Safe Deferred Memory Reclamation with Types

Memory management in lock-free data structures remains a major challenge in concurrent programming. Design techniques including read-copy-update (RCU) and hazard pointers provide workable solutions, and are widely used to great effect. These techniques rely on the concept of a grace period: nodes that should be freed are not deallocated immediately, and all threads obey a protocol to ensure that the deallocating thread can detect when all possible readers have completed their use of the object. This provides an approach to safe deallocation, but only when these subtle protocols are implemented correctly. We present a static type system to ensure the correct use of RCU memory management: that nodes removed from a data structure are always scheduled for subsequent deallocation, and that nodes are scheduled for deallocation at most once. As part of our soundness proof, we give an abstract semantics for RCU memory management primitives which captures the fundamental properties of RCU. Our type system allows us to give the first proofs of memory safety for RCU linked list and binary search tree implementations without requiring full verification.

==> chapters/FigsBST.tex <==
Concurrent Red-Black tree is used in crucial places inside operating system kernels like Virtual Memory(VM) region trees where they have great impact on scalability of multithreaded VM-intensive applications.  We analyse this important data
structure under RCU semantics and we try to explore free linearisability properties when we apply our type system. 

\textsf{\textbf{Readers}}. With RCU technique developing a reader is almost as easy as developing a non-concurrent reader.  The only restrictions placed on readers are that they do not hold any references to the data structure outside critical section.


\textsf{\textbf{Mutators}}. Lock-free proceeding of \textsf{Readers} can be provided with keeping Red-Black tree consistent by \textsf{Mutators}. 
\begin{itemize}
\item Mutator must not allow a reader to see partial changes to a node. Mutator use copy-on-update to make all changes to a private copy of the node, then atomically switch the new node with the old one.
\item Readers must not get lost when the structure of the tree is changed. In the Zig restructure below, if a reader is at node \textsf{A} looking for node \textsf{B} at the same time the restructure happens, the reader will never find \textsf{B}. The reason is after restructure
	we have \textsf{B} is above \textsf{A} instead of below it. 
\item Discuss with Matt: Temporarily having the same item in the tree multiple times won't affect the lookups. A unique value is returned if first copy encountered and another unique value can be returned if second copy is encountered.
\end{itemize}

% Restructure operations to rebalance a red black tree. There are left and right versions of these, but they are symmetric so only the left version is shown here.
\begin{figure}
\centering
\[
\begin{array}{r@{\;\;\Longrightarrow_{transform}\;\;}ll}

\begin{tikzpicture}
\tikzstyle{hollow node}=[circle,draw,inner sep=1.5]
\tikzstyle{solid node}=[rectangle,draw,inner sep=2.5]
\tikzset{
	red node/.style={circle,draw=red,fill=red,inner sep=2.2},
	blue node/.style={rectangle,draw=blue,inner sep=2.5}
}
\node[solid node]{C}
	child{
		node[solid node]{B}			
			child{node[solid node]{A}
					child{node[hollow node]{1}}
					child{node[hollow node]{2}}					
			}
			child{node[hollow node]{3}}
	}
	child{node[hollow node]{4}}
	
;
\end{tikzpicture}
&
\begin{tikzpicture}
\tikzstyle{hollow node}=[circle,draw,inner sep=1.5]
\tikzstyle{solid node}=[rectangle,draw,inner sep=2.5]
\tikzset{
	red node/.style={circle,draw=red,fill=red,inner sep=2.2},
	blue node/.style={rectangle,draw=blue,inner sep=2.5}
}
\node[solid node]{B}
			child{node[solid node]{A}
					child{node[hollow node]{1}}
					child{node[hollow node]{2}}					
			}
			child{node[solid node]{C}
					 child{node[hollow node]{3}} 
					 child{node[hollow node]{4}}
			}		
			
;
\end{tikzpicture}
&
 \textrm{Diag Structure}
\\
\begin{tikzpicture}
\tikzstyle{hollow node}=[circle,draw,inner sep=1.5]
\tikzstyle{solid node}=[rectangle,draw,inner sep=2.5]
\tikzset{
	red node/.style={circle,draw=red,fill=red,inner sep=2.2},
	blue node/.style={rectangle,draw=blue,inner sep=2.5}
}
\node[solid node]{C}							
			child{node[solid node]{A}
					child{node[hollow node]{1}}
					child{node[hollow node]{B}
								child{node[hollow node]{2}}
								child{node[hollow node]{3}}
					}							
			}					
			child{node[hollow node]{4}}	
	
	
;
\end{tikzpicture}
&
\begin{tikzpicture}
\tikzstyle{hollow node}=[circle,draw,inner sep=1.5]
\tikzstyle{solid node}=[rectangle,draw,inner sep=2.5]
\tikzset{
	red node/.style={circle,draw=red,fill=red,inner sep=2.2},
	blue node/.style={rectangle,draw=blue,inner sep=2.5}
}
\node[solid node]{B}
			child{node[solid node]{A}
					child{node[hollow node]{1}}
					child{node[hollow node]{2}}					
			}
			child{node[solid node]{C}
					 child{node[hollow node]{3}} 
					 child{node[hollow node]{4}}
			}		
			
;
\end{tikzpicture}
&
 \textrm{Zig Structure}
\\

\end{array}
\]
\caption{Restructure operations used to rebalance a red black tree. There are left and right versions of these, but they are symmetric so only the left version is shown here.}
\end{figure}

\subsubsection{Swap}
Consider the delete of node \textsf{B} shown in  below. Since \textsf{B} is an internal, \textsf{B} will be swapped with \textsf{C} $(= next ($ \textsf{B} )$)$ prior to deletion.
\newpage

\begin{figure}
\centering
\begin{tikzpicture}
\tikzstyle{hollow node}=[circle,draw,inner sep=1.5]
\tikzstyle{solid node}=[rectangle,draw,inner sep=2.5]
\tikzset{
	red node/.style={circle,draw=red,fill=red,inner sep=2.2},
	blue node/.style={rectangle,draw=blue,inner sep=2.5}
}
\node[solid node]{F}
			child{node[solid node]{B}
					child{node[solid node]{A}}
					child{node[solid node]{E}
							child{node[solid node]{C}
								child{node[hollow node]{NULL}}
								child{node[solid node]{D}}
							}
							child{node[hollow node]{SUB-TREE}}	
					}					
			}
			child{node[hollow node]{SUB-TREE}}						
;
\end{tikzpicture}
\caption{Tree Before Deletion of node B}
\end{figure}



\textsf{C'} is allocated with color and children of B, but with key and data  values of C.  The \textsf{C'} is linked into tree as in place of \textsf{B}. The value of \textsf{C} can be  observed twice in tree. In this setting, readers who are below \textsf{B} and above \textsf{C'} can read the value of \textsf{C} safely.
This is because \textsf{C} is kept until all readers below \textsf{B} looking for value of \textsf{C} is are done. In other words, garbage collector thread waits for a grace period before removing \textsf{C} from the tree. This preserves that readers below \textsf{B} will complete their read prior to \textsf{C} being removed.

\begin{figure}
\centering
\begin{tikzpicture}[>=stealth',node distance=2.5cm,semithick,auto]
\tikzstyle{hollow node}=[circle,draw,inner sep=1.5]
\tikzstyle{sub node}=[triangle,draw,inner sep=1.5]
\tikzstyle{solid node}=[rectangle,draw,inner sep=2.5]

\tikzset{
	red node/.style={rectangle,draw=red,fill=red,inner sep=2.2},
	blue node/.style={rectangle,draw=blue,inner sep=2.5}
}
    \node[solid node]                  (F)                             {$F$};
    \node[solid node]            (Cp)    [below left of=F]            {$C'$};
    \node[red node]            (B)    [right of=Cp]           {$B$};
   \node[solid node]            (A)    [below left of=Cp]     {$A$};
    \node[solid node]            (E)    [below right of=B]           {$E$};
    \node[red node]            (C)    [below left of=E]     {$C$};
    \node[solid node]            (D)    [below right of=C]           {$D$};
    \node[hollow node]            (N)    [below left of=C]     {$NULL$};
    \node[hollow node]            (STF)  [right of= F] {$SUB-TREE$};
   \node[hollow node]            (STE)  [ right of= E] {$SUB-TREE$};

    \path[-]   (F)     edge                        node        {}              (Cp)
                (Cp)    edge                        node        {}    (A)
                (Cp)    edge                        node        {}    (E)
                (B)    edge                        node        {}    (A)
                (B)    edge                        node        {}    (E)
                (E)    edge                        node        {}    (D)
                (C)    edge                        node        {}    (D)
                (C)    edge                        node        {}    (N)
		(E)	edge				node		{}	(STE)
		(F)	edge				node 	{}	(STF)
;
\end{tikzpicture}
\caption{Tree after deletion of node B. The red nodes are scheduled for reclamation.}
\end{figure}
[TODO: Informal Reasonings on Rotations, Evaluation Order]


==> chapters/ProofsLemmasBeforeColin <==

\subsection{Soundness Lemmas}
\begin{Lemma}[Overwrite-Current]\scriptsize
\begin{align*}
\llbracket x:=x.f \rrbracket \lfloor \llbracket \Gamma,x:\mathsf{rcuItr} \rrbracket_{\textsf{R,M},tid} * \{m\}\rfloor  \subseteq \\
\lfloor \llbracket \Gamma,x:\mathsf{rcuItr} \rrbracket_{\textsf{R,M},tid}  * \mathcal{R}(\{m\})\rfloor
\end{align*}
\end{Lemma}
\begin{proof}
We prove here the simpler obligation, which together with Lemma \ref{lem:crit-lifting} (critical section lifting) implies the above:

{\scriptsize
\[
\llbracket x:=x.f \rrbracket \lfloor \llbracket \Gamma,x:\mathsf{rcuItr} \rrbracket_{tid} * \{m\}\rfloor  \subseteq
\lfloor \llbracket \Gamma,x:\mathsf{rcuItr} \rrbracket_{tid}  * \mathcal{R}(\{m\})\rfloor
\]
}

Assume
\[(\sigma,O,U,T)\in\llbracket \Gamma,x:\mathsf{rcuItr} \rrbracket_{tid} * \{m\}\]
Then
\[
\llbracket x:=x.f \rrbracket(\sigma)\Downarrow_{tid}\sigma'
\]
where
\[
\sigma'=\sigma[s\mapsto(\sigma.s[(x,tid)\mapsto \sigma.h(\sigma.s(x,tid),f)])]
\]
We must choose $O'$, $U'$, and $T'$ such that
\[(\sigma',O',U',T')\in\llbracket \Gamma,x:\mathsf{rcuItr} \rrbracket_{tid} * \{m\}\]
Let $U'=U$ and $T'=T$, and
\[O'=O\cup(\sigma.h(\sigma.s(x,tid),f)\mapsto\mathsf{iterator}\;tid)\]
\todo{there should be field maps in this lemma...}
\colin{T-WriteS doesn't seem to have the required side-conditions on $\Gamma$.  Either $\Gamma$ should be dropped from this rule (pushing the problem to \textsf{WellFramed} and the frame rule) or T-WriteS should gain appropriate side-conditions.  The appropriate side conditions should really be equivalent to what \textsf{WellFramed} would impose, so I propose dropping it.}
\iso{I couldn't understand this comment. So is it the case that our well-formed framing lemma and its proof does not captures this case ? I am not clear on this. }
\colin{T-WriteS doesn't seem to manage the field maps correctly.  The map in the input environment can have \emph{any} field map, since we don't care about its contents for safety.  And the map in the output environment should be empty, since we know nothing about the node $x$ now refers to.}
\iso{Yes, you are right, it needs to be empty mapping.}
\end{proof}


\begin{Lemma}[Read-Heap]\scriptsize
\begin{align*}
\llbracket y:=x.f \rrbracket( \lfloor \llbracket \Gamma,y:\_,x:\mathsf{rcuItr} \rrbracket_{\textsf{R,M},tid} * \{m\}\rfloor)  \subseteq \\
\lfloor \llbracket \Gamma,y:\mathsf{rcuItr},x:\mathsf{rcuItr} \rrbracket_{\textsf{R,M},tid}  * \mathcal{R}(\{m\})\rfloor
\end{align*}
\end{Lemma}
\begin{proof}
    \todo{also missing field maps}
\end{proof}

\begin{Lemma}[Heap-Update-Unlink]\scriptsize
\begin{align*}
  \llbracket x.f:=z \rrbracket (\lfloor \llbracket \Gamma, \, x:\mathsf{rcuItr}\,\rho\,\N ( [f \rightharpoonup  y]), y:\mathsf{rcuItr} \, \rho' \,\N([ f \rightharpoonup z]), \\
                                                              z:\mathsf{rcuItr} \, \rho'' \,\_ \rrbracket_{M,tid} * \{m\}\rfloor)  \subseteq \\
                                                              \lfloor \llbracket \Gamma, \,  x:\mathsf{rcuItr} \, \rho \, \N([ f \rightharpoonup z]),\\
                                                              y:\mathsf{unlinked}, \\
                                                              z:\mathsf{rcuItr} \, \rho' \, \_ \rrbracket  * \mathcal{R}(\{m\})\rfloor
\end{align*}
\end{Lemma}
\begin{proof}\scriptsize

We can assume
\begin{gather}\label{3ua1}
  \begin{aligned}
    (\sigma, O, U, T) \, \in & \llbracket \Gamma, \, x:\mathsf{rcuItr}\,\rho\,\N ( [f \rightharpoonup  y]), y:\mathsf{rcuItr} \, \rho' \,\N([ f \rightharpoonup z]) , \\
    &z:\mathsf{rcuItr} \, \rho'' \,\_ \rrbracket_{M,tid} * \{m\}
    \end{aligned} \\
\textsf{WellFormed}(\sigma,O,U,T)
\label{3ua2}
\end{gather}

And we show that there exists $O', U', T'$ such that

\begin{gather}\label{3up1}
\textsf{WellFormed}(  \sigma [ \sigma.h(\sigma.s(x,tid),f )\mapsto \sigma.s(z,tid) ] , O', U', T')
\end{gather}

From \ref{3ua1} we can assume

\begin{gather} \label{3u1a1}
  \begin{aligned}
    (\sigma, O_{1}, U_{1}, T_{1} ) \in & \llbracket \Gamma,\, x:\mathsf{rcuItr}\,\rho\,\N ( [f \rightharpoonup  y]), y:\mathsf{rcuItr} \, \rho' \,\N([ f \rightharpoonup z]), \\
    &z:\mathsf{rcuItr} \, \rho'' \,\_  \rrbracket_{M,tid} \end{aligned}\\
\label{3u2a1}
(\sigma, O_{2}, U_{2}, T_{2}) = m
\\
\label{3ua3}
O_{1} \bullet O_{2} = O
\\
\label{3ua4}
U_{1} \cup U_{2} = U
\\
\label{3ua5}
T_{1} \cup T_{2} = T
\\
\label{3ua6}
\textsf{WellFormed}(\sigma,O_{1},U_{1},T_{1})
\\
\label{3ua7}
\textsf{WellFormed}(\sigma,O_{2},U_{2},T_{2})
\end{gather}

To prove \ref{3up1} we choose

\begin{gather}\label{3xup}
  O' = O [\sigma.s(y,tid) \mapsto O(\sigma.s(y,tid)) \setminus \mathsf{iterator} \, tid \cup \{ \mathsf{unlinked}\} ]\\
  \label{3xup1}
  U' = U\\
  \label{3xup2}
  T' = T
\end{gather}


We must prove there exists $O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2}$ such that

\begin{gather}\label{3u1p1}
\begin{aligned}
(\sigma',O'_{1},U'_{1}, T'_{1})  \in \llbracket \Gamma, \,  x:\mathsf{rcuItr} \, \rho \,\N([ f \rightharpoonup z]), \\y:\mathsf{unlinked}, z:\mathsf{rcuItr} \, \rho' \, \_ \rrbracket_{M,tid}
\end{aligned}\\
\label{3u2p1}
(\sigma',O'_{2},U'_{2}, T'_{2}) \in \mathcal{R}(\{m\})
\\
\label{3up3}
O'_{1} \bullet O'_{2} = O'
\\
\label{3up4}
U'_{1} \cup U'_{2} = U'
\\
\label{3up5}
T'_{1} \cup T'_{2} = T
\\
\label{3up6}
\textsf{WellFormed}(\sigma',O'_{1},U'_{1},T'_{1}) \\
\label{3up7}
\textsf{WellFormed}(\sigma',O'_{2},U'_{2},T'_{2})
\end{gather}
We choose \[O_{2}' = O_{2}, U_{1}' = U_{1}, U_{2}' = U_{2}, T_{1}' = T_{1}, T_{2}' = T_{2}\] so that \ref{3up4} follows from \ref{3ua4} and for the rest for the proof, we claim that

\begin{equation} \label{3ua8}
T_{1} = \{tid\} \land tid =  \sigma.l
\end{equation}
which follows directly from \ref{3ua1}.

We set $O'_1$ as
\begin{gather} \label{3xup3}
O'_1 = O_1 [  \sigma.s(y,tid) \mapsto \sigma.s(y,tid) \setminus \{\mathsf{iterator}\;tid \} \cup \{\mathsf{unlinked}\} ]
\end{gather}
As $O_{2}'$ is chosen as $O_{2}$ and we know equations \ref{3xup3}, \ref{3xup1} and \ref{3ua3}, we can show that \ref{3up3} holds.

From \ref{3u1a1} we can assume that there exists $\hat{O_1}$, $\hat{\hat{O_1}}$,  $\hat{\hat{\hat{O_1}}}$ and $\hat{\hat{\hat{\hat{O_1}}}}$ such that
\begin{gather}\label{3uahat1}
  (\sigma, \hat{O_1}, U_1,T_1) \in \llbracket \Gamma \rrbracket_{M,tid} \\
  \label{3uahat2}
  (\sigma, \hat{\hat{O_1}}, U_1 ,T_1) \in \llbracket x:\mathsf{rcuItr}\,\rho\,\N ( [f \rightharpoonup  y]) \rrbracket_{M,tid} \\
\label{3uahat3}
 (\sigma, \hat{\hat{\hat{O_1}}}, U_1 ,T_1) \in \llbracket y:\mathsf{rcuItr} \, \rho' \,\N([ f \rightharpoonup z]) \rrbracket_{M,tid} \\
\label{3uahat4}
  (\sigma, \hat{\hat{\hat{\hat{O_1}}}}, U_1 ,T_1) \in \llbracket z:\mathsf{rcuItr} \, \rho'' \,\_  \rrbracket_{M,tid} \rrbracket_{M,tid}\\
  \label{3uahat5}
  \hat{O_1} \bullet \hat{\hat{O_1}} \bullet \hat{\hat{\hat{O_1}}} \bullet \hat{\hat{\hat{\hat{O_1}}}} = O_1
  \end{gather}

To show \ref{3u1p1} we need to show that there exists $\hat{O}'_{1}$, $\hat{\hat{O}}'_{1}$, $\hat{\hat{\hat{O'_1}}}$ and $\hat{\hat{\hat{\hat{O'_1}}}}$

\begin{gather}
\label{3uphat1}
  (\sigma',\hat{O}'_{1},U_1, T_1) \in \llbracket \Gamma \rrbracket_{M,tid} \\
  \label{3uphat2}
   (\sigma',\hat{\hat{O}}'_{1},U_1, T_1) \in \llbracket   x:\mathsf{rcuItr} \, \rho \,\N([ f \rightharpoonup z]) \, \rrbracket_{M,tid} \\
\label{3uphat3}
(\sigma',\hat{\hat{\hat{O}}}'_{1},U_1, T_1) \in \llbracket   y:\mathsf{unlinked}\, \rrbracket_{M,tid} \\
\label{3uphat4}
(\sigma',\hat{\hat{\hat{\hat{O}}}}'_{1},U_1, T_1) \in \llbracket  z:\mathsf{rcuItr} \, \rho' \, \_ \rrbracket_{M,tid} \\
\label{3uphat5}
\hat{O'_1} \bullet \hat{\hat{O'_1}} \bullet \hat{\hat{\hat{O'_1}}} \bullet \hat{\hat{\hat{\hat{O'_1}}}} = O'_1
\end{gather}

We choose $\hat{O'}_1$ as $\hat{O}_1$, $\hat{\hat{O'}}_1$ as $\hat{\hat{O}}_1$ and $\hat{\hat{\hat{\hat{O'}}}}_1$ as $\hat{\hat{\hat{\hat{O}}}}_1$ so that \ref{3uphat1}, \ref{3uphat2} and \ref{3uphat4} follows from \ref{3uahat1}, \ref{3uahat2} and \ref{3uahat4}.

However, $\hat{\hat{\hat{O'}}}_1$ and $\hat{\hat{\hat{O}}}_1$ are different observations so \ref{3uphat3} does not follow from \ref{3uahat3}.
To prove \ref{3up6} we need to recall \ref{3ua6}, \ref{3xup3} and $tid = \sigma.l \land T_1 = \{tid\}$.
%%I am here
\begin{itemize}
\item \textsf{\ref{3up6}.Ownership}:trivial.
\item \textsf{\ref{3up6}.Reader-Writer-Iterator-Coexistence-Ownerhsip}:trivial.
\item \textsf{\ref{3up6}.Iterators-Free-List}:trivial.
\item \textsf{\ref{3up6}.Unlinked-Reachability}:We know that only updated map is $O'_1$ where the update is shown with equation \ref{3xup3}.
  We also know from \ref{3uphat3} that $y$ is observed as $\mathsf{unlinked}$. Unlinked observation of $y$ can be in premise of Unlinked-Reachability or in conclusion of the Unlinked-Reachability. Therefore, we need to show two cases :
  \begin{itemize}
  \item \textbf{Case-1} All nodes reaching to $y$ can be either observed as $\mathsf{unlinked}$ or in free-list:
    \begin{itemize}
    \item From type environments shown in figure \ref{fig:denotingtypeenviroment} and equations \ref{3uahat1}, \ref{3uahat2}, \ref{3uahat3}, \ref{3uahat4}, \ref{3uphat1}, \ref{3uphat2}, \ref{3uphat3} and \ref{3uphat4} we know that:
      \begin{itemize}
            \item \[\textsf{iterator } \, tid\in  O_1(s(x,tid))  \land x \notin U_1 \land s(y,tid) = h(s(x,tid), f) \]
              \[\textsf{iterator } \, tid\in  O'_1(s(x,tid))  \land x \notin U'_1 \land s(z,tid) = h(s(x,tid), f) \]
            \item \[\textsf{iterator } \, tid\in  O_1(s(y,tid))  \land y \notin U_1 \land s(z,tid) = h(s(y,tid), f) \]
              \[\textsf{unlinked }\in  O'_1(s(y,tid))  \land y \notin U'_1 \]
            \item \[\textsf{iterator } \, tid\in  O_1(s(z,tid))  \land z \notin U_1 \land s(\_,tid) = h(s(z,tid), f) \]
              \[\textsf{iterator } \, tid\in  O'_1(s(z,tid))  \land z \notin U'_1 \land s(\_,tid) = h(s(z,tid), f) \]
            \item Since $U_{1}'$ is chosen  $U_{1}$ and $T_{1}'$ is chosed as $T_{1}$, we know that the only map changed is shown in equation \ref{3xup3}
            \item Suppose $\exists_{f'}\ldotp f' \neq f$
              \[\textsf{iterator } \, tid\in  O_1(s(x,tid))  \land x \notin U_1 \land s(y,tid) = h(s(x,tid), f') \]
              \[\textsf{iterator } \, tid\in  O'_1(s(x,tid))  \land x \notin U'_1 \land s(y,tid) = h(s(x,tid), f') \]
              which ends in contradiction with $\textsf{unlinked} \in O'_1(s(y,tid))$.
      \end{itemize}
      \end{itemize}
  \item \textbf{Case-2} All nodes reachable from $y$ needs to be observed as $\mathsf{unlinked}$ : Under the context built for \textbf{Case-1} and from type environments we know that
     \[\textsf{unlinked }\in  O'_1(s(y,tid))  \land y \notin U'_1 \]
    There exists no \textsf{rcu} field access in this type environment so no heap node can be observed as $\mathsf{iterator } tid$ from a $y$ with a field access.
  \end{itemize}
\item \textsf{\ref{3up6}.Free-List-Reachability}:is trivial because free list is not updated by the action.
\item \textsf{\ref{3up6}.Writer-Unlink}:trivial.
\item \textsf{\ref{3up6}.Fresh-Reachable}:trivial.
\item \textsf{\ref{3up6}.Fresh-Writer}:trivial.
\item \textsf{\ref{3up6}.Writer-Not-Reader}: We know that $tid = \sigma.l$. Since operational semantics of heap update does not include change in owner of lock we know that
  \[ \sigma'.l = tid\]
  which implies \textsf{\ref{3up6}.Writer-Not-Reader}.
\item \textsf{\ref{3up6}.Readers-In-Free-List}: As we know from operational semantics, \textsf{free-list} is changed with add/subtraction of threads $t$ such that
  \[t \in R\]
  As we know that $tid = \sigma.l$ we can conclude that \textsf{\ref{3up6}.Writer-Not-Reader}.
\item \textsf{\ref{3up6}.To-Be-In-Free-List}:trivial.
\item \textsf{\ref{3up6}.MustBeAllocated}:trivial.
\item \textsf{\ref{3up6}.Heap-Domain}:trivial.
  \textsf{\ref{3up6}.Unique-Root}: \begin{itemize}
  \item From \ref{3up6} we know that \textsf{Unique-Root} invariant is preserved by observed type states in $O_1$ including $x,y,z$.
  \item We know that choosing $\hat{\hat{O'}}_1$ as $\hat{\hat{O}}_1$ and $\hat{\hat{\hat{\hat{O'}}}}_1$ as $\hat{\hat{\hat{\hat{O}}}}_1$ showed that \ref{3uphat1}, \ref{3uphat2} and \ref{3uphat4} follows from \ref{3uahat1}, \ref{3uahat2} and \ref{3uahat4} as we know from the equation \ref{3xup3} that the only changed map is $O'_1$ and the change is reflected in change from \ref{3uahat3} to \ref{3uphat3}.
  \item We unlink $y$ as shown in \ref{3uphat3} and unlinking occurs in between  $z$ and $x$ where both preserves the type states as shown in equations \ref{3uphat4} and \ref{3uphat2}.
    \item In this context, we know that $x$ points $z$ preserve \textsf{Unique-Root} in \ref{3ua6} and preserves in it in \ref{3up6}.
    \end{itemize}
\item \textsf{\ref{3up6}.Unique-Reachable}:[TODO: EASY - write down]

\end{itemize}
To show  \ref{3u2p1} we need to show that
\[(\sigma, O_2, U_2, T_2) \mathcal{R} (\sigma', O'_2, U'_2, T'_2)  \]
which by definition means that we must show
\begin{gather}\label{3ir1}
\sigma.l \in T_2 \implies \sigma.h = \sigma'.h \\
\label{3ir2}
\textsf{iterator} \, tid \in O_2(o) \implies o \in dom(\sigma'.h) \\
\label{3ir3}
O_2  = O'_2\\
\label{3ir4}
U_2 = U'_2\\
\label{3ir5}
T_2 = T'_2\\
\label{3ir6}
\forall_{t} \in T_2 \implies  \forall x \ldotp \sigma.s(x,t) = \sigma'.s(x,t)
\end{gather}
\begin{itemize}
\item We know that $tid \in T_1 \land \sigma.l = tid$ therefore $\forall_{t\in T_2}\ldotp t \neq tid$. Also recall that $T'_1$ is chosen as $T_1$ and $T'_2$ is chosen as $T_2$ where all implies \ref{3ir1}.
\item Recall that  $U'_2$ is chosen as $U_2$, $T'_2$ is chosen as $T_2$, $O'_2$ is chosen as $O_2$ therefore \ref{3ir3}-\ref{3ir5} holds.
\item Recall from equation \ref{3xup3} that the only changed map is $O_1$. Also recall that $O_2'$ is chosen as $O_2$ and $T'_2$ is chosen as $T_2$ which means $\forall_{x,f\fname,t\in T_2} \ldotp O_2(h(s(x,t),f)) = O'_2(h'(s'(x,t),f))$. Therefore \ref{3ir2} and \ref{3ir6} hold.
\end{itemize}
\end{proof}

\newcommand{\newln}{\\&\quad\quad{}}

\begin{Lemma}[Heap-Update-Link]\scriptsize
\begin{align*}
\llbracket x.f:=z \rrbracket( \lfloor \llbracket \Gamma,x:\mathsf{rcuItr} \, \N([ f \rightharpoonup y]) \, , \\
z:\mathsf{rcuFresh} \,\N([f \rightharpoonup y]) \rrbracket_{\textsf{M},tid} * \{m\}\rfloor)  \subseteq  \\
\lfloor \llbracket \Gamma,x:\mathsf{rcuItr} \, \N([f \rightharpoonup z]) \, , \\
z:\mathsf{rcuItr} \, \rho' \,\N([ f \rightharpoonup y])  \rrbracket_{\textsf{M},tid}  * \mathcal{R}(\{m\})\rfloor
\end{align*}
\end{Lemma}
\begin{proof}\scriptsize

We can assume
\begin{gather}\label{4ua1}
\begin{aligned}
(\sigma, O, U, T) \, \in \,& \llbracket \Gamma, \, x:\mathsf{rcuItr}\,\rho\,\N ( [f \rightharpoonup  y]), \\
&z:\mathsf{rcuFresh} \,\N([ f \rightharpoonup y])  \rrbracket_{M,tid} * \{m\}  \end{aligned}\\
\textsf{WellFormed}(\sigma,O,U,T)
\label{4ua2}
\end{gather}

And we show that there exists $O', U', T'$ such that

\begin{gather}\label{4up1}
  \textsf{WellFormed}(\sigma[ h(s(x,tid),f )\mapsto .s(z,tid)], h(.s(z,tid),f )\mapsto \sigma.s(y,tid) ] , O', U', T')
\end{gather}

From \ref{4ua1} we can assume

\begin{gather} \label{4u1a1}
(\sigma, O_{1}, U_{1}, T_{1} ) \in \llbracket \Gamma,\, x:\mathsf{rcuItr}\,\rho\,\N ( [f \rightharpoonup  y]), z:\mathsf{rcuFresh} \, \rho' \,\N([ f \rightharpoonup y]) \rrbracket_{M,tid} \\
\label{4u2a1}
(\sigma, O_{2}, U_{2}, T_{2}) = m
\\
\label{4ua3}
O_{1} \bullet O_{2} = O
\\
\label{4ua4}
U_{1} \cup U_{2} = U
\\
\label{4ua5}
T_{1} \cup T_{2} = T
\\
\label{4ua6}
\textsf{WellFormed}(\sigma,O_{1},U_{1},T_{1})
\\
\label{4ua7}
\textsf{WellFormed}(\sigma,O_{2},U_{2},T_{2})
\end{gather}

To prove \ref{4up1} we choose

\begin{gather}
\label{4xup}
O' = O [\sigma.s(z,tid) \mapsto O(\sigma.s(z,tid)) \setminus \{\mathsf{fresh}\}  \cup \{ \mathsf{iterator }tid\} ]\\
\label{4xup1}
U' = U\\
\label{4xup2}
T' = T
\end{gather}


We must prove there exists $O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2}$ such that

\begin{gather}\label{4u1p1}
(\sigma',O'_{1},U'_{1}, T'_{1})  \in \llbracket \Gamma, \,  x:\mathsf{rcuItr} \, \rho \,\N([ f \rightharpoonup z]),  z:\mathsf{rcuItr} \, \rho' \,\N([ f \rightharpoonup y]) \rrbracket_{M,tid}
\\
\label{4u2p1}
(\sigma',O'_{2},U'_{2}, T'_{2}) \in \mathcal{R}(\{m\})
\\
\label{4up3}
O'_{1} \bullet O'_{2} = O'
\\
\label{4up4}
U'_{1} \cup U'_{2} = U'
\\
\label{4up5}
T'_{1} \cup T'_{2} = T
\\
\label{4up6}
\textsf{WellFormed}(\sigma',O'_{1},U'_{1},T'_{1}) \\
\label{4up7}
\textsf{WellFormed}(\sigma',O'_{2},U'_{2},T'_{2})
\end{gather}
We choose \[O_{2}' = O_{2}, U_{1}' = U_{1}, U_{2}' = U_{2}, T_{1}' = T_{1}, T_{2}' = T_{2}\] so that \ref{4up4} follows from \ref{4ua4} and for the rest for the proof, we claim that

\begin{equation} \label{4ua8}
T_{1} = \{tid\} \land tid =  \sigma.l
\end{equation}
which follows directly from \ref{4ua1}.

We set $O'_1$ as
\begin{gather}
\label{4xup3}
O'_1 = O_1 [  \sigma.s(z,tid) \mapsto \sigma.s(z,tid) \setminus \{\mathsf{fresh}\} \cup \{\mathsf{iterator }tid\} ]
\end{gather}

As $O_{2}'$ is chosen as $O_{2}$ and we know equations \ref{4xup3}, \ref{4xup1} and \ref{4ua3}, we can show that \ref{4up3} holds.

From \ref{4u1a1} we can assume that there exists $\hat{O_1}$, $\hat{\hat{O_1}}$,  $\hat{\hat{\hat{O_1}}}$ and $\hat{\hat{\hat{\hat{O_1}}}}$ such that
\begin{gather}\label{4uahat1}
  (\sigma, \hat{O_1}, U_1,T_1) \in \llbracket \Gamma \rrbracket_{M,tid} \\
  \label{4uahat2}
  (\sigma, \hat{\hat{O_1}}, U_1 ,T_1) \in \llbracket x:\mathsf{rcuItr}\,\rho\,\N ( [f \rightharpoonup  y]) \rrbracket_{M,tid} \\
\label{4uahat3}
 (\sigma, \hat{\hat{\hat{O_1}}}, U_1 ,T_1) \in \llbracket z:\mathsf{rcuFresh} \, \N([ f \rightharpoonup u]) \rrbracket_{M,tid} \\
  \label{4uahat4}
  \hat{O_1} \bullet \hat{\hat{O_1}} \bullet \hat{\hat{\hat{O_1}}}  = O_1
  \end{gather}

To show \ref{4u1p1} we need to show that there exists $\hat{O}'_{1}$, $\hat{\hat{O}}'_{1}$ and $\hat{\hat{\hat{O'_1}}}$

\begin{gather}
\label{4uphat1}
  (\sigma',\hat{O}'_{1},U_1, T_1) \in \llbracket \Gamma \rrbracket_{M,tid} \\
  \label{4uphat2}
   (\sigma',\hat{\hat{O}}'_{1},U_1, T_1) \in \llbracket   x:\mathsf{rcuItr} \, \rho \,\N([ f \rightharpoonup z]) \, \rrbracket_{M,tid} \\
\label{4uphat3}
(\sigma',\hat{\hat{\hat{O}}}'_{1},U_1, T_1) \in \llbracket   z:\mathsf{rcuItr}\, \rho' \,\N([ f \rightharpoonup y]) \rrbracket_{M,tid} \\
\label{4uphat4}
\hat{O'_1} \bullet \hat{\hat{O'_1}} \bullet \hat{\hat{\hat{O'_1}}} \bullet \hat{\hat{\hat{\hat{O'_1}}}} = O'_1
\end{gather}

We choose $\hat{O'}_1$ as $\hat{O}_1$ and $\hat{\hat{O'}}_1$ as $\hat{\hat{O}}_1$  so that \ref{4uphat1} and \ref{4uphat2}  follow from \ref{4uahat1} and \ref{4uahat2}.

However, $\hat{\hat{\hat{O'}}}_1$ and $\hat{\hat{\hat{O}}}_1$ are different observations so \ref{4uphat3} does not follow from \ref{4uahat3}. To prove \ref{4up6} we need to recall \ref{4ua6}, \ref{3xup3} and $tid = \sigma.l \land T_1 = \{tid\}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{itemize}
\item \textsf{\ref{4up6}.Ownership}: [TODO : A wierd question to Colin]
\item \textsf{\ref{4up6}.Reader-Writer-Iterator-Coexistence-Ownerhsip}: trivial.
\item \textsf{\ref{4up6}.Iterators-Free-List} and \textsf{\ref{4up6}.Free-List-Reachability}: From equations \ref{4uahat3}, \ref{4uphat3} and \ref{4xup3} we know that $\textsf{fresh} \in O_1(s(z,tid))$ and $\textsf{iterator }tid \in O'_1(s'(z,tid))$. $T'_1$ is chosen as $T_1$ and recalling equation \ref{4ua8} together with operational semantics for free-list updates we conclude that $T$ in $\forall_{T}\ldotp (T,o) \in \sigma'.F$ is empty.
\item \textsf{\ref{4up6}.Unlinked-Reachability}:trivial.
\item \textsf{\ref{4up6}.Writer-Unlink}: Facts from type environment of the \textsf{rcuItr} shown in figure \ref{fig:denotingtypeenviroment}makes this proof trivial.
\item \textsf{\ref{4up6}.Fresh-Reachable}:trivial.
\item \textsf{\ref{4up6}.Fresh-By-Mutator}:trivial.
\item \textsf{\ref{4up6}.Writer-Not-Reader}:trivial.
\item \textsf{\ref{4up6}.Readers-In-Free-List}:trivial.
\item \textsf{\ref{4up6}.To-Be-In-Free-List}:trivial.
\item \textsf{\ref{4up6}.MustBeAllocated}:trivial.
\item \textsf{\ref{4up6}.Heap-Domain}: Facts from type environment of the \textsf{rcuItr} and \textsf{rcuFresh} shown in figure \ref{fig:denotingtypeenviroment} makes this proof trivial.
\item \textsf{\ref{4up6}.Unique-Root}:
  \begin{itemize}
  \item Recalling \ref{4ua6}, we know that there exists no observable type state that violates the \textsf{Unique-Root} invariant.
  \item As \ref{4uphat2} is shown as valid by choosing $\hat{\hat{O'}}_1$ as $\hat{\hat{O}}_1$ and recalling equation \ref{4xup3} shows that linking $z$ as fresh node preserves \textsf{Unique-Root} invariant.
  \end{itemize}
\item \textsf{\ref{4up6}.Unique-Reachable}:
  \begin{itemize}
   \item Recalling \ref{4ua6}, we know that there are no observed type states in $O_1$ violating the \textsf{Unique-Reachable} property.
   \item \todo{add to type env of fresh that there exists no rcu heap node pointing to it}.
     \item From \ref{4ua1} and \ref{4ua6} we know that $\rho$ is valid unique path. From \ref{4ua1} we also know that $x$ points to $y$ via field $f$. From path arithmetic that we introduce, we can suppose that we have $\rho' = \rho.f$.  In addition, \ref{4uphat2} is shown as valid by choosing $\hat{\hat{O'}}_1$ as $\hat{\hat{O}}_1$. Therefore recalling equation \ref{4xup3} shows preservation of \textsf{Unique-Reachability}.
  \end{itemize}
\end{itemize}
To show  \ref{4u2p1} we need to show that
\[(\sigma, O_2, U_2, T_2) \mathcal{R} (\sigma', O'_2, U'_2, T'_2)  \]
which by definition means that we must show
\begin{gather}\label{4ir1}
\sigma.l \in T_2 \implies \sigma.h = \sigma'.h \\
\label{4ir2}
\textsf{iterator} \, tid \in O_2(o) \implies o \in dom(\sigma'.h) \\
\label{4ir3}
O_2  = O'_2\\
\label{4ir4}
U_2 = U'_2\\
\label{4ir5}
T_2 = T'_2\\
\label{4ir6}
\forall_{t \in T_2, x} \ldotp \sigma.s(x,t) = \sigma'.s(x,t)
\end{gather}

\begin{itemize}
\item We know that $tid \in T_1 \land \sigma.l = tid$ therefore $\forall_{t\in T_2}\ldotp t \neq tid$. Also recall that $T'_1$ is chosen as $T_1$ and $T'_2$ is chosen as $T_2$ where all implies \ref{4ir1}.
\item Recall that  $U'_2$ is chosen as $U_2$, $T'_2$ is chosen as $T_2$, $O'_2$ is chosen as $O_2$ therefore \ref{4ir3}-\ref{4ir5} holds.
\item Recall from equation \ref{4xup3} that the only changed map is $O_1$. Also recall that $O_2'$ is chosen as $O_2$ and $T'_2$ is chosen as $T_2$ which means $\forall_{x,f\fname,t\in T_2} \ldotp O_2(h(s(x,t),f)) = O'_2(h'(s'(x,t),f))$. Therefore \ref{4ir2} and \ref{4ir6} hold.
\end{itemize}
\end{proof}

\begin{Lemma}[Stack-Read]\scriptsize
\begin{align*}
\llbracket y:=x \rrbracket( \lfloor \llbracket \Gamma,y:\_,x:\mathsf{rcuItr} \rho \, \N \rrbracket_{\textsf{R,M},tid} * \{m\}\rfloor)  \subseteq \\
\lfloor \llbracket \Gamma,y:\mathsf{rcuItr} \, \rho \, \N ,x:\mathsf{rcuItr} \rrbracket_{\textsf{R,M},tid}  * \mathcal{R}(\{m\})\rfloor
\end{align*}
\end{Lemma}

\begin{Lemma}[Heap-Allocate]\scriptsize
\begin{align*}
  \llbracket y := new \rrbracket (\lfloor \llbracket \Gamma,y:\_ \rrbracket_{\textsf{M},tid} * \{m\}\rfloor)  \subseteq \\
  \lfloor \llbracket \Gamma,y:\mathsf{rcuFresh} \, \N_{\emptyset} \rrbracket_{\textsf{M},tid}  * \mathcal{R}(\{m\})\rfloor
\end{align*}
\end{Lemma}


\begin{Lemma}[Asych-Free]\scriptsize
\begin{align*}
\llbracket  \mathsf{asyncDelayedFree}(x) \rrbracket (\lfloor \llbracket \Gamma,x:\mathsf{unlinked} \rrbracket_{\textsf{M},tid} * \{m\}\rfloor)  \subseteq \\
\lfloor \llbracket \Gamma,x:\mathsf{undef} \rrbracket_{\textsf{M},tid}  * \mathcal{R}(\{m\})\rfloor
\end{align*}
\end{Lemma}



==> chapters/RCUBSTExplanation.tex <==

\section{Red-Black Tree with RCU Types}
Red-Black(RB)  tree is an important data structure which is used in many performance critical system (e.g. Operating Systems). RB Trees are used in implementation of dictionaries which is a set of key-value pairs with \textsf{Insert}, \textsf{Delete}, \textsf{Read} operations. \textsf{Insert}, \textsf{Delete} are \textsf{update} operations, \textsf{Read} is a \textsf{look up} operation. A RB Tree keeps key-value pairs as its internal nodes, with totally ordered keys.RB Tree shown in Figure \ref{fig:rbtree} has $(k,v)$ as its internal node and all value $v$, \textsf{Value((key,value)) = v}, of a node has a unique key $k$, \textsf{Key((key,value)) = k},  which never changes. In RB Tree, all descendants in  the left sub-tree of $v$ have keys larger than the key of $v$. The successor of node $v$ is the node with the smallest key among nodes with keys larger than or equal to key of $v$ which is the purple node in Figure \ref{fig:rbtree}. 
\input{RBTreeStructure.tex}
RB Trees are mainly used in components where read-only transactions are intensive. RCU is a programming-pattern which scales up performance when read-only operations are intensive. Naturally, exploration of rb-tree implementation with RCU pattern resulted in many studies:
\begin{itemize}
\item \href{http://www.pdx.edu/sites/www.pdx.edu.computer-science/files/tr1006.pdf}{Relativistic Red-Black Tree}. First relativistic RBTree paper.
\item \href{http://www.cs.technion.ac.il/~mayaarl/full-version.pdf}{ArbelAttiyaConcurrent Updates} . Fine grain updates.
\end{itemize}
In this section, we present the implementation of rb-tree with types that we propose and show proofs of memory safety and some linearisability properties. General correctness properties that we expect from a rb-tree are:
\begin{itemize}
\item An in order traversal of a consistent tree will always give values of the tree sorted
\item Lookups will always find a node that exists in the tree
\end{itemize}
Thinking rb-tree from RCU perspective does not make implementation more complicated than normally it is.  A concurrent setting with RCU technique is basically includes:
\begin{itemize} 
\item \textsf{\textbf{Readers}}. With RCU technique developing a reader is almost as easy as developing a non-concurrent reader.  The only restrictions placed on readers are that they do not hold any references to the data structure outside critical section.
\item \textsf{\textbf{Mutators}}. Lock-free proceeding of \textsf{Readers} can be provided with keeping Red-Black tree consistent by \textsf{Mutators}. 
\item Mutator must not allow a reader to see partial changes to a node. Mutator use copy-on-update to make all changes to a private copy of the node, then atomically switch the new node with the old one.
\item The termination position of a search is defined to be the last node whose value is examined by the search before it is terminated. If a search for a value $v$ is terminated at node $n$ at  time $t$ then it search for value $v$ will always terminate at node $n$ for all searches when we isolate tree from updates
\item Readers must not get lost when the structure of the tree is changed. In Figure \ref{fig:succmoveanom}, assume that there exists a reader looking for node with key \textsf{k'} concurrently with a mutator thread which moves successor of \textsf{k}, \textsf{k'},as a result of \textsf{Delete} operation performed on \textsf{k}  then the reader will get lost and return false for \textsf{Read} operation on \textsf{k'} even it exists in the tree.
\item  Temporarily having the same item in the tree multiple times won't affect the lookups. A unique value is returned if first copy encountered and another unique value can be returned if second copy is encountered.
\item Only nodes which are  no longer reachable  by an existing search or  future search will be garbage collected and all such nodes will be garbage collected, Figure \ref{fig:del2}
\end{itemize}
\subsection{Red-Black Tree Implementation}
RB-Tree implementation has three functions:
\begin{itemize}
\item \textsf{Insert}$(key,value)$ adds $(key,value)$ pair to the tree as a leaf; returns $true$ if $key$ is not in the set and $false$ otherwise
\item \textsf{Delete}$(key)$ removes $(key,value)$ pair  from tree; returns $true$ if $key$ is in the tree and $false$ otherwise
\item \textsf{Read}$(key)$ returns $val$ if $(key,value)$ is in the set; otherwise it returns $false$
\end{itemize}
\paragraph{Read}Explain code in general and anomaly caused by the part of the code.
\input{RBTreeSuccMoveAnom.tex}
\paragraph{Insert} Explain code in general and anomaly caused by the part of the code.
\input{RBTreeInsertAnom.tex}
\paragraph{Delete} Explain code in general and anomaly caused by the part of  the code.
\input{RBTreeDeleteOneChildAnom.tex}
\input{RBTReeDeleteTwoChildAnom.tex}
\begin{table}[]
	\begin{tabular}{ c c }
		Read & Update \\		
\begin{lstlisting}
struct node_p{
  int key;
  struct node_p* child[2];
  int value;
}

node_p<rcu> root;
	
data Read(int key){
  data result;	
  rcuRead{
    node_p<rcuIterator> itr; 
    itr=root;
    int itrKey = itr->key; 
        
    while(itr != NULL && 
	itrKey != key ){

      if(itrKey > key)
	  itr = itr->child[0]
       if(itrKey < key)
          itr = itr->child[1];
	if(itr != NULL) 
         itrKey = itr->key;
    }
    result = itr->value;
  }
  return result;
}
\end{lstlisting} &		
\begin{lstlisting}
//Adds a node as leaf
void Insert(int key, int val){
 rcuMutate{
   node_p <rcuIterator> itr;
   node_p<rcuIterator> prev;
   prev = root;
   itr = prev->child[0]; //right
   itrKey = itr->key;
   direction = 0;
   int itrKey = itr->key;

   while (itr != NULL && 
          itrKey != key)
   {
    prev = itr;
    if (itrKey > key){
     itr = itr->child[0];
     direction = 0;
    }
    if (itrKey < key){
     itr = itr->child[1];
     direction = 1;
    }
    if (itr!=NULL) 
     itrKey = itr->key ;
  }
    if(itr != NULL)
     return false;

    // Add fresh node as leaf  
    node = new(key,val)
    prev->child[direction] = node
  }
  return true;
}
		\end{lstlisting} 
	\end{tabular}
	
\caption{RCU-Red-Black Tree Implementation.}
\label{tab:rcurbtree}
\end{table}

\begin{table}[]
	\begin{tabular}{ c }
		Update\\		
\begin{lstlisting}
void Delete(int key){  
 rcuMutate{  
   node_p<rcuIterator> prev = root;
   node_p <rcuIterator> itr  itr = prev->child[0]; //right;
   itrKey = itr->key;
   direction = 0;
   int itrKey = itr->key;  
   while (itr != NULL && itrKey != key){
    prev = itr;
    if (itrKey > key){ itr = itr->child[0]; direction = 0;}
    if (itrKey < key){ itr = itr->child[1]; direction = 1;}
    if (itr!=NULL) 
     itrKey = itr->key ;
   }
   if(itr == NULL)//Not found
    return false;
   // One child
   if(itr->child[0] == NULL){ prev->child[direction] = itr->child[1]; return true;}
   if(itr->child[1] == NULL){ prev->child[direction] = itr->child[0]; return true;}
   //Two children
   node_p<rcuIterator>  prevSucc = itr;  
   node_p<rcuIterator>  succ = itr->child[1];
   node_p<rcuIterator>  next = succ->child[0]; 
   while ( next!= NULL){
    prevSucc = succ;
    succ = next;
    next = next->child[0];
   }
   node = new(succ->key); // Update
   new->child[0]=curr->child[0];
   new->child[1]=curr->child[1];
   prev->child[direction]=new ;    
  } //rcuMutate ends
  asyncDelayedFree(Clean, prevSucc, itr, succ);   
 return true;
}
\end{lstlisting} 
	\end{tabular} \hfill	
\caption{RCU-Red-Black Tree Delete implementation.}
\label{tab:rcurbtreedel}
\end{table}
\begin{table}[]
	\begin{tabular}{ c }
		Async Free\\
\begin{lstlisting}
void Clean(node_p prev, node_p curr, node_p succ)
{
 // succ is the right child of curr
 if (prev == curr){
  new->child[1]=succ->child[1];
 }
 prev->child[0] = succ->child[1];
}
\end{lstlisting}
	\end{tabular} \hfill	
\caption{RCU-Red-Black Tree Clean function for removing old successor.}
\label{tab:rcurbtreecln}
\end{table}
\subsection{Proof for RCU RB-Tree}
\section{Conclusion}
\section{Related Work Notes}
Aspect-Oriented Linearizability Proofs:
Thomas A. Henzinger, Ali Sezgin, and Viktor Vafeiadis


Implicit ownership types for memory management


==> chapters/RCUBriefExplanation.tex <==
\section{Read-Copy-Update Programming}
Writing an efficient concurrent program is hard. One of well-known ways for providing efficiency is implementing non-blocking concurrent data structures. \textsf{Read-Copy-Update} is a programming pattern which provides implementing non-blocking concurrent data structures.
RCU and similar programming patterns have an optimistic memory access pattern which stems from allowing accesses to memory locations while they are being updated by the concurrent mutator thread. Reader threads do not need to hold locks for accessing linked list and there exists only one mutator thread accessing to linked list at a time. Mutual exclusiveness between mutator threads are provided via one global lock.

There are couple computing structures which are clients of RCU programming pattern
\begin{itemize}
\item Concurrent Linked-List
\item Concurrent Hash Tables [Resizable, scalable, concurrent hash tables via relativistic programming]
\item Concurrent Red-Black trees [Relativistic red-black trees]
\item Software Transactional Memory implementations
\end{itemize}
where we focus on RCU Linked-List throughout the paper.

Enforcing readers to see the modifications in a particular order, linearizability,  in red-black trees and hash tables in such optimistic concurrent setting as a correctness criteria is very important. 
\subsection{Informal Reasoning on Linked List}
\begin{table}[]
	\begin{tabular}{|p{7cm}|p{7cm}|}
		Read & Delete \\
		
\begin{lstlisting}
struct node_p{
  int data;
  node_p* next;
}		
node_p<rcu>* head;
	
data Read(data toRead){
  data result;	
  ReadBegin{
    node_p<rcuIterator>* itr; 
    itr=head;     
    while(itr != NULLl){
      if(itr->data == toRead)
	    break;
	  itr= itr->next;
    }
    result = itr->data;
  }
  return result;
}
		\end{lstlisting} &
		
		\begin{lstlisting}
void Delete(data toDel){

 WriteBegin{
   node_p <rcuIterator>* itr;
   node_p<rcuIterator>* prev;

   itr=prev=head;    
   if(itr != NULL){
    while(itr != NULL){
     if(itr->data == toDel)
       break;
     prev = itr;
     itr = itr->next;
    }
   }
    prev->next = itr->next;
    asyncDelayedFree(itr);
   }
}
		\end{lstlisting} 
	\end{tabular}
	
	\caption{Read-Copy-Update Client: Linked-List Implementation.}
	\label{tab:rculist}
\end{table}

Table ~\ref{tab:rculist} denotes the implementation of a \textsf{Read-Copy-Update} client singly linked list. 
In RCU based non-blocking linked list implementation, generally the implementation pattern looks similar to the one shown in Table . However, the implementation shown in Table ~\ref{tab:rculist} includes types parameterized under our type system rules.
\paragraph{Delete}  : \textsf{WriteBegin-WriteEnd} block in between lines (3-17) is defined as  a mutual exclusive scope where only one mutator thread can be inside. 

\textsf{asyncDelayedFree} at line 18 is not inside \textsf{rcuMutate}. In other words, asynchronous memory reclamation call is not handled inside a mutually exclusive block.  [TODO: Showing that atomic\{traverse;unlink;reclaim\} == rcuMutate\{traverse;unlink\} asyncDelayedFree]. See \textbf{mutator axioms} in section  ~\ref{mutatoraxioms}.

\paragraph{Read} : \textsf{ReadBegin-ReadEnd} block in between lines (9-18) is defined as a read only scope in which only reader threads can have access. Many reader threads can have access to this block simultaneously even though threre exists an iterator pointer from the mutator thread at the same time.  Pictorially, the interleaving of reader and writer threads are shown as in the following Figure ~\ref{fig:readlist} , Figure ~\ref{fig:mutatelist} and Figure ~\ref{fig:unlinkedlist} : 

\begin{figure}
\centering
\begin{tikzpicture}[>=stealth',node distance=2cm,semithick,auto]
\tikzstyle{hollow node}=[circle,draw,inner sep=1.5]
\tikzstyle{sub node}=[triangle,draw,inner sep=1.5]
\tikzstyle{solid node}=[rectangle,draw,inner sep=2.5]

\tikzset{
	red node/.style={rectangle,draw=red,fill=red,inner sep=2.2},
	blue node/.style={rectangle,draw=blue,inner sep=2.5},
	reader node/.style={circle,draw=blue,inner sep=1},
	writer node/.style={circle,draw=green,inner sep=1}
}
 
    \node[solid node] (R) {$R$};
    \node[hollow node] (5) [right of=R] {$5$};
    \node[hollow node] (7) [right of=5] {$7$};
   \node[hollow node] (8) [right of=7] {$8$};
    \node[hollow node] (2) [right of=8] {$2$};
    \node[hollow node] (1) [right of=2] {$1$};
    \node[hollow node] (11) [right of=1] {$11$};
    \node[hollow node] (4) [right of=11] {$4$};
  \node[reader node] (r1) [above right of= 1]  {$cr$};
    \node[reader node] (r2)  [above left of= 1] {$cr$};

    \path[->]   (R) edge node {} (5)
                (5) edge node {} (7)
		(7) edge node {} (8)
		(8) edge node {} (2)
		(2) edge node {} (1)
		(1) edge node {} (11)
		(11) edge node {} (4)                
		(r1) edge node {$\textsf{tid}_{r1}$} (1)
		(r2) edge node {$\textsf{tid}_{r2}$} (1)
;
\end{tikzpicture}
\caption{Two concurrent reader threads with $\textsf{tid}_{r1}$ and $\textsf{tid}_{r2}$ ids are on the node with value 1. These threads have their own iterators $\textsf{cr}$ on linked list. }
\label{fig:readlist}
\end{figure}

\begin{figure}
\centering
\begin{tikzpicture}[>=stealth',node distance=2cm,semithick,auto]
\tikzstyle{hollow node}=[circle,draw,inner sep=1.5]
\tikzstyle{sub node}=[triangle,draw,inner sep=1.5]
\tikzstyle{solid node}=[rectangle,draw,inner sep=2.5]

\tikzset{
	red node/.style={rectangle,draw=red,fill=red,inner sep=2.2},
	blue node/.style={rectangle,draw=blue,inner sep=2.5},
	reader node/.style={circle,draw=blue,inner sep=1},
	writer node/.style={circle,draw=green,inner sep=1}
}
 
      \node[solid node] (R) {$R$};
      \node[hollow node] (5) [right of=R] {$5$};
      \node[hollow node] (7) [right of=5] {$7$};
      \node[hollow node] (8) [right of=7] {$8$};
      \node[hollow node] (2) [right of=8] {$2$};
      \node[hollow node] (1) [right of=2] {$1$};
      \node[hollow node] (11) [right of=1] {$11$};
      \node[hollow node] (4) [right of=11] {$4$};
      \node[reader node] (r1) [above right of= 1]  {$cr$};
      \node[reader node] (r2)  [above left of= 1] {$cr$};
      \node[writer node] (wp) [below of=2] {$pr$}; 
      \node[writer node] (wc) [below of=1]{$cr$};

    \path[->]   (R) edge node {} (5)
                (5) edge node {} (7)
    		(7) edge node {} (8)
     		(8) edge node {} (2)
     		(11) edge node {} (4)   	
    		(1) edge node {} (11)
		(2) edge node {} (1)	
		(r1) edge node {$\textsf{tid}_{r1}$} (1)
		(r2) edge node {$\textsf{tid}_{r2}$} (1)
	        (wp) edge node  {$\textsf{tid}_{mut}$}  (2) 
		(wc) edge  node  {$\textsf{tid}_{mut}$}   (1)    
;
\end{tikzpicture}
\caption{A mutator thread with $\textsf{tid}_{mut}$ id is on linked list, $ l = \textsf{tid}_{mut}$, to delete the node with value 1.  Mutator thread has two iterators which are green $\textsf{pr}$ for showing previous node and  $\textsf{cr}$ for current node. }
\label{fig:mutatelist}
\end{figure}

\begin{figure}
\centering
\begin{tikzpicture}[>=stealth',node distance=2cm,semithick,auto]
\tikzstyle{hollow node}=[circle,draw,inner sep=1.5]
\tikzstyle{sub node}=[triangle,draw,inner sep=1.5]
\tikzstyle{solid node}=[rectangle,draw,inner sep=2.5]

\tikzset{
	red node/.style={rectangle,draw=red,fill=red,inner sep=2.2},
	blue node/.style={rectangle,draw=blue,inner sep=2.5},
	reader node/.style={circle,draw=blue,inner sep=1},
	writer node/.style={circle,draw=green,inner sep=1}
}
 
      \node[solid node] (R) {$R$};
      \node[hollow node] (5) [right of=R] {$5$};
      \node[hollow node] (7) [right of=5] {$7$};
      \node[hollow node] (8) [right of=7] {$8$};
      \node[hollow node] (2) [right of=8] {$2$};
      \node[hollow node] (1) [right of=2] {$1$};
      \node[hollow node] (11) [right of=1] {$11$};
      \node[hollow node] (4) [right of=11] {$4$};
      \node[reader node] (r1) [above right of= 1]  {$cr$};
      \node[reader node] (r2)  [above left of= 1] {$cr$};


    \path[->]  (R) edge node {} (5);
    \path[->]  (5) edge node {} (7);
    \path[->]  (7) edge node {} (8);
    \path[->]  (8) edge node {} (2);
    \path[->]  (11) edge node {} (4);   	
    \path[->] (2) edge [bend right] node {} (11);
    \path[dashed,->]  (1) edge node {} (11);
   
    \path[->]  (r1) edge node {$\textsf{tid}_{r1}$} (1);
    \path[->]  (r2) edge node {$\textsf{tid}_{r2}$} (1);
;
\end{tikzpicture}

\caption{Linked-List is in a state where mutator thread with $\textsf{tid}_{mut}$ id unlinked the node with value 1 and released  $\textsf{pr}$ and $\textsf{cr}$ pointers on linked list, exited $\textsf{rcuMutate}$, $l \neq \textsf{tid}_{mut}$ . A unique thread for garbage collection, $\textsf{tid}_{gc}$, shows grace until all readers exit $\textsf{rcuRead}$.  Assuming that  location of the node with value 1 is $o$ then ($\textsf{tid}_{r2}$ ,o) $\in$ $F$ and ($\textsf{tid}_{r2}$,o) $\in$ $F$ }
\label{fig:unlinkedlist}
\end{figure}

The crucial point on memory management to provide safe memory is deciding when to reclaim memory; e.g., deciding when it is safe to reclaim a node with value $1$ as in Figure ~\ref{fig:unlinkedlist}. RCU orchestrates threads reading, mutating and reclaiming a memory location in a data structure by letting a memory reclaimer wait for all reader threads to finish their $\textsf{rcuRead}$ sections before allocating the node.

Eventhough the protocols orchestrating threads in the RCU pattern can be expressed clearly in a few sentences, their implementations in non-blocking data structures are extremely subtle.  For example, in the non-blocking linked list implementation in Table ~\ref{tab:rculist}  unlinking a node in $\textsf{rcuMutate}$ involves more than a simple pointer setting. We can conclude that such an optimistic memory access pattern generates structures for which it is hard to reason for memory safety and other properties. We propose a $\textsf{Flow Sensitive}$ type system using $\textsf{Ownership Types}$ which enforces correct usage of RCU pattern  and comes with strong guarantees like $\textsf{Memory Safety}$ and some $\textsf{Linearisability}$ properties. 

\paragraph{Flow Sensitive} Our type system is flow sensitive, which means types of memory locations can be viewed [TODO: I do not like "view", find another] as different types under the permission of typing rules. For example, type $\textsf{undef}$ represents variables that can not be accessed until something is loaded into them. This is used in the flow sensitive type system to invalidate variables that should no longer be accessed. Another example is for the type, $\textsf{rcuIterator}$, which represents a pointer into an RCU data structure that can be used in either a $\textsf{rcuUpdate}$ or a $\textsf{rcuRead}$.
\paragraph{Ownership Types} A memory region can be observed either $\textsf{unlinked}$, $\textsf{fresh}$ or being accessed by a thread with an iterator on it , $\textsf{iterator tid}$.  If a memory region is observed as a part of RCU structure which means has field type $\textsf{rcu}$ then it is a unique part of $\textsf{rcu}$ typed structure or is $\textsf{unlinked}$  or is in the free list. More formal $\textbf{\textsf{Ownership}}$ definition is in section ~\ref{subsec:meminv} 
\paragraph{Linearisability} The fundemantal mechanism to guarantee some $\textsf{Linearisability}$ properties is providing $\textsf{linearity}$ for $\textsf{rcuIterator}$ of reader thread.  In other words, there is at most one $\textsf{rcuIterator}$ type for a thread for providing a reader thread not to read the same state more than once.  $\textbf{\textsf{Read Block Axioms}}$ in section ~\ref{readblockaxioms} has more rigorous definition of providing $\textsf{linearity}$. For the RCU-based Linked-List example, a generic $\textsf{Linearisability}$ condition that our type system provides is the condition for setting a value in the reader that can be satisfied by at most one node in the list.
\paragraph{Memory Safety} 

\end{document}


==> chapters/RCUProgLang.tex <==
\vspace*{\fill}
\section{Programming language}
In this section, we present a simple object oriented programming language with two block constants for modelling RCU. We provide a semantics of this language, and a type system to check for correct usage of RCU primitives.

We assume all objects contain all fields.  This means we do not have to worry about the correct typing of field manipulation, etc. that is covered by a standard type system such as found in C$^\sharp$ or Java. We will only focus on the aspects of the typing related to the correct operation of RCU. This means our type system extends C$^\sharp$ or Java like languages' type systems which can handle standard type errors such as field not-exists.

\lstdefinestyle{nonumbers}
{numbers=none}
\subsection{Types}
\label{subsection:subsec-types}
Our type system only considers field types
\[
\tau ::= \textsf{rcu} | \textsf{normal}
\]
We assume a function, $\textsf{FType}$ that maps each field to its type.

There are six types of local variable
\[
\tau_{local} ::=  \textsf{rcuItr} \mid \textsf{rcuFresh} \mid \textsf{tofree} \mid \textsf{unlinked} \mid \textsf{undef} \mid \textsf{free}
\]
in addition to a type for global variables
\[\tau_{global} ::= \textsf{rcuRoot}\]

We have typing context $\Gamma$ of the form $x_1: T_1, \ldots x_n : T_n$.

The system has three forms of typing judgement
\begin{itemize}
\item $\Gamma \vdash C$: standard typing outside rcu regions
\item $\Gamma \vdash_R C \dashv \Gamma'$: flow sensitive typing inside an rcu read region
\item $\Gamma \vdash_M C \dashv \Gamma'$: flow sensitive typing inside an rcu write region
\end{itemize}

Below, we introduce each type through small code fragments taken from our typing effort for binary search tree ~\cite{msdn_bst} in the Appendix \ref{appendix:bst_del}. We also explain related type rules which we find important for program statements in the code fragments. Our aim is
\begin{itemize}
\item to define each type through is components e.g. path and field mappings of the \textsf{rcuItr} type. How do these components work together coherently? 
\item to explain why we employ each of these components. How do they serve to correct \textsf{RCU} programming? - (\textbf{Service})
\item to explain the \textit{flow-sensitive} nature of the type system. We justify why the flow of change in types serves to the correct \textsf{RCU} programming - (\textbf{Service})
\item to investigate potential memory safety issues for each program statement in the code fragments. We discuss what memory inconsistencies they can cause and how type rules prevent it - (\textbf{Service})
\end{itemize}

The code fragments below are annotated with assertions about type environments between each statement (in the style of a proof outline in Hoare Logic) to demonstrate informally how types change before and after various statements. All of the formal definitions for the type components and rules can be found in the Figures \ref{fig:sub-typing}, \ref{fig:type-judgements}, \ref{fig:type-judgements-for-cf} and \ref{fig:transitionsbetweendifferenttypesystems}.

(\textit{\textbf{Reading a Global}} \textsf{RCU} \textit{\textbf{Root}}) - All \textsf{RCU} data structures have global unique roots so that we can attach an iterator pointer to the data structure from here to traverse it. The type \textsf{rcuRoot} represents variables a unique root. We read a \textsf{rcuRoot} typed pointer to a local variable. As we observe in the pre/post conditions of reading the global root in the Listing \ref{lst:readglobal}, \texttt{root} pointer's type does not change. A local varible \texttt{current} is our new pointer to iterate over the data structure. The type of \texttt{current} changes from \textsf{undef} to \textsf{rcuItr} after reading the global root. The type \textsf{undef} represents variables that cannot be accessed until something is loaded into them. A variable in the type \textsf{rcuItr} represents a pointer into an RCU data structure that can be used in either a read or write region. It is product of multiple components and denoted as
\[current: \mathsf{rcuItr}\; \rho \; \N \]
where \textsf{rcuItr} type does not only hold the fact that the reference points into the shared RCU data structure, but it also keeps a path component, $\rho$, which tracks the path from the data structure's root to the heap node pointed by the variable. A component $\N$ is set of field mappings taking field names to local variable names. Field mappings are added to the field map, when the object's fields are read. Against these definitions,  we can assert that the path of \texttt{current} pointer is empty, $\epsilon$, and there exists no field mappings in its $\N$ yet. (\textbf{Service}) - In general, we utilize the path information to ensure that we preserve well shaped heap for the data structures, e.g. acyclicity. In conjuction with the path component, we employ the field mappings to assist in checking whether proper linking/mapping exists between the related nodes shown by the pointers when unlinking occurs. We already see the incarnation of the service from the path and field mappings to the correct usage of \textsf{RCU} programming in the Listing \ref{lst:readglobal}. The type assertion for the \texttt{current} pointer in the post condition tells that the heap node pointed by it is at the root -- its path is $\epsilon$ -- and there is no field mapping -- $\N_{\emptyset} = \{\}$  -- which means there is no link to any other heap node from the node pointed by \texttt{current}. So, at this point, there is not enough and proper resource for doing actions such as \textit{unlinking}, \textit{reclaiming} and \textit{replacing} a node. At this point, the type system considers all these actions as invalid program actions.  
\begin{lstlisting}[caption={Reading a global variable},label={lst:readglobal}, numbers=left, numberstyle=\tiny\color{red}, numbersep=5pt]%, basicstyle=\scriptsize]

$\assert{root:\mathsf{rcuRoot}}, current:\mathsf{undef}$
BinaryTreeNode current = root;
$\assert{root:\mathsf{rcuRoot},current:\mathsf{rcuItr} \;\epsilon \; \{\}}$
\end{lstlisting}

(\textit{\textbf{Reading an Object Field and a Variable}}) - As expected, we explore the heap of the data structure via reading the objects' fields. For example, The assertion in the Listing \ref{lst:readobjectfield}-line\{1\} tells that the path to reach the heap node pointed by \texttt{current} is $Left$. Correlatively, the assertion in the Listing \ref{lst:readobjectfield}-line\{2\} tells that there exists a link from the heap node pointed by \textsf{parent} to the heap node pointed by \textsf{current}. Reading \texttt{current} to \texttt{parent} in the Listing \ref{lst:readobjectfield}-line\{3\} sets the path and field mappings of \texttt{parent} to be same with \texttt{current}. As we observe in the post condition in the Listing \ref{lst:readobjectfield}-line\{7,8\}, reading \texttt{current} to the \texttt{parent}'s $Left$ field adds the field mapping entry $Left \mapsto \texttt{current}$ to the field mapping set of \texttt{parent} and extends the path of the \texttt{current} with $Left$.
\begin{lstlisting}[caption={Reading a object field},label={lst:readobjectfield}, numbers=left, numberstyle=\tiny\color{red}, numbersep=5pt]%, basicstyle=\scriptsize]

....
$\assert{current:\mathsf{rcuItr}\; Left \; \{\}}$
$\assert{parent:\mathsf{rcuItr}\; \epsilon \;\{Left\mapsto current\}}$
parent = current
$\assert{current:\mathsf{rcuItr}\; Left \;\{\}}$
$\assert{parent:\mathsf{rcuItr}\; Left \;\{\}}$
current = parent.Left
$\assert{current:\mathsf{rcuItr}\; Left.Left \;\{\}}$
$\assert{parent:\mathsf{rcuItr}\;  Left \;\{Left\mapsto current\}}$
....
\end{lstlisting}

(\textit{\textbf{Choosing Fields to Read}}) - Thus far, we have always been precise on the representation of the object fields-- mention just one field name -- both in the path component and field mappings. However, we cannot always be precise in mentioning the field names in the \textsf{rcuItr} type. The assertions in the Listing \ref{lst:altfield}-line\{2,3\} mention field names in different way, $Left|Right$, than we have seen so far. (\textbf{Service}) - Our intention to represent the object fields this way is to make \textsf{RCU} types expressible enough to assert "either Left or Right field''. The assertion in the Listing \ref{lst:altfield}-line\{2\} tells that the heap node pointed by the \texttt{current} pointer is reached via either "Left or Right" field. From other perspective, the assertion in the Listing \ref{lst:altfield}-line\{3\} tells that the heap node pointed by \texttt{current} can be reached from the heap node pointed by \texttt{parent} via "either Left or Right" field. 

However, we should also note that being precise in the field names is so crucial for mutation actions. This means we need to know which fields are used to replace/unlink. Then, what is the mechanism to become more/less precise in the fields used in both path and field mappings of the \textsf{rcuItr} type? In the Listing \ref{lst:altfield}, we see a \textit{if-statement} with the condition $parent.Left == current$. This condition refines the assertions in the Listing \ref{lst:altfield}-line\{2,3\} to the ones in the line \{5,6\} for the \textit{then} branch and to the ones in the line \{13,14\} for the \textit{else} branch via making types more precise  on the object fields used in both the path component and field mappings. The next step is to type the body of the branches which we have already seen in the Listing \ref{lst:readobjectfield}. 

To capture the precision relation on object fields in the types, we define the relation in between the contexts in the Listing \ref{lst:altfield}-line-\{2,3\} line-\{[9,10],[17,18]\} line-\{20,21\} as \textit{subtyping} relation with rules \textsc{T-NSub1} and \textsc{T-NSub1} in the Figure \ref{fig:sub-typing}. To type check the \textsf{if-statement} in the Listing \ref{lst:altfield}, we use a simple type rule, \textsc{T-Branch1}, in the Figure \ref{fig:type-judgements-for-cf}.
\begin{lstlisting}[caption={Choosing fields to read},label={lst:altfield}, numbers=left, numberstyle=\tiny\color{red}, numbersep=5pt]%, basicstyle=\scriptsize]

....
$\assert{current:\mathsf{rcuItr}\; Left|Right \;\{\}}$
$\assert{parent:\mathsf{rcuItr}\;  \epsilon \;\{Left|Right\mapsto current\}}$
if(parent.Left == current){
  $\assert{current:\mathsf{rcuItr}\; Left \;\{\}}$
  $\assert{parent:\mathsf{rcuItr}\;  \epsilon \;\{Left\mapsto current\}}$
  parent = current;
  current = parent.Left;
  $\assert{current:\mathsf{rcuItr}\; Left.Left \;\{\}}$
  $\assert{parent:\mathsf{rcuItr}\;  Left \;\{Left\mapsto current\}}$
}
else{
  $\assert{current:\mathsf{rcuItr}\; Right \;\{\}}$
  $\assert{parent:\mathsf{rcuItr}\;  \epsilon \;\{Right\mapsto current\}}$
  parent = current;
  current = parent.Right;
  $\assert{current:\mathsf{rcuItr}\; Right.Right \;\{\}}$
  $\assert{parent:\mathsf{rcuItr}\;  Right \;\{Right\mapsto current\}}$
}
$\assert{current:\mathsf{rcuItr}\; Left|Right.Left|Right \;\{\}}$
$\assert{parent:\mathsf{rcuItr}\;  Left|Right \;\{Left|Right\mapsto current\}}$
....
\end{lstlisting}

(\textit{\textbf{Loop Summarization via Path Summarization}}) - Inside loops, we read object fields iteratively to explore the heap of a data structure. Naturally, It has effects on a path component of the \textsf{rcuItr} type. As we go along the loop, depth from a root of a data structure increases because we read object fields and these object fields accumulate on the path component e.g. reading the \texttt{current} to the $Left$ field to iterately. Another aspect of the loops is non-deterministic choice on the number of iterations. (\textbf{Service}) - To capture the effects of the loops properly in the type \textsf{rcuItr}, we \textit{summarize} the \textit{loop}'s effects on the paths of the iterator pointers used inside the loop. We see in the Listing \ref{lst:loop}-line\{3,4\} that the type assertions for the \texttt{parent} and \texttt{current} pointers have $(Left|Right)^{*}$ and $(Right|Left)^{*}.Left$ in their path components respectively. The portion of the path summary superscripted with $*$ -- denotes non-determinisim in the number of execution times -- denotes the common portion contibuted to all of the iterators used in the loop. The portion outside $*$, e.g. the last $Left$ of $(Left|Right)^{*}.Left$, is the portion which distinguishes the contribution of the loop to the iterator pointer's path component, e.g. the \texttt{current} pointer shares the path contribution $(Left|Right)^{*}$ with \texttt{parent} but it has $Left$ in its path component as it is pointed by \texttt{parent} via $Left$ component.

We reflect the change in the path of a type \textsf{rcuItr} to a subtyping relation via \textsc{T-PSub1}, \textsc{T-PSub2} and \textsc{T-PSub3}, in the Figure \ref{fig:sub-typing}. We also use simple structural type rule, \textsc{T-Loop1}, to type the \textit{while-statement} in the Listing \ref{lst:loop}.
\begin{lstlisting}[caption={Loop summarization via path summarization },label={lst:loop}, numbers=left, numberstyle=\tiny\color{red}, numbersep=5pt]%, basicstyle=\scriptsize]

....
while(current.data != data)
  $\assert{current:\mathsf{rcuItr}\; (Left|Right)^{*}.Left|Right \;\{\}}$
  $\assert{parent:\mathsf{rcuItr}\;  (Left|Right)^{*} \;\{Left|Right\mapsto current\}}$
  if(parent.Left == current){
    $\assert{current:\mathsf{rcuItr}\; (Left)^{*}.Left \;\{\}}$
    $\assert{parent:\mathsf{rcuItr}\;  (Left)^{*} \;\{Left\mapsto current\}}$
    parent = current;
    current = parent.Left;
    $\assert{current:\mathsf{rcuItr}\; (Left)^{*}.Left \;\{\}}$
    $\assert{parent:\mathsf{rcuItr}\;  (Left)^{*} \;\{Left\mapsto current\}}$
  }
  else{
    $\assert{current:\mathsf{rcuItr}\; (Right)^{*}.Right \;\{\}}$
    $\assert{parent:\mathsf{rcuItr}\;  (Right)^{*} \;\{Right\mapsto current\}}$
    parent = current;
    current = parent.Right;
    $\assert{current:\mathsf{rcuItr}\; (Right)^{*}.Right \;\{\}}$
    $\assert{parent:\mathsf{rcuItr}\;  (Right)^{*} \;\{Right\mapsto current\}}$
  }

  $\assert{current:\mathsf{rcuItr}\; (Left|Right)^{*}.Left|Right \;\{\}}$
  $\assert{parent:\mathsf{rcuItr}\;  (Left|Right)^{*} \;\{Left|Right\mapsto current\}}$
}
....
\end{lstlisting}

(\textit{\textbf{Points to}}\textsf{null}) - [TODO: ...]

(\textit{\textbf{Mutation - Unlinking a Heap Node}}) - Preserving invariants of a data structure, e.g. acyclicity in \textsf{BST}, against possible mutations under \textsf{RCU} semantics is challenging. Our types in coherent with the type rules provide safety -- memory safety -- guarantees against mutations. Unlinking an heap node is one way of mutating the heap. (\textbf{Service}) - The first crucial neccesity  to do a proper unlinking is to have three consecutive heap nodes. We assert the "proper linkage" in between the heap nodes involved in unlinking via assistance of path components and field mappings. Our type rule for unlinking, \textsc{T-UnlinkH}, is
\[\scriptsize
\inferrule
{
\textsf{FV}(\Gamma) \cap \{x,z,r\} \qquad \rho.f_1=\rho' \;\; \rho'.f_2=\rho'' \qquad \forall_{f\in dom(\N')} \ldotp f\neq f_2 \implies \N'([f\rightharpoonup \textsf{null}])   \\
\lnot(\exists_{n\in \Gamma, p''',f,m}\ldotp n:\textsf{rcuItr}\,\rho'''\,\N([f\rightharpoonup m]) \land ((\rho = \rho''') \lor (\rho' = \rho''') \lor (\rho''=\rho''') ) \land \{m\} \cap \{z,r\} \neq \emptyset  )
}
{
\Gamma,\, x:\textsf{rcuItr}\, \rho \, \N([f_1\rightharpoonup z]) \, ,
z:\textsf{rcuItr}\, \rho' \, \N'([f_2\rightharpoonup r]) \, ,  r:\textsf{rcuItr} \, \rho'' \, \N''\, 
\vdash_{M} x.f_1=r \dashv
z:\unlinked\, ,
x:\textsf{rcuItr} \, \rho \, \N(f_1\rightharpoonup z \setminus r)\, ,
r:\textsf{rcuItr} \, \rho' \, \N'',\, \Gamma
}
\]
 The rule asserts that $x$, $y$ and $z$ pointers are linked with the field mappings $\N([f_1\rightharpoonup z])$ of $x$, $\N'([f_2\rightharpoonup r])$ of $y$. In accordance with the field mappings, we assert that $x$ has the path $\rho$, $y$ has the path $\rho.f_1$. and $z$ has the path $\rho.f_1.f_2$. In the Listing \ref{lst:unlink}, we see the code fragment for unlinking the heap node pointed by \texttt{current}. The precondition in the Listing \ref{lst:unlink}-link\{2-4\} tells that the heap nodes pointed by \texttt{parent},  \texttt{current} and \texttt{currentL} are linked -- via the field mappings and they are consecutive -- via the path components.

Being able to localize the effects of the mutation is important in a sense that it prevents unexpected side effects of the mutation. So, sharing through aliasing to the resources under mutation, e.g. aliasing to \texttt{parent}, \texttt{current} and \texttt{currentL}, needs to be handled carefully. To understand the importance of the locality on the effect of the mutation, we illustrate the setting in the Listing \ref{lst:unlink} with some additional fictional resources such as stack pointer aliases in the Figure \ref{fig:frameout} and \ref{fig:unlinkframeout}. The square nodes filled with $R$ -- a root node -- and $H$ -- a heap node -- are heap nodes. The hollow nodes are stack pointers to the square heap nodes. All resources in red are the ones that form the resource context under the effect of unlinking which we call \textit{effect-zone}. The hollow red nodes -- \texttt{pr}, \texttt{cr} and \texttt{crl} -- point to the red square heap nodes which are involved in unlinking of the heap node pointed by \texttt{cr}. We have the $a_1$, $a_2$ and $a_3$ which are aliases with \texttt{parent}-$pr$, \texttt{current}-$cr$ and \texttt{currenL}-$crl$ respectively. We call them the \textit{path-aliases} as they share the same path form root to the node that they point. The red filled circle depicts \texttt{null}, the $l$ field depicts $Left$ and $r$ depicts $Right$ field in the Listing \ref{lst:unlink}.

To prevent the complications due to \textit{path-aliasing} and also variable name sharing in different contexts, the type rule first asserts
\[\textsf{FV}(\Gamma) \cap \{x,z,r\} \]
which simply states that there exists no variable named $x$(\texttt{parent} in the Listing \ref{lst:unlink}, $pr$ in the Figures \ref{fig:frameout} and \ref{fig:unlinkframeout}), $y$\texttt{current} in the Listing \ref{lst:unlink}, $cr$ in the Figures \ref{fig:frameout} and \ref{fig:unlinkframeout} and $z$\texttt{currentL} in the Listing \ref{lst:unlink}, $crl$ in the Figures \ref{fig:frameout} and \ref{fig:unlinkframeout} shared with $\Gamma$. Then it also asserts the \textit{framing} assertion
\[\lnot(\exists_{n\in \Gamma, p''',f,m}\ldotp n:\textsf{rcuItr}\,\rho'''\,\N([f\rightharpoonup m]) \land ((\rho = \rho''') \lor (\rho' = \rho''') \lor (\rho''=\rho''') ) \land (\{m\} \cap \{z,r\} \neq \emptyset  )\]
to restrict the aliasing. So, why do we need all these assertions? How would aliasing show up with our \textsf{RCU} types? What problems can aliasing generate with our \textsf{RCU} types? First, aliasing can occur via either through  object fields -- via field mappings -- or stack pointers -- via path components. We see the path aliases, $a_1$, $a_2$ and $a_3$, illustrated with dashed nodes and arrows to the heap nodes in the Figures \ref{fig:frameout} and \ref{fig:unlinkframeout}. They are depicted as dashed because they are not safe resources to use when unlinking the \texttt{current} so they are \textit{framed-out} via the part of the assertion 
\[\lnot((\rho = \rho''') \lor (\lor' = \lor''') \lor (\rho''=\rho''') )\]
which states non-existence of the \textit{path-aliases} to any of $x$, $z$ and $r$ in the rule which corresponds to $pr$, $cr$ and $crl$ respectively.
The reason for framing-out these dashed path aliases is obvious when we look at the changes from the Figure \ref{fig:frameout} to the Figure \ref{fig:unlinkframeout}. For example, the $a_1$ points to the $H_1$ which has object field $Left$-$l$ pointing to the $H_2$ which is also pointed by \texttt{current} as depicted in the Figure \ref{fig:frameout}. However, in the Figure \ref{fig:unlinkframeout}, the $l$ of the $H_1$ is pointing to the $H_3$ though the $a_1$ still points to the $H_1$. This change invalidates the field mapping $Left \mapsto current$ of the $a_1$ in the \textsf{rcuItr} type. One another safety achieved with framing shows up in a setting where \texttt{current} and $a_2$ are aliases. In the Figure \ref{fig:frameout}, both \texttt{current} and $a_2$ are in the \textsf{rcuItr} type and point to $H_2$. After the unlinking action in the Listing \ref{lst:unlink}-line\{6\}, the type of the \texttt{current} becomes \texttt{unlinked} although the $a_2$ is still in the \texttt{rcuItr} type. Framing out the $a_2$ prevents the inconsistency in its type under the unlinking operation. One interesting and not obvious inconsistency issue shows up due to the aliasing between the $a_3$ and the \texttt{currentL}-$crl$. Before the unlinking happens, both \texttt{currentL} and $a_3$ have the same path components -- assume it is $(Left)^{*}.Left.Left$ in the Listing \ref{lst:unlink}-line\{4\}. After the unlinking, the path of the \texttt{currentL}-$crl$ gets shortened as the path to heap node it points, $H_3$, changes  to $(Left)^{*}.Left$ as we see in the Listing \ref{lst:unlink}-line\{10\}. However, the path component of the $a_3$  would not change so the path component of the $a_3$ in the \textsf{rcuItr} would become inconsistent with the actual path reaching to the $H_3$.

In addition to \textit{path-aliasing}, there can also  the aliasing via \textit{field-mappings} which we call \textit{field-aliasing}. We see the field alising examples in the Figures \ref{fig:frameout} and \ref{fig:unlinkframeout}: $pr$ and $a_1$ are field aliases with $Left-l$ from $H_0$ points to $H_1$, $cr$ and $a_2$ are field aliases with $Left-l$ from $H_4$ points to $H_2$  and $crl$ and $a_3$ are field aliases with $Left-l$ from $H_5$ points to $H_3$. We do not discuss the problems that can occur due to the \textit{field-aliasing} as they are same with the ones due to \textit{path-aliasing}. What we focus on is how the type rule prevents \textit{field-aliases} that can cause problem in the unlinking setting. The portion of the framing assertion
\[\lnot(\{m\} \cap \{z,r\} \neq \emptyset  )\]
prevents potential problems due to field aliasing. This assertion states that there exists no object field $f$ which points to $m$ in the context $\Gamma$ such that $m$ can be neither 1- the variable points the heap node that is mutation(unlinking) -- \texttt{current}-$cr$ --  nor 2- the variable points that $f$ shows after unlinking -- \texttt{currentL}-$crl$. We should also note that it is expected to have object fields in $\Gamma$ to point to $pr$ -- which is to expect $m$ to be $pr$ -- as they are not in the effect zone of unlinking. For example, we see the object field $l$ points from $H_0$ to  $H_1$ in the Figures \ref{fig:frameout} and \ref{fig:unlinkframeout}.

Being aware of how much of the heap is under mutation is important, e.g. a whole subtree or a single node. Our type system ensures that there can be only just one heap node unlinked at a time by atomic field update action. To be able to ensure this, in addition to the proper linkage enforcement, the rule also asserts that all other object fields which are not under mutation must point to \texttt{null}
\[\forall_{f\in dom(\N')} \ldotp f\neq f_2 \implies \N'([f\rightharpoonup \textsf{null}])\]
For example, in the Listing \ref{lst:unlink}-line\{3\}, we see that the \texttt{current} has the $Left \mapsto currentL$ mapping so its $Right$ field must point to \texttt{null}. We also see this pictorially in the Figures \ref{fig:frameout} and \ref{fig:unlinkframeout}, the object field $Right$-$r$ from the $H_2$ points to red circle, \texttt{null}.

After the safe unlinking of the heap node happens, the type of the variable points this heap node changes from \textsf{rcuItr} to \textsf{unlinked} -- change from assertion in the Listing \ref{lst:unlink}-line\{3\} to one in the line\{9\}. This node cannot be accessed by the new coming reader threads the ones that are currently reading this node cannot access to the rest of the heap. We illustrate this with dashed red $cr$, $H_2$ and object fields in the Figure \ref{fig:unlinkframeout}.
 \begin{figure}[H]
 \centering
 \begin{subfigure}[b]{.4\linewidth}
\centering
 \begin{tikzpicture}[>=stealth',node distance=1.3cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]
 \tikzstyle{solids node}=[rectangle,draw=red,inner sep=1.5]
\tikzstyle{null node}=[circle,draw=red,fill=red]
 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1},
 	blue node/.style={rectangle,draw=black,inner sep=1},
 	reader node/.style={circle,draw=black,inner sep=1},
        redreader node/.style={circle,draw=red,inner sep=1},
        readerr node/.style={dashed,circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[solid node] (1) [right of=R] {$H_0$};
       \node[solids node] (2) [right of=1] {$H_1$};
       \node[solids node] (3) [right of=2] {$H_2$};
       \node[solids node] (4) [right of=3] {$H_3$};
       \node[solid node] (5) [above  of=3] {$H_4$};
       \node[null node] (nl) [above right of = 3]{};
       \node[solid node] (6) [above  of=4] {$H_5$};
       
       \node[redreader node] (r0) [below  of= 2]  {$pr$};
       \node[redreader node] (r1) [below  of= 3]  {$cr$};
       \node[redreader node] (r2)  [below  of= 4] {$crl$};

       \node[readerr node] (r0a) [above  of= 1]  {$a_1$};
       \node[readerr node] (r1a) [above   of= 2]  {$a_2$};
       \node[readerr node] (r2a)  [below right of= 4] {$a_3$};

       \node[reader node] (r1f) [above  of= 5]  {$a_4$};
       \node[reader node] (r2f)  [above  of= 6] {$a_5$};

     \path[->]  (R) edge node[below] {$l$} (1);
     \path[->]  (1) edge node[below] {$l$} (2);
     \path[draw=red,->]  (2) edge node[below] {$l$} (3);
     \path[draw=red,->]  (3) edge node[below] {$l$} (4);
     \path[dashed,->]  (5) edge node {$l$} (3);
     \path[dashed,->]  (6) edge node {$l$} (4);

     \path[draw=red,->]  (r0) edge node {} (2);
     \path[draw=red,->]  (r1) edge node  {}  (3);
     \path[draw=red,->]  (r2) edge  node  {}   (4);

     \path[dashed,->]  (r0a) edge node {} (2);
     \path[dashed,->]  (r1a) edge node  {}  (3);
     \path[dashed,->]  (r2a) edge  node  {}   (4);

     \path[->]  (r1f) edge node  {}  (5);
     \path[->]  (r2f) edge  node  {}   (6);
    \path[draw=red,->] (3) edge node[below] {$r$} (nl);
%\path[dotted,->] (1) edge[bend left] node  {$f^{*}$} (5)
 ;
 
 \end{tikzpicture}
 \caption{\textsf{Framing} before unlinking the heap node pointed by the \texttt{current}-$cr$.}
 \label{fig:frameout}
 \end{subfigure}\quad
\begin{subfigure}[b]{.4\linewidth}
 \centering
 \begin{tikzpicture}[>=stealth',node distance=1.3cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]
 \tikzstyle{solids node}=[rectangle,draw=red,inner sep=1.5]
  \tikzstyle{solidss node}=[dashed,rectangle,draw=red,inner sep=1.5]
 \tikzstyle{null node}=[circle,draw=red,fill=red]
 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1.5},
 	blue node/.style={rectangle,draw=black,inner sep=1.5},
 	reader node/.style={circle,draw=black,inner sep=1},
        redreader node/.style={circle,draw=red,inner sep=1},
                rredreader node/.style={dashed,circle,draw=red,inner sep=1},
        readerr node/.style={dashed,circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[solid node] (1) [right of=R] {$H_0$};
       \node[solids node] (2) [right of=1] {$H_1$};
       \node[solidss node] (3) [right of=2] {$H_2$};
       \node[solids node] (4) [right of=3] {$H_3$};
       \node[solid node] (5) [above  of=3] {$H_4$};
       \node[solid node] (6) [above  of=4] {$H_5$};
       \node[null node] (nl) [above right of = 3]{};

       \node[redreader node] (r0) [below  of= 2]  {$pr$};
       \node[rredreader node] (r1) [below  of= 3]  {$cr$};
       \node[redreader node] (r2)  [below  of= 4] {$crl$};

       \node[readerr node] (r0a) [above  of= 1]  {$a_1$};
       \node[readerr node] (r1a) [above   of= 2]  {$a_2$};
       \node[readerr node] (r2a)  [below right of= 4] {$a_3$};

       \node[reader node] (r1f) [above  of= 5]  {$a_4$};
       \node[reader node] (r2f)  [above  of= 6] {$a_5$};

     \path[->]  (R) edge node[below] {$l$} (1);
     \path[->]  (1) edge node[below] {$l$} (2);
     \path[draw=red,->]  (2) edge [bend right] node[below left] {$l$} (4);
     \path[dashed,draw=red,->]  (3) edge node[below] {$l$} (4);
     \path[dashed,->]  (5) edge node {$l$} (3);
     \path[dashed,->]  (6) edge node {$l$} (4);

     \path[draw=red,->]  (r0) edge node {} (2);
     \path[dashed,draw=red,->]  (r1) edge node  {}  (3);
     \path[draw=red,->]  (r2) edge  node  {}   (4);

     \path[dashed,->]  (r0a) edge node {} (2);
     \path[dashed,->]  (r1a) edge node  {}  (3);
     \path[dashed,->]  (r2a) edge  node  {}   (4);

     \path[->]  (r1f) edge node  {}  (5);
     \path[->]  (r2f) edge  node  {}   (6);
     \path[dashed,draw=red, ->] (3) edge node[below] {$r$} (nl);
 ;
 \end{tikzpicture}

 \caption{Safe unlinking of the heap node pointed by the \texttt{current}-$cr$ via \textsf{Framing}}
 \label{fig:unlinkframeout}
 \end{subfigure}
 \end{figure}
\begin{lstlisting}[caption={Unlinking a heap node},label={lst:unlink}, numbers=left, numberstyle=\tiny\color{red}, numbersep=5pt]%, basicstyle=\scriptsize]

....
$\assert{parent:rcuItr\; (Left)^{*} \; \{ Left \mapsto current\} }$
$\assert{current:rcuItr\; (Left)^{*}.Left \; \{Left\mapsto currentL, Right \mapsto null\}}$
$\assert{currentL:rcuItr\; (Left)^{*}.Left.Left \; \{\} }$

parent.Left = currentL;

$\assert{parent:rcuItr\; (Left)^{*} \; \{ Left \mapsto currentL\} }$
$\assert{current:unlinked }$
$\assert{currentL:rcuItr\; (Left)^{*}.Left \; \{\} }$
  
....
\end{lstlisting}

\textit{\textbf{Mutation - Reclaiming a Heap Node after a Grace Period}} - After the heap node pointed by the \texttt{current} pointer is unlinked, the crucial phase with respect to \textsf{RCU} semantic -- grace period for the reader threads -- starts. \textbf{Service} - We start the grace period with \texttt{SyncStart} as we see in the Listing \ref{lst:reclaim}-line\{3\}. In real implementations, \texttt{SynchStart}-\texttt{SyncStop} are one just one call to \texttt{sync\_rcu} to wait the grace period to end so there is no need for a change in the type of the \texttt{current} as we see in the Listing \ref{lst:reclaim}-line\{2,4\}. The change from \textsf{unlinked} to \textsf{freeable} in the type of the \texttt{current} pointer indicates that grace period for the heap node pointed by the \texttt{current} has finished. The grace period ends once the \texttt{SyncStop} returns as seen in the Listing \ref{lst:reclaim}-line\{5\}. Once the grace period ends, It is semantically convenient to to reclaim the heap node pointed by the \texttt{current} via calling \texttt{Free} as seen in the Listing \ref{lst:reclaim}-line\{7\}. We indicate the end of grace period and being able to reclaim the heap node via the change from the \textsf{freeable}, the Listing \ref{lst:reclaim}-line\{4\}, to \textsf{free}, the Listing \ref{lst:reclaim}-line\{6\}, in type of the \texttt{current} pointer. The reason why we type the \texttt{current} pointer as \textsf{freeable} after the grace period is to prevent the ability to call \texttt{Free} before the grace period ends -- we call \texttt{Free} only with a pointer in type \texttt{freeable}.    
\begin{lstlisting}[caption={Reclaiming a heap node after a grace period},label={lst:reclaim}, numbers=left, numberstyle=\tiny\color{red}, numbersep=5pt]%, basicstyle=\scriptsize]

....
$\assert{current:unlinked}$
SyncStart;
$\assert{current:unlinked}$
SyncStop;
$\assert{current:free}$
Free(current);
$\assert{current:undef}$
....

\end{lstlisting}

\textit{\textbf{Creating a Fresh Node}} - In the Listing \ref{lst:alloc}-line\{2\}, we allocate a new node and set its fields line\{4,6\}. The type $\textsf{rcuFresh} \, \N_{\emptyset}$ in the line\{3\} represents the variable \textsf{currentF} pointing to a freshly allocated heap node, fields of which are not so far. \textbf(Service) - A \textsf{rcuFresh} pointer can be used either in setting the fields of a fresh object or linking the fresh object. We will investigate the fresh object linking in the next analysis but, first we anaylze how we set the  fields of the fresh object. In the Listing \ref{lst:alloc}-line\{4,6\}, we set the fields of the object pointed by \texttt{currentF} and we end up having the type in the line\{7\} which seems quite similar to the type \textsf{rcuItr} with empty path. Then the important question to ask is "Why do we need a separate type \textsf{rcuFresh}?". What would happen if we also typed the freshly allocated node with \textsf{rcuItr}? To understand and answer the questions easily, we illustrate the setting in the Listing \ref{lst:alloc} in the Figure \ref{fig:alloc}. The dashed green $H_f$ denotes the freshly allocated heap node pointed by green dashed pointer $cf$ -- line\{2\} in the Listing \ref{lst:alloc}. The green dashed $Left-l$ is set to point to the heap node pointed by the \texttt{currentL} and the green dashed $Right-r$ is set to point the heap node pointed by the \texttt{lmParent}. What if all of these dashed green pointers and heap nodes were black -- Why don't we just use the type \textsf{rcuItr} for heap allocation? If all were black -- which means all the heap nodes are pointed by \textsf{rcuItr} typed variables -- then we would violate \textit{well-shapedness} related invariants of the data structure. In our \textsf{BST} example, we would invalidate invariants such as the single entry point to the data structure -- both \texttt{root} and \textsf{currentF} would be used as entry points -- and the single path to all heap nodes in the data structure -- both $H_2$ and $H_4$ have 2 paths reaching to them. 

Note that we can neither read a \textsf{rcuFresh} variable nor read a field of the object it points. So we do not allow to create aliases to the fresh variable and the object it points. This restriction localizes our reasoning over the effects due to linking to just one fresh pointer and the object it points. Otherwise, we would need to bookeep the aliases of the fresh pointer and the object fields of it because once we linked the fresh object to the data structure via using one of its fresh pointer, the fresh pointer gets the type \textsf{rcuItr} and it would require us to change the aliases' types from \textsf{rcuFresh} to \textsf{rcuItr} to prevent inconsistency in between the types of the aliases.
 \begin{figure}[H]
 \centering
 \begin{tikzpicture}[>=stealth',node distance=1.3cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]
 \tikzstyle{solids node}=[rectangle,draw=red,inner sep=1.5]
  \tikzstyle{solidss node}=[dashed,rectangle,draw=red,inner sep=1.5]
  \tikzstyle{freshollow node}=[dashed,circle,draw=green,inner sep=1]

 \tikzstyle{fresh node}=[dashed,rectangle,draw=green,inner sep=1.5]
  
 \tikzstyle{null node}=[circle,draw=red,fill=red]
 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1.5},
 	blue node/.style={rectangle,draw=black,inner sep=1.5},
 	reader node/.style={circle,draw=black,inner sep=1},
        redreader node/.style={circle,draw=red,inner sep=1},
        readerr node/.style={dashed,circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[solid node] (0) [right of=R] {$H_0$};
       \node[solid node] (1) [right of=0] {$H_1$};
       \node[fresh node] (2) [above of=1] {$H_f$};
       \node[solid node] (3) [right of=1] {$H_2$};
       \node[solid node] (4) [above  of=3] {$H_4$};
       %\node[solid node] (6) [above  of=4] {$H_5$};
       %\node[null node] (nl) [above of = 3]{};

       \node[reader node] (r0) [below  of= 0]  {$pr$};
       \node[reader node] (r1) [below  of= 1]  {$cr$};
       \node[freshollow node] (f)  [left  of= 2] {$cf$};
        \node[reader node] (crl)  [below right  of= 3] {$crl$};
        \node[reader node] (lm) [right  of= 4]  {$lm$};


      % \node[reader node] (r1f) [above  of= 5]  {$a_4$};
      % \node[reader node] (r2f)  [above  of= 6] {$a_5$};

     \path[->]  (R) edge node[below] {$l$} (0);
     \path[->]  (0) edge node[below] {$l$} (1);
     \path[->]  (crl) edge  node {} (3);
     \path[dashed,draw=green,->]  (f) edge node {} (2);
     \path[dashed,draw=green,->]  (2) edge node {$r$} (4);
     \path[dashed,draw=green,->]  (2) edge node {$l$} (3);
     \path[->]  (1) edge node {$r$} (4);
     \path[->]  (1) edge node {$l$} (3);
     
     \path[->]  (r0) edge node {} (0);
     \path[->]  (r1) edge node  {}  (1);
     \path[->]  (lm) edge  node  {}   (4);

     %\path[dashed,->]  (r1a) edge node {} (0);
     %\path[dashed,->]  (r2a) edge node  {}  (1);
     %\path[dashed,->]  (r2a) edge  node  {}   (4);

 %    \path[->]  (r1f) edge node  {}  (5);
     %\path[->]  (r2f) edge  node  {}   (6);
     %\path[draw=red, ->] (2) edge node[below] {$r$} (nl);
 ;
 \end{tikzpicture}
 \caption{Allocating a \textit{fresh} heap node pointed by the \texttt{currentF}-$cf$}
 \label{fig:alloc}
 \end{figure}
\begin{lstlisting}[caption={Allocating a fresh node},label={lst:alloc}, numbers=left, numberstyle=\tiny\color{red}, numbersep=5pt]%, basicstyle=\scriptsize]

....
BinaryTreeNode currentF = new;
$\assert{currentF:rcuFresh }$
currentF.Right = lmParent;
$\assert{currentF:rcuFresh \; \{Right\mapsto lmParent\}}$
currentF.Left = currentL;
$\assert{currentF:rcuFresh \; \{Right\mapsto lmParent, Left\mapsto currentL\}}$
....
\end{lstlisting}

\textit{\textbf{Mutation - Linking a Fresh Node}} - Linking a fresh heap node pointed by a \textsf{rcuFresh} mutates the heap so it needs to handle carefully. To understand the conditions to be satisfied for safe linking, we extend the setting in the Figure \ref{fig:alloc} with some fictional \textit{path-aliases} $a_0$ and $a_1$ to the pointers $pr$ and $cr$ respectively in the Figures \ref{fig:frframeout} and \ref{fig:freshframeout}. We also add fictional \textit{field-aliases} from $H_5$ pointed by $a_5$ to $H_0$ and from $H_6$ pointed by $a_6$ to $H_1$. We do not discuss the problems due to both \textit{path-aliasing} and \textit{field-aliasing} as they are same with ones we discussed for unlinking. Similar to the transition from the Figure \ref{fig:frameout} to \ref{fig:unlinkframeout}, the transition from the Figure \ref{fig:frframeout} to \ref{fig:freshframeout} illustrates the effects of the heap mutation (linking a fresh node). (\textbf{Service}) - It also helps to explain the type rule for linking a fresh node 
\[
\scriptsize
\inferrule[]
{
\rho.f  = \rho'  \qquad \N' = \N'' \qquad  \textsf{FV}(\Gamma) \cap \{p,o,n\}  =\emptyset \\
\lnot(\exists_{x,y \in \Gamma, \rho'',f'} \ldotp (x:\textsf{rcuItr}\,\rho''\,\N'''([f'\rightharpoonup y])) \land ((\rho'' = \rho)\lor(\rho'' = \rho')) \land (y\neq o) )
}
{
\Gamma,\,
 p:\textsf{rcuItr}\, \rho \, \N([f\rightharpoonup o]) \, ,
  o:\textsf{rcuItr}\, \rho' \, \N' \, , n:\textsf{rcuFresh} \, \N''
  \vdash_{M} p.f = n \dashv
  p:\textsf{rcuItr}\, \rho \, \N(f \rightharpoonup o \setminus n) \, ,
  n:\textsf{rcuItr}\, \rho' \, \N'' \,
  o:\unlinked\, ,  \Gamma
}
\]
where we can assume of $p$ as $pr$, $o$ as $cr$ and $n$ as $cf$. The reasoning we do for the \textit{path-aliases} in unlinking is also valid in fresh node linking. We have the framing assertion
\[\lnot(\exists_{x,y \in \Gamma, \rho'',f'} \ldotp (x:\textsf{rcuItr}\,\rho''\,\N'''([f'\rightharpoonup y])) \land ((\rho'' = \rho)\lor(\rho'' = \rho')) \land (y\neq o) )\]
where it prevents path aliasing -- nonexistence of $a_0$ and $a_1$ -- via its portion
\[((\rho'' = \rho)\lor(\rho'' = \rho'))\]
and field mapping aliasing -- nonexistence of any object field in the context $\Gamma$ pointing to $cr$ ($o$ in the type rule) -- via
\[(y\neq o)\]

Among other memory safety issues related to the fresh heap node linking, there is one that we want to raise attention to. When we look at the Figure \ref{fig:frframeout}, we see that same object fields from $H_1$ and $H_f$, which are pointed by $current-cr$ and $currentF-cf$ respectively, point to exactly the same heap nodes $H_2$ and $H_4$, which are pointed by $crl$ and $lm$ respectively. This is asserted in the field mappings of \texttt{current} and \texttt{currentF} in the Listing \ref{lst:fresh}-lined\{3,4\}. We see the same assertion in the type rule as
\[\N' = \N''\]
So, why do we need this assertion? Why do we need to capture all field mappings of the node-to-be-unlinked/replaced by the fresh one's field mappings? In fact, if we did not capture all the field mapping of the node to be unlinked/replaced, then we would leak more heap nodes in addition to the one we intend to e.g. the heap node pointed by $cl$. However, our type system allows mutation of a single heap node at a time. We see, in the Figure \ref{fig:freshframeout}, that the only replaced/unlinked heap node is the one pointed by $cr$. We also observe the change in the type assertions -- from type \textsf{rcuItr} in the Listing \ref{lst:unlink}-line\{3\} to type \textsf{unlinked} in the line\{8\}. We should also note that replacement does not change the reachability of any nodes except the one replaced. This leads to an interesting observation: there is not problem in having many pointers to the heap nodes $H_2$ and $H_4$ as pointers to them do not have change in their path components -- e.g. crl and lm do not have change in their path components. 
 \begin{figure}[H]
 \centering
\begin{subfigure}[b]{.4\linewidth}
 \centering
 \begin{tikzpicture}[>=stealth',node distance=1.3cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]
 \tikzstyle{solids node}=[rectangle,draw=red,inner sep=1.5]
  \tikzstyle{solidss node}=[dashed,rectangle,draw=red,inner sep=1.5]
  \tikzstyle{freshollow node}=[dashed,circle,draw=green,inner sep=1]

 \tikzstyle{fresh node}=[dashed,rectangle,draw=green,inner sep=1.5]
  
 \tikzstyle{null node}=[circle,draw=red,fill=red]
 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1.5},
 	blue node/.style={rectangle,draw=black,inner sep=1.5},
 	reader node/.style={circle,draw=black,inner sep=1},
        redreader node/.style={circle,draw=red,inner sep=1},
        readerr node/.style={dashed,circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[solids node] (0) [right of=R] {$H_0$};
       \node[solids node] (1) [right of=0] {$H_1$};
       \node[fresh node] (2) [above of=1] {$H_f$};
       \node[solid node] (3) [right of=1] {$H_2$};
       \node[solid node] (4) [above  of=3] {$H_4$};
              \node[solid node] (5) [above left of=0] {$H_5$};
       \node[solid node] (6) [above left of = 1]{$H_6$};
      

       \node[redreader node] (r0) [below  of= 0]  {$pr$};
       \node[redreader node] (r1) [below  of= 1]  {$cr$};
       \node[freshollow node] (f)  [above  of= 2] {$cf$};
        \node[reader node] (crl)  [right  of= 3] {$crl$};
       \node[reader node] (lm) [right  of= 4]  {$lm$};
       \node[readerr node] (r1a) [below   of= R]  {$a_0$};
       \node[readerr node] (r2a)  [below of= 3] {$a_1$};

       \node[reader node] (r1f) [above  of= 5]  {$a_5$};
       \node[reader node] (r2f)  [above  of= 6] {$a_6$};

     \path[->]  (R) edge node[below] {$l$} (0);
     \path[draw=red,->]  (0) edge node[below] {$l$} (1);
     \path[->]  (crl) edge  node {} (3);
     \path[dashed,draw=green,->]  (f) edge node {} (2);
     \path[dashed,draw=green,->]  (2) edge node {$r$} (4);
     \path[dashed,draw=green,->]  (2) edge node {$l$} (3);


     \path[dashed,->]  (5) edge node {$l$} (0);
     \path[dashed,->]  (6) edge node {$l$} (1);


     \path[draw=red,->]  (1) edge node {$r$} (4);
     \path[draw=red,->]  (1) edge node {$l$} (3);
     
     \path[draw=red,->]  (r0) edge node {} (0);
     \path[draw=red,->]  (r1) edge node  {}  (1);
     \path[->]  (lm) edge  node  {}   (4);

     \path[dashed,->]  (r1a) edge node {} (0);
     \path[dashed,->]  (r2a) edge node  {}  (1);
     
     \path[->]  (r1f) edge  node  {}   (5);
     \path[->]  (r2f) edge  node  {}   (6);


     %\path[draw=red, ->] (2) edge node[below] {$r$} (nl);
 ;
 \end{tikzpicture}

 \caption{Safe linking of the \textit{fresh} heap node pointed by the \texttt{currentF}-$cf$}
 \label{fig:frframeout}
 \end{subfigure} \quad
 \begin{subfigure}[b]{.4\linewidth}
 \centering
 \begin{tikzpicture}[>=stealth',node distance=1.3cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]
 \tikzstyle{solids node}=[rectangle,draw=red,inner sep=1.5]
  \tikzstyle{solidss node}=[dashed,rectangle,draw=red,inner sep=1.5]
  \tikzstyle{freshollow node}=[dashed,circle,draw=green,inner sep=1]

 \tikzstyle{fresh node}=[dashed,rectangle,draw=green,inner sep=1.5]
  
 \tikzstyle{null node}=[circle,draw=red,fill=red]
 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1.5},
 	blue node/.style={rectangle,draw=black,inner sep=1.5},
 	reader node/.style={circle,draw=black,inner sep=1},
        redreader node/.style={circle,draw=red,inner sep=1},
        readerr node/.style={dashed,circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1},
               rredreader node/.style={dashed,circle,draw=red,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[solids node] (0) [right of=R] {$H_0$};
       \node[solidss node] (1) [right of=0] {$H_1$};
       \node[solid node] (2) [above of=1] {$H_f$};
       \node[solid node] (3) [right of=1] {$H_2$};
       \node[solid node] (4) [above  of=3] {$H_4$};
       \node[solid node] (5) [above of=R] {$H_5$};
       \node[solid node] (6) [above of = 0]{$H_6$};

       \node[redreader node] (r0) [below  of= 0]  {$pr$};
       \node[rredreader node] (r1) [below  of= 1]  {$cr$};
       \node[reader node] (f)  [above  of= 2] {$cf$};
        \node[reader node] (crl)  [ right  of= 3] {$crl$};
       \node[reader node] (lm) [right  of= 4]  {$lm$};
       \node[readerr node] (r1a) [below   of= R]  {$a_0$};
       \node[readerr node] (r2a)  [below of= 3] {$a_1$};

      \node[reader node] (r1f) [above  of= 5]  {$a_5$};
      \node[reader node] (r2f)  [above  of= 6] {$a_6$};

     \path[->]  (R) edge node[below] {$l$} (0);
    % \path[draw=red,->]  (0) edge node[below] {$l$} (1);
     \path[->]  (crl) edge  node {} (3);
     \path[->]  (f) edge node {} (2);
     \path[->]  (2) edge node {$r$} (4);
     \path[->]  (2) edge node {$l$} (3);
     \path[dashed,draw=red,->]  (1) edge node {$r$} (4);
     \path[dashed,draw=red,->]  (1) edge node {$l$} (3);




     \path[draw=red,->]  (r0) edge node {} (0);
     \path[dashed,draw=red,->]  (r1) edge node  {}  (1);
     \path[->]  (lm) edge  node  {}   (4);

     \path[dashed,->]  (r1a) edge node {} (0);
     \path[dashed,->]  (r2a) edge node  {}  (1);
          \path[dashed,->]  (5) edge node {$l$} (0);
     \path[dashed,->]  (6) edge node {$l$} (1);


     %\path[dashed,->]  (r2a) edge  node  {}   (4);

     \path[draw=red,->]  (0) edge node  {$l$}  (2);


     \path[->]  (r1f) edge  node  {}   (5);
     \path[->]  (r2f) edge  node  {}   (6);


 ;
 \end{tikzpicture}

 \caption{Safe replacement of the heap node pointed by \texttt{current}-$cr$ by the \textit{fresh} heap node pointed by the \texttt{currentF}-$cf$}
 \label{fig:freshframeout}
 \end{subfigure}
 \end{figure}
\begin{lstlisting}[caption={Replacing a heap node with a fresh one},label={lst:fresh}, numbers=left, numberstyle=\tiny\color{red}, numbersep=5pt]%, basicstyle=\scriptsize]

....
$\assert{parent:rcuItr\; (Left|Right)^{*} \; \{ Left\mapsto current\} }$
$\assert{current:rcuItr\; (Left|Right)^{*}.Left \; \{Right\mapsto lmParent, Left \mapsto currentL \} }$
$\assert{currentF:rcuFresh \; \{Right\mapsto lmParent, Left\mapsto currentL\}}$
//current's right child a left child of parent
parent.Left = currentF; 
$\assert{parent:rcuItr\; (Left|Right)^{*} \; \{ Left\mapsto currentF\} }$
$\assert{current:unlinked }$
$\assert{currentF:rcuItr \; (Left|Right)^{*}.Left \; \{Right\mapsto lmParent, Left\mapsto currentL\}}$
....
\end{lstlisting}

%\;\;

%%%%%%%%%%%%%%%%%%%%%%%%SUB TYPING JUDGEMENTS%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
\scriptsize{
\begin{mathpar}
\typelocalmap \and \typeglobal \and \rcutypes \and \types \and  \ftypedecl \and
\pth \and  \cpath \and \rpath \and \rpth 
\end{mathpar}
\medskip
%%%%%%%%%%%%%%%%%%%%
\fbox{$\vdash \, \N \subt \N'$} \;\;
$
\inferrule
{
\text{T} = \textsf{rcuItr} \, \rho \, \N([f_2 \rightharpoonup y]) \;\;
 \text{T}'=\textsf{rcuItr} \, \rho \, \N'([f^{*} \rightharpoonup y])
}
{\vdash \, \N \subt \N'}
\;(\textsc{T-NSub2})
$
\medskip
$
\inferrule
{
\text{T} = \textsf{rcuItr} \, \rho \, \N([f_1 \rightharpoonup y]) \;\;
 \text{T}'=\textsf{rcuItr} \, \rho \, \N'([f^{*} \rightharpoonup y])
}
{\vdash \, \N \subt \N'}
\;(\textsc{T-NSub1})
$
\medskip
%%%%%%%%%%%%%%%%%%%%
\fbox{$\vdash \, \rho \subt \rho'$} \;\;
$
\inferrule
{
\rho' = \rho.\rho''
}
{
 \vdash  \rho \subt \rho'
}
\;(\textsc{T-PSub1})
$
\medskip
$
\inferrule
{
\rho' = \rho.\rho''
}
{
 \vdash  \rho'' \subt \rho'
}
\;(\textsc{T-PSub2})
$
\medskip
%%%%%%%%%%%%%%%%%%%%
$
\inferrule
{
}
{
\vdash  \rho \subt \rho
}
\;(\textsc{T-PSub3})
$
\medskip
%%%%%%%%%%%%%%%%%%%%
$
\inferrule
{
\vdash  \rho \subt \rho'' \;\; \vdash  \rho'' \subt \rho'
}
{
\vdash  \rho \subt \rho'
}
\;(\textsc{T-PSub4})
$
\medskip
%%%%%%%%%%%%%%%%%%%%
\fbox{$\vdash \, T \subt T'$} \;\;
$
\inferrule
{
}
{
\vdash \textsf{rcuItr}\; \_   \subt \textsf{undef}
}
\;(\textsc{T-TSub})
$
\medskip
%%%%%%%%%%%%%%%%%%%%
$
\inferrule
{
\vdash\rho\subt \rho' \qquad \vdash \N \subt \N'
}
{
\vdash \textsf{rcuItr} \, \rho \, \N  \subt   \textsf{rcuItr} \, \rho' \, \N'
}
\;(\textsc{T-NPSub})
$
\medskip
%%%%%%%%%%%%%%%%%%%%
\fbox{$\vdash \, \Gamma \subt \Gamma'$} \;\;
$
\inferrule
{
\vdash\Gamma \subt \Gamma' \;\; \vdash \text{T}  \subt \text{T'}
}
{
\vdash \Gamma\, , x:\text{T}  \subt \Gamma'\, , x:\text{T'}
}
\;(\textsc{T-CSub})
$
\medskip
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
$
\inferrule
{
}
{
\vdash  \epsilon \subt \epsilon
}
\;(\textsc{T-ESub})
$
\medskip
%%%%%%%%%%%%%%%%%%%%
}
\caption{Sub-Typing Judgements}
\label{fig:sub-typing}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%SUB TYPING JUDGEMENTS ENDS%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%TYPE JUDEGEMENT%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*} \scriptsize
\begin{mathpar}
 \fmapextendn \and
\fmapname  \and \fmapdiff \and \fmapwithf \and \fmapextend \and \fmapempty \and \fmapfieldemp
\end{mathpar}
\medskip
%%%%%%%%%%%%%%%%%%%%
\begin{mathpar}
\fbox{$\Gamma \vdash s \dashv \Gamma'$}
\and
\inferrule[\scriptsize(T-Root)]
{ \textsf{FV}(\Gamma) \cap \{r,y\}  =\emptyset}
{\Gamma\,,r:\textsf{rcuRoot}\,,y:\textsf{undef} \vdash_{M,R} y = r \dashv y: \textsf{rcuItr}\, \epsilon \, \N_{\emptyset}\,,r:\textsf{rcuRoot}\,,\Gamma}
\and
\inferrule[\scriptsize(T-ReadS)]
{ \textsf{FV}(\Gamma) \cap \{z,x\}  =\emptyset}
{
\Gamma\,,  z:\textsf{rcuItr}\,\_ \, ,\rcuitrT{x}{G}{k}{k+1}{\_} \vdash_{M,R} z=x \dashv  \rcuitrT{x}{G}{k}{k+1}{\_}\, , \rcuitrT{z}{G}{k}{k+1}{\_} \,, \Gamma
}
\and
\inferrule[\scriptsize(T-ReadH)]
{
\rho.f=\rho' \\
 \textsf{FV}(\Gamma) \cap \{z,x\} =\emptyset
}
{
 \Gamma\, , z:\textsf{rcuItr}\,\_ \,,  x:\textsf{rcuItr} \, \rho \, \N   \vdash_{M,R}
 	z=x.f
 \dashv  x:\textsf{rcuItr} \, \rho \, \N([f\rightharpoonup z])\, ,z:\textsf{rcuItr} \, \rho' \, \N_{\emptyset} \, , \Gamma
}
\and
\inferrule[\scriptsize(T-Alloc)]
{
\mathsf{FV}(\Gamma) \cap \{x\} = \emptyset
}
{
 \Gamma\,, x:\textsf{undef} \vdash_{M} x = \NEW \dashv x:\textsf{rcuFresh} \, \N_{\emptyset} \, ,  \Gamma
}
\and
\inferrule[\scriptsize(T-Free)]
{
}
{
x:\textsf{free} \vdash_{M} \textsf{Free}(x) \dashv x:\textsf{undef}
}
\and
\inferrule[\scriptsize(T-SyncStart)]
{
}
{
\Gamma \vdash_{M} \textsf{SyncStart} \dashv \Gamma
}
\and
\inferrule[\scriptsize(T-SyncStop)]
{
\Gamma' = \forall x:\textsf{unlinked} \in \Gamma \ldotp \Gamma \setminus \{x:\textsf{unlinked}\} \cup \{x:\textsf{freeable}\}
}
{
\Gamma \vdash_{M} \textsf{SyncStop} \dashv \Gamma'
}
\and
\inferrule[\scriptsize(T-Exchange)]
{
 \Gamma, \, y:T' , \, x:T, \, \Gamma' \vdash \bar{s} \dashv   \Gamma''
}
{
\Gamma, \, x:T , \, y:T' , \, \Gamma' \vdash \bar{s} \dashv   \Gamma''
}
\and
\inferrule[\scriptsize(T-WriteFH)]
{
\textsf{FV}(\Gamma) \cap \{p,z,x\}  =\emptyset
}
{
 \Gamma, p:\textsf{rcuFresh}\,\N_{f,\emptyset},\; x:\textsf{rcuItr}\;\; \rho \;\; \N([f\rightharpoonup z])
  \vdash_{M} p.f = x.f \dashv
  \rcunf{p}{f}{z} \, , x:\textsf{rcuItr}\, \rho \, \N([f\rightharpoonup z]), \, \Gamma
}
\and
\inferrule[\scriptsize(T-UnlinkH)]
{
\textsf{FV}(\Gamma) \cap \{x,z,r\} \qquad \rho.f_1=\rho' \;\; \rho'.f_2=\rho'' \qquad \forall_{f\in dom(\N')} \ldotp f\neq f_2 \implies \N'([f\rightharpoonup \textsf{null}])   \\
\lnot(\exists_{n,m \in \Gamma, p''',f}\ldotp n:\textsf{rcuItr}\,\rho'''\,\N'''([f\rightharpoonup m]) \land ((\rho = \rho''') \lor (\rho' = \rho''') \lor (\rho''=\rho''') ) \land \{m\} \cap \{z,r\} \neq \emptyset  )
}
{
\Gamma,\,x:\textsf{rcuItr}\, \rho \, \N([f_1\rightharpoonup z]) \, ,
z:\textsf{rcuItr}\, \rho' \, \N'([f_2\rightharpoonup r]) \, ,  r:\textsf{rcuItr} \, \rho'' \, \N''\, 
\vdash_{M} x.f_1=r \dashv
z:\unlinked\, ,
x:\textsf{rcuItr} \, \rho \, \N(f_1\rightharpoonup z \setminus r)\, ,
r:\textsf{rcuItr} \, \rho' \, \N'',\, \Gamma
}
\and
\inferrule[\scriptsize(T-LinkF)]
{
\rho.f  = \rho'  \qquad \N' = \N'' \qquad  \textsf{FV}(\Gamma) \cap \{p,o,n\}  =\emptyset \\
\lnot(\exists_{x \in \Gamma, \rho'',f',y} \ldotp (x:\textsf{rcuItr}\,\rho''\,\N'''([f'\rightharpoonup y])) \land ((\rho'' = \rho)\lor(\rho'' = \rho')) \land (y\neq o) )
}
{
\Gamma,\,
 p:\textsf{rcuItr}\, \rho \, \N([f\rightharpoonup o]) \, ,
  o:\textsf{rcuItr}\, \rho' \, \N' \, , n:\textsf{rcuFresh} \, \N''
  \vdash_{M} p.f = n \dashv
  p:\textsf{rcuItr}\, \rho \, \N(f \rightharpoonup o \setminus n) \, ,
  n:\textsf{rcuItr}\, \rho' \, \N'' \,
  o:\unlinked\, ,  \Gamma
}
\and
\inferrule[\scriptsize(T-Seq)]
{
\Gamma_1 \vdash \bar{s_1} \dashv_{M,R}   \Gamma_2  \qquad   \Gamma_2 \vdash_{M,R} \bar{s_2} \dashv   \Gamma_3
}
{
\Gamma_1  \vdash_{M,R} \bar{s_1} \; ; \; \bar{s_2} \dashv  \Gamma_3
}
\and
\inferrule[\scriptsize(T-Par)]
{
 \Gamma_1 \vdash_{R} \bar{s_1} \dashv   \Gamma'_1  \qquad   \Gamma_2 \vdash_{M,R} \bar{s_2} \dashv   \Gamma'_2
}
{
 \Gamma_1, \; \Gamma_2  \vdash \bar{s_1} || \bar{s_2} \dashv  \Gamma'_1 \; , \Gamma'_2
}
\and
\inferrule[\scriptsize(T-Skip)]
{
}
{
 \Gamma \vdash_{M,R} \textsf{skip} \dashv   \Gamma
}
\end{mathpar}
\caption{Type Judgements}
\label{fig:type-judgements}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%TYPE JUDGEMENTS ENDS%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%COND TYPE JUDGEMENTS%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
\scriptsize
\begin{mathpar}
\fbox{$\Gamma \vdash \bar{s} \dashv \Gamma'$} \and
\inferrule[\scriptsize(T-Branch1)]
{
  x.f_1==z \and
 \Gamma\, ,x:\textsf{rcuItr}\,\rho \, \N([f_1 \rightharpoonup  z]) \vdash \bar{s}_1 \dashv\Gamma_4 \and
  \Gamma\, ,x:\textsf{rcuItr}\, \rho \, \N([f_2 \rightharpoonup z]) \vdash \bar{s}_2 \dashv \Gamma_4
}
{
\Gamma\, ,x:\textsf{rcuItr}\, \rho \, \N([f_1\mid f_2 \rightharpoonup z]) \vdash \textsf{if}(x.f_1==z)  \textsf{ then } \bar{s}_1 \textsf{ else } \bar{s}_2 \dashv \Gamma_4
}
\and
\inferrule[\scriptsize(T-Branch2)]
{
\Gamma(x)= \textsf{bool} \\
 \Gamma \vdash \bar{s}_1 \dashv\Gamma' \and \Gamma \vdash \bar{s}_2 \dashv \Gamma'
}
{
\Gamma \vdash \textsf{if}(x) \textsf{ then } \bar{s}_1  \textsf{ else } \bar{s}_2 \dashv \Gamma'
}
\and
\inferrule[\scriptsize(T-Branch3)]
{
 \Gamma,\,x:\textsf{rcuItr} \, \rho \, \N([f\rightharpoonup \textsf{null}]) \vdash \bar{s}_1 \dashv \Gamma' \and \Gamma,\,x:\textsf{rcuItr} \, \rho \, \N([f\rightharpoonup \_]) \vdash \bar{s}_2 \dashv \Gamma'
}
{
\Gamma,\,x:\textsf{rcuItr} \, \rho \, \N([f\rightharpoonup \_]) \vdash \textsf{if}(x.f == \textsf{null}) \textsf{ then } \bar{s}_1  \textsf{ else } \bar{s}_2 \dashv \Gamma'
}
\and
\inferrule[\scriptsize(T-Frame)]
{
\Gamma_1 \vdash \bar{s} \dashv \Gamma_2   \and
\textsf{WellFramed}(\Gamma, \Gamma_1) \and \textsf{WellFramed}(\Gamma, \Gamma_2)
}
{
\Gamma, \; \Gamma_1 \vdash \bar{s} \dashv \Gamma, \; \Gamma_2
}
\and
\inferrule[\scriptsize(T-Conseq)]
{
 \Gamma \subt \Gamma'  \and \Gamma' \vdash \bar{s} \dashv \Gamma'' \and \Gamma'' \subt \Gamma'''
}
{
 \Gamma \vdash \bar{s} \dashv \Gamma'''
}
\and
\inferrule[\scriptsize(T-Loop1)]
{
\Gamma(x) = \textsf{bool} \and
\Gamma \vdash \bar{s} \dashv \Gamma 
}
{
\Gamma \vdash \textsf{while}(x)\{\bar{s}\} \dashv  \Gamma
}
\and
\inferrule[\scriptsize(T-Loop2)]
{
\Gamma,\, x:\textsf{rcuItr}\;\rho \; \N([f\rightharpoonup \_]) \vdash \bar{s} \dashv \Gamma, x:\textsf{rcuItr}\;\rho' \; \N([f\rightharpoonup \_])
}
{
\Gamma,\, x:\textsf{rcuItr}\;\rho \; \N([f\rightharpoonup \_]) \vdash \textsf{while}(x.f \neq \textsf{null})\{\bar{s}\} \dashv   x:\textsf{rcuItr}\;\rho' \; \N([f\rightharpoonup \textsf{null}]) ,\,  \Gamma
}
\end{mathpar}
\caption{Type Judgements for Control-Flow.}
\label{fig:type-judgements-for-cf}
\end{figure*}
%%%%%%%%%%%%%%%COND TYPE JUDGEMENTS ENDS%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
(\textit{\textbf{Transitions in between}} \textsf{rcu} \textit{\textbf{and}} \textsf{normal} \textit{\textbf{Types}}) - There are two rules shown in the Figure \ref{fig:transitionsbetweendifferenttypesystems} for moving between the different type systems: one for entering a write region, and one for a read region. The type rules for outside an RCU region are otherwise straightforward and restrict $\Gamma$ to only mention variables of type $\textsf{normal}$; that is, we cannot read or write to rcu structures.

%%%%%%%%%%%%%%TYPE SYSTEM TRANSITIONS%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
\scriptsize{
\medskip
%%%%%%%%%%%%%%%%%%%%
$
\inferrule
{
\Gamma\, , y : \textsf{rcuItr} \vdash_R \bar{s} \dashv \Gamma'
}
{
\Gamma \vdash \textsf{RCURead}\, x.f \textsf{ as }y\textsf{ in }\{\bar{s}\}
}
\;(\textsc{ToRCURead})
$
\medskip
%%%%%%%%%%%%%%%%%%%%
$
\inferrule
{
 \Gamma\, , y : \textsf{rcuItr} \vdash_M \bar{s} \dashv \Gamma' \;\; \ftype{}{\textsf{rcu}} \;\;  \textsf{NoFresh}(\Gamma') \;\; \textsf{NoUnlinked}(\Gamma')
}
{
\Gamma \vdash \textsf{RCUWrite}\, x.f \textsf{ as }y\textsf{ in } \{ \bar{s} \}
}
\;(\textsc{ToRCUWrite})
$
\medskip
%%%%%%%%%%%%%%%%%%%%
}
\caption{RCU and Normal Type Systems}
\label{fig:transitionsbetweendifferenttypesystems}
\end{figure*}






































%%%%%Old stuff%%%%%%%%%%%%%%%%%
\begin{comment}
This section defines and explains the type rules for programs written with  RCU types defined in section \ref{subsection:subsec-types}. We start with explaining the type rules for the atomic actions shown in the figure \ref{fig:type-judgements}. Next, we introduce the subtyping relations shown in the figure \ref{fig:sub-typing} together with explaining the type rules for control flow constructs of programming languages shown in the figure \ref{fig:type-judgements-for-cf}.
\paragraph{Mutation on heap} \textsc{T-WriteFH} ensures that field of a \textsf{rcuFresh} typed variable is written properly. In figure \ref{fig:del2.2} \textsf{rcuFresh} typed $f'$ has its fields set to fields of a variable, $k$, in type \textsf{rcuItr}. This means that fields of \textsf{rcuFresh} typed variables are set to point to valid heap locations. At this point, we need to raise the attention to the fact that both \textsf{rcuFresh} and \textsf{rcuItr} are type representations for valid \textsf{RCU} heap locations but only one \textsf{rcuItr} typed pointer can access to the \textsf{RCU} data structure. The importance of this subtlety shows up in reasoning on the well-formedness of the data structure in the heap. For instance, in figure \ref{fig:del2.2}, there seems to be two access points to the tree which seems to violate well-formedness of the binary search tree but we actually know that there is no way to access the rest of the \textsf{RCU} data structure via \textsf{rcuFresh} pointer. \textsc{T-LinkF} rules ensures proper linking of a fresh heap location to the \textsf{RCU} data structure which is basically the transition from figure \ref{fig:del2.2} to \ref{fig:del2.3}. To make this transition properly, we need to make sure that all fields of the unlinked node, $k$, is captured by the fields of the variable in type \textsf{rcuFresh}, $f'$. This prevents memory leakage during fresh heap node linking. \textsc{T-LinkFH} ensures safe linking of a fresh heap node into the \textsf{RCU} data structure where no unlinking occurs as pointing field of the fresh node is convenient to have all nodes linearized on the same path after linking.\textsc{T-UnlinkH} ensures proper unlinking of a node inside \textsf{RCU} data structure. It allows us to ensure that there exists memory leakage only for the unlinked heap which needs \emph{grace} to be shown by writer thread. The rule provides this guarantee through enforcing all other fields of the node we unlinked to be \textsf{null} as shown in transition from figure \ref{fig:del1.1} to \ref{fig:del1.2}.
\input{chapters/FigBSTDeleteOneChildAnom.tex}
\input{chapters/FigBSTDeleteTwoChildAnom.tex}
\paragraph{Grace period and destroying memory} \textsc{T-SyncStart} and \textsc{T-SyncStop} ensure that type context is not changed during the grace period. \textsc{T-Free} ensures the correct memory reclamation under \textsf{RCU} setting by asserting that the heap node to be reclaimed must be in type of \textsf{unlinked}.
\paragraph{Sub-Type Rules} Subtying relation in our types has two folds 
\begin{itemize}
\item \textsc{T-TSub} is the relation between \textsf{rcuItr} and \textsf{undef}. The most crucial point that we want to capture with this relation is typing of the reclaimed memory locations with aliases. For instance, when we consider the following code snippet, which unlinks and the reclaims the memory location pointed by both \texttt{itr} and \texttt{itrC}
\begin{lstlisting}[style=nonumbers]
....
$\assert{\rcuit{prev}{}{\rho'}{\{next\mapsto itr\}}}$
$\assert{\rcuit{itr}{}{\rho'.next}{\{next\mapsto itrN\}}}$
node_p <rcuItr>* itrC = itr;
$\assert{\rcuit{itr}{}{\rho'.next}{\{next\mapsto itrN\}}}$
$\assert{\rcuit{itrC}{}{\rho'.next}{\{next\mapsto itrN\}}}$
node_p <rcuItr>*  prev->next = itrN;
$\assert{ \texttt{itr}:\textsf{unlinked}}$
SyncStart;
SyncStop;
Free(itr);
$\assert{ \texttt{itr}:\textsf{undef}}$
//Crucuial point in typing itrC
....
\end{lstlisting}
At this point the typing for \texttt{itrC}, which is an alias with \texttt{itr} is handled with subtyping relation in between \textsf{undef} and \textsf{rcuItr}.

\item \textsc{T-NBSub} is the relation defined over each component of \textsf{rcuItr} type where:
\begin{itemize}
\item Relations \textsc{T-PSub1-3} are defined over path-$\rho$. Subtyping relation over paths is crucial for typing loop structures. We do abstraction over the number of times that loop is executed and typing of \texttt{itr} is handled with subtyping relations over path. 
\begin{lstlisting}[style=nonumbers]
....
$\assert{head:\mathsf{rcuRoot}}$
node_p <rcuItr>* itr = head;
$\assert{head:\mathsf{rcuRoot}}$
$\assert{\rcuit{itr}{}{\epsilon}{\{\}}}$
while(*){
	 itr = itr->next;
}
$\assert{\rcuit{itr}{}{\rho^{k}}{\{\}}}$  
....
\end{lstlisting}
\item Relations \textsc{T-NSub1-2} are defined over field map-$\N$. Subtyping relation over field mappings is crucial for typing conditional structures. We do abstraction over the field names in field mappings via providing a mapping from set of field names instead of single field name. For instance,
\begin{lstlisting}[style=nonumbers]
....
$\assert{head:\mathsf{rcuRoot}}$
node_p <rcuItr>* itr = head;
node_p <rcuItr>* itrN = itr->left;
$\assert{head:\mathsf{rcuRoot},\rcuit{itr}{}{\epsilon}{\{left\mapsto itrN\}}}$
$\assert{ \rcuit{itrN}{}{left}{\emptyset} }$
if(itr->left == itrN){
	 itr->left = itrN;
	itrN = itrN->left;
}
else{
	itr->right = itrN
	itrN= itrN->right;
}
$\assert{\rcuit{itr}{}{\epsilon}{\{left | right \mapsto itrN\}}}$  
$\assert{\rcuit{itrN}{}{\rho}{\emptyset}}$
....
\end{lstlisting}
We use subtyping relation to handle the typing of conditinals, specifically typing of \texttt{itr} and \texttt{itrN} before and after the execution of conditional statement.  
\end{itemize}
\end{itemize}
Subtyping is lifted up to the type contexts in rule \textsc{T-CSub}.
\paragraph{Control-Flow-Type Rules} Our typing rules for loop and conditional statements are standard rules. As explained corner cases for these statements are captured with subtyping relations. 

\end{comment}

\begin{comment}

\textsf{rcuFresh} represents a pointer to a freshly allocated object.
\[\rcunfdecl\]
Similar to the \textsf{rcuItr} type, It keeps a field map  as a compnent of the type but it does not keep path component as \textsf{rcuItr} does. For example, suppose that we have a variable $x$ in type \textsf{rcuItr} with the components $\rho$ and $\N[\text{next}\rightharpoonup y]$ and a newly allocated heap pointed by a fresh variable $z$ in type \textsf{rcuFresh} with field map component $\N_{\emptyset}$. Setting fields of a fresh variable is more interesting than allocating the space in the heap for it. We consider the case where we set $z$'s \texttt{next} field to to be showing $x$'s \texttt{next} field


where \textsf{next} of $x$ and $z$ is in domain of field maps of \textsf{rcuItr} and \textsf{rcuFresh} respectively. We would like to raise attention to the following points:
\begin{itemize}
\item Accessing two fields shown in the listing above is valid as \textsf{rcuFresh} type and its field maps are thread local. Actually there exists only one heap access which is $\text{x}\mapsto\text{next}$.
\item There is still no access to the \textsf{rcu} data structure from $z$ as field names inside \textsf{rcuFresh} type's field maps are thread local.
\end{itemize}
Once we link the $z$ to be shown by \texttt{next} field of the $x$

we make $z$ observed as part of \textsf{RCU} heap as its type is change from \textsf{rcuFresh} to \textsf{rcuItr}. We also see the harmony in using \textsf{rcuFresh} and \textsf{rcuItr} in \emph{Binary Search Tree}. In figure \ref{fig:del2.2}, $f'$ is a new allocated heap node which is the copy of $k'$. The state of the BST in figure \ref{fig:del2.2} seems not to be in \emph{wellformed} state as there seems to be two roots of the tree and unique reachability paths of the nodes from the root of the BST seems invalid. However, as we know that \textsf{rcuFresh} is thread local or another way of saying is that $f'$ is not published as \textsf{rcuItr} yet so \emph{wellformed} is still preserved.

\end{comment}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%OLD TYPE RULES%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\medskip
%%%%%%%%%%%%%%%%%%%%
$
\inferrule
{
 \ftype{ }{\textsf{rcu}} \qquad \mid\rho\mid + 1= \mid \rho' \mid  \qquad \mid \rho' \mid + 1 = \mid \rho'' \mid \qquad \rho.f=\rho'\qquad \rho'.f=\rho''\qquad\textsf{FV}(\Gamma) \cap \{z,x,r\}  =\emptyset\qquad\;(\textsc{T-LinkFH})
}
{
 \Gamma\, ,
z:\textsf{rcuItr}\, \rho \, \N([f\rightharpoonup x]) \, ,
x:\textsf{rcuItr}\, \rho' \, \N \, ,
r:\textsf{rcuFresh} \, \N([f\rightharpoonup x]) \,
  \vdash_{M} z.f = r \dashv
z:\textsf{rcuItr}\, \rho \, \N(f\rightharpoonup x\setminus r) \,,
r:\textsf{rcuItr}\, \rho' \, \N([f\rightharpoonup x]) \, ,
x:\textsf{rcuItr}\, \rho'' \, \N
 \, , \Gamma
}
%\;(\textsc{T-LinkFH})
$
\end{comment}


==> chapters/RCUProgLangNew_v1.tex <==
\makeatletter % allow us to mention @-commands
\def\arcr{\@arraycr}
\makeatother
\section{Type System \& Programming Language}
In this section, we present a simple object oriented programming language with two block constructs for modelling \textsf{RCU}. We provide a programming language and a type system to enforce correct usage of RCU primitives. In the following subsections, We stress two aspects of our type system.
First, to ensure memory safety, we must show how our type system makes programs preserve the following two properties:
\begin{itemize}
\item A heap node can only be freed, if it is no longer accessible from an RCU data structure
\item Local variables may not point inside an RCU data structure unless they are inside an \textsf{RCU} read or write block
\end{itemize}
To achieve this we ensure the reachability and access which can be suitably restricted. We explain how our types support a delayed ownership transfer for the deallocation.
Second, to ensure that our type system can type useful programs, we must show how it works on well known data structures such as binary search trees and list-based bags. To achieve the level of expressibility for typing these data structures, we use a refinement types like system to ensure having approximation on loop abstractions and control flow joins.
In our system, all objects contain all fields.  This means we do not have to worry about the correct typing of field manipulation, etc. which is covered by a standard type system such as found in C. We will only focus on the aspects of the typing related to the correct operation of RCU. This means our type system extends C like languages' type systems which can handle standard type errors such as field not-exists.
We explain the two main aspects of our type system in the following subsections. In Section \ref{subsection:rcu-typing} we introduce the \textsf{RCU} types and the need for substyping. In Section \ref{subsection:type-action}, we see how types represent programs via showing the code snippets from our type checking effort list-based bag example. Then, in Section \ref{subsection:type-rules}, we discuss possible memory safety issues in the \textsf{RCU} setting, introduce the type rules and how they prevent these issues. At last, we discuss our type system by code fragments peculiar to the \textsf{BST}. 
\subsection{\textsf{RCU} Typing}
\label{subsection:rcu-typing}
Here, we present an high-level introduction of the types in our system. There are five types of local variable
\[
\tau_{local} ::=  \textsf{rcuItr}\;\rho\;\N \mid \textsf{rcuFresh}\;\N  \mid \textsf{unlinked} \mid \textsf{undef} \mid \textsf{freeable}
\]
and we assume a function, $\textsf{FType}$ that maps each field to its type. In addition, we have a type for global variables
\[\tau_{global} ::= \textsf{rcuRoot}\]
\textit{\textbf{rcuItr}} -is the type given to references pointing into a shared RCU data structure. An \textsf{rcuItr} reference can be used in either a read or write region. It indicates both that the reference points into the shared \textsf{RCU} data structure and that the heap location referenced by the \textsf{rcuItr} reference is reachable by following the following the path $\rho$ from the root. A component $\N$ is a set of field mappings taking the field name to local variable names. Field mappings are added to the set when the object's fields are read. Field mapping set and path components are important for keeping track of heap locations through \textit{reached-by} and \textit{points-to} relations so that effects of mutations using references in \textsf{rcuItr} type are localized.
In general, we utilize path information to ensure that we preserve well shaped heap for the data structures, e.g. acyclicity. In conjuction with the path component, we employ the field mappings to assist in checking whether proper linking/mapping exists between the related nodes shown by the pointers when unlinking occurs.

\textit{\textbf{unlinked}} - is the type given to references pointing at unlinked heap locations inside an \textsf{RCU} write block. An object reference by a reference in unlinked type means that the object is now disconnected from the data structure, unreachable. A heap location referenced by unlinked reference may also be accessed by reader threads using a reference in \textsf{rcuItr} simultaneously. This means that an object referenced by an unlinked reference may reside in the free list which defers reclamation/deallocation of the object until all reader threads pointing to the object simultaneously at the time of unlinking  are done with the object. However, from now on the object is inaccessible for the incoming reader threads.

\textit{\textbf{freeable}} - is the type given to references pointing at unlinked heap location which is convenient to reclaim as there are no reader threads to wait. This enforces the right time -- after syncronising with all readers threads on the object (to be reclaimed) exit the \textsf{RCU} read block -- to reclaim the object in the \textsf{RCU} setting. Only freeable objects can be reclaimed.

\textit{\textbf{undef}} - is the type given to references where the content of the referenced location is inaccessible. A freeable object becomes undefined after it is reclaimed.

\textit{\textbf{rcuFresh}} - is the type given to references pointing at freshly allocated heap location. Similar to the \textsf{rcuItr} type, it has field mappings set $\N$. We set the field mappings in the set of an existsing \textsf{rcuFresh} reference to be the same as field mappings in the set of an \textsf{rcuItr} reference when we replace the heap referenced by the \textsf{rcuItr} with the heap referenced by \textsf{rcuFresh} for memory safe replacement.

\textit{\textbf{rcuRoot}} - is the type given to references pointing at the heap location which is the data structure unique global root. An undefined reference can be loaded with a value -- it becomes \textsf{rcuItr} -- once we read the global unique root to it.
%%%%%%%%%%%%%%%%%%%%%%%%SUB TYPING JUDGEMENTS%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}\tiny
%\begin{subfigure}[b]{.4\linewidth}
\begin{mathpar}
 \fmapextendn \and \fmapname  \and \fmapdiff \and \fmapwithf \and \fmapextend \and \fmapempty \and \fmapfieldemp \and \typelocalmap \and \typeglobal \and \rcutypes \and \types \and  \ftypedecl \and \rpth 
\and
\fbox{$\vdash \, \N \subt \N'$} \;\;
\inferrule[\scriptsize{T-NSub3}]
{
\N'([f \rightharpoonup y]) \;\;
\N_{f,\emptyset}
}
{\vdash \, \N\subt \N'}
\and
\inferrule[\scriptsize{T-NSub4}]
{
 \N' \;\;
 \N_{\emptyset}
}
{\vdash \, \N \subt \N'}
\and
\inferrule[\scriptsize{T-NSub2}]
{
 \N([f_2 \rightharpoonup y]) \;\;
\N'([f^{*} \rightharpoonup y])
}
{\vdash \, \N\subt \N'}
\and
\inferrule[\scriptsize{T-NSub1}]
{
\N([f_1 \rightharpoonup y]) \;\;
 \N'([f^{*} \rightharpoonup y])
}
{\vdash \, \N \subt \N'}
\and
\inferrule[\scriptsize{T-NSub5}]
{
}
{\vdash \, \N \subt \N}
\and
\fbox{$\vdash \, \rho \subt \rho'$} \;\;
\inferrule[\scriptsize{T-PSub1}]
{
\rho'=\rho''.f_1 \qquad \rho = \rho''.f_1|f_2
}
{
 \vdash  \rho' \subt \rho
}
\and
\inferrule[\scriptsize{T-PSub2})]
{
\rho'=\rho''.f_2  \qquad \rho= \rho''.f_1|f_2
}
{
 \vdash  \rho' \subt \rho
}
\and
\fbox{$\vdash \, \rho \subt \rho'$} \;\;
\inferrule[\scriptsize{T-TSub}]
{
T=\textsf{rcuItr}\; \_ \qquad T'=\textsf{undef}
}
{
\vdash T   \subt T' 
}
\and
\inferrule[\scriptsize{T-TSub1}]
{
\vdash\rho\subt \rho' \qquad \vdash \N \subt \N' \\
T =\textsf{rcuItr} \, \rho \, \N \qquad T'=\textsf{rcuItr} \, \rho' \, \N'
}
{
\vdash T  \subt  T'
}
\and
\fbox{$\vdash \, \Gamma \subt \Gamma'$} \;\;
\inferrule[\scriptsize{T-CSub1}]
{
\vdash\Gamma \subt \Gamma' \;\; \vdash \text{T}  \subt \text{T'}
}
{
\vdash \Gamma\, , x:\text{T}  \subt \Gamma'\, , x:\text{T'}
}
\and
\inferrule[\scriptsize{T-CSub2}]
{
\Gamma' = \Gamma[\rho.f^{k}/\rho.f^{k}.f]
}
{
 \vdash  \Gamma \subt \Gamma'
}
\and
\inferrule[\scriptsize{T-ESub}]
{
}
{
\vdash  \epsilon \subt \epsilon
}\and
%\end{mathpar}
%\caption{Sub-Typing Judgements}
%\label{fig:sub-typing}
%\end{subfigure}\quad
%\begin{subfigure}[b]{.4\linewidth}
%\tiny
%\begin{mathpar}
\fbox{$\Gamma \vdash \bar{s} \dashv \Gamma'$} \and
\inferrule[\scriptsize(T-Branch1)]
{
  x.f_1==z \and
 \Gamma\, ,x:\textsf{rcuItr}\,\rho \, \N([f_1 \rightharpoonup  z]) \vdash \bar{s}_1 \dashv\Gamma_4 \and
  \Gamma\, ,x:\textsf{rcuItr}\, \rho \, \N([f_2 \rightharpoonup z]) \vdash \bar{s}_2 \dashv \Gamma_4
}
{
\Gamma\, ,x:\textsf{rcuItr}\, \rho \, \N([f_1\mid f_2 \rightharpoonup z]) \vdash \textsf{if}(x.f_1==z)  \textsf{ then } \bar{s}_1 \textsf{ else } \bar{s}_2 \dashv \Gamma_4
}
\and
\inferrule[\scriptsize(T-Branch2)]
{
\Gamma(x)= \textsf{bool} \\
 \Gamma \vdash \bar{s}_1 \dashv\Gamma' \and \Gamma \vdash \bar{s}_2 \dashv \Gamma'
}
{
\Gamma \vdash \textsf{if}(x) \textsf{ then } \bar{s}_1  \textsf{ else } \bar{s}_2 \dashv \Gamma'
}
\and
\inferrule[\scriptsize(T-Branch3)]
{
 \Gamma,\,x:\textsf{rcuItr} \, \rho \, \N([f\rightharpoonup y \setminus \textsf{null}]) \vdash \bar{s}_1 \dashv \Gamma' \and \Gamma,\,x:\textsf{rcuItr} \, \rho \, \N([f\rightharpoonup y]) \vdash \bar{s}_2 \dashv \Gamma'
}
{
\Gamma,\,x:\textsf{rcuItr} \, \rho \, \N([f\rightharpoonup y]) \vdash \textsf{if}(x.f == \textsf{null}) \textsf{ then } \bar{s}_1  \textsf{ else } \bar{s}_2 \dashv \Gamma'
}
\and
\inferrule[\scriptsize(T-Conseq)]
{
 \Gamma \subt \Gamma'  \and \Gamma' \vdash \bar{s} \dashv \Gamma'' \and \Gamma'' \subt \Gamma'''
}
{
 \Gamma \vdash \bar{s} \dashv \Gamma'''
}
\and
\inferrule[\scriptsize(T-Loop1)]
{
\Gamma(x) = \textsf{bool} \and
\Gamma \vdash \bar{s} \dashv \Gamma 
}
{
\Gamma \vdash \textsf{while}(x)\{\bar{s}\} \dashv  \Gamma
}
\and
\inferrule[\scriptsize(T-Loop2)]
{
\Gamma,\, x:\textsf{rcuItr}\;\rho \; \N([f\rightharpoonup \_]) \vdash \bar{s} \dashv \Gamma, x:\textsf{rcuItr}\;\rho' \; \N([f\rightharpoonup \_])
}
{
\Gamma,\, x:\textsf{rcuItr}\;\rho \; \N([f\rightharpoonup \_]) \vdash \textsf{while}(x.f \neq \textsf{null})\{\bar{s}\} \dashv   x:\textsf{rcuItr}\;\rho' \; \N([f\rightharpoonup \textsf{null}]) ,\,  \Gamma
}
\and
\inferrule[\scriptsize(T-ReIndex)]
{
}
{
\Gamma \vdash \bar{s}_{k} \dashv  \Gamma[\rho.f^{k}/\rho.f^{k}.f]
}\and
%\end{mathpar}
%\caption{Type Judgements for Control-Flow.}
%\label{fig:type-judgements-for-cf}
%\end{subfigure}\quad
%%%%%%%%%%%%%%%%%%%%%%%%TYPE JUDEGEMENT%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{subfigure}[b]{.4\linewidth}
%\begin{mathpar}
\inferrule[\scriptsize(T-Root)]
{ \textsf{FV}(\Gamma) \cap \{r,y\}  =\emptyset}
{\Gamma\,,r:\textsf{rcuRoot}\,,y:\textsf{undef} \vdash_{M,R} y = r \dashv y: \textsf{rcuItr}\, \epsilon \, \N_{\emptyset}\,,r:\textsf{rcuRoot}\,,\Gamma}
\;\;
\inferrule[\scriptsize(T-ReadS)]
{ \textsf{FV}(\Gamma) \cap \{z,x\}  =\emptyset}
{
\Gamma\,, z:\textsf{rcuItr}\,\_ \, ,\rcuitrT{x}{G}{k}{k+1}{\_} \vdash_{M,R} z=x \dashv  \rcuitrT{x}{G}{k}{k+1}{\_}\, , \rcuitrT{z}{G}{k}{k+1}{\_} \,, \Gamma
}
\and
\inferrule[\scriptsize(T-ReadH)]
{
\rho.f=\rho' \\
 \textsf{FV}(\Gamma) \cap \{z,x\} =\emptyset
}
{
 \Gamma\, , z:\textsf{rcuItr}\,\_ \, ,  x:\textsf{rcuItr} \, \rho \, \N   \vdash_{M,R}
 	z=x.f
 \dashv  x:\textsf{rcuItr} \, \rho \, \N[f\mapsto z]\, ,z:\textsf{rcuItr} \, \rho' \, \N_{\emptyset} \, , \Gamma
}
\and
\inferrule[\scriptsize(T-Alloc)]
{
\mathsf{FV}(\Gamma) \cap \{x\} = \emptyset
}
{
 \Gamma\,, x:\textsf{undef} \vdash_{M} x = \NEW \dashv x:\textsf{rcuFresh} \, \N_{\emptyset} \, ,  \Gamma
}
\;\;
\inferrule[\scriptsize(T-Free)]
{
}
{
x:\textsf{freeable} \vdash_{M} \textsf{Free}(x) \dashv x:\textsf{undef}
}\;\;
\inferrule[\scriptsize(T-Exchange)]
{
 \Gamma, \, y:T' , \, x:T, \, \Gamma' \vdash \bar{s} \dashv   \Gamma''
}
{
\Gamma, \, x:T , \, y:T' , \, \Gamma' \vdash \bar{s} \dashv   \Gamma''
}
\and
\inferrule[\scriptsize(T-Sync)]
{
\textsf{FV}(\Gamma) \cap \textsf{FV}(\Gamma'')  = \emptyset \\
\lnot(\exists_{x \in \Gamma''} \ldotp x:\textsf{unlinked}) \\
\forall x \in \Gamma \ldotp  x:\textsf{unlinked} \quad \Gamma'  = \forall_{x\in \Gamma }\ldotp \Gamma \setminus \{x:\textsf{unlinked}\} \cup \{x:\textsf{freeable}\} \\
\Gamma'',\Gamma \vdash_{M}\textsf{SyncStart}\dashv\Gamma'',\Gamma \qquad \Gamma'',\Gamma \vdash_{M}\textsf{SyncStop}\dashv\Gamma'',\Gamma' \qquad
}
{
\Gamma'',\Gamma \vdash_{M} \textsf{SyncStart};\textsf{SyncStop} \dashv \Gamma',\Gamma''
}
\and
\inferrule[\scriptsize(T-WriteFH)]
{
\textsf{FV}(\Gamma) \cap \{p,z,x\}  =\emptyset \\ z:\textsf{rcuItr} \; \rho.f \; \_
}
{
 \Gamma, p:\textsf{rcuFresh}\,\N_{f,\emptyset},\; x:\textsf{rcuItr}\;\; \rho \;\; \N([f\rightharpoonup z])
  \vdash_{M} p.f = z \dashv
  \rcunf{p}{f}{z} \, , x:\textsf{rcuItr}\, \rho \, \N([f\rightharpoonup z]), \, \Gamma
}
\and
\inferrule[\scriptsize(T-UnlinkH)]
{
\textsf{FV}(\Gamma) \cap \{x,z,r\} \qquad \rho.f_1=\rho' \;\; \rho'.f_2=\rho'' \qquad \forall_{f\in dom(\N')} \ldotp f\neq f_2 \implies \N'([f\rightharpoonup \textsf{null}]) \lor \N'_{f,\emptyset}   \\
\begin{array}{l}
\forall_{n\in \Gamma,m,\N''', p''',f}\ldotp n:\textsf{rcuItr}\,\rho'''\,\N'''([f\rightharpoonup m]) \implies 
\left\{\begin{array}{l}
(((\rho \neq \rho''' \land \rho' \neq \rho''' \land \rho'' \neq \rho''')  ) \land (\{m\} \cap \{z,r\} = \emptyset ) ) \arcr
\land (\forall_{\rho''''\neq \epsilon} \ldotp \rho'''\neq \rho''.\rho'''' )
\end{array}\right.
\end{array}
}
{
\Gamma,\,x:\textsf{rcuItr}\, \rho \, \N([f_1\rightharpoonup z]) \, ,
z:\textsf{rcuItr}\, \rho' \, \N'([f_2\rightharpoonup r]) \, ,  r:\textsf{rcuItr} \, \rho'' \, \N''\, 
\vdash_{M} x.f_1=r \dashv
z:\unlinked\, ,
x:\textsf{rcuItr} \, \rho \, \N(f_1\rightharpoonup z \setminus r)\, ,
r:\textsf{rcuItr} \, \rho' \, \N'',\, \Gamma
}
\and
\inferrule[\scriptsize(T-LinkF)]
{
\rho.f  = \rho'  \qquad \N' = \N'' \qquad  \textsf{FV}(\Gamma) \cap \{p,o,n\}  =\emptyset \\
\lnot(\exists_{x \in \Gamma, \N''', \rho'',f',y} \ldotp (x:\textsf{rcuItr}\,\rho''\,\N'''([f'\rightharpoonup y])) \land ((\rho'' = \rho)\lor(\rho'' = \rho')) \land (y\neq o \land (\forall_{x_i \in codom(\N')} \ldotp y \neq x_i  ) ) )
}
{
\Gamma,\,
 p:\textsf{rcuItr}\, \rho \, \N([f\rightharpoonup o]) \, ,
  o:\textsf{rcuItr}\, \rho' \, \N' \, , n:\textsf{rcuFresh} \, \N''
  \vdash_{M} p.f = n \dashv
  p:\textsf{rcuItr}\, \rho \, \N(f \rightharpoonup o \setminus n) \, ,
  n:\textsf{rcuItr}\, \rho' \, \N'' \,
  o:\unlinked\, ,  \Gamma
}
\and
\inferrule[\scriptsize(T-Seq)]
{
\Gamma_1 \vdash \bar{s_1} \dashv_{M,R}   \Gamma_2  \qquad   \Gamma_2 \vdash_{M,R} \bar{s_2} \dashv   \Gamma_3
}
{
\Gamma_1  \vdash_{M,R} \bar{s_1} \; ; \; \bar{s_2} \dashv  \Gamma_3
}
\and
\inferrule[\scriptsize(T-Par)]
{
 \Gamma_1 \vdash_{R} \bar{s_1} \dashv   \Gamma'_1  \qquad   \Gamma_2 \vdash_{M,R} \bar{s_2} \dashv   \Gamma'_2
}
{
 \Gamma_1, \; \Gamma_2  \vdash \bar{s_1} || \bar{s_2} \dashv  \Gamma'_1 \; , \Gamma'_2
}
\and
\inferrule[\scriptsize(T-Skip)]
{
}
{
 \Gamma \vdash_{M,R} \textsf{skip} \dashv   \Gamma
}
\and
\inferrule[\scriptsize(ToRCURead)]
{
\Gamma\, , y : \textsf{rcuItr} \vdash_R \bar{s} \dashv \Gamma'
}
{
\Gamma \vdash \textsf{RCURead}\, x.f \textsf{ as }y\textsf{ in }\{\bar{s}\}
}
\and
\inferrule[\scriptsize(ToRCUWrite)]
{
 \Gamma\, , y : \textsf{rcuItr} \vdash_M \bar{s} \dashv \Gamma' \;\; \ftype{}{\textsf{rcu}} \;\;  \textsf{NoFresh}(\Gamma') \;\; \textsf{NoUnlinked}(\Gamma')
}
{
\Gamma \vdash \textsf{RCUWrite}\, x.f \textsf{ as }y\textsf{ in } \{ \bar{s} \}
}
\end{mathpar}
\label{fig:ts}
\caption{Type Rule for \textsf{RCU} Programming}
\end{figure}
%%%%%%%%%%%%%%%COND TYPE JUDGEMENTS ENDS%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Subtyping}
We know that there is non-determinisim in the number of the loop execution times. To capture this non-determinisim in the \textsf{rcuItr} types, we approximate over the number of loop executions and abstract the contribution of the loop execution to the \textsf{rcuItr} typed references' path components. The abstraction on the path  makes it possible to write loop invariants that grow paths by traversing the heap. Assertions of the \texttt{add} function in lines 19 and 20 in Listing \ref{fig:rculist} show the \textit{loop}'s effects on paths of iterator pointers used inside the loop, \texttt{current} and \texttt{parent}. The \textsf{rcuItr} reference \texttt{parent}'s assertion in the line 20 has $(Next)^{k}$ on the path component in addition to the path component of its assertion before the loop in the line 17. The $k$ in the $(Next)^{k}$ is our approximation to the number of loop executions with side condition $k>=0$. We define the path capturing this abstraction as $\cpath$. The \textsf{rcuItr} reference \texttt{current}'s assertion in the line 19 has $(Next)^{k}.Next$ on the path component in addition to the path component of its assertion before the loop in the line 16. The $Next$ portion of the $(Next)^{k}.Next$ distinguishes the relationship between \texttt{current} and \texttt{parent}. Under these mechanisms, we end up having the loop invariants in  assertions of the \texttt{current} and \texttt{parent} in lines 19 and 20. We apply reindexing(\textsc{T-ReIndex}) with respect to $k$ on the path components after loop execution to preserve loop invariant. The relation between the context to be reindexed(lines 23 and 24 of the \texttt{add} function in Figure \ref{fig:rculist}) and the context forming the loop invariant (lines 19 and 20 of the \texttt{add} function in Figure \ref{fig:rculist}) is captured by subtyping relation(\textsc{T-CSub2}).

(\textit{\textbf{Approximation on Fields}}) - We sometimes need to overapproximate, both for control flow joins or later to throw away detailed information (like field map contents, or coercing to undef) in order to prune accessible aliases. Since our list based bag example's objects have single field($Next$), we take small code snippet from our \textsf{BST} type checking effort in Appendix \ref{appendix:bst_del} in which objects have two fields $Left$ and $Right$. Field mappings take field names to local variable names. They are added to the field map, $\N$, when the object's fields are read. In Listing \ref{lst:altfield}, we see that \texttt{parent} reads \texttt{current} to its different fields in different branches of the \textit{if-statement}. We see the join of the type assertions in lines 6 and 11 to the one in the line 12. We overapproximate on the fields $Left|Right$ (either $Left$ or $Right$) both in the path of the \texttt{current} and in the field mappings of \texttt{parent} and \texttt{current}. We capture this overapproximation through subtyping relations(\textsc{T-NSub1-5} and \textsc{T-PSub1-2}).

(\textit{\textbf{Choosing Fields to Read}}) - Thus far, we have always been precise on the representation of the object fields-- mention just one field name -- both in the path component and field mappings. However, we cannot always be precise in mentioning the field names in the \textsf{rcuItr} type. The assertion in Listing \ref{lst:altfield} line 1 mentions field names in different way, $Left|Right$, than we have seen so far. Our intention to represent the object fields this way is to make \textsf{RCU} types expressible enough to assert "either Left or Right field''. The assertion for the \texttt{current} in Listing \ref{lst:altfield} line 1 tells that the heap node pointed by the \texttt{current} pointer is reached via either "Left or Right" field. From other perspective, the assertion for the \texttt{parent} in the same line tells that the heap node pointed by \texttt{current} can be reached from the heap node pointed by \texttt{parent} via "either the Left or the Right" field.
However, we should also note that being precise in the field names is so crucial for mutation actions. This means we need to know which fields are used to replace/unlink a heap node. Then, what is the mechanism to become more/less precise in the fields used in both path and field mappings of the \textsf{rcuItr} type? In Listing \ref{lst:altfield}, we see a \textit{if-statement} with the condition $parent.Left == current$. This condition refines the assertions in Listing \ref{lst:altfield} line 1 to the one in the line 3 for the \textit{then} branch and to the one in the line 8 for the \textit{else} branch via making types more precise on the object fields.
To capture the precision relation on object fields in the types, we use \textit{subtyping}.
\begin{lstlisting}[caption={Choosing fields to read},label={lst:altfield}, numbers=left, numberstyle=\tiny\color{red}, numbersep=5pt]%, basicstyle=\scriptsize]

$\assert{current:\mathsf{rcuItr}\; Left|Right \;\{\},\;\;parent:\mathsf{rcuItr}\;  \epsilon \;\{Left|Right\mapsto current\}}$
if(parent.Left == current){
  $\assert{current:\mathsf{rcuItr}\; Left \;\{\} ,\;\; parent:\mathsf{rcuItr}\;  \epsilon \;\{Left\mapsto current\}}$
  parent = current;
  current = parent.Left;
  $\assert{current:\mathsf{rcuItr}\; Left.Left \;\{\}, \;\; parent:\mathsf{rcuItr}\;  Left \;\{Left\mapsto current\}}$
}else{
  $\assert{current:\mathsf{rcuItr}\; Right \;\{\}, \;\; parent:\mathsf{rcuItr}\;  \epsilon \;\{Right\mapsto current\}}$
  parent = current;
  current = parent.Right;
  $\assert{current:\mathsf{rcuItr}\; Right.Right \;\{\}, \;\; parent:\mathsf{rcuItr}\;  Right \;\{Right\mapsto current\}}$
}$\assert{current:\mathsf{rcuItr}\; Left|Right.Left|Right \;\{\}, \;\; parent:\mathsf{rcuItr}\;  Left|Right \;\{Left|Right\mapsto current\}}$
\end{lstlisting}

(\textit{\textbf{Points to}}\textsf{null}) - \todo{Motivate and explain}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Types in Action}
\label{subsection:type-action}
%%%%%%%%%%%%%%%%%%%%%%TYPE JUDGEMENTS ENDS%%%%%%%%%%%%%%%%%%%%%%%%%%%
We have typing context $\Gamma$ of the form $x_1 : T_1, \ldots x_n : T_n$.

The system has three forms of typing judgement
\begin{itemize}
\item $\Gamma \vdash C$: standard typing outside rcu regions
\item $\Gamma \vdash_R C \dashv \Gamma'$: flow sensitive typing inside an rcu read region
\item $\Gamma \vdash_M C \dashv \Gamma'$: flow sensitive typing inside an rcu write region
\end{itemize}
Below, we introduce our types through the list-based bag implementation in Figure \ref{fig:rculist} ~\cite{McKenney2015SomeEO}.  We aim to
\begin{itemize}
\item explain why we employ each of these components. How do they serve to certify memory safety in \textsf{RCU} programs? How do they represent the program?
\item explain the \textit{flow-sensitive} nature of the type system. 
\end{itemize}
The code fragments below are annotated with assertions about type environments between each statement (in the style of a proof outline in Hoare Logic) to demonstrate informally how types change before and after various statements. All of the formal definitions for the type components and rules can be found in the Figures \ref{fig:ts} and \ref{fig:transitionsbetweendifferenttypesystems}.

(\textit{\textbf{Reading a Global}} \textsf{RCU} \textit{\textbf{Root}}) - All \textsf{RCU} data structures have global unique roots so that we can attach an iterator pointer to the data structure to traverse it. The type \textsf{rcuRoot} represents a variable referencing a unique root. We read a \textsf{rcuRoot} typed pointer to a local variable. As we observe in the pre/post conditions of reading the global root in assertions of the \texttt{remove} function in lines 3 and 5, \texttt{root} pointer's type does not change. A local variable \texttt{current} is our new pointer to iterate over the data structure. The type of \texttt{current} changes from \textsf{undef} in line 3 to \textsf{rcuItr} in line 6 after reading the global root. The path of \texttt{current} pointer is empty, $\epsilon$, and there exists no field mappings in its field mapping set.  The type assertion for the \texttt{current} pointer in the post condition says that the heap node pointed by it is at the root -- its path is $\epsilon$ -- and there is no field mapping -- \{\}  -- which means there is no link to any other heap node from the node referenced by the \texttt{current}. So, at this point, there are not enough resources for actions such as \textit{unlinking}, \textit{reclaiming} and \textit{replacing} a node.

(\textit{\textbf{Reading an Object Field and a Variable}}) - As expected, we explore the heap of the data structure via reading the objects' fields. For example, the assertion of the \textsf{remove} function in line 7 says that the path to reach the heap node pointed by \texttt{current} is $Next$. The assertion in line 8 for \texttt{parent} tells that there exists a link from the referent of \textsf{parent} to the referent of \textsf{current}. As we observe in the post condition in the lines 7 and 8, reading \texttt{current} to the \texttt{parent}'s $Next$ field in line 6 adds the field mapping entry $Next \mapsto \texttt{current}$ to the field mapping set of \texttt{parent} and extends the path of the \texttt{current} with $Next$.

(\textit{\textbf{Mutation - Unlinking a Heap Node}}) - When we unlink a heap node, the type of the reference to it changes from \textsf{rcuItr} to \textsf{unlinked}. We observe this change for \texttt{current} reference in the assertions of the \texttt{remove} in lines 22 and 26.

(\textit{\textbf{Mutation - Reclaiming a Heap Node after a Grace Period}}) - After the referent of \texttt{current} is unlinked, the crucial phase with respect to \textsf{RCU} semantic -- grace period for the reader threads -- starts. We start the grace period with \texttt{SyncStart} as we see in line 28 of the \texttt{remove} function. In real implementations, \texttt{SyncStart}-\texttt{SyncStop} are just one call to \texttt{synchronize\_rcu} to wait the grace period to end so there is no need for a change in the type of the \texttt{current}. The change from \textsf{unlinked} to \textsf{freeable} in the type of the \texttt{current} pointer indicates that grace period for the heap node referenced by the \texttt{current} has finished. The grace period ends once the \texttt{SyncStop} returns as seen in line 29. Once the grace period ends, It is semantically convenient to to reclaim the heap node referenced by the \texttt{current} via calling \texttt{Free} as seen in line 31. We indicate the end of grace period and being able to reclaim the heap node via the change in type of \texttt{current} reference from \textsf{unlinked} in line 26, to \textsf{freeable} in line 30.

(\textit{\textbf{Creating a Fresh Node}}) - Some data structure implementations needs allocation and linking of a new heap node e.g. replacing a new node with an existing one in BST or adding a new node to a bag. In line 8 of the \texttt{add} method, we allocate a new node and set its fields in lines 10 and 29. The type of the variable \textsf{nw} in line 9 represents a freshly allocated heap node, whose fields are not set yet. A \textsf{rcuFresh} pointer can be used either in setting the fields of a fresh object or linking the fresh object. We will investigate  linking a fresh object in the next analysis but, first we anaylze how we set the fields of the fresh object. In  line 29, we set the fields of the object referenced by \texttt{nw} and we end up having the type in line 30 which seems similar to a type \textsf{rcuItr} with empty path. We will justify why we have separate type \textsf{rcuFresh} instead of typing the freshly allocated heap with \textsf{rcuItr} when we explain the type rules.
\subsection{Type Rules}
\label{subsection:type-rules}
Our aim in this section is to investigate potential memory safety issues, discuss what memory inconsistencies they can cause and how type rules prevent it and justify why the flow of change in types serves to the correct \textsf{RCU} programming.

(\textit{\textbf{Mutation - Unlinking a Heap Node}}) - Preserving invariants of a data structure against possible mutations under \textsf{RCU} semantics is challenging. Unlinking a heap node is one way of mutating the heap. To understand the importance of the locality on the effect of the mutation, we illustrate the setting of \texttt{remove} function in \ref{fig:rculist} with some additional fictional resources such as stack pointer aliases in Figures  \ref{fig:frameout} and \ref{fig:unlinkframeout}. The square nodes filled with $R$ -- a root node -- and $H$ -- a heap node -- are heap nodes. The hollow nodes are stack pointers to the square heap nodes. All resources in red form the memory foot print of unlinking. The hollow red nodes -- $pr$, $cr$ and $crl$ -- point to the red square heap nodes which are involved in unlinking of the heap node pointed by \texttt{cr}. We have $a_1$, $a_2$ and $a_3$ which are aliases with \texttt{parent}-$pr$, \texttt{current}-$cr$ and \texttt{currenL}-$crl$ respectively. We call them the \textit{path-aliases} as they share the same path from root to the node that they reference. The $n$ field depicts $Next$.
 \begin{figure}[H]
 \centering
 \begin{subfigure}[b]{.4\linewidth}
\centering
 \begin{tikzpicture}[>=stealth',node distance=1.3cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]
 \tikzstyle{solids node}=[rectangle,draw=red,inner sep=1.5]
\tikzstyle{null node}=[circle,draw=red,fill=red]
 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1},
 	blue node/.style={rectangle,draw=black,inner sep=1},
 	reader node/.style={circle,draw=black,inner sep=1},
        redreader node/.style={circle,draw=red,inner sep=1},
        readerr node/.style={dashed,circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[solid node] (1) [right of=R] {$H_0$};
       \node[solids node] (2) [right of=1] {$H_1$};
       \node[solids node] (3) [right of=2] {$H_2$};
       \node[solids node] (4) [right of=3] {$H_3$};
       \node[solid node] (5) [above  of=3] {$H_4$};
       \node[solid node] (6) [above  of=4] {$H_5$};
       
       \node[redreader node] (r0) [below  of= 2]  {$pr$};
       \node[redreader node] (r1) [below  of= 3]  {$cr$};
       \node[redreader node] (r2)  [below  of= 4] {$crl$};

       \node[readerr node] (r0a) [above  of= 1]  {$a_1$};
       \node[readerr node] (r1a) [above   of= 2]  {$a_2$};
       \node[readerr node] (r2a)  [below right of= 4] {$a_3$};

       \node[reader node] (r1f) [above  of= 5]  {$a_4$};
       \node[reader node] (r2f)  [above  of= 6] {$a_5$};

     \path[->]  (R) edge node[below] {$n$} (1);
     \path[->]  (1) edge node[below] {$n$} (2);
     \path[draw=red,->]  (2) edge node[below] {$n$} (3);
     \path[draw=red,->]  (3) edge node[below] {$n$} (4);
     \path[dashed,->]  (5) edge node {$n$} (3);
     \path[dashed,->]  (6) edge node {$n$} (4);

     \path[draw=red,->]  (r0) edge node {} (2);
     \path[draw=red,->]  (r1) edge node  {}  (3);
     \path[draw=red,->]  (r2) edge  node  {}   (4);

     \path[dashed,->]  (r0a) edge node {} (2);
     \path[dashed,->]  (r1a) edge node  {}  (3);
     \path[dashed,->]  (r2a) edge  node  {}   (4);

     \path[->]  (r1f) edge node  {}  (5);
     \path[->]  (r2f) edge  node  {}   (6);
   
%\path[dotted,->] (1) edge[bend left] node  {$f^{*}$} (5)
 ;
 
 \end{tikzpicture}
 \caption{\textsf{Framing} before unlinking the heap node pointed by \texttt{current}-$cr$.}
 \label{fig:frameout}
 \end{subfigure}\quad
\begin{subfigure}[b]{.4\linewidth}
 \centering
 \begin{tikzpicture}[>=stealth',node distance=1.3cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]
 \tikzstyle{solids node}=[rectangle,draw=red,inner sep=1.5]
  \tikzstyle{solidss node}=[dashed,rectangle,draw=red,inner sep=1.5]
 \tikzstyle{null node}=[circle,draw=red,fill=red]
 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1.5},
 	blue node/.style={rectangle,draw=black,inner sep=1.5},
 	reader node/.style={circle,draw=black,inner sep=1},
        redreader node/.style={circle,draw=red,inner sep=1},
                rredreader node/.style={dashed,circle,draw=red,inner sep=1},
        readerr node/.style={dashed,circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[solid node] (1) [right of=R] {$H_0$};
       \node[solids node] (2) [right of=1] {$H_1$};
       \node[solidss node] (3) [right of=2] {$H_2$};
       \node[solids node] (4) [right of=3] {$H_3$};
       \node[solid node] (5) [above  of=3] {$H_4$};
       \node[solid node] (6) [above  of=4] {$H_5$};

       \node[redreader node] (r0) [below  of= 2]  {$pr$};
       \node[rredreader node] (r1) [below  of= 3]  {$cr$};
       \node[redreader node] (r2)  [below  of= 4] {$crl$};

       \node[readerr node] (r0a) [above  of= 1]  {$a_1$};
       \node[readerr node] (r1a) [above   of= 2]  {$a_2$};
       \node[readerr node] (r2a)  [below right of= 4] {$a_3$};

       \node[reader node] (r1f) [above  of= 5]  {$a_4$};
       \node[reader node] (r2f)  [above  of= 6] {$a_5$};

     \path[->]  (R) edge node[below] {$n$} (1);
     \path[->]  (1) edge node[below] {$n$} (2);
     \path[draw=red,->]  (2) edge [bend right] node[below left] {$n$} (4);
     \path[dashed,draw=red,->]  (3) edge node[below] {$n$} (4);
     \path[dashed,->]  (5) edge node {$n$} (3);
     \path[dashed,->]  (6) edge node {$n$} (4);

     \path[draw=red,->]  (r0) edge node {} (2);
     \path[dashed,draw=red,->]  (r1) edge node  {}  (3);
     \path[draw=red,->]  (r2) edge  node  {}   (4);

     \path[dashed,->]  (r0a) edge node {} (2);
     \path[dashed,->]  (r1a) edge node  {}  (3);
     \path[dashed,->]  (r2a) edge  node  {}   (4);

     \path[->]  (r1f) edge node  {}  (5);
     \path[->]  (r2f) edge  node  {}   (6);

 ;
 \end{tikzpicture}

 \caption{Safe unlinking of the heap node pointed by \texttt{current}-$cr$ via \textsf{Framing}}
 \label{fig:unlinkframeout}
 \end{subfigure}
 \caption{Safe unlinking of the heap node}\vspace{-2mm}
 \end{figure}
The type rule for unlinking must assert the "proper linkage" in between the heap nodes involved in unlinking. We see the proper linkage relation between in Figure \ref{fig:frameout} as red $n$ links between $H_1$, $H_2$ and $H_3$ which are referenced by $pr$, $cr$ and $crl$ respectively. Our type rule for unlinking(\textsc{T-UnlinkH}) asserts that $x$ (\texttt{parent}), $y$ (\texttt{current}) and $z$ (\texttt{currentL}) pointers are linked with field mappings $\N([f_1\rightharpoonup z])$ ($Next \mapsto current$) of $x$, $\N'([f_2\rightharpoonup r])$ ($Next \mapsto currentL$) of $y$. In accordance with the field mappings, the type rule also asserts that $x$ has the path $\rho$ ($(Next)^{k}$), $y$ has the path $\rho.f_1$ ($(Next)^{k}.Next$) and $z$ has the path $\rho.f_1.f_2$ ($(Next)^{k}.Next.Next$).
Being able to localize the effects of the mutation is important in a sense that it prevents unexpected side effects of the mutation. So, sharing through aliasing to the resources under mutation, e.g. aliasing to \texttt{parent}, \texttt{current} and \texttt{currentL}, needs to be handled carefully. Aliasing can occur via either through  object fields -- via field mappings -- or stack pointers -- via path components. We see path aliases, $a_1$, $a_2$ and $a_3$, illustrated with dashed nodes and arrows to the heap nodes in Figures \ref{fig:frameout} and \ref{fig:unlinkframeout}. They are depicted as dashed because they are not safe resources to use when unlinking so they are \textit{framed-out} by the type system via $\rho \neq \rho''' \land \rho' \neq \rho''' \land \rho'' \neq \rho'''$ which ensures the non-existence of the \textit{path-aliases} to any of $x$, $z$ and $r$ in the rule which corresponds to $pr$, $cr$ and $crl$ respectively. 
Any heap node reached from root by following a path($\rho'''$) deeper than the path reaching to the last heap node($crl$) in the footprint cannot be pointed by the heap nodes($pr$, $cr$ and $crl$) in the footprint. We require this restriction to prevent inconsistency on the type of pointers having $\rho'''$ as path component($\forall_{\rho''''\neq \epsilon} \ldotp \rho''' = \rho''.\rho'''' \implies \lnot(\exists_{f'}\ldotp ( \N(f')=n \lor \N'(f')=n  \lor \N''(f')=n ))$). The reason for framing-out these dashed path aliases is obvious when we look at the changes from the Figure \ref{fig:frameout} to Figure \ref{fig:unlinkframeout}. For example, $a_1$ points to $H_1$ which has object field $Next$-$n$ pointing to $H_2$ which is also pointed by \texttt{current} as depicted in the Figure \ref{fig:frameout}. However, in Figure \ref{fig:unlinkframeout}, $n$ of $H_1$ is pointing to $H_3$ though $a_1$ still points to $H_1$. This change invalidates the field mapping $Next \mapsto current$ of $a_1$ in the \textsf{rcuItr} type. One another safety achieved with framing shows up in a setting where \texttt{current} and $a_2$ are aliases. In the Figure \ref{fig:frameout}, both \texttt{current} and $a_2$ are in the \textsf{rcuItr} type and point to $H_2$. After the unlinking action, the type of the \texttt{current} becomes \texttt{unlinked} although $a_2$ is still in the \texttt{rcuItr} type. Framing out $a_2$ prevents the inconsistency in its type under the unlinking operation. One interesting and not obvious inconsistency issue shows up due to the aliasing between $a_3$ and the \texttt{currentL}-$crl$. Before the unlinking happens, both \texttt{currentL} and $a_3$ have the same path components (assuming that it is $(Next)^{k}.Next.Next$ line 23 in \texttt{remove} function). After unlinking, the path of \texttt{currentL}-$crl$ gets shortened as the path to heap node it points, $H_3$, changes  to $(Next)^{k}.Next$ as we see in line 27 in \texttt{remove} function. However, the path component of $a_3$  would not change so the path component of $a_3$ in the \textsf{rcuItr} would become inconsistent with the actual path reaching to $H_3$.
In addition to \textit{path-aliasing}, there can also be aliasing via \textit{field-mappings} which we call \textit{field-aliasing}. We see field alising examples in Figures \ref{fig:frameout} and \ref{fig:unlinkframeout}: $pr$ and $a_1$ are field aliases with $Next-n$ from $H_0$ points to $H_1$, $cr$ and $a_2$ are field aliases with $Next-n$ from $H_4$ points to $H_2$  and $crl$ and $a_3$ are field aliases with $Next-n$ from $H_5$ points to $H_3$. We do not discuss the problems that can occur due to the \textit{field-aliasing} as they are same with the ones due to \textit{path-aliasing}. What we focus on is how the type rule prevents \textit{field-aliases}. The type rule asserts $\lnot(\{m\} \cap \{z,r\} \neq \emptyset)$ to make sure that there exists no object field from any other context pointing either to the variable points the heap node that is mutation(unlinking) -- \texttt{current}-$cr$ -- or to the variable which points to the new $Next$ of the \texttt{parent} after unlinking -- \texttt{currentL}-$crl$. We should also note that it is expected to have object fields in other contexts to point to $pr$ as they are not in the effect zone of unlinking. For example, we see the object field $n$ points from $H_0$ to  $H_1$ in Figures \ref{fig:frameout} and \ref{fig:unlinkframeout}.
We should note that the type system must also forbid sharing the variable names variables in different contexts $\textsf{FV}(\Gamma) \cap \{x,z,r\} = \emptyset$.\\
Once we unlink the heap node, it cannot be accessed by the new coming reader threads the ones that are currently reading this node cannot access to the rest of the heap. We illustrate this with dashed red $cr$, $H_2$ and object fields in Figure \ref{fig:unlinkframeout}.
Although it is not quite obvious in the list-based bag example which we have been focusing on so far, being aware of how much of the heap is under mutation is important, e.g. a whole subtree or a single node. Our type system ensures that there can be only just one heap node unlinked at a time by atomic field update action. To be able to ensure this, in addition to the proper linkage enforcement, the rule also asserts that all other object fields which are not under mutation must either not exists or point to \texttt{null} via $\forall_{f\in dom(\N')} \ldotp f\neq f_2 \implies \N'([f\rightharpoonup \textsf{null}]) \lor \N'_{f,\emptyset}$.
It is much easier to understand why we need this assertion when we consider a data structure implementation whose objects needs more than one field. A binary search tree is a good candidate to understand this setting. To understand this setting more pictorially, we also elaborate Figures \ref{fig:frameout} and \ref{fig:unlinkframeout} with the red filled circle which depicts \texttt{null}, the $l$ field which depicts $Left$ and $r$ which depicts $Right$ field in the Figures \ref{fig:bframeout} and \ref{fig:bunlinkframeout}. We see in these Figures that to unlink the referent of \texttt{current} using $Left$ field of the \texttt{parent}. With respec to the type rule, the proper set of field mappings of the \texttt{current} include $Left \mapsto currentL$ and $Right \mapsto \texttt{null}$. We also see this pictorially in Figures as the object field $Right$-$r$ from the $H_2$ points to red circle, \texttt{null}. So it is obvious that if we had a subtree instead of a red filled circle -- \texttt{null} -- we would be leaking more than a single node by unlinking.
 \begin{figure}[H]
 \centering
 \begin{subfigure}[b]{.4\linewidth}
\centering
 \begin{tikzpicture}[>=stealth',node distance=1.3cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]
 \tikzstyle{solids node}=[rectangle,draw=red,inner sep=1.5]
\tikzstyle{null node}=[circle,draw=red,fill=red]
 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1},
 	blue node/.style={rectangle,draw=black,inner sep=1},
 	reader node/.style={circle,draw=black,inner sep=1},
        redreader node/.style={circle,draw=red,inner sep=1},
        readerr node/.style={dashed,circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[solid node] (1) [right of=R] {$H_0$};
       \node[solids node] (2) [right of=1] {$H_1$};
       \node[solids node] (3) [right of=2] {$H_2$};
       \node[solids node] (4) [right of=3] {$H_3$};
       \node[solid node] (5) [above  of=3] {$H_4$};
       \node[null node] (nl) [above right of = 3]{};
       \node[solid node] (6) [above  of=4] {$H_5$};
       
       \node[redreader node] (r0) [below  of= 2]  {$pr$};
       \node[redreader node] (r1) [below  of= 3]  {$cr$};
       \node[redreader node] (r2)  [below  of= 4] {$crl$};

       \node[readerr node] (r0a) [above  of= 1]  {$a_1$};
       \node[readerr node] (r1a) [above   of= 2]  {$a_2$};
       \node[readerr node] (r2a)  [below right of= 4] {$a_3$};

       \node[reader node] (r1f) [above  of= 5]  {$a_4$};
       \node[reader node] (r2f)  [above  of= 6] {$a_5$};

     \path[->]  (R) edge node[below] {$l$} (1);
     \path[->]  (1) edge node[below] {$l$} (2);
     \path[draw=red,->]  (2) edge node[below] {$l$} (3);
     \path[draw=red,->]  (3) edge node[below] {$l$} (4);
     \path[dashed,->]  (5) edge node {$l$} (3);
     \path[dashed,->]  (6) edge node {$l$} (4);

     \path[draw=red,->]  (r0) edge node {} (2);
     \path[draw=red,->]  (r1) edge node  {}  (3);
     \path[draw=red,->]  (r2) edge  node  {}   (4);

     \path[dashed,->]  (r0a) edge node {} (2);
     \path[dashed,->]  (r1a) edge node  {}  (3);
     \path[dashed,->]  (r2a) edge  node  {}   (4);

     \path[->]  (r1f) edge node  {}  (5);
     \path[->]  (r2f) edge  node  {}   (6);
    \path[draw=red,->] (3) edge node[below] {$r$} (nl);
%\path[dotted,->] (1) edge[bend left] node  {$f^{*}$} (5)
 ;
 
 \end{tikzpicture}
 \caption{\textsf{Framing} before unlinking the heap node pointed by \texttt{current}-$cr$.}
 \label{fig:bframeout}
 \end{subfigure}\quad
\begin{subfigure}[b]{.4\linewidth}
 \centering
 \begin{tikzpicture}[>=stealth',node distance=1.3cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]
 \tikzstyle{solids node}=[rectangle,draw=red,inner sep=1.5]
  \tikzstyle{solidss node}=[dashed,rectangle,draw=red,inner sep=1.5]
 \tikzstyle{null node}=[circle,draw=red,fill=red]
 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1.5},
 	blue node/.style={rectangle,draw=black,inner sep=1.5},
 	reader node/.style={circle,draw=black,inner sep=1},
        redreader node/.style={circle,draw=red,inner sep=1},
                rredreader node/.style={dashed,circle,draw=red,inner sep=1},
        readerr node/.style={dashed,circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[solid node] (1) [right of=R] {$H_0$};
       \node[solids node] (2) [right of=1] {$H_1$};
       \node[solidss node] (3) [right of=2] {$H_2$};
       \node[solids node] (4) [right of=3] {$H_3$};
       \node[solid node] (5) [above  of=3] {$H_4$};
       \node[solid node] (6) [above  of=4] {$H_5$};
       \node[null node] (nl) [above right of = 3]{};

       \node[redreader node] (r0) [below  of= 2]  {$pr$};
       \node[rredreader node] (r1) [below  of= 3]  {$cr$};
       \node[redreader node] (r2)  [below  of= 4] {$crl$};

       \node[readerr node] (r0a) [above  of= 1]  {$a_1$};
       \node[readerr node] (r1a) [above   of= 2]  {$a_2$};
       \node[readerr node] (r2a)  [below right of= 4] {$a_3$};

       \node[reader node] (r1f) [above  of= 5]  {$a_4$};
       \node[reader node] (r2f)  [above  of= 6] {$a_5$};

     \path[->]  (R) edge node[below] {$l$} (1);
     \path[->]  (1) edge node[below] {$l$} (2);
     \path[draw=red,->]  (2) edge [bend right] node[below left] {$l$} (4);
     \path[dashed,draw=red,->]  (3) edge node[below] {$l$} (4);
     \path[dashed,->]  (5) edge node {$l$} (3);
     \path[dashed,->]  (6) edge node {$l$} (4);

     \path[draw=red,->]  (r0) edge node {} (2);
     \path[dashed,draw=red,->]  (r1) edge node  {}  (3);
     \path[draw=red,->]  (r2) edge  node  {}   (4);

     \path[dashed,->]  (r0a) edge node {} (2);
     \path[dashed,->]  (r1a) edge node  {}  (3);
     \path[dashed,->]  (r2a) edge  node  {}   (4);

     \path[->]  (r1f) edge node  {}  (5);
     \path[->]  (r2f) edge  node  {}   (6);
     \path[dashed,draw=red, ->] (3) edge node[below] {$r$} (nl);
 ;
 \end{tikzpicture}

 \caption{Safe unlinking of the heap node pointed by \texttt{current}-$cr$ via \textsf{Framing}}
 \label{fig:bunlinkframeout}
 \end{subfigure}
 \caption{Safe unlinking: Unlinking a single node.}\vspace{-2mm}
 \end{figure}
\textit{\textbf{Creating a Fresh Node}} - We defered answering the questions: "Why do we need a separate type \textsf{rcuFresh}?" and "What would happen if we also typed the freshly allocated node with \textsf{rcuItr}?". To understand and answer the questions easily, we illustrate the setting for creating a fresh \textsf{BST} heap node and linking it in Figures \label{fig:frframeout} and \label{fig:freshframeout} --whole typing can be found in Appendix \ref{appendix:bst_del}. The dashed green $H_f$ denotes the freshly allocated heap node pointed by green dashed pointer \texttt{currentF}-$cf$. The dashed green $Left-l$ is set to point to the referent of \texttt{currentL}-$cl$ and the green dashed $Right-r$ is set to point to the referent of the heap node pointed by \texttt{lmParent}-$lm$. What if all of these dashed green pointers and heap nodes were black -- Why don't we just use the type \textsf{rcuItr} for heap allocation? If all were black -- which means all the heap nodes are pointed by \textsf{rcuItr} typed variables -- then we would violate \textit{well-shapedness} related invariants of the data structure. In our \textsf{BST} example, we would invalidate invariants such as the single entry point to the data structure -- both \texttt{root} and \textsf{currentF} would be used as entry points -- and the single path to all heap nodes in the data structure -- both $H_2$ and $H_4$ have 2 paths reaching to them. 
Note that we can neither read a \textsf{rcuFresh} variable nor read a field of the object it points. So we do not allow to create aliases to the fresh variable and the object it points. This restriction localizes our reasoning over the effects due to linking to just one fresh pointer and the object it points. Otherwise, we would need to bookkeep the aliases of the fresh pointer and the object fields of it because once we linked the fresh object to the data structure via using one of its fresh pointer, the fresh pointer gets the type \textsf{rcuItr} and it would require us to change the aliases' types from \textsf{rcuFresh} to \textsf{rcuItr} to prevent inconsistency in between the types of aliases.\begin{comment}
 \begin{figure}[H]
 \centering
 \begin{tikzpicture}[>=stealth',node distance=1.3cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]
 \tikzstyle{solids node}=[rectangle,draw=red,inner sep=1.5]
  \tikzstyle{solidss node}=[dashed,rectangle,draw=red,inner sep=1.5]
  \tikzstyle{freshollow node}=[dashed,circle,draw=green,inner sep=1]

 \tikzstyle{fresh node}=[dashed,rectangle,draw=green,inner sep=1.5]
  
 \tikzstyle{null node}=[circle,draw=red,fill=red]
 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1.5},
 	blue node/.style={rectangle,draw=black,inner sep=1.5},
 	reader node/.style={circle,draw=black,inner sep=1},
        redreader node/.style={circle,draw=red,inner sep=1},
        readerr node/.style={dashed,circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[solid node] (0) [right of=R] {$H_0$};
       \node[solid node] (1) [right of=0] {$H_1$};
       \node[fresh node] (2) [above of=1] {$H_f$};
       \node[solid node] (3) [right of=1] {$H_2$};
       \node[solid node] (4) [above  of=3] {$H_4$};
       %\node[solid node] (6) [above  of=4] {$H_5$};
       %\node[null node] (nl) [above of = 3]{};

       \node[reader node] (r0) [below  of= 0]  {$pr$};
       \node[reader node] (r1) [below  of= 1]  {$cr$};
       \node[freshollow node] (f)  [left  of= 2] {$cf$};
        \node[reader node] (crl)  [below right  of= 3] {$crl$};
        \node[reader node] (lm) [right  of= 4]  {$lm$};


      % \node[reader node] (r1f) [above  of= 5]  {$a_4$};
      % \node[reader node] (r2f)  [above  of= 6] {$a_5$};

     \path[->]  (R) edge node[below] {$l$} (0);
     \path[->]  (0) edge node[below] {$l$} (1);
     \path[->]  (crl) edge  node {} (3);
     \path[dashed,draw=green,->]  (f) edge node {} (2);
     \path[dashed,draw=green,->]  (2) edge node {$r$} (4);
     \path[dashed,draw=green,->]  (2) edge node {$l$} (3);
     \path[->]  (1) edge node {$r$} (4);
     \path[->]  (1) edge node {$l$} (3);
     
     \path[->]  (r0) edge node {} (0);
     \path[->]  (r1) edge node  {}  (1);
     \path[->]  (lm) edge  node  {}   (4);

     %\path[dashed,->]  (r1a) edge node {} (0);
     %\path[dashed,->]  (r2a) edge node  {}  (1);
     %\path[dashed,->]  (r2a) edge  node  {}   (4);

 %    \path[->]  (r1f) edge node  {}  (5);
     %\path[->]  (r2f) edge  node  {}   (6);
     %\path[draw=red, ->] (2) edge node[below] {$r$} (nl);
 ;
 \end{tikzpicture}
 \caption{Allocating a \textit{fresh} heap node pointed by \texttt{currentF}-$cf$}
 \label{fig:alloc}\vspace{-2mm}
 \end{figure}\end{comment}
 
\textit{\textbf{Mutation - Linking a Fresh Node}} - Linking a fresh heap node reference by a \textsf{rcuFresh} pointer mutates the heap so it needs to be handled carefully. We do not discuss the problems that can come up due to both \textit{path-aliasing} and \textit{field-aliasing} as they are same with ones we discussed for unlinking. Similar to the transition from Figure \ref{fig:bframeout} to Figure \ref{fig:bunlinkframeout}, transition from the Figure \ref{fig:frframeout} to \ref{fig:freshframeout} illustrates the effects of the heap mutation (linking a fresh node). The reasoning we make for aliasing in unlinking is also valid in fresh node linking with one exception. To frame linking/replacing action, we do not use abstraction(havocing path) on path reaching to heap nodes deeper than the ones involved in memory footprint which we do for unlinking an heap node. Our type rule for ensuring safe linking(\textsc{T-LinkF})prevents path aliasing  precisely -- nonexistence of $a_0$ and $a_1$ -- via asserting $\lnot((\rho'' = \rho)\lor(\rho'' = \rho'))$ and field mapping aliasing -- nonexistence of any object field from any other context pointing to $cr$ ($o$ in the type rule) -- via asserting $(y\neq o)$.
Among other memory safety issues related to the fresh heap node linking, there is one that we want to raise attention to. When we look at Figure \ref{fig:frframeout}, we see that same object fields from $H_1$ and $H_f$, which are pointed by \texttt{current} ($cr$) and \texttt{currentF} ($cf$) respectively, point to exactly the same heap nodes $H_2$ and $H_4$, which are pointed by $crl$ and $lm$ respectively. This discharges the assertion $\N' = \N''$ in the type rule. So, why do we need this assertion? (Why do we need to capture all field mappings of the node-to-be-unlinked/replaced by the fresh one's field mappings?) In fact, if we did not capture all the field mapping of the node to be unlinked/replaced, we would leak more heap nodes in addition to the one we intend to e.g. the heap node pointed by $cl$. However, our type system allows mutation of a single heap node at a time. We see, in Figure \ref{fig:freshframeout}, that the only replaced/unlinked heap node is the one pointed by $cr$. We should also note that replacement does not change the reachability of any nodes except the one replaced. This leads to an interesting observation: there is not problem in having many pointers to the heap nodes $H_2$ and $H_4$ as pointers to them do not have change in their path components -- e.g. $crl$ and $lm$ do not have change in their path components. 
 \begin{figure}[H]
 \centering
\begin{subfigure}[b]{.4\linewidth}
 \centering
 \begin{tikzpicture}[>=stealth',node distance=1.3cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]
 \tikzstyle{solids node}=[rectangle,draw=red,inner sep=1.5]
  \tikzstyle{solidss node}=[dashed,rectangle,draw=red,inner sep=1.5]
  \tikzstyle{freshollow node}=[dashed,circle,draw=green,inner sep=1]

 \tikzstyle{fresh node}=[dashed,rectangle,draw=green,inner sep=1.5]
  
 \tikzstyle{null node}=[circle,draw=red,fill=red]
 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1.5},
 	blue node/.style={rectangle,draw=black,inner sep=1.5},
 	reader node/.style={circle,draw=black,inner sep=1},
        redreader node/.style={circle,draw=red,inner sep=1},
        readerr node/.style={dashed,circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[solids node] (0) [right of=R] {$H_0$};
       \node[solids node] (1) [right of=0] {$H_1$};
       \node[fresh node] (2) [above of=1] {$H_f$};
       \node[solid node] (3) [right of=1] {$H_2$};
       \node[solid node] (4) [above  of=3] {$H_4$};
              \node[solid node] (5) [above left of=0] {$H_5$};
       \node[solid node] (6) [above left of = 1]{$H_6$};
      

       \node[redreader node] (r0) [below  of= 0]  {$pr$};
       \node[redreader node] (r1) [below  of= 1]  {$cr$};
       \node[freshollow node] (f)  [above  of= 2] {$cf$};
        \node[reader node] (crl)  [right  of= 3] {$crl$};
       \node[reader node] (lm) [right  of= 4]  {$lm$};
       \node[readerr node] (r1a) [below   of= R]  {$a_0$};
       \node[readerr node] (r2a)  [below of= 3] {$a_1$};

       \node[reader node] (r1f) [above  of= 5]  {$a_5$};
       \node[reader node] (r2f)  [above  of= 6] {$a_6$};

     \path[->]  (R) edge node[below] {$l$} (0);
     \path[draw=red,->]  (0) edge node[below] {$l$} (1);
     \path[->]  (crl) edge  node {} (3);
     \path[dashed,draw=green,->]  (f) edge node {} (2);
     \path[dashed,draw=green,->]  (2) edge node {$r$} (4);
     \path[dashed,draw=green,->]  (2) edge node {$l$} (3);


     \path[dashed,->]  (5) edge node {$l$} (0);
     \path[dashed,->]  (6) edge node {$l$} (1);


     \path[draw=red,->]  (1) edge node {$r$} (4);
     \path[draw=red,->]  (1) edge node {$l$} (3);
     
     \path[draw=red,->]  (r0) edge node {} (0);
     \path[draw=red,->]  (r1) edge node  {}  (1);
     \path[->]  (lm) edge  node  {}   (4);

     \path[dashed,->]  (r1a) edge node {} (0);
     \path[dashed,->]  (r2a) edge node  {}  (1);
     
     \path[->]  (r1f) edge  node  {}   (5);
     \path[->]  (r2f) edge  node  {}   (6);


     %\path[draw=red, ->] (2) edge node[below] {$r$} (nl);
 ;
 \end{tikzpicture}

 \caption{Safe linking of the \textit{fresh} heap node pointed by \texttt{currentF}-$cf$}
 \label{fig:frframeout}
 \end{subfigure} \quad
 \begin{subfigure}[b]{.4\linewidth}
 \centering
 \begin{tikzpicture}[>=stealth',node distance=1.3cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]
 \tikzstyle{solids node}=[rectangle,draw=red,inner sep=1.5]
  \tikzstyle{solidss node}=[dashed,rectangle,draw=red,inner sep=1.5]
  \tikzstyle{freshollow node}=[dashed,circle,draw=green,inner sep=1]

 \tikzstyle{fresh node}=[dashed,rectangle,draw=green,inner sep=1.5]
  
 \tikzstyle{null node}=[circle,draw=red,fill=red]
 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1.5},
 	blue node/.style={rectangle,draw=black,inner sep=1.5},
 	reader node/.style={circle,draw=black,inner sep=1},
        redreader node/.style={circle,draw=red,inner sep=1},
        readerr node/.style={dashed,circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1},
               rredreader node/.style={dashed,circle,draw=red,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[solids node] (0) [right of=R] {$H_0$};
       \node[solidss node] (1) [right of=0] {$H_1$};
       \node[solid node] (2) [above of=1] {$H_f$};
       \node[solid node] (3) [right of=1] {$H_2$};
       \node[solid node] (4) [above  of=3] {$H_4$};
       \node[solid node] (5) [above of=R] {$H_5$};
       \node[solid node] (6) [above of = 0]{$H_6$};

       \node[redreader node] (r0) [below  of= 0]  {$pr$};
       \node[rredreader node] (r1) [below  of= 1]  {$cr$};
       \node[reader node] (f)  [above  of= 2] {$cf$};
        \node[reader node] (crl)  [ right  of= 3] {$crl$};
       \node[reader node] (lm) [right  of= 4]  {$lm$};
       \node[readerr node] (r1a) [below   of= R]  {$a_0$};
       \node[readerr node] (r2a)  [below of= 3] {$a_1$};

      \node[reader node] (r1f) [above  of= 5]  {$a_5$};
      \node[reader node] (r2f)  [above  of= 6] {$a_6$};

     \path[->]  (R) edge node[below] {$l$} (0);
    % \path[draw=red,->]  (0) edge node[below] {$l$} (1);
     \path[->]  (crl) edge  node {} (3);
     \path[->]  (f) edge node {} (2);
     \path[->]  (2) edge node {$r$} (4);
     \path[->]  (2) edge node {$l$} (3);
     \path[dashed,draw=red,->]  (1) edge node {$r$} (4);
     \path[dashed,draw=red,->]  (1) edge node {$l$} (3);




     \path[draw=red,->]  (r0) edge node {} (0);
     \path[dashed,draw=red,->]  (r1) edge node  {}  (1);
     \path[->]  (lm) edge  node  {}   (4);

     \path[dashed,->]  (r1a) edge node {} (0);
     \path[dashed,->]  (r2a) edge node  {}  (1);
          \path[dashed,->]  (5) edge node {$l$} (0);
     \path[dashed,->]  (6) edge node {$l$} (1);


     %\path[dashed,->]  (r2a) edge  node  {}   (4);

     \path[draw=red,->]  (0) edge node  {$l$}  (2);


     \path[->]  (r1f) edge  node  {}   (5);
     \path[->]  (r2f) edge  node  {}   (6);


 ;
 \end{tikzpicture}

 \caption{Safe replacement of the heap node pointed by \texttt{current}-$cr$ by the \textit{fresh} heap node pointed by \texttt{currentF}-$cf$}
 \label{fig:freshframeout}
 \end{subfigure}
 \label{fig:alloc}\vspace{-2mm}
 \end{figure}
\textit{\textbf{Mutation - Reclaiming a Heap Node after a Grace Period}} - The reason why we have type \textsf{freeable} after the grace period is to prevent the ability to call \texttt{Free} before the grace period ends. This means that we cannot give ownership of a heap node to heap right after unlinking. Our type system ensures this via enforcing that we call \texttt{Free} only with a pointer in type \textsf{freeable}.

To get \textsf{freeable} pointer, first we wait the grace period \texttt{SyncStart};\texttt{SyncStop} for unlinked heap nodes to end. The \texttt{SyncStart} does not have any effect on type of the variables.

(\textit{\textbf{Referencing inside \textsf{RCU} Blocks} } ) - There are two rules shown in Figure \ref{fig:ts} for moving between the different type systems: one for entering a write region, and one for a read region. The type rules for outside an RCU region are otherwise straightforward and restrict $\Gamma$ to only mention variables of type $\textsf{normal}$; that is, we cannot read or write to \textsf{RCU} structures.


==> chapters/RCURules.tex <==
\makeatletter % allow us to mention @-commands
\def\arcr{\@arraycr}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%SUB TYPING JUDGEMENTS%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}\tiny
%\begin{subfigure}[b]{.4\linewidth}
\begin{mathpar}
 \fmapextendn \and \fmapname  \and \fmapdiff \and \fmapwithf \and \fmapextend \and \fmapempty \and \fmapfieldemp \and \typelocalmap \and \typeglobal \and \rcutypes \and \types \and  \ftypedecl \and \rpth 
\and
\fbox{$\vdash \, \N \subt \N'$} \;\;
\inferrule[\scriptsize{T-NSub3}]
{
\N'([f \rightharpoonup y]) \;\;
\N_{f,\emptyset}
}
{\vdash \, \N\subt \N'}
\and
\inferrule[\scriptsize{T-NSub4}]
{
 \N' \;\;
 \N_{\emptyset}
}
{\vdash \, \N \subt \N'}
\and
\inferrule[\scriptsize{T-NSub2}]
{
 \N([f_2 \rightharpoonup y]) \;\;
\N'([f^{*} \rightharpoonup y])
}
{\vdash \, \N\subt \N'}
\and
\inferrule[\scriptsize{T-NSub1}]
{
\N([f_1 \rightharpoonup y]) \;\;
 \N'([f^{*} \rightharpoonup y])
}
{\vdash \, \N \subt \N'}
\and
\inferrule[\scriptsize{T-NSub5}]
{
}
{\vdash \, \N \subt \N}
\and
\fbox{$\vdash \, \rho \subt \rho'$} \;\;
\inferrule[\scriptsize{T-PSub1}]
{
\rho'=\rho''.f_1 \qquad \rho = \rho''.f_1|f_2
}
{
 \vdash  \rho' \subt \rho
}
\and
\inferrule[\scriptsize{T-PSub2})]
{
\rho'=\rho''.f_2  \qquad \rho= \rho''.f_1|f_2
}
{
 \vdash  \rho' \subt \rho
}
\and
\fbox{$\vdash \, \rho \subt \rho'$} \;\;
\inferrule[\scriptsize{T-TSub}]
{
T=\textsf{rcuItr}\; \_ \qquad T'=\textsf{undef}
}
{
\vdash T   \subt T' 
}
\and
\inferrule[\scriptsize{T-TSub1}]
{
\vdash\rho\subt \rho' \qquad \vdash \N \subt \N' \\
T =\textsf{rcuItr} \, \rho \, \N \qquad T'=\textsf{rcuItr} \, \rho' \, \N'
}
{
\vdash T  \subt  T'
}
\and
\fbox{$\vdash \, \Gamma \subt \Gamma'$} \;\;
\inferrule[\scriptsize{T-CSub1}]
{
\vdash\Gamma \subt \Gamma' \;\; \vdash \text{T}  \subt \text{T'}
}
{
\vdash \Gamma\, , x:\text{T}  \subt \Gamma'\, , x:\text{T'}
}
\and
\inferrule[\scriptsize{T-CSub2}]
{
\Gamma' = \Gamma[\rho.f^{k}/\rho.f^{k}.f]
}
{
 \vdash  \Gamma \subt \Gamma'
}
\and
\inferrule[\scriptsize{T-ESub}]
{
}
{
\vdash  \epsilon \subt \epsilon
}\and
%\end{mathpar}
%\caption{Sub-Typing Judgements}
%\label{fig:sub-typing}
%\end{subfigure}\quad
%\begin{subfigure}[b]{.4\linewidth}
%\tiny
%\begin{mathpar}
\fbox{$\Gamma \vdash \bar{s} \dashv \Gamma'$} \and
\inferrule[\scriptsize(T-Branch1)]
{
  x.f_1==z \and
 \Gamma\, ,x:\textsf{rcuItr}\,\rho \, \N([f_1 \rightharpoonup  z]) \vdash \bar{s}_1 \dashv\Gamma_4 \and
  \Gamma\, ,x:\textsf{rcuItr}\, \rho \, \N([f_2 \rightharpoonup z]) \vdash \bar{s}_2 \dashv \Gamma_4
}
{
\Gamma\, ,x:\textsf{rcuItr}\, \rho \, \N([f_1\mid f_2 \rightharpoonup z]) \vdash \textsf{if}(x.f_1==z)  \textsf{ then } \bar{s}_1 \textsf{ else } \bar{s}_2 \dashv \Gamma_4
}
\and
\inferrule[\scriptsize(T-Branch2)]
{
\Gamma(x)= \textsf{bool} \\
 \Gamma \vdash \bar{s}_1 \dashv\Gamma' \and \Gamma \vdash \bar{s}_2 \dashv \Gamma'
}
{
\Gamma \vdash \textsf{if}(x) \textsf{ then } \bar{s}_1  \textsf{ else } \bar{s}_2 \dashv \Gamma'
}
\and
\inferrule[\scriptsize(T-Branch3)]
{
 \Gamma,\,x:\textsf{rcuItr} \, \rho \, \N([f\rightharpoonup y \setminus \textsf{null}]) \vdash \bar{s}_1 \dashv \Gamma' \and \Gamma,\,x:\textsf{rcuItr} \, \rho \, \N([f\rightharpoonup y]) \vdash \bar{s}_2 \dashv \Gamma'
}
{
\Gamma,\,x:\textsf{rcuItr} \, \rho \, \N([f\rightharpoonup y]) \vdash \textsf{if}(x.f == \textsf{null}) \textsf{ then } \bar{s}_1  \textsf{ else } \bar{s}_2 \dashv \Gamma'
}
\and
\inferrule[\scriptsize(T-Frame)]
{
\Gamma_1 \vdash \bar{s} \dashv \Gamma_2   \and
\textsf{WellFramed}(\Gamma, \Gamma_1) \and \textsf{WellFramed}(\Gamma, \Gamma_2)
}
{
\Gamma, \; \Gamma_1 \vdash \bar{s} \dashv \Gamma, \; \Gamma_2
}
\and
\inferrule[\scriptsize(T-Conseq)]
{
 \Gamma \subt \Gamma'  \and \Gamma' \vdash \bar{s} \dashv \Gamma'' \and \Gamma'' \subt \Gamma'''
}
{
 \Gamma \vdash \bar{s} \dashv \Gamma'''
}
\and
\inferrule[\scriptsize(T-Loop1)]
{
\Gamma(x) = \textsf{bool} \and
\Gamma \vdash \bar{s} \dashv \Gamma 
}
{
\Gamma \vdash \textsf{while}(x)\{\bar{s}\} \dashv  \Gamma
}
\and
\inferrule[\scriptsize(T-Loop2)]
{
\Gamma,\, x:\textsf{rcuItr}\;\rho \; \N([f\rightharpoonup \_]) \vdash \bar{s} \dashv \Gamma, x:\textsf{rcuItr}\;\rho' \; \N([f\rightharpoonup \_])
}
{
\Gamma,\, x:\textsf{rcuItr}\;\rho \; \N([f\rightharpoonup \_]) \vdash \textsf{while}(x.f \neq \textsf{null})\{\bar{s}\} \dashv   x:\textsf{rcuItr}\;\rho' \; \N([f\rightharpoonup \textsf{null}]) ,\,  \Gamma
}
\and
\inferrule[\scriptsize(T-ReIndex)]
{
}
{
\Gamma \vdash \bar{s}_{k} \dashv  \Gamma[\rho.f^{k}/\rho.f^{k}.f]
}\and
%\end{mathpar}
%\caption{Type Judgements for Control-Flow.}
%\label{fig:type-judgements-for-cf}
%\end{subfigure}\quad
%%%%%%%%%%%%%%%%%%%%%%%%TYPE JUDEGEMENT%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{subfigure}[b]{.4\linewidth}
%\begin{mathpar}
\inferrule[\scriptsize(T-Root)]
{ \textsf{FV}(\Gamma) \cap \{r,y\}  =\emptyset}
{\Gamma\,,r:\textsf{rcuRoot}\,,y:\textsf{undef} \vdash_{M,R} y = r \dashv y: \textsf{rcuItr}\, \epsilon \, \N_{\emptyset}\,,r:\textsf{rcuRoot}\,,\Gamma}
\;\;
\inferrule[\scriptsize(T-ReadS)]
{ \textsf{FV}(\Gamma) \cap \{z,x\}  =\emptyset}
{
\Gamma\,, z:\textsf{rcuItr}\,\_ \, ,\rcuitrT{x}{G}{k}{k+1}{\_} \vdash_{M,R} z=x \dashv  \rcuitrT{x}{G}{k}{k+1}{\_}\, , \rcuitrT{z}{G}{k}{k+1}{\_} \,, \Gamma
}
\and
\inferrule[\scriptsize(T-ReadH)]
{
\rho.f=\rho' \\
 \textsf{FV}(\Gamma) \cap \{z,x\} =\emptyset
}
{
 \Gamma\, , z:\textsf{rcuItr}\,\_ \, ,  x:\textsf{rcuItr} \, \rho \, \N   \vdash_{M,R}
 	z=x.f
 \dashv  x:\textsf{rcuItr} \, \rho \, \N[f\mapsto z]\, ,z:\textsf{rcuItr} \, \rho' \, \N_{\emptyset} \, , \Gamma
}
\and
\inferrule[\scriptsize(T-Alloc)]
{
\mathsf{FV}(\Gamma) \cap \{x\} = \emptyset
}
{
 \Gamma\,, x:\textsf{undef} \vdash_{M} x = \NEW \dashv x:\textsf{rcuFresh} \, \N_{\emptyset} \, ,  \Gamma
}
\and
\inferrule[\scriptsize(T-Free)]
{
}
{
x:\textsf{freeable} \vdash_{M} \textsf{Free}(x) \dashv x:\textsf{undef}
}\;\;
\inferrule[\scriptsize(T-Exchange)]
{
 \Gamma, \, y:T' , \, x:T, \, \Gamma' \vdash \bar{s} \dashv   \Gamma''
}
{
\Gamma, \, x:T , \, y:T' , \, \Gamma' \vdash \bar{s} \dashv   \Gamma''
}
\and
\inferrule[\scriptsize(T-Sync)]
{
\textsf{FV}(\Gamma) \cap \textsf{FV}(\Gamma'')  = \emptyset \\
\lnot(\exists_{x \in \Gamma''} \ldotp x:\textsf{unlinked}) \\
\forall x \in \Gamma \ldotp  x:\textsf{unlinked} \quad \Gamma'  = \forall_{x\in \Gamma }\ldotp \Gamma \setminus \{x:\textsf{unlinked}\} \cup \{x:\textsf{freeable}\} \\
\Gamma'',\Gamma \vdash_{M}\textsf{SyncStart}\dashv\Gamma'',\Gamma \qquad \Gamma'',\Gamma \vdash_{M}\textsf{SyncStop}\dashv\Gamma'',\Gamma' \qquad
}
{
\Gamma'',\Gamma \vdash_{M} \textsf{SyncStart};\textsf{SyncStop} \dashv \Gamma',\Gamma''
}
\and
\inferrule[\scriptsize(T-WriteFH)]
{
\textsf{FV}(\Gamma) \cap \{p,z,x\}  =\emptyset \\ z:\textsf{rcuItr} \; \rho.f \; \_
}
{
 \Gamma, p:\textsf{rcuFresh}\,\N_{f,\emptyset},\; x:\textsf{rcuItr}\;\; \rho \;\; \N([f\rightharpoonup z])
  \vdash_{M} p.f = z \dashv
  \rcunf{p}{f}{z} \, , x:\textsf{rcuItr}\, \rho \, \N([f\rightharpoonup z]), \, \Gamma
}
\and
\inferrule[\scriptsize(T-UnlinkH)]
{
\textsf{FV}(\Gamma) \cap \{x,z,r\} \qquad \rho.f_1=\rho' \;\; \rho'.f_2=\rho'' \qquad \forall_{f\in dom(\N')} \ldotp f\neq f_2 \implies \N'([f\rightharpoonup \textsf{null}]) \lor \N'_{f,\emptyset}   \\
\begin{array}{l}
\forall_{n\in \Gamma,m,\N''', p''',f}\ldotp n:\textsf{rcuItr}\,\rho'''\,\N'''([f\rightharpoonup m]) \implies 
\left\{\begin{array}{l}
(((\rho \neq \rho''' \land \rho' \neq \rho''' \land \rho'' \neq \rho''')  ) \land (\{m\} \cap \{z,r\} = \emptyset ) ) \arcr
\land (\forall_{\rho''''\neq \epsilon} \ldotp \rho''' = \rho''.\rho'''' \implies \lnot(\exists_{f'}\ldotp ( \N(f')=n \lor \N'(f')=n  \lor \N''(f')=n )))
\end{array}\right.
\end{array}
}
{
\Gamma,\,x:\textsf{rcuItr}\, \rho \, \N([f_1\rightharpoonup z]) \, ,
z:\textsf{rcuItr}\, \rho' \, \N'([f_2\rightharpoonup r]) \, ,  r:\textsf{rcuItr} \, \rho'' \, \N''\, 
\vdash_{M} x.f_1=r \dashv
z:\unlinked\, ,
x:\textsf{rcuItr} \, \rho \, \N(f_1\rightharpoonup z \setminus r)\, ,
r:\textsf{rcuItr} \, \rho' \, \N'',\, \Gamma
}
\and
\inferrule[\scriptsize(T-LinkF)]
{
\rho.f  = \rho'  \qquad \N' = \N'' \qquad  \textsf{FV}(\Gamma) \cap \{p,o,n\}  =\emptyset \\
\lnot(\exists_{x \in \Gamma, \N''', \rho'',f',y} \ldotp (x:\textsf{rcuItr}\,\rho''\,\N'''([f'\rightharpoonup y])) \land ((\rho'' = \rho)\lor(\rho'' = \rho')) \land (y\neq o \land (\forall_{x_i \in codom(\N')} \ldotp y \neq x_i  ) ) )
}
{
\Gamma,\,
 p:\textsf{rcuItr}\, \rho \, \N([f\rightharpoonup o]) \, ,
  o:\textsf{rcuItr}\, \rho' \, \N' \, , n:\textsf{rcuFresh} \, \N''
  \vdash_{M} p.f = n \dashv
  p:\textsf{rcuItr}\, \rho \, \N(f \rightharpoonup o \setminus n) \, ,
  n:\textsf{rcuItr}\, \rho' \, \N'' \,
  o:\unlinked\, ,  \Gamma
}
\and
\inferrule[\scriptsize(T-Seq)]
{
\Gamma_1 \vdash \bar{s_1} \dashv_{M,R}   \Gamma_2  \qquad   \Gamma_2 \vdash_{M,R} \bar{s_2} \dashv   \Gamma_3
}
{
\Gamma_1  \vdash_{M,R} \bar{s_1} \; ; \; \bar{s_2} \dashv  \Gamma_3
}
\and
\inferrule[\scriptsize(T-Par)]
{
 \Gamma_1 \vdash_{R} \bar{s_1} \dashv   \Gamma'_1  \qquad   \Gamma_2 \vdash_{M,R} \bar{s_2} \dashv   \Gamma'_2
}
{
 \Gamma_1, \; \Gamma_2  \vdash \bar{s_1} || \bar{s_2} \dashv  \Gamma'_1 \; , \Gamma'_2
}
\and
\inferrule[\scriptsize(T-Skip)]
{
}
{
 \Gamma \vdash_{M,R} \textsf{skip} \dashv   \Gamma
}
\end{mathpar}
%\caption{Type Rules for other program statements}
%\label{fig:type-judgements}
%\end{subfigure}
\label{fig:ts}
\caption{Type Rule for \textsf{RCU} Programming}
\end{figure}
%%%%%%%%%%%%%%%COND TYPE JUDGEMENTS ENDS%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> chapters/RCUSemanticsOld.tex <==
\section{Semantics}
\label{sec:semantics}
In this section, we outline the details of a simple RCU implementation, and provide the semantics for it. Note that the implementation provided below is focused on illustrating how RCU works, rather than efficiency, and It captures the core semantics of RCU.  As the paper focuses on the correct usage of RCU, rather than the correctness of the implementation, we do not discuss how to efficiently realise the semantics~\cite{Mckenney01read-copyupdate}.
\begin{figure}\scriptsize %\fontsize{4}{12}
\grammar
\meta
% Well formed programs, declarations...
\caption{\texttt{Programming Language} for \textsf{RCU} programming.}
\label{fig:prog-lang}
\end{figure}
RCU allows a single mutator thread and  multiple  reader threads to traverse a data structure. When a writer mutates some state, it waits  until all concurrent reads are completed to free the mutated state. To represent this in our semantics, we augment the  machine state,$\textsf{MState}$, ranged over by $\sigma$, consists of:
\begin{itemize}
\item A stack $s$, of type $\textsf{Var} \times \textsf{TID} \rightharpoonup \textsf{Loc}$
\item A heap, $h$, of type $\textsf{Loc} \times \textsf{FName} \rightharpoonup \textsf{Val}$
\item A write lock, $l$, of type $\textsf{TID} \uplus \{\textsf{unlocked}\}$
\item A root location $rt$ of type $\textsf{Loc}$
\item A read set, $R$, of type $\mathcal{P}(\textsf{TID})$
\item A bounding set, $B$, of type $\mathcal{P}(\textsf{TID})$ and
\item A to-free map, $F$, of type $\textsf{Loc} \rightharpoonup \mathcal{P}(\textsf{TID})$
\end{itemize}
The write lock, $l$, enforces mutual exclusion between write-side critical sections.
The root location, $rt$, is the root of  an \textsf{RCU} data structure. We model only a single global RCU data structure, as the generalization to multiple structures is straightforward but complicates formal development later in the paper.
The read set, $R$, tracks the thread IDs of all threads currently executing a read block. 
The bounding set , $B$, tracks which threads the writer is \emph{actively} waiting for during a grace period --- it is empty if the writer is not waiting.
The final component of the machine state is the free map, $F$, which tracks for each location in memory the set of reader threads that may still hold stack references to it.  It is not required for execution of code, and for validating an implementation could be ignored, but we use it later with our type system to help prove that memory deallocation is safe.
\begin{figure*}%%%%%%%%%%%%OPdERATIONAL SEMANTICS%%%%%%%%%%%%%%
\tiny
%\begin{mathpar}
%\atomeval \and \heap \and \stack \and \wlock \and \rlock \and \fset \and \mstatedecl
%\end{mathpar}
\[\begin{array}{c@{\;}rl@{\Downarrow_{\mathit{tid}}}ll}
(\textsc{HUpdate}) & \llbracket\texttt{x.f=y}\rrbracket   &(s,h,l,rt,R,B,F)& (s,h[s(x,tid),f \mapsto s(y,tid)],l,rt,R,B,F) &\textrm{where}~ rt \neq s(y,tid)\\
(\textsc{HRead})   & \llbracket\texttt{y=x.f}\rrbracket   &(s,h,l,rt,R,B,F)& (s[(y,tid) \mapsto h(s(x,tid),f)],h,l,rt,R,B,F) & \\
(\textsc{SUpdate}) & \llbracket\texttt{y=x}\rrbracket     &(s,h,l,rt,R,B,F)& (s[(y,tid) \mapsto (x,tid)],h,l,rt,R,B,F) &\\
(\textsc{HAllocate}) & \llbracket\texttt{y=new}\rrbracket &(s,h,l,rt,R,B,F)& (s,h[\ell\mapsto\mathsf{nullmap}],l,rt,R,B,F) & \textrm{where}~ rt \neq s(y,tid) \\
(\textsc{RCU-W-Begin}) & \llbracket\texttt{WriteBegin}\rrbracket & (s,h,\mathsf{unlocked},rt,R,B,F) &(s,h,\mathit{tid},rt,R,B,F) & \textrm{where}~\mathit{tid}\notin R\\
(\textsc{RCU-W-End}) & \llbracket\texttt{WriteEnd}\rrbracket & (s,h,\mathrm{tid},rt,R,B,F) & (s,h,\mathsf{unlocked},rt,R,B,F) & \textrm{where}~\mathit{tid}\notin R\\
(\textsc{RCU-R-Begin}) & \llbracket\texttt{ReadBegin}\rrbracket & (s,h,l,rt,R,B,F) & (s,h,l,rt,R\uplus tid,B,F) & \textrm{where}~\mathit{tid}\neq l\\
(\textsc{RCU-R-End}) & \llbracket\texttt{ReadEnd}\rrbracket & (s,h,l,rt,R\uplus\{tid\},B,F) & (s,h,l,rt,R,B\setminus \{tid\},F / tid)  &
\textrm{where}~\mathit{tid}\neq l\\
(\textsc{RCU-Synch-Start}) & \llbracket\texttt{SyncStart}\rrbracket & (s,h,l,rt,R,\emptyset,F) & (s,h,l,rt,R,R,F\cup\{s(x,tid)\mapsto R \mid (x,tid)\in\mathsf{dom}(s)\} & \textrm{where}~\mathit{tid} \notin R \\ %\forall_{t\in R}\ldotp t \notin r
(\textsc{RCU-Synch-Stop}) & \llbracket\texttt{SyncStop}\rrbracket & (s,h,l,rt,R,\emptyset,F) & (s,h,l,rt,R,\emptyset,F) & \textrm{where}~\mathit{tid} \notin R \\
(\textsc{Free}) & {\llbracket\texttt{Free}(x)\rrbracket} & (s,h,l,rt,R,B,F\cup \{s(x,tid)\mapsto \{\emptyset\} \}) & (s,h,l,rt,R,B,F\setminus \{s(x,tid)\mapsto \{\emptyset\} \} ) & \textrm{where}~\mathit{tid} \notin R \\
\end{array}
\]
\[\textrm{where}~ \textsf{F} / tid \textrm{ is provided as } \{o \mapsto T \setminus \{tid\} | \{o \mapsto T \} \in F \}\]
\caption{Operational Semantics for RCU Programming Model }
\label{fig:operationalsemrcu}
\end{figure*}%%%%%%%%%%%%%%%%%%%%%OPERATIONAL SEMANTICS ENDS%%%%%%%%%%%%%%%%%%
In the figure \ref{fig:operationalsemrcu}, we give operational semantics for \emph{atomic} actions; conditionals, loops, and sequencing all have standard semantics, and parallel composition  uses sequentially-consistent interleaving semantics.

\paragraph{Basic Actions} The first few atomic actions, for writing and reading fields, assigning among local variables, and allocating new objects, are typical of formal semantics for heaps and mutable local variables.
\paragraph{Writer Thread Actions}
A writer thread's critical section is bounded by \lstinline|WriteBegin| and \lstinline|WriteEnd|, which acquire and release the lock that enforces mutual exclusion between writers.  \lstinline|WriteBegin| requires the lock to be unlocked in order to reduce, so a thread whose next action is \lstinline|WriteBegin| will block if another thread currently holds the lock.

Standard RCU APIs include a primitive \texttt{synchronize\_rcu()} to wait for a grace period for the current readers.  We decompose this here into two actions, \lstinline|SyncStart| and \lstinline|SyncStop|, for reasons both pedagogical (to separate the start of the grace period from its completion), and technical (our proof framework makes this formulation most convenient).
\lstinline|SyncStart| makes two changes.  First, it initializes the blocking set to the current set of readers --- the set of threads that may have already observed any nodes the writer has unlinked.
\lstinline|SyncEnd| does not change state, but requires the blocking set to be empty to run, and thus blocks when it is non-empty.  Reader threads are responsible for shrinking the blocking set. Once the grace period ends, the unlinked/mutated node is reclaimed with \lstinline|Free|.
\paragraph{Reader Thread Actions}
A reader thread, like the writer thread, has a critical section, in this case bounded by \lstinline|ReadBegin| and \lstinline|ReadEnd|.  \lstinline|ReadBegin| simply records the current thread's presence as an active reader.
\lstinline|ReadEnd| removes the current thread from the set of active readers, and also removes it (if present) from the blocking set --- if a writer was waiting for a certain reader to finish its critical section, this ensures the writer no longer waits once that reader has finished its active read-side critical section.
\paragraph{Implementing Grace Periods}
\lstinline|ReadBegin|, \lstinline|ReadEnd|, \lstinline|SyncStart|, and \lstinline|SyncStop| work together to implement grace periods.  \lstinline|ReadBegin| ensures the set of active readers is known.  When a writer thread needs to wait through a grace period \lstinline|SyncStart;SyncStop;| will initialize the set $B$ of threads the writer waits for to the set of active readers when \lstinline|SyncStart| is executed (recording the readers that may have observed any nodes unlinked by the writer), and \lstinline|SyncStop| waits for that set of threads to become empty.
\lstinline|ReadEnd| ``informs'' the writer thread of its exit from the critical section by removing itself from $B$, and once every reader that overlapped the \lstinline|SyncStart| has completed its critical section, the blocking set will be empty and the writer will resume.

These semantics do permit a reader in the blocking set to finish its read-side critical section and enter a \emph{new} read-side critical section before the writer wakes.  In this case, \emph{the writer waits only for the first critical section of that reader to complete}, since entering the new critical section adds the thread's ID back to $R$, but not $B$.
\begin{comment}
Next, we introduce the instantiation of concrete program states and transitions in between these states for our introductory example, bag example shown in the figure \ref{fig:rculist}. Figures \ref{fig:readlist}-\ref{fig:prereclaim} show the crucial program states in \textsf{RCU} setting.
 \begin{figure}[H]
\centering
 \begin{tikzpicture}[>=stealth',node distance=1.5cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]

 \tikzset{
 	red node/.style={rectangle,draw=black,fill=black,inner sep=1.5},
 	blue node/.style={rectangle,draw=black,inner sep=1.5},
 	reader node/.style={circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1}
 }

     \node[solid node] (R) {$R$};
     \node[hollow node] (5) [right of=R] {$5$};
    \node[hollow node] (8) [right of=5] {$8$};
     \node[hollow node] (2) [right of=8] {$2$};
     \node[hollow node] (1) [right of=2] {$1$};
    \node[hollow node] (11) [right of=1] {$11$};
     %\node[hollow node] (4) [right of=11] {$4$};
   \node[reader node] (r1) [above right of= 1]  {$cr$};
     \node[reader node] (r2)  [above left of= 1] {$cr$};

     \path[->]   (R) edge node {} (5)
                 (5) edge node {} (8)
 		(8) edge node {} (2)
 		(2) edge node {} (1)
 		(1) edge node {} (11)
 	%	(11) edge node {} (4)
 		(r1) edge node {$\textsf{tid}_{r1}$} (1)
 		(r2) edge node {$\textsf{tid}_{r2}$} (1)
 ;
 \end{tikzpicture}
 \caption{$R$ is unique root of the \textsf{RCU} singly linked list. Two concurrent reader threads with $\textsf{tid}_{r1}$ and $\textsf{tid}_{r2}$ ids are on the node with value 1. These threads have their own iterators $\textsf{cr}$ on linked list. }
 \label{fig:readlist}
 \end{figure}
 In the figure \ref{fig:readlist}, there are two reader threads in read block, $R\uplus \{tid_{r1},tid_{r2}\}$.

 \begin{figure}[H]
 \centering
 \begin{tikzpicture}[>=stealth',node distance=1.5cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]

 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1.5},
 	blue node/.style={rectangle,draw=black,inner sep=1.5},
 	reader node/.style={circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[hollow node] (5) [right of=R] {$5$};

       \node[hollow node] (8) [right of=5] {$8$};
       \node[hollow node] (2) [right of=8] {$2$};
       \node[hollow node] (1) [right of=2] {$1$};
       \node[hollow node] (11) [right of=1] {$11$};
      % \node[hollow node] (4) [right of=11] {$4$};
       \node[reader node] (r1) [above right of= 1]  {$cr$};
       \node[reader node] (r2)  [above left of= 1] {$cr$};
       \node[writer node] (wp) [below of=2] {$pr$};
       \node[writer node] (wc) [below of=1]{$cr$};

     \path[->]   (R) edge node {} (5)
     		(5) edge node {} (8)
      		(8) edge node {} (2)
      	%	(11) edge node {} (4)
     		(1) edge node {} (11)
 		(2) edge node {} (1)
 		(r1) edge node {$\textsf{tid}_{r1}$} (1)
 		(r2) edge node {$\textsf{tid}_{r2}$} (1)
 	        (wp) edge node  {$\textsf{tid}_{mut}$}  (2)
 		(wc) edge  node  {$\textsf{tid}_{mut}$}   (1)
 ;
 \end{tikzpicture}
 \caption{$\textsf{tid}_{mut}$ traverses the list to deletes the node with value 1.}
 \label{fig:mutatelist}
 \end{figure}

 Writer thread in in the figure \ref{fig:mutatelist}, $tid_{mut}$, is shown in program state as $l=tid_{mut}$.
 \begin{figure}[H]
 \centering
 \begin{tikzpicture}[>=stealth',node distance=1.5cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]

 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1.5},
 	blue node/.style={rectangle,draw=black,inner sep=1.5},
 	reader node/.style={circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=black,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[hollow node] (5) [right of=R] {$5$};
       \node[hollow node] (8) [right of=5] {$8$};
       \node[hollow node] (2) [right of=8] {$2$};
       \node[hollow node] (1) [right of=2] {$1$};
       \node[hollow node] (11) [right of=1] {$11$};
       %\node[hollow node] (4) [right of=11] {$4$};
       \node[reader node] (r1) [above right of= 1]  {$cr$};
       \node[reader node] (r2)  [above left of= 1] {$cr$};
       \node[writer node] (wp) [below of=2] {$pr$};
       \node[writer node] (wc) [below of=11]{$cr$};

     \path[->]  (R) edge node {} (5);
     \path[->]  (5) edge node {} (8);
     \path[->]  (8) edge node {} (2);
    % \path[->]  (11) edge node {} (4);
     \path[->] (2) edge [bend right] node {} (11);
     \path[dashed,->]  (1) edge node {} (11);

     \path[->]  (r1) edge node {$\textsf{tid}_{r1}$} (1);
     \path[->]  (r2) edge node {$\textsf{tid}_{r2}$} (1);
     \path[->]  (wp) edge node  {$\textsf{tid}_{mut}$}  (2);
     \path[->]  (wc) edge  node  {$\textsf{tid}_{mut}$}   (11);
 ;
 \end{tikzpicture}
 \caption{$\textsf{tid}_{mut}$ unlinks the node with value 1.}
 \label{fig:unlinkedlist}
 \end{figure}
\ref{fig:unlinkedlist} shows heap update. Writer thread updates the field of the node pointed by 2 to show the node pointed by 11, $h[s(2,tid_{mut}),f \mapsto s(11,tid_{mut})]$. At this point, read set, $R=\{tid_{r1},tid_{r2}\}$, shows the node 1 which is \emph{unlinked}.

After heap update, \lstinline{SyncStart} exexutes to start the \emph{grace period} for the read set, $R=\{tid_{r1}, tid_{r2}\}$. $B$ is set to $R$, $B=\{tid_{r1}, tid_{r2}\}$. $B$ keeps the threads that need to be waited for, and it reclaims the mutated heap location, $S(1)$. In addition to bounding set, $B$, \lstinline{SyncStart} also updates the free map, $F$, with mapping read set to unlinked nodes which have a potential to be reclaimed, $F=\{(R,S(1))\}$.

Grace period lasts until the \lstinline{SyncStop} returns. \emph{Pre-state} to call \lstinline{SycnStop} has bounding set empty, $B = \{\emptyset\}$. This means that all bounding threads exit read block with executing \textsf{ReadEnd}. Exiting read block removes exiting thread's identifier from bouding set which changes $B=\{tid_{r1},tid_{r2}\}$, to $B\setminus \{tid_{r1},tid_{r2}\}$.
 \begin{figure}[H]
 \centering
 \begin{tikzpicture}[>=stealth',node distance=1.5cm,semithick,auto]
 \tikzstyle{hollow node}=[circle,draw,inner sep=1]
 \tikzstyle{sub node}=[triangle,draw,inner sep=1]
 \tikzstyle{solid node}=[rectangle,draw,inner sep=1.5]

 \tikzset{
 	red node/.style={rectangle,draw=black,fill=red,inner sep=1.5},
 	blue node/.style={rectangle,draw=black,inner sep=1.5},
 	reader node/.style={circle,draw=black,inner sep=1},
 	writer node/.style={circle,draw=green,inner sep=1}
 }

       \node[solid node] (R) {$R$};
       \node[hollow node] (5) [right of=R] {$5$};
       \node[hollow node] (8) [right of=5] {$8$};
       \node[hollow node] (2) [right of=8] {$2$};
       \node[hollow node] (1) [right of=2] {$1$};
       \node[hollow node] (11) [right of=1] {$11$};
       %\node[hollow node] (4) [right of=11] {$4$};

     \path[->]  (R) edge node {} (5);
     \path[->]  (5) edge node {} (8);
     \path[->]  (8) edge node {} (2);
     %\path[->]  (11) edge node {} (4);
     \path[->] (2) edge [bend right] node {} (11);
     \path[dotted,->]  (1) edge node {} (11);


 ;
 \end{tikzpicture}
 \qquad
 \qquad
 \tikzset{
     font=\sffamily,
     BLOCK/.style={
         draw,
         align=center,
         text height=0.4cm,
         draw=red!50,
         fill=red!20,
         rectangle split,
         rectangle split horizontal,
         rectangle split parts=#1,
     }
 }
 \qquad
 \qquad
 \begin{tikzpicture}
     \node (h1) {to-free list};
     \node[BLOCK=3, below=0 of h1]{
       \nodepart{one}...\nodepart{two} F[s(1,\textsf{tid}) $\rightharpoonup$ $\emptyset$ )]
         \nodepart{three}...};
 \end{tikzpicture}
 \caption{Bounding threads, $\textsf{tid}_{r1}$ and $\textsf{tid}_{r2}$ exit \textsf{ReadBlock}. }
 \label{fig:prereclaim}
 \end{figure}
Once \emph{grace-period} finishes as shown in the figure \ref{fig:prereclaim}, the mutated node can be reclaimed. \lstinline{Free}(1) reclaims the memory via unmapping the mutated heap location, $F \setminus S(1)$. Write thread exists write block with executing \lstinline{WriteEnd} which basically sets the lock, $l$, in program state from $l=tid_{mut}$ to $l=\textsf{unlocked}$.
\begin{figure}\scriptsize
\[
\begin{array}{c}
  \desugarwrite \\
  \desugarread \\
  \desugarsync
 \end{array}
\]
\caption{Desugaring \textsf{RCUWrite}, \textsf{RCURead} and \textsf{Synchronize\_rcu}}
\label{fig:desugaringrcureadwrite}
\end{figure}
\end{comment}
\subsection{Relationship to Real Implementations}
Real implementations of RCU are far more sophisticated than our formal semantics above. Our simple global lock semantics for write critical sections has so many drawbacks in terms limiting the scalability and performance. The motivation of \textsf{RCU} is having very cheap reader critical sections but the number of reader theards can be a lot and this can be a problem. Although readers' performance are not effected badly, writer thread must show the grace period to all of these \emph{active/pre-existsting} readers in such a way that it must \emph{defer} the reclamation phase blocking (or in some implementations registering callback to be invoked after grace period) until all active readers are done with their jobs. Acquiring a global lock during each grace period severly affects scalibility and performance. To overcome this problem, a \emph{tree based} hieararchical mechanism is implemented to handle each thread's (CPU's) \emph{quiescent-state} information and \emph{grace-period}. In Tree RCU, the data strcuture is used in such a way that it records each CPU's quiescent states. The \textsf{rcu} node tree propagates these states up to the root, and then propagates grace-period information down to the leaves. Quiescent-state information does not propagate upwards from a given node until a quiescent state has been reported by each CPU covered by the subtree rooted at that node. This propagation scheme dramatically reduces the lock contention experienced by the upper levels of the tree ~\cite{LiangMKM16}
  
In addition, efficient implementations go to great lengths to minimize the cost of the read-side critical section operations while tracking the same information.  Direct implementation of our semantics would yield unacceptable performance, since both \lstinline|ReadBegin| and \lstinline|ReadEnd| modify shared data structures.  Typically, implementations are structured so each reader thread (or CPU) maintains its own \emph{fragment} of the global state, which is only updated by that thread, but is read by the write-side primitives.
In the ideal case, the boundaries of the read-side critical section coincide with some other operation the reader must already do for other purposes, such as disabling interrupts~\tocite{}. As a result, some descriptions of RCU implementations do not explicitly discuss equivalents to \lstinline|ReadStart| and \lstinline|ReadEnd|, because the implementation piggybacks on existing state already present for non-RCU purposes.

Conceptually, each reader thread maintains a count of how many times it has passed through the RCU data structure as a reader (a count of how many read-side critical sections it has executed).  The writer waits for a grace period by effectively taking an atomic snapshot of all readers' counts, and waiting until all have been incremented.  

Real implementations, of course, must also tolerate the weak memory model of whatever processor they run on, leading them to use. For example, the primitive to dereference a memory location shown by a pointer and the primitive to update the memory location shown by a pointer contain architecture-specific memory barrier instructions and compiler directives to enforce correct ordering. Both primitives reduce to simple assignment statements on sequentially consistent systems. Dereferencing is volatile access except on DEC Alpha, which also requires a memory barrier \todo{CITE}.

The Linux implementation of the communication in between reader thread and writer thread is based on waiting for context switches. The implementation uses calls \lstinline|SyncStart| and returns back from \lstinline|SyncStop| after all CPUs have passed through at least one context switch. The synchronous version of the primitive to wait reader threads is \textsf{synchronize\_rcu}. For performance reasons, the Linux implementation has also asynchronous version of this primitive named \textsf{call\_rcu}. Detecting context switches requires maintaining state shared between CPUs. A CPU must update state, which other CPUs read, that indicate it executed a context switch ~\cite{Mckenney_rcuusage}.


==> chapters/RCUTypesBST.tex <==

\textsf{BST} is an important data structure which is used in many performance critical system (e.g. Operating Systems). \textsf{BST}s are used in implementation of dictionaries which is a set of key-value pairs with \textsf{Insert}, \textsf{Delete}, \textsf{Read} operations. \textsf{Insert}, \textsf{Delete} are \textsf{update} operations, \textsf{Read} is a \textsf{look up} operation. A BST Tree keeps key-value pairs as its internal nodes, with totally ordered keys.\textsf{BST} shown in Figure \ref{fig:rbtree} has $(k,v)$ as its internal node and all value $v$, \textsf{Value((key,value)) = v}, of a node has a unique key $k$, \textsf{Key((key,value)) = k},  which never changes. In BST Tree, all descendants in  the left sub-tree of $v$ have keys larger than the key of $v$. The successor of node $v$ is the node with the smallest key among nodes with keys larger than or equal to key of $v$ which is the purple node in Figure ~\ref{fig:rbtree}. 
\input{RBTReeStructure.tex}
\textsf{BST}s are mainly used in components where read-only transactions are intensive. RCU is a programming-pattern which scales up performance when read-only operations are intensive. Naturally, exploration of rb-tree implementation with RCU pattern resulted in many studies:
\begin{itemize}
\item \href{http://www.pdx.edu/sites/www.pdx.edu.computer-science/files/tr1006.pdf}{Relativistic Red-Black Tree}. First relativistic RBTree paper.
\item \href{http://www.cs.technion.ac.il/~mayaarl/full-version.pdf}{ArbelAttiyaConcurrent Updates} . Fine grain updates.
\end{itemize}
In this section, we present the implementation of \textsf{BST} with our RCU types and show proofs of memory safety. General correctness properties that we expect from a BST are:
\begin{itemize}
\item An in order traversal of a consistent tree will always give values of the tree sorted
\item Lookups will always find a node that exists in the tree
\end{itemize}
Thinking \textsf{BST} from RCU perspective does not make implementation more complicated than normally it is.  A concurrent setting with RCU technique is basically includes:
\begin{itemize} 
\item \textsf{\textbf{Readers}}. With RCU technique developing a reader section is almost as easy as developing a non-concurrent reader section.  The only restrictions placed on readers are that they do not hold any references to the data structure outside critical section.
\item \textsf{\textbf{Mutators}}. Lock-free proceeding of \textsf{Readers} can be provided with keeping BST tree consistent by \textsf{Mutators}. 
\item Mutator must not allow a reader to see partial changes to a node. Mutator use copy-on-update to make all changes to a private copy of the node, then atomically switch the new node with the old one.
\item The termination position of a search is defined to be the last node whose value is examined by the search before it is terminated. If a search for a value $v$ is terminated at node $n$ at  time $t$ then it search for value $v$ will always terminate at node $n$ for all searches when we isolate tree from updates
\item Readers must not get lost when the structure of the tree is changed. In Figure ~\ref{fig:succmoveanom}, suppose that there exists a reader looking for node with key \textsf{k'} concurrently with a mutator thread which moves successor of \textsf{k}, \textsf{k'},to the previous position of \textsf{k}. Result of the \textsf{Delete} operation performed on \textsf{k} cause the reader gets lost and returns false for \textsf{Read} operation on \textsf{k'} even though it exists in the tree.
\item  Temporarily having the same item in the tree multiple times do not affect the lookups. A unique value is returned if first copy encountered and another unique value can be returned if second copy is encountered.
\item Only nodes which are  no longer reachable  by an existing search or  future search will be garbage collected and all such nodes will be garbage collected, Figures ~\ref{fig:del1}, ~\ref{fig:del2}
\end{itemize}
\subsubsection{Binary-Search-Tree Implementation}
\textsf{BST} implementation has three functions:
\begin{itemize}
\item \textsf{Insert}$(key,value)$ adds $(key,value)$ pair to the tree as a leaf; returns $true$ if $key$ is not in the set and $false$ otherwise
\item \textsf{Delete}$(key)$ removes $(key,value)$ pair  from tree; returns $true$ if $key$ is in the tree and $false$ otherwise
\item \textsf{Read}$(key)$ returns $val$ if $(key,value)$ is in the set; otherwise it returns $false$
\end{itemize}
\paragraph{Read:}  
\input{RBTReeSuccMoveAnom.tex}
\paragraph{Insert:}
\input{RBTReeInsertAnom.tex}
\paragraph{Delete:} 
\input{RBTReeDeleteOneChildAnom.tex}
\input{RBTReeDeleteTwoChildAnom.tex}
\begin{figure*}\tiny
\[
\proofoutstep{\rcuitr{prev}{sui}{k}{k+1}{\_},itr:\_}{ %read next
   \proofoutstep{\rcuitr{itr}{sui}{k}{k+1}{\_}\;,prev:\_}{ %read stack  
   \proofoutstep{\rcuitr{prev}{sui}{k}{k+1}{\_}\;,itr:\_}{
    \proofoutstep{\rcuitr{sui}{root}{k}{k+1}{\_}\;,prev:\_}{
      \proofoutstep{root:\uiglobal,sui:\udef}{
        sui\texttt{=}root\texttt{;}\\
	}{\textsc{T-UniqueGlobalRead}}
        {\rcuitr{sui}{root}{k}{k+1}{\_}}\\
        prev\texttt{=}sui\texttt{.child[1];}\\
        }{\textsc{T-UniqueStackRead}}
        {\rcuitr{sui}{root}{k}{k+1}{prev}\;,\rcuitr{prev}{sui}{k+1}{k+2}{\_}}\\
        itr\texttt{=}prev\texttt{.child[1]}\\
        }{\textsc{T-ReadNext}}
        {\rcuitr{prev}{sui}{k}{k+1}{itr}\;,\rcuitr{itr}{sui}{k+1}{k+2}{\_}}\\
        \;\;\;\;direction\texttt{=}1\texttt{;}\\
        \;\;\;\;itrKey\texttt{=}itr.key\texttt{;}\\
        //\texttt{\textcolor{red}{loop for finding the node to read starts}}\\
        \;\;\;\;prev\texttt{=}itr\texttt{;}\\
        }{\textsc{T-ReadStack}}
        {\rcuitr{itr}{sui}{k}{k+1}{\_}, \rcuitr{prev}{sui}{k}{k+1}{\_}} \\
        \;\;\;\;direction\texttt{ = (itrKey > key ? 0 : 1) }\texttt{;}\\
        \;\;\;\;itr\texttt{=}prev\texttt{.child[}direction\texttt{]}\texttt{;}\\ %read next
        \;\;\;\;itrKey\texttt{=}itr\texttt{.key}\texttt{;}\\ %read next
        //\texttt{\textcolor{red}{loop for finding the node to read ends}}\\
        }{\textsc{T-ReadNext}}
        {\rcuitr{itr}{sui}{k+1}{k+2}{\_},\rcuitr{prev}{sui}{k}{k+1}{itr}}
\]
\caption{Typing derivation for traversing Binary Search Tree.}
\label{fig:traverse-bst}
\end{figure*}

\begin{figure*}\tiny
\[
\proofoutstep{\rcuitr{itr}{sui}{k}{k+1}{\_},succ:\_}{ %read next
 \proofoutstep{\rcuitr{itr}{sui}{k}{k+1}{\_}\;,prevSucc:\_}{ 
\proofoutstep{itr:\unlinked}{
\proofoutstep{\rcuitr{prev}{sui}{k}{k+1}{itr}\;,\rcuitr{itr}{sui}{k+1}{k+2}{itrNext}}{
\proofoutstep{\rcuitr{prev}{sui}{k}{k+1}{\_}\;,itr:\_}{
\proofoutstep{\rcuitr{itr}{sui}{k}{k+1}{\_}\;,prev:\_}{
\proofoutstep{\rcuitr{prev}{sui}{k}{k+1}{\_}\;,itr:\_}{
    \proofoutstep{\rcuitr{sui}{root}{k}{k+1}{\_}\;,prev:\_}{
      \proofoutstep{root:\uiglobal,sui:\udef}{
        sui\texttt{=}root\texttt{;}\\
	}{\textsc{T-UniqueGlobalRead}}
        {\rcuitr{sui}{root}{k}{k+1}{\_}}\\
        prev\texttt{=}sui\texttt{.child[1];}\\
        }{\textsc{T-UniqueStackRead}}
        {\rcuitr{sui}{root}{k}{k+1}{prev}\;,\rcuitr{prev}{sui}{k+1}{k+2}{\_}}\\
        itr\texttt{=}prev\texttt{;}\\
        }{\textsc{T-ReadStack}}
        {\rcuitr{prev}{sui}{k}{k+1}{\_}\;,\rcuitr{itr}{sui}{k}{k+1}{\_}}\\
        itrKey\texttt{=} itr\texttt{.key};\\
        //\texttt{\textcolor{red}{loop for finding the node to delete starts}}\\
        prev\texttt{=}itr\texttt{;}\\
        }{\textsc{T-ReadStack}}
        {\rcuitr{prev}{sui}{k}{k+1}{\_}\;,\rcuitr{itr}{sui}{k}{k+1}{\_}}\\
         \;\;\;\;direction\texttt{ = (itrKey > key ? 0 : 1) }\texttt{;}\\
         itr\texttt{=}prev\texttt{.child[1]}\\
         }{\textsc{T-ReadNext}}
        {\rcuitr{prev}{sui}{k}{k+1}{itr}\;,\rcuitr{itr}{sui}{k+1}{k+2}{\_}}\\
        \;\;\;\;itrKey\texttt{=}itr\texttt{.key}\texttt{;}\\ %read next
        //\texttt{\textcolor{red}{loop for finding the node to delete ends}}\\
        \texttt{if(}itr\texttt{ == NULL)return false;} //\texttt{Not found}\\
        \texttt{if(}itr\texttt{.child[0] == NULL) \{ } \\ 
         \;\;\;\;itrNext\texttt{=} itr\texttt{.child[1];} \\
         \;\;\;\;prev\texttt{.child[direction]}\texttt{=}itr\texttt{.child[1];}\\
         }{\textsc{T-UnlinkANode}}
        {\rcuitr{prev}{sui}{k}{k+1}{itrNext}\;,itr:\unlinked}\\
        \texttt{asyncDelayedFree(}itr\texttt{); return true; \} }
        //\texttt{ Unlinking  a single child, child[0], ends. Same for child[1]}\\
        }{\textsc{T-AsyncFree}}
        {\rcuitr{prev}{sui}{k}{k+1}{itrNext}\;,itr:\udef}\\
         \;\;\;\;prevSucc\texttt{=} itr\texttt{;} \\
        }{\textsc{T-ReadStack}}
        {\rcuitr{itr}{sui}{k}{k+1}{\_}, \rcuitr{prevSucc}{sui}{k}{k+1}{\_}}\\
         \;\;\;\;succ\texttt{=} itr\texttt{.child[0];} \\
            }{\textsc{T-ReadNext}}
        {\rcuitr{succ}{sui}{k+1}{k+2}{itr}\;,\rcuitr{itr}{sui}{k}{k+1}{\_}}
        \]
\caption{Typing derivation for deleting a node in  Binary Search Tree. Phase-1: Deleting node with one child}
\label{fig:delete-bst-phase1}
\end{figure*}

\begin{figure*}\tiny
\[
\proofoutstep{}{
\proofoutstep{}{
\proofoutstep{}{
\proofoutstep{}{
\proofoutstep{itr:\unlinked}{
\proofoutstep{\rcuitr{prev}{sui}{k}{k+1}{z},\rcuf{newNode}{f}}{
 \proofoutstep{newNode:\rcuf}{
 \proofoutstep{newNode:\_}{ 
 \proofoutstep{\rcuitr{follower}{sui}{k}{k+1}{\_}}{ 
 \proofoutstep{\rcuitr{follower}{sui}{k}{k+1}{\_}\;,succ:\_}{ 
 \proofoutstep{\rcuitr{succ}{sui}{k}{k+1}{\_}\;,prevSucc:\_}{ 
\proofoutstep{\rcuitr{succ}{sui}{k}{k+1}{\_},follower:\_}{ %read next
         \;\;\;\;follower\texttt{=} succ\texttt{.child[1];} \\
         }{\textsc{T-ReadNext}}
        {\rcuitr{succ}{sui}{k+1}{k+2}{itr}\;,\rcuitr{follower}{sui}{k}{k+1}{\_}}\\
        //\texttt{\textcolor{red}{loop for finding the succ node starts}}\\
         \;\;\;\;prevSucc\texttt{=} succ\texttt{;} \\
         }{\textsc{T-ReadStack}}
         {\rcuitr{succ}{sui}{k}{k+1}{\_}, \rcuitr{prevSucc}{sui}{k}{k+1}{\_}}\\
         \;\;\;\;succ\texttt{=} follower\texttt{;} \\
          }{\textsc{T-ReadStack}}
         {\rcuitr{succ}{sui}{k}{k+1}{\_}, \rcuitr{follower}{sui}{k}{k+1}{\_}}\\
         \;\;\;\;follower\texttt{=} follower\texttt{.child[1];} \\
           //\texttt{\textcolor{red}{loop for finding the succ node ends}}\\
          }{\textsc{T-OverWriteCurrent}}
         {\rcuitr{follower}{sui}{k+1}{k+2}{\_}}\\
         \;\;\;\;newNode\texttt{=}\textsf{new}\texttt{;}\\
          }{\textsc{T-Allocate}}
         {newNode:\rcuf}\\
         //\texttt{Trivial read of next fields}\\
         \;\;\;\;x\texttt{=} itr\texttt{.child[0];} \\
         \;\;\;\;y\texttt{=} itr\texttt{.child[1];} \\
         \;\;\;\;newNode\texttt{.child[0]}\texttt{=} x\texttt{;} \\
         \;\;\;\;newNode\texttt{.child[1]}\texttt{=} y\texttt{;} \\
         }{\textsc{T-SetFresField}}
         {\rcunf{newNode}{f}{x}, \rcunf{newNode}{f}{y}}\\
         \;\;\;\;prev.\texttt{.child[direction]}\texttt{=} newNode\texttt{;}\\
         }{\textsc{T-LinkFresh}}
         {z:\unlinked,\rcuitr{prev}{sui}{k}{k+1}{newNode}, \rcuitr{newNode}{sui}{k+1}{k+2}{\_}}\\
         \texttt{asyncDelayedFree(}itr\texttt{);}\\           
         }{\textsc{T-AsyncFree}}
         {itr:\udef}\\         
         \texttt{if(}prev\texttt{==}itr\texttt{) \{ }\\
         //\texttt{ Take this part again. [Proof up to this point.]}\\
         \;\;\;\;newNode.\texttt{.child[0]}\texttt{=}succ\texttt{.child[0];}\\
         }{\textsc{T-UnlinkANode}}
         {}\\
          \texttt{asyncDelayedFree(}succ\texttt{); \} // remove old succ case 1}\\
         }{\textsc{T-AsyncFree}}
         {succ:\udef}\\
         \texttt{else \{ }\\
         \;\;\;\;prevSucc.\texttt{.child[1]}\texttt{=}succ\texttt{.child[1];}\\
         }{\textsc{T-UnlinkANode}}
         {}\\
          \texttt{asyncDelayedFree(}succ\texttt{); //remove old succ case 2}\\
         }{\textsc{T-AsyncFree}}
         {succ:\udef}
\]
\caption{Typing derivation for deleting a node in  Binary Search Tree. Phase-2: Deleting node with two children}
\label{fig:delete-bst-phase2}
\end{figure*}
%%Temporarily commented out
%\input{staticCheckBST.tex}



==> chapters/RCUTypesBSTProof.tex <==
\begin{comment}
%\begin{table}[H]
	%\begin{tabular}{l}
		%Read\\

\begin{lstlisting}[mathescape,caption={RCU-BST \textsf{Read} function with assertions added.}\label{lst:rcubstreadassertions},language=C]
struct node_p{
  int key;
  struct node_p* child[2];
  int data;
}

node_p<rcu> root;
	
int Read(int key){
 int result;	
 <@\textcolor{orange}{ReadBegin}@>
  node_p<<@\textcolor{orange}{rcuIterator}@>> itr; 
  itr=root;
  int itrKey = itr->key; 
  while(itr != NULL && itrKey != key ){
    if(itrKey > key)
    	$\textrm{assert}$
    	$[$ 
	 $\Gamma\,,itr:\textsf{rcuIterator}$ $\vdash_{R} \hilight{itr := itr\textendash\textgreater child[0]}  \dashv$ $itr:\textsf{rcuIterator}\,,\Gamma$                                
    		    $\textrm{provided} \, \textsf{ftype}(child) = \textsf{rcu}$
	$]$
    if(itrKey < key)
   	$\textrm{assert}$
  	$[$
   	$\Gamma\,,itr:\textsf{rcuIterator}$ $\vdash_{R} \hilight{itr := itr\textendash\textgreater child[1]}  \dashv$ $itr:\textsf{rcuIterator}\,,\Gamma$                                
   	              $\textrm{provided} \, \textsf{ftype}(child) = \textsf{rcu}$
   	$]$      
      if(itr != NULL) 
      itrKey = itr->key;
    }
    result = itr->data;
  <@\textcolor{orange}{ReadEnd}@>
  return result;
}
\end{lstlisting}
%	\end{tabular} \hfill	
%\caption{RCU-BST \textsf{Read} function with assertions added.}
%\label{tab:rcubstreadassertions}
%\end{table}

%\begin{table}[hbt]
	%\begin{tabular}{ c }
		%Update\\
\begin{lstlisting}[mathescape,caption={RCU-BST \textsf{Insert} function with assertions added.}\label{lst:rcubstinsertassertions},language=C]
void Insert(int k, int val){
 <@\textcolor{orange}{WriteBegin}@>
   node_p<<@\textcolor{orange}{rcuIterator}@>> itr;
   node_p<<@\textcolor{orange}{rcuIterator}@>> prev;
   prev = root;
    $\textrm{assert}$
     $[$
     $\Gamma\,,itr:\_\,,prev:\textsf{rcuIterator}$ $\vdash_{M} \hilight{itr := prev\textendash\textgreater child[0]} \dashv$ $prev:\textsf{rcuNext}\,child\,itr\,, itr:\textsf{rcuIterator}\,, \Gamma$ 
     $]$
   itrKey = itr->key;
   direction = 0;
   int itrKey = itr->key;
   while (itr != NULL &&  itrKey != key) {
    prev = itr;
    if (itrKey > key){
    $\textrm{assert}$
     $[$ $\Gamma\,, itr:\_ ,prev:\textsf{rcuIterator}$ $ \vdash_{M} \hilight{prev = itr;itr := prev\textendash\textgreater child[0]} \dashv$ $prev:\textsf{rcuNext}\,child\,itr\,, itr:\textsf{rcuIterator}\,, \Gamma$ 
     $]$
     direction = 0;
    }
    if (itrKey < key){
   $\textrm{assert}$
    $[$ $\Gamma\,, itr:\_ \,prev:\textsf{rcuIterator}$ $\vdash_{M} \hilight{prev = itr;itr := prev\textendash\textgreater child[1]} \dashv$ $prev:\textsf{rcuNext}\,child\,itr \,, itr:\textsf{rcuIterator}\,, \Gamma$ $]$    
    direction = 1;
    }
    if (itr!=NULL) 
     itrKey = itr->key ;
  }
    if(itr != NULL)
     return false;
   // Add fresh node as leaf  
  node_p<<@\textcolor{orange}{rcuFresh}@>> newNode;
  $\textrm{assert}$ $[$ $\Gamma\,, newNode:\_ \vdash_{M} \hilight{newNode := new} \dashv newNode:\textsf{fresh}, \Gamma$ $]$   
  $\textrm{assert}$ $[$ $\Gamma\,,newNode:\textsf{fresh}\, key \_ \vdash_{M} \hilight{newNode.key := k } \dashv newNode:\textsf{fresh}\,key\,k$ $]$
  $\textrm{assert}$ $[$ $\Gamma\,, newNode: \textsf{fresh}\, data\_ \vdash_{M} \hilight{newNode.data := val} \dashv newNode:\textsf{fresh}\,data\,val$ $]$
  $\textrm{assert}$ $[$ $\Gamma\,, newNode:\textsf{fresh}\, child \_ \vdash_{M} \hilight{newNode.child[0] := NULL} \dashv newNode:\textsf{fresh}\,child\,NULL$ $]$
  $\textrm{assert}$ $[$  $\Gamma\,, newNode:\textsf{fresh}\, child \_ \vdash_{M} \hilight{newNode.child[1] := NULL} \dashv newNode:\textsf{fresh}\,child\,NULL$ $]$  

  $\textrm{assert}$
   $[$ 
   $\Gamma\,,prev:\textsf{rcuNext}\,child\,NULL\,,newNode:fresh\,child\,NULL$
   $\vdash_{M}  \hilight{ prev.child[direction] := newNode} \dashv$
   $prev:\textsf{rcuNext}\,child\,newNode \,, newNode:\textsf{rcuNext}\,child\,NULL \, , \Gamma$
   $]$
  node_p<<@\textcolor{orange}{WriteEnd}@>>
  return true;
}
\end{lstlisting}
%	\end{tabular} \hfill	
%\caption{RCU-BST \textsf{Insert} function with assertions added.}
%\label{tab:rcubstinsertassertions}
%\end{table}
%\usepackage{longtable}
%\begin{table}[]
%	\begin{tabular}{ c } 
\begin{lstlisting}[linewidth=\linewidth,mathescape,caption={RCU-BST \textsf{Delete} function with assertions added.}\label{lst:rcubstdelassertions},language=C] 
void Delete(int key){  
 node_p<<@\textcolor{orange}{WriteBegin}@>>
   node_p<<@\textcolor{orange}{rcuIterator}@>> prev = root;
   node_p<<@\textcolor{orange}{rcuIterator}@>> itr;
   $\textrm{assert}$
    $[$ $\Gamma\,,itr:\_ \,,prev:\textsf{rcuIterator}$ $\vdash_{M} \hilight{itr := prev\textendash\textgreater child[0]} \dashv$ $prev:\textsf{rcuNext}\,child\,prev\,, itr:\textsf{rcuIterator}\,,\Gamma$ $]$
   itrKey = itr->key;
   direction = 0;
   int itrKey = itr->key;  
   while (itr != NULL && itrKey != key){
    prev = itr;
    if (itrKey > key){
    $\textrm{assert}$
      $[$ $\Gamma\,, itr:\_ \,,prev:\textsf{rcuIterator}$ $ \vdash_{M} \hilight{itr := prev\textendash\textgreater child[0]} \dashv$ $prev:\textsf{rcuNext}\,child\,itr\,, itr:\textsf{rcuIterator}\,, \Gamma$ $]$
      direction = 0;
    }
    if (itrKey < key){ 
    $\textrm{assert}$
     $[$ $\Gamma\,, itr:\_ \,,prev:\textsf{rcuIterator}$ $\vdash_{M} \hilight{itr := prev\textendash\textgreater\textendash\textgreater child[1]} \dashv$ $prev:\textsf{rcuNext}\,child\,itr, itr:\textsf{rcuIterator}\,,\Gamma$ $]$
      direction = 1;
    }
    if (itr!=NULL) 
     itrKey = itr->key ;
   }
   if(itr == NULL)//Not found
    return false;
   // One child
   if(itr->child[0] == NULL){
    $\textrm{assert}$
     $[$ $\Gamma\,,prev:\textsf{rcuNext}\,child\,itr\,,itr:\textsf{rcuNext}\,child\,itr.child$ $\vdash_{M} \hilight{prev.child[direction] := itr.child[1]} \dashv$ $itr:\textsf{unlinked}\,,prev:\textsf{rcuNext}\,child\,itr.child\,,\Gamma$ $]$ 
     }//rcu mutate ends
   $\textrm{assert}$
   $[$ $\Gamma\,,itr:\textsf{unlinked} \vdash_{M} \hilight{asyncFree(itr)}\dashv itr:\textsf{undef}\,,\Gamma$ $]$
     node_p<<@\textcolor{orange}{WriteEnd}@>>
     return true;
   }
   if(itr->child[1] == NULL){
    $\textrm{assert}$
     $[$ $\Gamma\,,prev:\textsf{rcuNext}\,child\,itr\,,itr:\textsf{rcuNext}\,child\,itr.child$ $\vdash_{M} \hilight{prev.child[direction] := itr.child[0]} \dashv$ $itr:\textsf{unlinked}\,,prev:\textsf{rcuNext}\,child\,itr.child\,,\Gamma$ $]$    
     }//rcu mutate ends
   $\textrm{assert}$
    $[$ $\Gamma\,, itr:\textsf{unlinked} \vdash_{M} \hilight{asyncFree(itr)} \dashv itr:\textsf{undef} \,,\Gamma$ $]$
    node_p<<@\textcolor{orange}{WriteEnd}@>>
    return true;
}
   //Two children
   node_p<<@\textcolor{orange}{rcuIterator}@>> prevSucc = itr;  
   node_p<<@\textcolor{orange}{rcuIterator}@>> succ = itr->child[0];
   node_p<<@\textcolor{orange}{rcuIterator}@>> next = succ->child[1]; 
   // Think this loop more
   while ( next!= NULL){
    prevSucc = succ;
    succ = next;
    next = next->child[1];
   }
   node_p<<@\textcolor{orange}{rcuFresh}@>> newNode;
   $\textrm{assert}$
   $[$ $\Gamma\,,newNode:\_\vdash_{M}\hilight{newNode := new}\dashv newNode:\textsf{fresh}\,,\Gamma$ $]$
   
   $\textrm{assert}$
    $[$ $\Gamma\,,newNode:\textsf{fresh}\,key\,\_\vdash_{M}\hilight{newNode.key := succ\textendash\textgreater key}\dashv newNode:\textsf{fresh}\,key\,succ.key\,,\Gamma$ $]$

   $\textrm{assert}$
    $[$ $\Gamma\,,newNode:\textsf{fresh}\,child\,\_\vdash_{M}\hilight{newNode.child[0] := itr\textendash\textgreater child[0]}\dashv newNode:\textsf{fresh}\,child\,itr.child[0]\,,\Gamma$ $]$

   $\textrm{assert}$
    $[$ $\Gamma\,,newNode:\textsf{fresh}\,child\,\_ vdash_{M}\hilight{newNode.child[1] := itr\textendash\textgreater child[1]}\dashv newNode:\textsf{fresh}\,child\,itr.child[1]\,,\Gamma$ $]$

   $\textrm{assert}$
    $[$ $\Gamma\,,prev:\textsf{rcuNext}\,child\,itr\,,itr:\textsf{rcuNext}\,child\,itr.child$ $\vdash_{M} \hilight{prev\textendash\textgreater child[direction]=newNode} \dashv$ $itr:\textsf{unlinked}\,,prev:\textsf{rcuNext}\,child\,itr.child\,,\Gamma$ $]$

   if(prevSucc == itr)
    $\textrm{assert}$
     $[$ $\Gamma\,,newNode:\textsf{rcuNext}\,child\,succ\,,succ:\textsf{rcuNext}\,child\,succ.child$ 
     $\vdash_{M} \hilight{newNode.child[0] := succ\textendash\textgreater child[0]} \dashv$ 
     $succ:\textsf{unlinked}\,, newNode:\textsf{rcuNext}\,child\,succ.child\,,\Gamma$ 
     $]$     
   else 
    $\textrm{assert}$
     $[$ $\Gamma\,,prevSucc:\textsf{rcuNext}\,child\,succ\,,succ:\textsf{rcuNext}\,child\,succ.child$ 
     $\vdash_{M} \hilight{prevSucc.child[1] := succ\textendash\textgreater child[0]} \dashv$ 
     $succ:\textsf{unlinked}\,,newNode:\textsf{rcuNext}\,child\,succ.child\,,\Gamma$ 
     $]$
  node_p<<@\textcolor{orange}{WriteEnd}@>> //Mutator Block Ends 
  asyncFree(itr,succ);   
  return true;
}
\end{lstlisting}
\todo{Redo the proof  with taking some informal notes}
%	\end{tabular} \hfill	
%\caption{RCU-BST \textsf{Delete} function with assertions added.}
%\label{tab:rcubstdelassertions}
%\end{longtable}
\end{comment}


==> chapters/RCUTypesEvaluation.tex <==
\section{Type Checking on RCU Data Structures}
We run the type-rules of our system on a RCU linked list and RCU Binary Search Tree (BST) in which types of variables are annotated with our type qualifiers. Type checker basically checks whether state of types before and after each command execution is admissible with respect to semantics of correct RCU usage we define in \ref{fig:operationalsematoms}, \ref{fig:operationalsemmemrecl}, \ref{fig:operationalsemrcuenterexit}.

We structure our type checking around judgements in $p\{C\}q$ structure where $p$ and $q$ are predicates over state of type of RCU variables and $C$ is command.
\label{sec:lleval}
\subsection{Type Checking RCU Linked List}
\input{staticCheckLL.tex}
%\subsection{Binary Search Tree with RCU Types}
\input{BST.tex}


==> chapters/RCUTypesLLProof.tex <==
\begin{figure*}\tiny
  \[
  \proofoutstep{\rcuitr{itr}{sui}{k}{k+1}{\_}}{
    \proofoutstep{\rcuitr{sui}{head}{k}{k+1}{\_}\;,itr:\_}{
      \proofoutstep{head:\uiglobal,sui:\udef}{
        sui\texttt{=}head\texttt{;}\\
	}{\textsc{T-UniqueGlobalRead}}
                   {\rcuitr{sui}{head}{k}{k+1}{\_}}\\
        itr\texttt{=}sui\texttt{.next;}\\
    }{\textsc{T-UniqueStackRead}}
                 {\rcuitr{sui}{head}{k}{k+1}{itr}\;,\rcuitr{itr}{sui}{k+1}{k+2}{\_}}\\
         //\texttt{\textcolor{red}{loop for finding the node to read starts}}\\
        \;\;\;\;itr\texttt{=}itr\texttt{.next}\texttt{;}\\
        //\texttt{\textcolor{red}{loop for finding the node to read ends}}\\
  }{\textsc{T-OverWriteCurrent}}
   {\rcuitr{itr}{sui}{k+1}{k+2}{\_}}
\]
\caption{Typing derivation for traversing list.}
\label{fig:traverse-ll}
\end{figure*}
\begin{figure*}\small
     \[
     \proofoutstep{\rcuitr{itr}{sui}{k+1}{k+2}{r}\;\rcuitr{prev}{sui}{k}{k+1}{itr}}{
      \proofoutstep{\rcuitr{itr}{sui}{k}{k+1}{\_}}{
        \proofoutstep{\rcuitr{itr}{sui}{k}{k+1}{\_}\;,prev:\_}{
          \proofoutstep{\rcuitr{itr}{sui}{k}{k+1}{\_}\;,prev:\_}{
           \texttt{...}\\
           prev\texttt{=}itr\texttt{;}\\
           }{\textsc{T-ReadStack}}
           {\rcuitr{itr}{sui}{k}{k+1}{\_}\;,\rcuitr{prev}{sui}{k}{k+1}{\_}}\\
            //\texttt{\textcolor{red}{loop for finding the node to delete starts}}\\
            prev\texttt{=}itr\texttt{;}\\
            }{\textsc{T-ReadStack}}
            {\rcuitr{itr}{sui}{k}{k+1}{\_}\;,\rcuitr{prev}{sui}{k}{k+1}{\_}}\\
            \;\;\;\;\;\;\;\;itr\texttt{=}itr\texttt{.next}\texttt{;}\\
            }{\textsc{T-OverWriteCurrent}}
            {\rcuitr{itr}{sui}{k+1}{k+2}{\_}}\\
            \;\;\;\;\;\;\;  //\texttt{\textcolor{red}{loop for finding the node to delete ends}}\\
            \;\;\;\;\;\;\;r\texttt{=}itr\texttt{.next}\texttt{;}\\
            \;\;\;\;\;\;\;prev\texttt{.next}\texttt{=}r\texttt{;}\\
     }{\textsc{T-UnlinkANode}}
                  {\rcuitr{prev}{sui}{k}{k+1}{r}\;,itr:\unlinked}
                  \]   
\caption{Typing derivation for updating list- Phase-1: Traversing and unlinking the node.}
\label{fig:update-ll-unlink}
\end{figure*}

\begin{figure*}\small
  \[
  \proofoutstep{itr:\unlinked}{
    \texttt{asyncDelayedFree}(itr)\texttt{;}\\
  }{\textsc{T-AsyncFree}}
               {itr:\udef}
               \]
\caption{Typing derivation for updating list-Phase-2: Reclaiming the memory location where the $\unlinked$ node resides.}
\label{fig:update-ll}
\end{figure*}
\begin{comment}
  In \ref{lst:typcheckread}, there exists only one command which touches to a RCU variable, \textsf{itr}, which has RCU qualified type, \textsf{rcuIterator}. Informally, while iterating  over linked list with one iterator, we set it to show next heap location and invalidate the pointer showing the next previous location on heap. To achieve this as type safe, type of \textsf{itr} needs to be preserved as \textsf{rcuIterator} which is checked against \texttt{Overwrite-Curr} typing rule in figure \ref{fig:typingrulesRCURead}.
  
In listing ~\ref{lst:typcheckwrite}, we use two iterators to delete a node. We want these two iterators, \textsf{itr} and \textsf{prev} , to be showing the consecutive heap locations. This property is checked with first assertion in the loop against  \texttt{Write-Traverse} typing rule in figure ~\ref{fig:typingrulesRCUWrite}. Once the node, representing a heap location in linked list, to be deleted is found then it is unlinked. We check the change in state of types due to unlinking a node againsts \texttt{Unlink-Node} typing rule. Once all reader threads are done with the unlinked node, RCU runtime call asynchronous memory reclamation call, \textsf{asyncFree}, and adds the node to the free list. To add a node to a free list, it must be in \textsf{unlinked} type. After the node gets added to free list, its type becomes \textsf{undef}. The last assertion which checks this type property against \texttt{Free-Unlinked-Node} typing rule.
\end{comment}
Some explanations for lltype checking ...
\newpage


==> chapters/RCUTypesRelatedWork.tex <==
\section{Concluding Remarks \& Related Work}
\label{sec:relatedwork}
Related work for correctness of code involving RCU memory management includes relevant work in concurrent program logics, model checking, and type systems.

\mypar{Modeling RCU}
Alglave et al.~\cite{Alglave:2018:FSC:3173162.3177156} propose a memory model to be assumed by the platform-independent parts of the Linux kernel, regardless of the underlying hardware's memory model.
As part of this, they give the first formalization of what it means for an RCU implementation to be correct (previously this was difficult to state, as the guarantees in principle could vary by underlying CPU architecture). Essentially, that reader critical sections do not span grace periods.  They prove by hand that the Linux kernel RCU implementation~\cite{DBLP:conf/cav/AlglaveKT13,abssem} satisfies this property. 
According to their definition, our model in Section \ref{sec:semantics} is a valid RCU implementation (assuming sequential consistency).
To the best of our knowledge, ours is the first abstract \emph{operational} model for a Linux kernel-style RCU implementation --- others are implementation-specific~\cite{Mandrykin:2016:TDV:3001219.3001297} or axiomatic like Alglave et al.'s. Tassarotti et al. models a well-known way of implementing RCU synchronization without hurting readers' performance, \textsf{Quiescent State Based Reclamation}(QSBR)~\cite{urcu_ieee} where synchronization in between the writer thread and reader threads provided via per-thread counters. 

\mypar{Program Logics} Fu et al.~\cite{shao_temp} extend Rely-Guarantee/Separation-Logic ~\cite{vafeiadis07,Feng:2007:RCS:1762174.1762193,Feng:2009:LRR:1480881.1480922} with the \textit{past-tense} temporal operator to eliminate the need for using the history variable and lift the standard separation conjuction to assert over on execution histories instead of state to capture the high level intuitive specification of Michael's non-blocking stack~\cite{Michael:2004:HPS:987524.987595}. Gotsman et al.~\cite{Gotsman:2013:VCM:2450268.2450289} take a similar approach and present a formalization of memory management using grace periods in an extension to separation logic, specifically an extension of Vafeiadis and Parkinson's \textsf{RGSep}~\cite{vafeiadis07}. Gotsman et al. take assertions from temporal logic to capture the essence of relaxed memory reclamation algorithms and have simpler proofs than Fu et al. have~\cite{shao_temp} for Micheal's non-blocking stack~\cite{Michael:2004:HPS:987524.987595} implementation under a sequentially consistent memory model. Another notably important point is handling \textit{batched-deallocation}, which Gotsman et al.~\cite{Gotsman:2013:VCM:2450268.2450289} and Tassarotti et al.~\cite{verrcu} can handle. Likewise, our logical state includes \textit{free list} which is an abstract map used mostly for reasoning about the \textit{bounding-threads} of the concrete RCU state-- reified logical state-- and RCU synchronization for safe reclamation through the global invariants and the type denotations. There is an almost direct mapping between Gotsman et al.'s \textsf{detached} and \textsf{in\_sum} sets for hazard pointers model and our logical abstract \textit{free list}. This crucial mapping implies that our type system can also directly be applied to hazard pointers and we think that it is a good future direction to investigate the applicability of our type system to different clients of different \textit{deferred} memory reclamation schemes~\cite{Wen:2018:IMR:3178487.3178488,Michael:2004:HPS:987524.987595,Mckenney:2004:EDD:1048173,UCAM-CL-TR-579}. Mandrykin et al.~\cite{Mandrykin:2016:TDV:3001219.3001297} use \textsf{VCC}~\cite{Cohen:2009:VPS:1616077.1616080} to verify an implementation of RCU primitives using specifications relating to a specific implementation, and do not verify client code.

\mypar{Weak Memory Models} Tassarotti et al.~\cite{verrcu} uses a protocol based program logic based on separation and ghost variables called \textsf{GPS}~\cite{Turon:2014:GNW:2660193.2660243} to verify user-level \textsf{RCU} singly linked list under \emph{release-acquire} semantics, which is a weaker memory model than sequential-consistency. They enforce the safe synchronization protocol in between the readers and the writer thread through \textit{release-writes} and \textit{acquire-reads} of the counters as a part of the QSRB model. We do capture all the guarantees from these \textit{release-acquire} orderings in our model via \textit{logical observations} -- e.g. (\textsf{iterator} $tid$, \textsf{unlinked} and \textsf{freeable}) -- the writer thread makes on the heap. Based on our comparative understanding taking Tassarotti's work as a reference, although we do not show it formally within the scope of this paper, we do not see any fundamental reason for not having our model to work under \textit{release-acquire} semantics.

\mypar{Separation of Concerns for Client Verification}: We think that instantiating a basis logic requires an effort on providing clean separation between client verification and full functional correctness of a model. \textit{This effort is subtle and important}. Meyer et al. ~\cite{myr} presents a methodology to separate \textit{linearasibility} proofs for Michael\&Scott's queue~\cite{Michael:1996:SFP:248052.248106} and DGLM~\cite{Doherty:2004:DSB:1007912.1007945} from memory reclamation model via establishing an over approximation for the \textit{epoch-based} and \textit{hazard-pointers} reclamation model. We hope our generic abstractions for linked-data structures inspire them when they integrate linked-data structure abstractions(e.g. linked-list) to their methodology. Regarding specifying client's action, Tassarotti et al. provide \textit{abstract-predicates} -- e.g. WriterSafe -- which might not be so reusable for an arbitrary RCU client -- e.g. binary search tree -- as they include linked list specific logical constructions together with the constructions for QSRB model. On the other hand, we manage to keep our types for client specification not only relatively simple but also reusable for different clients (e.g. a linked list in Appendix \ref{appendix:bag_paul} and a binary search tree in Appendix \ref{appendix:bst_del} via careful instantiation of Views framework: logical state including thread's observations, global memory invariants in Appendix \ref{sec:lemmas} and the denotations of our types in Figure \ref{fig:denotingtypeenviroment} Section \ref{sec:soundness}. 
%The writer thread \textit{release-writes} to its own counter to start synchronization(corresponds to setting the bounding threads to be same with the set of readers) and by doing so it publishes the fact that the updated heap node is no more reachable for the new coming reader threads. When a reader thread \textit{acquire-reads} the updated writer counter, it \textit{release-writes} the value to its own counter to announce that it is done with the heap node and is now \textit{quiescent}(corresponds to removing the reader's identifier both from the readers' set and bounding threads' set when exiting read-side critical section). After updating its counter, the writer thread repeatedly \textit{acquire-reads} the readers' counter to check whether they are all \textit{quiescent}(corresponds to the empty set of bounding threads). If so, then it is safe for the writer thread to reclaim the unreachable old heap node. We do capture all of these \textit{release-acquire} orderings based on the \textit{logical observations}(\textsf{iterator} $tid$, \textsf{unlinked} and \textsf{freeable}) of the writer thread on the heap and its importance is twofold:
%\begin{itemize}
%\item  Although we do not show it formally within the scope of this paper, we do not see any fundamental reason for having our model to work under \textit{release-acquire} semantics.
%\item Tassarotti et al. provide \textit{abstract-predicates} -- e.g. WriterSafe -- (which mainly corresponds to our global memory invariants in Appendix \ref{sec:lemmas} and the denotations of our types in Figure \ref{fig:denotingtypeenviroment} Section \ref{sec:soundness}) to be asserted and discharged for each of the RCU client actions and these abstract predicates might not be so reusable for another RCU client -- e.g. binary search tree -- as they include linked list specific logical constructions. Regarding memory safety of RCU clients, it is important to emphasise that we use the same types for different clients(e.g. a linked list in Appendix \ref{appendix:bag_paul} and a binary search tree in Appendix \ref{appendix:bst_del}) without having to prove the RCU properties (e.g. unreachable nodes, proper orderings etc.) separately for each different RCU client: since we introduce the logical observation and memory safety properties within the \textit{meta-theory}(logical RCU state, global memory invariants and the denotations of the types) and prove all of the RCU properties as a part of the soundness proof just for once.
%\end{itemize}

\mypar{Realizing Our Abstract RCU Model} Efficient implementations minimizes the cost of the read-side critical section operations: entering/exiting to the read-side critical section. Typically, implementations are structured so each reader thread (or CPU) maintains its own \emph{fragment} of the shared global state, which is only updated by that thread, but is read by the write-side primitives. For example, Tassarotti et al.~\cite{verrcu} model the readers' counters as an array of counters where the content of each cell corresponds to the counter of a specific reader thread in QSRB model. On the other hand, a direct implementation of our semantics would yield unacceptable performance, since both entering(\lstinline|ReadBegin|) and exiting(\lstinline|ReadEnd|) modify shared data structures for the \textit{bounding-threads} and \textit{readers} sets. A slight variation on our semantics would use a bounding set  that tracked such a snapshot of counts, and a vector of per-thread counts in place of the reader set. Blocking grace period completion until the snapshot was strictly older than all current reader counts would be more clearly equivalent to these implementations. Our current semantics are simpler than this alternative, while also equivalent.However, we know that if we had this slight variation in the implementation for the \lstinline|ReadBegin| and \lstinline|ReadEnd| then all actions(traverse and read the node value) from a reader thread would \textit{reduce} to an \textit{atomic} read of a data value(logical atomicity of readers' actions). Since we do not provide the careful implementation for the the \lstinline|ReadBegin| and \lstinline|ReadEnd| we cannot provide the \textit{atomicity} proof as well.
%(\textit{\textbf{RCU Model and Model Checking}}) - %Alglave et al. gives first semantics for the Linux kernel's implementation of \textsf{RCU}~\cite{abssem,Alglave:2018:FSC:3173162.3177156,DBLP:conf/cav/AlglaveKT13}. It captures details(behaviours on memory models etc.) of \textsf{RCU} implementation in Linux Kernel so it is much detailed and close to real implementation than our semantics is. However, our semantics abstracts the one Alglave et al. presents without loosing the \textit{fundamental law of} \textsf{RCU}  ~\cite{Alglave:2018:FSC:3173162.3177156} against which we show that our type system enforces correct usage of \textsf{RCU} API to guarantee memory safety(proper reclamation) and properties like \textit{acyclicity} for data structures implemented with using the API soundly. 

\mypar{Model Checking}
Desnoyers et al. propose a virtual architecture to model out of order memory accesses and instruction scheduling~\cite{Desnoyers:2013:MSM:2506164.2506174} and use the \textsf{SPIN} model checker to verify a user-mode implementation of RCU~\cite{urcu_ieee}. This method requires manual translation from C to SPIN modelling language.
Liang et al. presents an approach to verify the \emph{grace period} guarantee of \textsf{Tree RCU} in Linux kernel~\cite{LiangMKM16}. \textsf{Tree RCU} is an hieararchical \textsf{RCU} model which is a remedy to contention of writer threads in the single global lock model. 
Similarly, Kokologiannakis et al.~\cite{Kokologiannakis:2017:SMC:3092282.3092287} use a stateless model checker for testing the core of \textsf{Tree RCU}.
Liang's approach has limited support for lists and callback handling which are important when we consider the correctness for writer primitives which are based on callback handling. Kokologiannakis's approach overcomes all these limitations and shows considerable performance when compared with Liang's approach using \textsf{CBMC}. 
%Our method do not consider optimized \textsf{RCU} implementation such as \textsf{Tree RCU} as we focus on enforcing correct usages of \textsf{RCU} primitives instead of giving formal semantics to optimized efficient \textsf{RCU} implementation.
Both focus on validating a particular RCU implementation, whereas we focus on verifying memory safety of clients independent of implementation.
  
\mypar{Type Systems}
Howard et al.~\cite{Howard:2011:RES:2001252.2001267} enhance \textsf{STM} in Haskell to a technique called \textit{Relativistic Programming} which aims low overhead linearly scalable concurrent threads. Unlike our system which types binary search tree in \textsf{RCU} setting, they claim  handling trees (look-up followed by update) as a future work.
A follow up paper from Cooper et al.~\cite{Cooper2015RelativisticPI} presents a \textsf{Haskell} library called \emph{Monadic RP}, for relativistic programming. Similar to our approach, Monadic RP provides types and relativistic programming constructs for write/read critical sections which enforce correct usage of relativistic programming pattern. 
They also have only checked a linked list.
Thus our work is the first type system for ensuring correct use of RCU primitives that is known to handle more complex structures than linked lists.
%\subsection{More on Efficiency in Real RCU Implementations}
%\label{sec:effici}
%\iso{I am no sure this part should be in the ESOP version.}
%Our simple global lock semantics for write critical sections has so many drawbacks in terms limiting the scalability and performance. The motivation of \textsf{RCU} is having very cheap reader critical sections but the number of reader theards can be a lot and this can be a problem. Although readers' performance are not effected badly, writer thread must show the grace period to all of these \emph{active/pre-existsting} readers in such a way that it must \emph{defer} the reclamation phase blocking (or in some implementations registering callback to be invoked after grace period) until all active readers are done with their jobs. Acquiring a global lock during each grace period severly affects scalibility and performance. To overcome this problem, a \emph{tree based} hieararchical mechanism is implemented to handle each thread's (CPU's) \emph{quiescent-state} information and \emph{grace-period}. In Tree RCU, the data strcuture is used in such a way that it records each CPU's quiescent states. The \textsf{rcu} node tree propagates these states up to the root, and then propagates grace-period information down to the leaves. Quiescent-state information does not propagate upwards from a given node until a quiescent state has been reported by each CPU covered by the subtree rooted at that node. This propagation scheme dramatically reduces the lock contention experienced by the upper levels of the tree ~\cite{LiangMKM16}
%
%Real implementations, of course, must also tolerate the weak memory model of whatever processor they run on, leading them to use. For example, the primitive to dereference a memory location shown by a pointer and the primitive to update the memory location shown by a pointer contain architecture-specific memory barrier instructions and compiler directives to enforce correct ordering. Both primitives reduce to simple assignment statements on sequentially consistent systems. Dereferencing is volatile access except on DEC Alpha, which also requires a memory barrier \todo{CITE}.
%
%The Linux implementation of the communication in between reader thread and writer thread is based on waiting for context switches. The implementation uses calls \lstinline|SyncStart| and returns back from \lstinline|SyncStop| after all CPUs have passed through at least one context switch. The synchronous version of the primitive to wait reader threads is \textsf{synchronize\_rcu}. For performance reasons, the Linux implementation has also asynchronous version of this primitive named \textsf{call\_rcu}. Detecting context switches requires maintaining state shared between CPUs. A CPU must update state, which other CPUs read, that indicate it executed a context switch ~\cite{Mckenney_rcuusage}.


==> chapters/RCUTypesSoundness.tex <==
\section{Soundness}
\label{sec:soundness}
Here we give overview for our strategy to prove soundness of the system. To prove soundness we use the Views Framework~\cite{views} and all Views encoding, definitions, proofs and invariants for \textit{wellformedness} can be found in detail in Appendix \ref{sec:lemmas}. 

We do our reasoning for soundness over instrumented states which we define logical states, $\textsf{LState}$ to be
\begin{itemize}
\item A machine state, $\sigma=(s,h,l,rt,R,B,F)$;
\item An observation map, O, of type $ \textsf{Loc} \to \mathcal{P}(\textsf{obs})$
\item Undefined variable map, $U$, of type $\mathcal{P}(\textsf{Var}\times \textsf{TID})$
\item Set of threads, $T$, of type $\mathcal{P}(\textsf{TIDS})$
\end{itemize}
Each memory region can be observed in one of the following type states within a snapshot taken at any time $\textsf{obs} := \texttt{iterator} \; \mathrm{tid} \mid \texttt{unlinked} \mid \texttt{fresh} \mid \texttt{freeable} \mid \texttt{root}$. We are interested in \textsf{RCU} typed of heap domain which we define as:$\textsf{RCU} = \{ o \mid \textsf{ftype}(f) = \textsf{rcu} \land \exists o' \ldotp h(o',f) = o \}$
A thread's (or scope's) \emph{view} of memory is a subset of the instrumented(logical states), which satisfy certain well-formedness criteria relating the physical state and the additional meta-data ($O$, $U$, and $T$):  $\mathcal{M} \stackrel{def}{=} \{ m \in (\textsf{MState} \times O \times U \times T) \mid  \textsf{WellFormed}(m) \}$.
We do our reasoning for soundness over instrumented states and define an erasure relation $\lfloor - \rfloor :\mathsf{MState} \implies \textsf{LState}$ that projects instrumented states to the common components with \textsf{MState}.

Well-formedness imposes restrictions over the representation of the \textsf{RCU} structure in memory and type of threads for actions defined in operational semantics. For instance, \emph{an unlinked heap location cannot be reached from a root of an \textsf{RCU} data structure}. We define well-formedness as conjuction of memory axioms define in Section \ref{sec:memaxioms} Appendix \ref{sec:lemmas}.
\begin{figure}\tiny
\[
\begin{array}{l@{\;\;=\;\;}l}
 \llbracket \, x : \textsf{rcuItr}\,\rho\,\N \,  \rrbracket_{tid}
&
\left\{
\begin{array}{l|l}
\sigma,O,U,T,F
&(\textsf{iterator} \, tid\in  O(\sigma.s(x,tid)))  \land (x \notin U)  \land \\
& (\forall_{f_i\in dom(\N), x_i\in codom(\N) } \ldotp \sigma.s(x_i,tid) = \sigma.h(\sigma.s(x,tid), f_i) \land \textsf{iterator}\in O(s(x_i,tid))) \land \\
&(\forall_{\rho', \rho''}\ldotp \rho'.\rho'' = \rho \implies  \textsf{iterator}\,tid \in O(h^{*}(\sigma.rt,\rho'))) \land h^{*}(\sigma.rt,\rho)  \sigma.s(x,tid)\\

\end{array}
\right\}
\\
\llbracket \, x : \textsf{unlinked} \, \rrbracket_{tid}
&
\left\{
\begin{array}{l|l}
\sigma,O,U,T
&(\textsf{unlinked}\in  O(\sigma.s(x,tid)) \land \sigma.l = tid \land x \notin U)
%\land \\ &((\forall_{o'f'} \ldotp h(o',f')= s(x,tid) \implies (\textsf{unlinked} \in O(o') \lor \textsf{freeable} \in O(o'))))
\end{array}
\right\}
\\
\llbracket \, x : \textsf{freeable} \, \rrbracket_{tid}
&
\left\{
\begin{array}{l|l}
\sigma,O,U,T
&\textsf{freeable}\in  O(\sigma.s(x,tid)) \land \sigma.l = tid \land x \notin U \land \{x\mapsto \{\emptyset\}\} \in \sigma.F
\end{array}
\right\}
\\
\llbracket \, x : \textsf{rcuFresh} \, \N \, \,  \rrbracket_{tid}
&
\left\{
\begin{array}{l|l}
\sigma,O,U,T
&(\textsf{fresh}\in  O(s(x,tid)) \land x \notin U ) \land \\
&(\forall_{f_i\in dom(\N), x_i\in codom(\N) } \ldotp \sigma.s(x_i,tid) = \sigma.h(\sigma.s(x,tid), f_i) \land \textsf{iterator}\,tid \in O(s(x_i,tid))) \\
& \forall_{f}
\end{array}
\right\}
\\
\llbracket  x : \textsf{undef}\rrbracket_{tid}
&
\left\{
\begin{array}{l|l}
\sigma,O,U,T
&
(x,tid) \in U
\end{array}
\right\}
\\
\llbracket \, x : \textsf{rcuRoot}\rrbracket
&
\left\{
\begin{array}{l|l}
\sigma,O,U,T
&
((\sigma.rt \notin U \land (x,\_) = \sigma.rt \land \sigma.rt \in dom(\sigma.h) \land O(\sigma.rt) \in \textsf{root} )
\end{array}
\right\}
\end{array}
\]
$  \bullet  = (\bullet_{\sigma},\bullet_O,\cup,\cup)$ \quad
  $O_{1} \bullet_O O_{2}(loc) \overset{\mathrm{def}}{=}  O_{1}(loc) \cup O_{2}(loc)$\quad
  $ (s_1 \bullet_s s_2) \overset{\mathrm{def}}{=}  s_1 \cup s_2 \texttt{   when   } dom(s_1) \cap dom(s_2) = \emptyset$ \\
  $(F_1 \bullet_F F_2) \overset{\mathrm{def}}{=}  F_1  \cup F_2 \texttt{   when   } dom(F_1) \cap dom(F_2) = \emptyset$ \\
$
\begin{array}{l}
(h_1\bullet_h h_2)(o,f)\overset{\mathrm{def}}{=}  \left\{
\begin{array}{ll}  
\mathrm{undef} & \textrm{if}~h_1(o,f)=v \land h_2(o,f)=v' \land v' \neq v\\
v & \textrm{if}~h_1(o,f)=v \land h_2(o,f)=v\\
v & \textrm{if}~h_1(o,f)=\mathrm{undef}\land h_2(o,f)=v\\
v & \textrm{if}~h_1(o,f)=v\land h_2(o,f)=\mathrm{undef}\\
\mathrm{undef} & \textrm{if}~h_1(o,f)=\mathrm{undef}\land h_2(o,f)=\mathrm{undef}
\end{array}
\right\}
\end{array}
\;\;
\begin{array}{l}
((s,h,l,rt,R,B,F), O, U, T) \mathcal{R}_{0}((s',h',l',rt',R',B',F'), O', U', T') \overset{\mathrm{def}}{=}
\\ \bigwedge\left\{
	\begin{array}{l}
	  l  \in  T \rightarrow (h = h' \land l=l')\\
	  l\in T\rightarrow F=F'\\
          l\in T\rightarrow T \cap B= T'\cap B'\\
	  \forall tid,o\ldotp\textsf{iterator} \, tid \in O(o) \rightarrow o \in dom(h) \\
	  \forall tid,o\ldotp\textsf{iterator} \, tid \in O(o) \rightarrow o \in dom(h') \\
	  O = O' \land U = U' \land T = T'\land rt = rt' \\

	  \forall x, t \in T \ldotp s(x,t) = s'(x,t)
	\end{array}
\right\}
\end{array}
$

\caption{Type Environments, Composition($\bullet$) and Thread Interference Relation($\mathcal{R}_{0}$)}
\label{fig:denotingtypeenviromentp}
\vspace{-2mm}
\end{figure}
Every type environment represents a set of possible views (well-formed logical states) consistent with the types in the environment.  We make this precise with a denotation function
\[\llbracket-:-\rrbracket_- : \mathsf{Var}\rightarrow\mathsf{Type}\rightarrow\mathsf{TID}\rightarrow\mathcal{P}(\mathcal{M})\] that yields the set of states corresponding to a given type environment. This is defined in terms of denotation of individual variable assertions given in Figure \ref{fig:denotingtypeenviromentp}. To define the former, we first need to state what it means to combine logical machine states.

Composition of instrumented states is an operation $\bullet$ : $\mathcal{M} \longrightarrow \mathcal{M} \longrightarrow \mathcal{M}$ that is commutative and associative, and defined component-wise in terms of composing physical states, observation maps, undefined sets, and thread sets as shown in Figure \ref{fig:denotingtypeenviromentp}. An important property of composition is that it preserves validity of logical states:
\begin{lemma}[Well Formed Composition]
\label{lem:wf-compositionp}
Any successful composition of two well-formed logical states is well-formed:\[\forall_{x,y,z}\ldotp \mathsf{WellFormed}(x) \implies \mathsf{WellFormed}(y) \implies x\bullet y = z \implies \mathsf{WellFormed(z)}\]
\end{lemma}
Different threads' views of the state may overlap (e.g., on shared heap locations, or the reader thread set), but one thread may modify that shared state. Subsets of the logical views that are \emph{stable} with respect to expected interference from other threads or contexts.  We define the interference as (the transitive reflexive closure of) a binary relation $\mathcal{R}$ on $\mathcal{M}$ as $M \in \mathcal{P}(\mathcal{M}) | \mathcal{R}(M) \subseteq M\}$
Thread interference relation -- $\mathcal{R} \subseteq \mathcal{M} \times \mathcal{M}$ --  defines permissible interference on an instrumented state. The relation must distribute over composition:
\[ \forall m_{1}, m_{2}, m\ldotp (m_{1} \bullet  m_{2})\mathcal{R}m \Longrightarrow \begin{array}{ll}  \exists  m'_{1} m'_{2} \ldotp m_{1} \mathcal{R} m'_{1} \land m_{2} \mathcal{R} m'_{2} \land  m \in m'_{1} \bullet m'_{2} \end{array}\]
where $\mathcal{R}$ is transitive-reflexive closure of $\mathcal{R}_{0}$ shown at Figure \ref{fig:denotingtypeenviromentp}. $\mathcal{R}_0$ (and therefore $\mathcal{R}$) also ``preserves'' validity:
\begin{lemma}[Valid $\mathcal{R}_0$ Interference]
For any $m$ and $m'$, if $\mathsf{WellFormed}(m)$ and $m\mathcal{R}_0m'$, then $\mathsf{WellFormed}(m')$.
\end{lemma}
\begin{lemma}[Stable Environment Denotation]
For any \emph{closed} environment $\Gamma$ $($i.e., $\forall x\in\mathsf{dom}(\Gamma)\ldotp, \mathsf{FV}(\Gamma(x))\subseteq\mathsf{dom}(\Gamma)$ $):$
\[
\mathcal{R}(\llbracket\Gamma\rrbracket_{\mathsf{M},tid})\subseteq\llbracket\Gamma\rrbracket_{\mathsf{M},tid}
\]
Alternatively, we say that environment denotation is \emph{stable} (closed under $\mathcal{R}$).
\end{lemma}
The Views Framework defines a program logic (Hoare logic) with judgments of the form $\{ p \} C \{ q \}$ for views p and q and commands $C$.  Commands include atomic actions, and soundness of such judgments for atomic actions is a parameter to the framework.  The framework itself provides for soundness of rules for sequencing, fork-join parallelism, and other general rules.
To prove type soundness for our system, we define a denotation of \emph{type judgments} in terms of the Views logic, and show that every valid  typing derivation translates to a valid derivation in the Views logic:
\[\forall\Gamma,C,\Gamma',\mathit{tid}\ldotp\Gamma\vdash_{M,R} C\dashv \Gamma' \Rightarrow \{\llbracket\Gamma\rrbracket_\mathit{tid}\} \llbracket C\rrbracket_\mathit{tid}\{\llbracket\Gamma'\rrbracket_\mathit{tid}\}\].
\begin{theorem}[Axiom Soundness]
For each axiom, $\Gamma_{1} \vdash_{\textsf{RMO}} \alpha \dashv \Gamma_{2}$, we must show
\[
\forall m\ldotp   \llbracket \alpha \rrbracket  (\lfloor \llbracket \Gamma_{1} \rrbracket_{tid}  * \{m\} \rfloor )\subseteq  \lfloor \llbracket \Gamma_{2} \rrbracket_{tid} * \mathcal{R}(\{m\}) \rfloor
\]
\end{theorem}
\begin{proof}
By case analysis on the atomic action $\alpha$ followed by inversion on typing derivation.
\end{proof}
The use of $*$ validates the frame rule (\todo{ref}), and makes this obligation akin to an interference-tolerant version of the small footprint property from traditional separation logics~\tocite{lics02,localaction}.


==> chapters/RCUTypesSoundnessLemmas.tex <==
%!TEX root = ../paper.tex
\section{Soundness Proof of Atomic and Structural Program Actions}
\subsection{Proof of Lemmas}
\label{sec:prooflemmas}
\begin{lemma}[Well Formed Composition]
\label{lem:wf-composition}
Any successful composition of two well-formed logical states is well-formed:\[\forall_{x,y,z}\ldotp \mathsf{WellFormed}(x) \implies \mathsf{WellFormed}(y) \implies x\bullet y = z \implies \mathsf{WellFormed(z)}\]
\end{lemma}
\begin{proof}
By assumption, we know that \textsf{Wellformed}(x) and \textsf{Wellformed}(y) hold. We need to show that composition of two well-formed states preserves well-formedness which is to show that for all $z$ such that $x\bullet y = z$, \textsf{Wellformed}(z) holds.
  Both $x$ and $y$ have compontents $((s_x,h_x,l_x,rt_x,R_x,B_x),O_x,U_x,T_x,F_x)$ and $((s_y,h_y,l_y,rt_y,R_y,B_y),O_y,U_y,T_y,F_y)$, respectively. $\bullet_s$ operator over stacks $s_x$ and $s_y$ enforces $dom(s_x) \cap dom(s_y) = \emptyset$ which enables to make sure that wellformed mappings in $s_x$ does not violate wellformed mappings in $s_y$ when we union these mappings for $s_z$. Same argument applies for $\bullet_F$ operator over $F_x$ and $F_y$. Disjoint unions of wellformed $R_x$ with wellformed $R_y$ and wellformed $B_x$ with wellformed $B_y$ preserves wellformedness in composition as it is disjoint union of different wellformed elements of sets. Wellformed unions of $O_x$ with $O_y$,  $U_x$ with $U_y$  and $T_x$ with $T_y$ preserve wellformedness. When we compose $h_x(s(x,tid),f)$ and $h_y(s(x,l),f)$, it is easy to show that we preserve wellformedness if both threads agree on the heap location. Otherwise, if the heap location is undefined for one thread but a value for the other thread then composition considers the value. If a heap location is undefined for both threads then this heap location is also undefined for the location. All the cases for heap composition still preserves the wellformedness from the assumption that $x$ and $y$ are wellformed. 
  \end{proof}
\begin{lemma}[Valid $\mathcal{R}_0$ Interference]
For any $m$ and $m'$, if $\mathsf{WellFormed}(m)$ and $m\mathcal{R}_0m'$, then $\mathsf{WellFormed}(m')$.
\end{lemma}
\begin{proof}
  By assumption, we know that $m = (s,h,l,rt,R,B),O,U,T,F)$ is wellformed. We also know that $m'= (s',h',l',rt',R',B'),O',U',T',F')$ is related to $m$ via $R_{0}$. By assumptions in $R_{0}$ and semantics, we know that $O$,$R$,$T$ and $U$ which means that these components do not have any effect on wellformedness of the $m$. In addition, change on stack, $s$, does not affect the wellformedness as
\[\forall x,t \in T \ldotp s(x,t) = s'(x,t) \]
Moreover, from semantics we know that $l$ and $h$ can only be changed by writer thread and from $R_0$
\[l  \in  T \rightarrow (h = h' \land l=l')\]
\[  l\in T\rightarrow F=F'\]
and by assumptions from the lemma($\mathsf{WellFormed}(m)$.\textbf{RINFL}) we can conclude that $F$,$l$ and $h$ do not have effect on wellformedness of the $m$.
\end{proof}
\begin{lemma}[Stable Environment Denotation-M]\label{lemma:stblw}
For any \emph{closed} environment $\Gamma$ (i.e., $\forall x\in\mathsf{dom}(\Gamma)\ldotp, \mathsf{FV}(\Gamma(x))\subseteq\mathsf{dom}(\Gamma)$):
\[
\mathcal{R}(\llbracket\Gamma\rrbracket_{\mathsf{M},tid})\subseteq\llbracket\Gamma\rrbracket_{\mathsf{M},tid}
\]
Alternatively, we say that environment denotation is \emph{stable} (closed under $\mathcal{R}$).
\end{lemma}
\begin{proof}
  By induction on the structure of $\Gamma$.  The empty case holds trivially.  In the other case where $\Gamma=\Gamma',x:T$, we have by the inductive hypothesis that
  \[\llbracket\Gamma'\rrbracket_{\mathsf{M},tid}\] is stable, and must show that
  \[\llbracket\Gamma'\rrbracket_{\mathsf{M},tid}\cap\llbracket{x:\tau}\rrbracket_{tid}\] is as well.  This latter case proceeds by case analysis on $T$.

We know that $O$, $U$, $T$, $R$, $s$ and $rt$ are preserved by $R_0$. By unfolding the type environment in the assumption we know that $tid = l$. So we can derive conclusion for preservation of $F$ and $h$ and $l$ by
\[l  \in  T \rightarrow (h = h' \land l=l')\]
\[  l\in T\rightarrow F=F'\]
Cases in which denotations, $\llbracket x:T \rrbracket$, touching these \emph{R$_0$ preserved} maps are trivial to show.
  \begin{case} - \textsf{unlinked}, \textsf{undef}, $\textsf{rcuFresh}\, \N$ and \textsf{freeable} trivial.
\begin{case} - $\textsf{rcuItr}\,\rho\,\N$: All the facts we know so far from $R_0$, $tid=l$ and additional fact we know from $R_0$:
  \[\forall tid,o\ldotp\textsf{iterator} \, tid \in O(o) \rightarrow o \in dom(h) \]
  \[\forall tid,o\ldotp\textsf{iterator} \, tid \in O(o) \rightarrow o \in dom(h')\]
  prove this case.
  \end{case}
  \end{case}
  \begin{case} - \textsf{root}: All the facts we know so far from $R_0$, $tid=l$ and additional fact we know from $R_0$:
    \[ \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h) \]
    \[ \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h') \]
    prove this case.
    \end{case}
\end{proof}
\begin{lemma}[Stable Environment Denotation-R]
For any \emph{closed} environment $\Gamma$ (i.e., $\forall x\in\mathsf{dom}(\Gamma)\ldotp, \mathsf{FV}(\Gamma(x))\subseteq\mathsf{dom}(\Gamma)$):
\[
\mathcal{R}(\llbracket\Gamma\rrbracket_{\mathsf{R},tid})\subseteq\llbracket\Gamma\rrbracket_{\mathsf{R},tid}
\]
Alternatively, we say that environment denotation is \emph{stable} (closed under $\mathcal{R}$).
\end{lemma}
\begin{proof}
Proof is similar to one for Lemma \ref{lemma:stblw} where there is only one simple case, $\llbracket x:\textsf{rcuItr} \rrbracket$. 
\end{proof}
\begin{theorem}[Axiom Soundness]
For each axiom, $\Gamma_{1} \vdash_{\textsf{RMO}} \alpha \dashv \Gamma_{2}$, we must show
\[
\forall m\ldotp   \llbracket \alpha \rrbracket  (\lfloor \llbracket \Gamma_{1} \rrbracket_{tid}  * \{m\} \rfloor )\subseteq  \lfloor \llbracket \Gamma_{2} \rrbracket_{tid} * \mathcal{R}(\{m\}) \rfloor
\]
\end{theorem}
\begin{proof}
By case analysis on the atomic action $\alpha$ followed by inversion on typing derivation.
\end{proof}

Type soundness proceeds according to the requirements of the Views Framework, primarily embedding each type judgment into the Views logic:
\begin{lemma}\label{lemma:embedr}
\[  \forall\Gamma,C,\Gamma',\mathit{t}\ldotp\Gamma\vdash_R C\dashv \Gamma' \Rightarrow
\llbracket\Gamma\rrbracket_\mathit{t}\cap\llbracket{R}\rrbracket_t\vdash \llbracket C\rrbracket_\mathit{t}\dashv\llbracket\Gamma'\rrbracket_\mathit{t}\cap\llbracket{R}\rrbracket_t
\]
\end{lemma}
\begin{proof}
  Proof is similar to the one for Lemma \ref{lemma:embedw} except the denotation for type system definition is $\llbracket R \rrbracket_t = \{\{((s,h,l,rt,R,B),O,U,T,F)| t \in R \}$ which shrinks down the set of all logical states to the one that can only be defined by types($\textsf{rcuItr}$) in read type system. 
  \end{proof}
\begin{lemma}\label{lemma:embedw}
  \[
\forall\Gamma,C,\Gamma',\mathit{t}\ldotp\Gamma\vdash_M C\dashv \Gamma' \Rightarrow
\llbracket\Gamma\rrbracket_\mathit{t}\cap\llbracket{M}\rrbracket_t\vdash \llbracket C\rrbracket_\mathit{t}\dashv\llbracket\Gamma'\rrbracket_\mathit{t}\cap\llbracket{M}\rrbracket_t
\]
\end{lemma}
\begin{proof}
  Induction on derivation of $\Gamma \vdash_M C \dashv \Gamma'$ and then inducting on the type of first element of the environment. For the nonempty case, $\Gamma'',x:T$ we do case analysis on $T$. Type environment for write-side actions includes only: $\textsf{rcuItr} \, \rho \, \N$, $\textsf{undef}$, $\textsf{rcuFresh}$, $\textsf{unlinked}$ and $\textsf{freeable}$. Denotations of these types include the constraint $t=l$ and other constraints specific to the type's denotation. The set of logical state defined by the denotation of the type is \emph{subset} of intersection of the set of logical states defined by $\llbracket M \rrbracket_{t} \cap \llbracket x:T \rrbracket_{t}$ which shrinks down the logical states defined by  $\llbracket M \rrbracket_{t}= \{((s,h,l,rt,R,B),O,U,T,F)| t = l\}$ to the set of logical states defined by denotation $\llbracket x:T \rrbracket_t$.
  \end{proof}
\begin{lemma}[Write-Side Critical Section Lifting]
\label{lem:crit-lifting}
For each $\alpha$ whose semantics does not affect the write lock, if
\[\forall m\ldotp   \llbracket \alpha \rrbracket  (\lfloor \llbracket \Gamma_{1} \rrbracket_{tid}  * \{m\} \rfloor )\subseteq  \lfloor \llbracket \Gamma_{2} \rrbracket_{tid} * \mathcal{R}(\{m\}) \rfloor\]
then
%\[\forall m\ldotp   \llbracket \alpha \rrbracket  (\lfloor \llbracket \Gamma_{1} \rrbracket_{\textsf{R},tid}  * \{m\} \rfloor )\subseteq  \lfloor \llbracket \Gamma_{2} \rrbracket_{\textsf{R},tid} * \mathcal{R}(\{m\}) \rfloor\]
\[\forall m\ldotp   \llbracket \alpha \rrbracket  (\lfloor \llbracket \Gamma_{1} \rrbracket_{\textsf{M},tid}  * \{m\} \rfloor )\subseteq  \lfloor \llbracket \Gamma_{2} \rrbracket_{\textsf{M},tid} * \mathcal{R}(\{m\}) \rfloor\]
\end{lemma}
\begin{proof}
Each of these shared actions $\alpha$ preserves the lock  component of the physical state, the only component constrained by $\llbracket-\rrbracket_{M,tid}$ beyond $\llbracket-\rrbracket_{tid}$.
For the read case, we must prove from the assumed subset relationship that for an aritrary $m$:
\[\llbracket \alpha \rrbracket  (\lfloor \llbracket \Gamma_{1} \rrbracket_{tid}\cap\llbracket\textsf{M}\rrbracket_{tid}  * \{m\} \rfloor )\subseteq  \lfloor \llbracket \Gamma_{2} \rrbracket_{tid}\cap\llbracket\textsf{M}\rrbracket_{tid} * \mathcal{R}(\{m\}) \rfloor\]
By assumption, transitivity of $\subseteq$, and the semantics for the possible $\alpha$s,
the left side of this containment is already a subset of
\[\lfloor \llbracket \Gamma_{2} \rrbracket_{tid} * \mathcal{R}(\{m\}) \rfloor\]
What remains is to show that the intersection with $\llbracket\mathsf{M}\rrbracket_{tid}$ is preserved by the atomic action.
This follows from the fact that none of the possible $\alpha$s modifies the global lock.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Complete Memory Axioms}
\label{sec:memaxioms}
\begin{enumerate}
\item{Ownership} invariant in Figure \ref{fig:ownership} invariant asserts that none of the valid heap locations can be observed as undefined.
\begin{figure}[!htb]
\[
\textbf{OW}(\sigma,O,U,T,F) =
\left\{
\begin{array}{ll}
 	 & \forall_{o,o'f,f'} \ldotp  \sigma.h(o,f) = v \land \sigma.h(o',f') = v \\
	& \land v \in \textsf{OID}  \land  \textsf{FType}(f) = \textsf{RCU} \implies \\
 	&\left\{
		\begin{array}{cl}
			&  o=o' \land f=f' \\
			& \lor\textsf{unlinked} \in O(o) \\
		  & \lor \textsf{unlinked} \in O(o') \\
                  & \lor \textsf{freeable} \in O(o)\\
                  & \lor \textsf{freeable} \in O(o')\\
		        & \lor \textsf{fresh} \in O(o)) \\
                        & \lor \textsf{fresh} \in O(o')
		\end{array}
		\right.%\} 
\end{array}
\right.%\}
\]
\caption{Ownership}
\label{fig:ownership}
\end{figure}
\item{Reader-Writer-Iterators-CoExistence} invariant in Figure \ref{fig:rwitrexistence} asserts that  if a heap location is not undefined then all reader threads and the writer thread may observe the heap location as \textsf{iterator}. Observations that the writer thread can make specifically are \textsf{fresh}, \textsf{unlinked} or \textsf{freeable}. Semantic denotation of the \textsf{freeable} observation asserts that the observed heap location is in the free list and and there exists no thread holding a reference to it. If some references from the reader threads to an observed heap location in the free list may exist -- captured by \textsf{unlinked} state -- then these threads \textit{bound} the writer thread for the reclamation of the heap location.
\begin{figure}[!htb]
\[
\textbf{RWOW}(\sigma,O,U,T,F)=
\left\{
\begin{array}{ll}
	 \forall x,tid,o \ldotp \sigma.s(x,tid) = o  
         \land (x,tid) \notin U \implies \\ \left\{
		\begin{array}{ll}
 			& \textsf{iterator } \, tid \in O(o) \\
 		  & \lor (\sigma.l=tid \land (\textsf{unlinked} \in O(o) ) \\
		  & \lor (\sigma.l=tid  \land \textsf{freeable} \in O(o)))  \\
       & \lor (\sigma.l=tid \land \textsf{fresh} \in O(o))     
		\end{array}
	\right.%\}
\end{array}
\right.%\}
\]
\caption{Reader-Writer-Iterator-Coexistence-Ownership}
\label{fig:rwitrexistence}
\end{figure}
\item{Alias-With-Root} invariant in Figure \ref{fig:aliaswithroot} asserts that the unique root location can only be aliased with thread local references through which the unique root location is observed as \textsf{iterator}.
\begin{figure}[!htb]
\[
\textbf{AWRT}(\sigma,O,U,T,F)=
\left\{
(\forall_{y,tid} \ldotp h^{*}(\sigma.rt,\epsilon) = s(y,tid)  \implies \textsf{iterator}\, tid \in O(s(y,tid)))
	\right.%\}
\]
\caption{Alias with Unique Root}
\label{fig:aliaswithroot}
\end{figure}
\item{Iterators-Free-List} invariant in Figure \ref{fig:itrfreelist} asserts that if a heap location is observed as \textsf{iterator} by a thread -- $tid$ -- and it is in free list with a set of bounding threads -- $T'$ -- then $tid$ is an element of this set of bounding threads.
\begin{figure}[!htb]
\[
\textbf{IFL}(\sigma,O,U,T,F)=
\left\{
	\forall tid, o \ldotp  \textsf{iterator} \, tid \in O(o)  \land \forall_{T'\subseteq T} \ldotp \sigma.F([o \mapsto T'])  \implies tid \in T' 
\right.%\}
\]
\caption{Iterators-Free-List}
\label{fig:itrfreelist}
\end{figure}
\item{Unlinked-Reachability} invariant in Figure \ref{fig:unlinkreach} asserts that if a heap node is observed as \textsf{unlinked}, all heap locations from which you can reach to the \textsf{unlinked} one are also unlinked or in the free list.
\begin{figure}[!htb]
\[
\textbf{ULKR}(\sigma,O,U,T,F) =
\left\{
\begin{array}{ll}
  \forall o \ldotp \textsf{unlinked} \in O(o) \implies \\
  \left\{
	\begin{array}{cl}
	  \forall o',f '\ldotp \sigma.h(o',f') = o \implies \\
          \left\{
			\begin{array}{cl}
				&\textsf{unlinked} \in O(o') \lor\\
				& \textsf{freeable} \in O(o')
			\end{array}
		\right.%\}
	\end{array}
	\right.%\}
\end{array}
\right.%\}
\]
\caption{Unlinked-Reachability}
\label{fig:unlinkreach}
\end{figure}
\item{Free-List-Reachability} invariant in Figure \ref{fig:freelistchain} asserts that if a heap location -- $o$ is in the free list then all heap locations -- $o'$ -- from which you can reach to the one in the free list are also in the free list. The set of threads -- $T'$ -- referencing to $o'$ are included in the set of threads($T$) referencing to the $o$.
\begin{figure}[!htb]
\[
\textbf{FLR}(\sigma,O,U,T,F) =
\left\{
\begin{array}{ll}
  \forall o \ldotp F([o \mapsto T]) \implies \\
  \left\{
   		\begin{array}{cl}
		  \forall o',f' \ldotp \sigma.h(o',f') = o \implies \\
                \left\{
   \begin{array}{cl}
   	 		&\exists_{T'\subseteq T} \ldotp  F([o'\mapsto T']) 
   \end{array}
   \right.
                  \end{array}
 	\right.%\}
\end{array}
\right.%\}
\]
\caption{Free-List-Reachability}
\label{fig:freelistchain}
\end{figure}
\item{Mutator-Iterator-Unlinked} invariant in Figure \ref{fig:mutunliked} states that  writer thread cannot observe a heap location as \textsf{unlinked}. It captures the fact that there exists a single writer that can mutate the heap at a time.
\begin{figure}[!htb]
\[
\textbf{WULK}(\sigma,O,U,T,F) =
\left\{
\begin{array}{ll}
\forall o \ldotp \textsf{iterator} \, \sigma.l \in O(o)  \implies \textsf{unlinked} \notin O(o)
\end{array}
\right.%\}
\]
\caption{Writer-Unlink}
\label{fig:mutunliked}
\end{figure}
\item{Fresh-Reachable} invariant in Figure \ref{fig:freach} states that there exists no heap location that can reach to a freshly allocated heap location together with fact on nonexistence of aliases to it.
\begin{figure}[!htb]
  \[
  \textbf{FR}(\sigma,O,U,T,F) =
 \begin{array}{ll}
   \forall_{tid,x,o} \ldotp (\sigma.s(x,tid) = o \land \textsf{fresh} \in O(o) ) \implies \\
	\begin{array}{cl}
          (\forall_{y,o',f',tid'}. (h(o',f') \neq o) \lor  (s(y,tid) \neq)  o \lor (tid'\neq tid \implies s(y,tid') \neq o ))
        \end{array}
        \end{array}
\]
\caption{Fresh-Reachable}
\label{fig:freach}
\end{figure}

\item{Fresh-By-Mutator} invariant in Figure \ref{fig:fmut} states that heap allocation can be done only by writer thread.
  \begin{figure}[!htb]
  \[
\textbf{WF}(\sigma,O,U,T,F) =
 \forall_{tid,x,o} \ldotp (\sigma.s(x,tid) = o \land \textsf{fresh} \in O(o) ) \implies  tid = \sigma.l 
\]
\caption{Fresh-Writer}
\label{fig:fmut}
  \end{figure}
\item{Fresh-Not-Reader} invariant in Figure \ref{fig:fnotreader} states that heap location allocated freshly cannot be observed as \textsf{unlinked} or \textsf{iterator}.
  \begin{figure}[!htb]
  \[
\textbf{FNR}(\sigma,O,U,T,F) =
 \forall_{o} \ldotp (\textsf{fresh} \in O(o) ) \implies  (\forall_{x,tid} \ldotp \textsf{iterator}\,tid  \notin O(o)  ) \land \textsf{unlinked} \notin O(o) 
\]
\caption{Fresh-Not-Reader}
\label{fig:fnotreader}
  \end{figure}
\item{Fresh-Points-Iterator} invariant in Figure \ref{fig:fsinglefield} states that any field of fresh allocated object can only be set to point heap node which can be observed as \textsf{iterator} (not \textsf{unlinked or freeable}).  This invariant captures the fact $\N = \N'$ asserted in the type rule for fresh node linking(\textsc{T-LinkF}). 
  \begin{figure}[!htb]
  \[
\textbf{FPI}(\sigma,O,U,T,F) =
 \forall_{o} \ldotp (\textsf{fresh} \in O(o)  \land \exists_{f,o'}\ldotp h(o,f)=o') \implies (\forall_{tid} \ldotp  \textsf{iterator}\,tid \in O(o')) 
\]
\caption{Fresh-Points-Iterator}
\label{fig:fsinglefield}
  \end{figure}
   
\item{Writer-Not-Reader} invariant in Figure \ref{fig:wnr} states that a writer thread identifier can not be a reader thread identifier.
  \begin{figure}[!htb]
    \[
\textbf{WNR}(\sigma,O,U,T,F) =
\left\{
\begin{array}{ll}
 \sigma.l \notin \sigma.R
\end{array}
\right.%\}
\]
    \caption{Writer-Not-Reader}
\label{fig:wnr}
  \end{figure}
  \item{Readers-Iterator} invariant in the Figure \ref{fig:riter} states that a reader threads can only make \textsf{iterators} observation on a heap location.
  \begin{figure}[!htb]
    \[
\textbf{RITR}(\sigma,O,U,T,F) =
\left\{
\begin{array}{ll}
 \forall_{tid \in \sigma.R,o}\ldotp \textsf{iterator} \, tid \in O(o) 
\end{array}
\right.%\}
\]
    \caption{Writer-Not-Reader}
\label{fig:riter}
  \end{figure}
\item{Readers-In-Free-List} invariant in Figure \ref{fig:readerinflist} states that for any mapping from a location to a set of threads in the free list we know the fact that  this set of threads is a subset of bounding threads( which itself is subset of reader threads).
\begin{figure}[!htb]
  \[
\textbf{RINFL}(\sigma,O,U,T,F) =
\left\{
\begin{array}{ll}
  \forall_{o} \ldotp F([o \mapsto T]) \implies T \subseteq \sigma.B
\end{array}
\right.%\}
\]
\caption{Readers-In-Free-List}
\label{fig:readerinflist}
\end{figure}
\item{Heap-Domain} invariant in the Figure \ref{fig:dreachable} defines the domain of the heap.
\begin{figure}[!htb]
\[
\textbf{HD}(\sigma,O,U,T,F) =
\forall_{o,f',o'} \ldotp  \sigma.h(o,f) = o' \implies  o' \in dom(\sigma.h)
\]
    \caption{Heap-Domain}
\label{fig:dreachable}
\end{figure}
\item{Unique-Root} invariant in Figure \ref{fig:uroot} states that a heap location which is observed as \textsf{root} has no incoming edges from any nodes in the domain of the heap and all nodes accessible from root is is observed as \textsf{iterator}. This invariant is part of enforcement for \emph{acyclicity}.
  \begin{figure}[!htb]
\[
\textbf{UNQRT}(\sigma,O,U,T,F) =
  \left\{ \begin{array}{ll}
 \forall_{\rho \neq \epsilon} \ldotp \textsf{iterator} \, tid \in O( h^{*}(\sigma.rt,\rho) \land \lnot(\exists_{f'} \ldotp \sigma.rt = h( h^{*}(\sigma.rt,\rho),f'))
\end{array} \right.%\}
\]
    \caption{Unique-Root}
\label{fig:uroot}
\end{figure}
\item{Unique-Path} invariant in Figure \ref{fig:upath} states that every node is reachable from root node with an unique path. This invariant is a part of \emph{wellshapedness}(e.g. acyclicity) enforcement on the heap layout of the data structure. The justification for having this invariant is explained in \textbf{ULKR}.
  \begin{figure}[!htb]
\[
\textbf{UNQR}(\sigma,O,U,T,F) =
\left\{
\begin{array}{ll}
    \forall_{\rho, \rho'}  \ldotp  h^{*}(\sigma.rt,\rho) \neq h^{*}(\sigma.rt, \rho') \implies  \rho \neq \rho' 
\end{array}
\right.%\}
\]
\caption{Unique-Reachable}
\label{fig:upath}
\end{figure}
\end{enumerate}
 Each of these memory invariants captures different aspects of validity of the memory under \textsf{RCU} setting, $\textsf{WellFormed}(\sigma,O,U,T,F) $, is defined as conjunction of all memory axioms.

 \subsection{Soundness Proof of Atoms}
 \label{lem:lematom}
 In this section, we do proofs to show the soundness of each type rule for each atomic actions.
 \begin{lemma}[\textsc{Unlink}]\small
   \label{lemma:unlink}
\begin{align*}
  \llbracket x.f_1:=r \rrbracket (\lfloor \llbracket \Gamma, \, x:\mathsf{rcuItr}\,\rho\,\N ( [f_1 \rightharpoonup  z]), z:\mathsf{rcuItr} \, \rho' \,\N'([ f_2 \rightharpoonup r]), \;
  r:\mathsf{rcuItr} \, \rho'' \,\N'' \rrbracket_{M,tid} * \{m\}\rfloor)     \subseteq \\
                                                              \lfloor \llbracket \Gamma, \,  x:\mathsf{rcuItr} \, \rho \, \N( f_1 \rightharpoonup z \setminus r),\;
                                                              z:\mathsf{unlinked}, \;
                                                              r:\mathsf{rcuItr} \, \rho' \, \N'' \rrbracket  * \mathcal{R}(\{m\})\rfloor
\end{align*}
 \end{lemma}
 \begin{proof}
We assume
\begin{gather}\label{ahu1}
  \begin{aligned}
    (\sigma, O, U, T, F) \, \in &  \llbracket \Gamma, \, x:\mathsf{rcuItr}\,\rho\,\N ,\, z:\mathsf{rcuItr} \, \rho' \,\N', \\
    &r:\mathsf{rcuItr} \, \rho'' \,\N'' \rrbracket_{M,tid} * \{m\}
    \end{aligned} \\
\textsf{WellFormed}(\sigma,O,U,T,F)
\label{ahu2}
\end{gather}

From assumptions in the type rule of \textsc{T-UnlinkH} we assume that
\begin{gather}
  \rho.f_1=\rho' \text{ and } \rho'.f_2=\rho'' \text{ and } \N(f_1) = z \text{ and } \N'(f_2)=r
    \label{ahu4} \\
\forall_{f\in dom(\N')} \ldotp f\neq f_2 \implies  \N'(f) = \textsf{null}
      \label{ahu5} \\
\begin{array}{l}\footnotesize
\forall_{n\in \Gamma,m,\N''', p''',f}\ldotp n:\textsf{rcuItr}\,\rho'''\,\N'''([f\rightharpoonup m]) \implies %\arcr
\left\{\begin{array}{l}
((\neg\mathsf{MayAlias}(\rho''',\{\rho,\rho',\rho''\})  ) \land (m\not\in\{z,r\} ) ) \arcr
\land (\forall_{\rho''''\neq \epsilon} \ldotp \neg\mathsf{MayAlias}(\rho''', \rho''.\rho'''') )
\end{array}\right.
\end{array}
        \label{ahu6}
\end{gather}
We split the composition in  \ref{ahu1} as 
\begin{gather} \label{ahu11}
  \begin{aligned}
    (\sigma_1, O_{1}, U_{1}, T_{1},F_1 ) \in  &\llbracket \Gamma, \, x:\mathsf{rcuItr}\,\rho\,\N ,\, z:\mathsf{rcuItr} \, \rho' \,\N',\\
    &r:\mathsf{rcuItr} \, \rho'' \,\N'' \rrbracket_{M,tid} \end{aligned}\\
\label{ahu12}
(\sigma_2, O_{2}, U_{2}, T_{2},F_2) = m
\\
\label{ahusig}
\sigma_1 \bullet_s \sigma_2 = \sigma \\
\label{ahu13}
O_{1} \bullet_{O} O_{2} = O
\\
\label{ahu14}
U_{1} \cup U_{2} = U
\\
\label{ahu15}
T_{1} \cup T_{2} = T
\\
\label{ahff}
F_{1} \uplus F_2 = F
\\
\label{ahu16}
\textsf{WellFormed}(\sigma_1,O_{1},U_{1},T_{1},F_1)
\\
\label{ahu17}
\textsf{WellFormed}(\sigma_2,O_{2},U_{2},T_{2},F_2)
\end{gather}

We must show  $\exists_{\sigma'_1,\sigma'_2, O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2}, F'_1,F'_2}$ such that
\begin{gather}\label{phu5}
\begin{aligned}
(\sigma_1',O'_{1},U'_{1}, T'_{1},F'_1)  \in \llbracket \Gamma, \,  x:\mathsf{rcuItr} \, \rho \,\N([f_1 \rightharpoonup r]) ,\, z:\mathsf{unlinked}, r:\mathsf{rcuItr} \, \rho' \, \N'' \rrbracket_{M,tid}
\end{aligned}\\
\\
\label{phuN}
\N(f_1)= r
\\
\label{phu6}
(\sigma_2',O'_{2},U'_{2}, T'_{2}, F'_2) \in \mathcal{R}(\{m\})
\\
\label{ahusig'}
\sigma'_1 \bullet_s \sigma'_2 = \sigma' \\
\label{phu7}
O'_{1} \bullet_{O} O'_{2} = O'
\\
\label{phu8}
U'_{1} \cup U'_{2} = U'
\\
\label{phu9}
T'_{1} \cup T'_{2} = T'
\\
\label{phff}
F'_{1} \uplus F'_2 = F'
\\
\label{phu10}
\textsf{WellFormed}(\sigma_1',O'_{1},U'_{1},T'_{1},F'_1) \\
\label{phu11}
\textsf{WellFormed}(\sigma_2',O'_{2},U'_{2},T'_{2},F'_2)
\end{gather}
We also know from operational semantics that the machine state has changed as
\begin{gather}\label{ahus}
\sigma_1' =  \sigma_1[h(s(x,tid),f_1 ) \mapsto s(r,tid) ]
\end{gather}
and \ref{ahus} is determined by operational semantics. 

The only change in the observation map is on $s(y,tid)$ from $\textsf{iterator}\;tid$ to $\textsf{unliked}$
\begin{gather}\label{ahus1}
  O'_1 =  O_1(s(y,tid))[\textsf{iterator}\;tid \mapsto \textsf{unlinked}]
\end{gather}
\ref{ahus2} follows from \ref{ahu1}
\begin{gather}\label{ahus2}
  T_1 = \{tid\} \text{ and } tid = \sigma.l
\end{gather}

$\sigma'_1$ is determined by operational semantics. The undefined map, free list and $T_1$ need not change so we can pick $U'_1$ as $U_1$, $T'_1$ as $T_1$ and $F'_1$ as $F_1$. Assuming \ref{ahu11} and choices on maps makes $(\sigma_1',O'_{1},U'_{1}, T'_{1})$ in denotation
\[\llbracket \Gamma, \,  x:\mathsf{rcuItr} \, \rho \,\N([ f \rightharpoonup r]), z:\mathsf{unlinked}, r:\mathsf{rcuItr} \, \rho' \, \N'' \rrbracket_{M,tid}\]

In the rest of the proof, we prove \ref{phu10}, \ref{phu11} and show the composition of $(\sigma'_1, O'_1, U'_1,T'_1,F'_1)$ and  $(\sigma'_2, O'_2, U'_2,T'_2,F'_2)$. To prove \ref{phu10}, we need to show that each of the memory axioms in Section \ref{sec:memaxioms} holds for the state $(\sigma',O'_1,U_1',T_1',F'_1)$.

Let $o_x$ be $\sigma.s(x,tid)$, $o_y$ be $\sigma.s(y,tid)$ and $o_z$ be $\sigma.s(z,tid)$.
\begin{case}\label{unqr} - \textbf{UNQR} \ref{ahus3} and \ref{ahus4} follow from framing assumption(\ref{ahu4}-\ref{ahu6}), denotations of the precondition(\ref{ahu11}) and \ref{ahu16}.\textbf{UNQR}
  \begin{gather}\label{ahus3}
    \rho \neq \rho' \neq \rho'' 
  \end{gather}
and   
  \begin{gather}\label{ahus4}
    o_x \neq o_y \neq o_z 
  \end{gather}
  where $o_x$, $o_y$ and $o_z$ are equal to $\sigma.h^{*}(\sigma.rt,\rho)$, $\sigma.h^{*}(\sigma.rt,\rho,f_1)$ and $\sigma.h^{*}(\sigma.rt,\rho.f_1.f_2)$ respectively and they($o_x,o_y,o_z$ and $\rho,\rho'$) are unique.

We must prove 
\begin{gather}\label{phuc1}
     h'^{*}(\sigma.rt,\rho) \neq h'^{*}(\sigma.rt, \rho.f_1)  \implies \rho \neq \rho.f_1 
\end{gather}
to show that uniqueness is preserved.

We know from operational semantics that root has not changed so
\[\sigma.rt = \sigma'.rt\]

From denotations (\ref{phu5}) we know that all heap locations reached by following $\rho$ and $\rho.f_1$ are observed as $\textsf{iterator}\, tid$ including the final reached heap locations($\textsf{iterator}\,tid \in O'_1(\sigma'.h^{*}(\sigma.rt,\rho))$ and $\textsf{iterator}\,tid \in O_1'(\sigma'.h^{*}(\sigma.rt,\rho.f_1))$). \ref{phuN} is determined directly by operational semantics.

$\textsf{unlinked}\in O'_1(o_y)$ follows from \ref{ahus1} and \ref{ahus} which makes path $\rho.f_1.f_2$ invalid(from denotation(\ref{phu5}), all heap locations reaching to  $O_1'(o_r)$ from root($\sigma.rt$) are observed as  $\textsf{iterator}\, tid$ so this proves that  $\textsf{unlinked}\in O'_1(o_y)$)  cannot be observed on the path to the $o_r$ which implies that $f_2$ cannot be part of the path and uniqueness of the paths to $o_x$ and $o_r$ is preserved. So we conclude \ref{ahus5} and \ref{ahus6}
  \begin{gather}\label{ahus5}
    \rho \neq \rho'
  \end{gather}
    \begin{gather}\label{ahus6}
    o_x \neq o_y \neq o_z 
  \end{gather}
from which \ref{phuc1} follows.
\end{case}
\begin{case} - \textbf{OW} By \ref{ahu16}.\textbf{OW}, \ref{ahus}, \ref{ahus1}.
\end{case}
\begin{case} - \textbf{RWOW} By \ref{ahu16}.\textbf{RWOW}, \ref{ahus} and \ref{ahus1}.
\end{case}
\begin{case} - \textbf{IFL} By \ref{ahu16}.\textbf{WULK}, \ref{ahu16}.\textbf{RINFL}, \ref{ahu16}.\textbf{IFL}, \ref{ahus1} and choice of $F'_1$.
\end{case}
\begin{case} - \textbf{FLR} By choice of $F'_1$ and \ref{ahu16}. 
\end{case}
\begin{case} - \textbf{WULK} By \ref{phu5},  \ref{ahus1} and \ref{ahus2}.
\end{case}
\begin{case} - \textbf{WF}, \textbf{FPI} and \textbf{FR} Trivial.
\end{case}
\begin{case} - \textbf{AWRT} By \ref{phu5}.
\end{case}
\begin{case} - \textbf{HD} By \ref{phu10}.\textbf{OW}(proved), \ref{ahu16}.\textbf{HD}  and \ref{ahus}. 
\end{case}
\begin{case} - \textbf{WNR} By \ref{ahu16}.\textbf{WNR}, \ref{ahus}, \ref{ahus1} and \ref{ahus2}.
\end{case}
\begin{case} - \textbf{RINFL} By \ref{phu5}, \ref{ahu16}.\textbf{RINFL}, choice of $F'_1$ and \ref{ahus}.
\end{case}
\begin{case} - \textbf{ULKR} We must prove \ref{phuc2}
  \begin{gather}\label{phuc2}
    \begin{aligned}
      \forall_{o',f'} \ldotp \sigma'.h(o',f') = o_y \implies & \textsf{unlinked} \in O'_1(o')  \\
      &\lor (\textsf{freeable} \in O'_1(o'))
      \end{aligned}
\end{gather}
which follows from \ref{phu5}, \ref{ahu16}.\textbf{OW}, operational semantics(\ref{ahus}) and \ref{ahus1}. If $o'$ were observed as \textsf{iterator} then that would conflict with \ref{phu10}.\textbf{UNQR}. 
\end{case}
\begin{case} - \textbf{UNQRT}: By \ref{ahu16}.\textbf{UNQRT}, \ref{ahus1} and \ref{ahus}.
\end{case}
To prove \ref{phu6} we need to show interference relation
\[(\sigma, O_2, U_2, T_2,F_2) \mathcal{R} (\sigma', O'_2, U'_2, T'_2,F'_2)  \]
which by definition means that we must show 
\begin{gather}\label{phu17}
  \sigma_2.l  \in  T_2 \rightarrow (\sigma_2.h =\sigma'_2.h \land \sigma_2.l=\sigma'_2.l)\\
  \label{phu18}
  l\in T_2\rightarrow F_2=F_2'\\
  \label{phu20}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma_2.h) \\
  \label{phu21}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma'_2.h) \\
  \label{phu22}
  O_2 = O_2' \land U_2 = U_2' \land T_2 = T_2' \land \sigma_2.R = \sigma'_2.R \land \sigma_2.rt = \sigma'_2.rt \\
  \label{phu23}
  \forall x, t \in T_2 \ldotp \sigma_2.s(x,t) = \sigma'_2.s(x,t) \\
  \label{phurt1}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h) \\
  \label{phurt2}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h') 
\end{gather}
To prove all relations (\ref{phu17}-\ref{phu23}) we assume \ref{ahus2} which is to assume $T_2$ as subset of reader threads. Let $\sigma'_2$ be $\sigma_2$. $O_2$ need not change so we pick $O'_2$  as $O_2$. Since $T_2$ is subset of reader threads, we pick $T_2$ as  $T'_2$. We pick $F'_2$ as $F_2$.

\ref{phu17} and \ref{phu18} follow from \ref{ahus2} and choice of $F_2'$. \ref{phurt1}, \ref{phurt2} and \ref{phu22} are determined by choice of $\sigma'_2$, operational semantic and choices made on maps related to the assertions.

By assuming \ref{ahu17} we show \ref{phu11}. \ref{phu20} and \ref{phu21} follow trivially. \ref{phu23} follows from choice of $\sigma'_2$, \ref{ahus} and \ref{ahus2}. 

To prove \ref{phu7} consider two cases: $O'_1 \cap O'_2 = \emptyset$ and $O'_1 \cap O'_2 \neq \emptyset$. The first case is trivial. The second case is where we consider 
\[
\textsf{iterator}\,tid \in O'_2(o_y)
\]
We also know from \ref{ahus1} that
\[\textsf{unliked} \in O'_1(o_y)\]
Both together with \ref{ahu13} and \ref{phu5} proves \ref{phu7}.

To show \ref{ahusig'} we consider two cases: $\sigma'_1.h \cap \sigma'_2.h = \emptyset$ and $\sigma'_1.h \cap \sigma'_2.h \neq \emptyset$. First is trivial. Second follows from \ref{phu10}.\textbf{OW}-\textbf{HD} and \ref{phu11}.\textbf{OW}-\textbf{HD}. \ref{phu8}, \ref{phu9} and \ref{phff} are trivial by choices on related maps and semantics of composition operations on them. All compositions shown let us to derive conclusion for $(\sigma'_1, O'_1, U'_1, T'_1,F'_1) \bullet (\sigma'_2, O'_2, U'_2, T'_2,F'_2) $.
   \end{proof}
 \begin{lemma}[\textsc{LinkFresh}]
   \label{lemma:linkf}
   \begin{align*}
  \llbracket p.f := n \rrbracket (\lfloor \llbracket \Gamma,\,
 p:\textsf{rcuItr}\, \rho \, \N \, ,
  r:\textsf{rcuItr}\, \rho' \, \N' \, , n:\textsf{rcuFresh} \, \N''\rrbracket_{M,tid} * \{m\}\rfloor)  \subseteq \\
  \lfloor \llbracket \Gamma \,,p:\textsf{rcuItr}\, \rho \, \N([f \rightharpoonup r \setminus  n]) \, , n:\textsf{rcuItr}\, \rho' \, \N'' \, ,r:\unlinked \rrbracket  * \mathcal{R}(\{m\})\rfloor
\end{align*}
 \end{lemma}
 \begin{proof}
 We assume
\begin{gather}\label{ahu1f}
  \begin{aligned}
    (\sigma, O, U, T,F) \, \in &  \llbracket \Gamma,\,
 p:\textsf{rcuItr}\, \rho \, \N \, ,
  r:\textsf{rcuItr}\, \rho' \, \N' \, , n:\textsf{rcuFresh} \, \N'' \rrbracket_{M,tid} * \{m\}
    \end{aligned} \\
\textsf{WellFormed}(\sigma,O,U,T,F)
\label{ahu2f}
\end{gather}
From assumptions in the type rule of \textsc{T-LinkF} we assume that
\begin{gather}
\textsf{FV}(\Gamma) \cap \{p,r,n\}  =\emptyset 
  \label{ahu3f} \\
\rho.f  = \rho' \text{ and } \N(f) = r
    \label{ahu4f} \\
\N' = \N''
\label{ahu5f} \\
\begin{aligned}
\forall_{x \in \Gamma, \N''', \rho'',f',y} \ldotp (x:\textsf{rcuItr}\,\rho''\,\N'''([f'\rightharpoonup y])) \implies (\neg\mathsf{MayAlias}(\rho'',\{\rho,\rho'\}) \land (y\neq o  ))  
\label{ahu6f}
  \end{aligned}
\end{gather}
We split the composition in  \ref{ahu1f} as 
\begin{gather} \label{ahu11f}
  \begin{aligned}
    (\sigma_1, O_{1}, U_{1}, T_{1} ,F_1) \in & \llbracket \Gamma,\,
 p:\textsf{rcuItr}\, \rho \, \N \, ,
  r:\textsf{rcuItr}\, \rho' \, \N' \, , n:\textsf{rcuFresh} \, \N'' \rrbracket_{M,tid} \end{aligned}\\
\label{ahu12f}
(\sigma_2, O_{2}, U_{2}, T_{2},F_2) = m
\\
\label{ahu13f}
O_{1} \bullet_{O} O_{2} = O
\\
\label{ahusigf}
\sigma_1 \bullet_s \sigma_2 = \sigma \\
\label{ahu14f}
U_{1} \cup U_{2} = U
\\
\label{ahu15f}
T_{1} \cup T_{2} = T
\\
\label{ahufff}
F_1 \uplus F_2 = F
\\
\label{ahu16f}
\textsf{WellFormed}(\sigma_1,O_{1},U_{1},T_{1},F_1)
\\
\label{ahu17f}
\textsf{WellFormed}(\sigma_2,O_{2},U_{2},T_{2},F_2)
\end{gather}
We must show $\exists_{\sigma'_1, \sigma'_2, O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2}, F'_1, F'_2}$ such that
\begin{gather}\label{phu5f}
\begin{aligned}
(\sigma_1',O'_{1},U'_{1}, T'_{1},F'_1)  \in \llbracket p:\textsf{rcuItr}\, \rho \, \N \, , n:\textsf{rcuItr}\, \rho' \, \N'' \, , r:\unlinked\, ,  \Gamma \rrbracket_{M,tid}
\end{aligned}
\\
\label{phuNf}
\N(f)=n 
\\
\label{phu6f}
(\sigma_2',O'_{2},U'_{2}, T'_{2}, F'_2) \in \mathcal{R}(\{m\})
\\
\label{phu7f}
O'_{1} \bullet_{O} O'_{2} = O'
\\
\label{ahusigf'}
\sigma'_1 \bullet_s \sigma'_2 = \sigma' \\
\label{phu8f}
U'_{1} \cup U'_{2} = U'
\\
\label{phu9f}
T'_{1} \cup T'_{2} = T'
\\
\label{phufff}
F'_1 \uplus F'_2 = F'
\\
\label{phu10f}
\textsf{WellFormed}(\sigma_1',O'_{1},U'_{1},T'_{1},F'_1) \\
\label{phu11f}
\textsf{WellFormed}(\sigma_2',O'_{2},U'_{2},T'_{2},F'_2)
\end{gather}
We also know from operational semantics that the machine state has changed as
\begin{gather}\label{ahusf}
\sigma_1' =  \sigma_1[h(s(p,tid),f ) \mapsto s(n,tid) ]
\end{gather}
\ref{phuNf} is determined directly from operational semantics.

We know that changes in observation map are
\begin{gather}\label{ahus1f}
O'_1 =  O_1(s(r,tid))[\textsf{iterator}\;tid \mapsto \textsf{unlinked}]
\end{gather}
and
\begin{gather}\label{ahus2f}
O'_1 =  O_1(s(n,tid))[\textsf{fresh} \mapsto \textsf{iterator}\,tid]
\end{gather}

\ref{ahus3f} follows from \ref{ahu1f}
\begin{gather}\label{ahus3f}
  T_1 = \{tid\} \text{ and } tid = \sigma.l
\end{gather}
Let $T'_1$ be $T_1$, $F'_1$ be $F_1$ and $\sigma'_1$ be determined by operational semantics. The undefined map need not change so we can pick $U'_1$ as $U_1$. Assuming \ref{ahu11f} and choices on maps makes $(\sigma_1',O'_{1},U'_{1}, T'_{1})$ in denotation
\[\llbracket p:\textsf{rcuItr}\, \rho \, \N(f \rightharpoonup r \setminus n) \, , n:\textsf{rcuItr}\, \rho' \, \N'' \, , r:\unlinked\, ,  \Gamma \rrbracket_{M,tid}\]

In the rest of the proof, we prove \ref{phu10f}, \ref{phu11f} and show the composition of $(\sigma'_1, O'_1, U'_1,T'_1)$ and  $(\sigma'_2, O'_2, U'_2,T'_2)$. To prove \ref{phu10f}, we need to show that each of the memory axioms in Section \ref{sec:memaxioms} holds for the state $(\sigma',O'_1,U_1',T_1')$.

\begin{case}\label{unqrf} - \textbf{UNQR} 
Let $o_p$ be $\sigma.s(p,tid)$, $o_r$ be $\sigma.s(r,tid)$ and $o_n$ be $\sigma.s(n,tid)$. 
  \ref{ahus3f} and \ref{ahus4f} follow from framing assumption(\ref{ahu3f}-\ref{ahu6f}), denotations of the precondition(\ref{ahu11f}), \ref{ahu16}.\textbf{FR} and \ref{ahu16f}.\textbf{UNQR}
  \begin{gather}\label{ahusbf}
    \rho \neq \rho.f \neq \forall_{\N'([f_i \rightharpoonup x_i])}\ldotp \rho.f.f_i
  \end{gather}
and   
  \begin{gather}\label{ahus4f}
    o_p \neq o_r \neq o_n \neq o_i \text{  where  } o_i=h(o_r,f_i)
  \end{gather}
where $o_p$,  $o_r$ are  $\sigma.h^{*}(\sigma.rt,\rho)$, $\sigma.h^{*}(\sigma.rt,\rho.f)$ respectively and they(heap locations in \ref{ahus4f} and paths in \ref{ahusbf}) are unique(From \ref{ahu16f}.\textbf{FR}, we assume that there exists no field alias/path alias to heap location freshly allocated $o_n$). 

We must prove 
\begin{gather}\label{phuc1f}
    \rho \neq \rho.f \neq \rho.f.f_i \iff \sigma'.h^{*}(\sigma.rt,\rho) \neq \sigma'.h^{*}(\sigma.rt, \rho.f) )  \neq \sigma'.h^{*}(\sigma.rt, \rho.f.f_i) )
\end{gather}

We know from operational semantics that root has not changed so
\[\sigma.rt = \sigma'.rt\]

From denotations (\ref{phu5f}) we know that all heap locations reached by following $\rho$ and $\rho.f$ are observed as $\textsf{iteartor}\,tid$ including the final reached heap locations($\textsf{iterator}\,tid \in O'_1(\sigma'.h^{*}(\sigma.rt,\rho))$, $\textsf{iterator}\,tid \in O'_1(\sigma'.h^{*}(\sigma.rt,\rho.f))$ and $\textsf{iterator}\,tid \in O'_1(\sigma'.h^{*}(\sigma.rt,\rho.f.f_i))$). The preservation of uniqueness follows from \ref{ahus1f}, \ref{ahus2f}, \ref{ahusf} and \ref{ahu16f}.\textbf{FR}.

from which we conclude \ref{ahus5f} and \ref{ahus6f}
  \begin{gather}\label{ahus5f}
    \rho \neq \rho.f \neq \rho.f.f_i
  \end{gather}
    \begin{gather}\label{ahus6f}
    o_p \neq o_n \neq o_r 
  \end{gather}
from which \ref{phuc1f} follows.
\end{case}
\begin{case} - \textbf{OW} By \ref{ahu16f}.\textbf{OW}, \ref{ahusf}, \ref{ahus1f} and \ref{ahus2f}.
\end{case}
\begin{case} - \textbf{RWOW} By \ref{ahu16f}.\textbf{RWOW}, \ref{ahusf}, \ref{ahus1f} and \ref{ahus2f}
\end{case}
\begin{case} - \textbf{AWRT} Trivial.
\end{case}
\begin{case} - \textbf{IFL}  By \ref{ahu16f}.\textbf{WULK}, \ref{ahus1f}, \ref{ahus2f} choice of $F'_1$ and operational semantics.
\end{case}
\begin{case} - \textbf{FLR} By choice of $F'_1$ and \ref{ahu16f}. 
\end{case}
\begin{case} - \textbf{FPI} By \ref{phu5f}.
\end{case}
\begin{case} - \textbf{WULK} Determined by operational semantics By \ref{ahu16f}.\textbf{WULK}, \ref{ahus1f}, \ref{ahus2f} and operational semantics.
\end{case}
\begin{case} - \textbf{WF} and \textbf{FR} Trivial.
\end{case}
\begin{case} - \textbf{HD} 
\end{case}
\begin{case} - \textbf{WNR} By \ref{ahus3f} and operational semantics.
\end{case}
\begin{case} - \textbf{RINFL} Determined by operational semantics(\ref{ahusf}) and \ref{ahu16f}.\textbf{RINFL}.
\end{case}
\begin{case} - \textbf{ULKR} We must prove 
  \begin{gather}\label{phuc2f}
\begin{aligned}
\forall_{o',f'} \ldotp \sigma'.h(o',f') = o_r \implies &\textsf{unlinked} \in O'_1(o') \\
 & \textsf{freeable} \in O'_1(o')
                \end{aligned}
\end{gather}
which follows from \ref{phu5f}, \ref{ahu16f}.\textbf{OW} and determined by operational semantics(\ref{ahusf}), \ref{ahus1f}, \ref{ahus2f}.  If $o'$ were observed as \textsf{iterator} then that would conflict with \ref{phu10f}.\textbf{UNQR}.
\end{case}
\begin{case} - \textbf{UNQRT} By \ref{ahu16f}.\textbf{UNQRT}, \ref{ahus1f}, \ref{ahus2f} and \ref{ahusf}.
\end{case}

To prove \ref{phu6f}, we need to show  interference relation
\[(\sigma, O_2, U_2, T_2,F_2) \mathcal{R} (\sigma', O'_2, U'_2, T'_2,F'_2)  \]
which by definition means that we must show 
\begin{gather}\label{phu17f}
  \sigma_2.l  \in  T_2 \rightarrow (\sigma_2.h =\sigma'_2.h \land \sigma_2.l=\sigma'_2.l)\\
  \label{phu18f}
  l\in T_2\rightarrow F_2=F_2'\\
  \label{phu20f}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma_2.h) \\
  \label{phu21f}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma'_2.h) \\
  \label{phu22f}
  O_2 = O_2' \land U_2 = U_2' \land T_2 = T_2' \land \sigma_2.R = \sigma'_2.R \land \sigma_2.rt = \sigma'_2.rt \\
  \label{phu23f}
  \forall x, t \in T_2 \ldotp \sigma_2.s(x,t) = \sigma'_2.s(x,t) \\
    \label{phufrt1}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h) \\
  \label{phufrt2}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h') 
\end{gather}
To prove all relations (\ref{phu17f}-\ref{phu23f}) we assume \ref{ahus3f} which is to assume $T_2$ as subset of reader threads. Let $\sigma'_2$ be $\sigma_2$, $F'_2$ be $F_2$. $O_2$ need not change so we pick $O'_2$  as $O_2$. Since $T_2$ is subset of reader threads, we pick $T_2$ as  $T'_2$. By assuming \ref{ahu17f}  we show \ref{phu11f}. \ref{phu20f} and \ref{phu21f} follow trivially. \ref{phu23f} follows from choice of $\sigma'_2$,  \ref{ahusf} and \ref{ahus3f}.

\ref{phu17f} and \ref{phu18f} follow from \ref{ahus3f} and choice of $F_2'$. \ref{phu22f}, \ref{phufrt1} and \ref{phufrt2} are determined by  choice of $\sigma'_2$, operational semantics and choices made on maps related to the assertions.

To prove \ref{phu7f} consider two cases: $O'_1 \cap O'_2 = \emptyset$ and $O'_1 \cap O'_2 \neq \emptyset$. The first case is trivial. The second case is where we consider \ref{intersect1} and \ref{intersect2}
\begin{gather}\label{intersect1}
\textsf{iterator}\,tid \in O'_2(o_r)
\end{gather}
From \ref{ahus1f} we know that
\[\textsf{unliked} \in O'_1(o_r)\]
Both together with \ref{ahu13f} and \ref{phu5f} proves \ref{phu7f}.

For case \ref{intersect2}
\begin{gather}\label{intersect2}
\textsf{fresh} \in O_2(o_n)
\end{gather}
From \ref{ahus2f} we know that
\[\textsf{iterator}\, tid \in O'_1(o_n)\]
Both together with \ref{ahu13f} and \ref{phu5f} proves \ref{phu7f}.

To show \ref{ahusigf'} we consider two cases: $\sigma'_1 \cap \sigma'_2 = \emptyset$ and $\sigma'_1 \cap \sigma'_2 \neq \emptyset$. First is trivial. Second follows from \ref{phu10f}.\textbf{OW}-\textbf{HD} and \ref{phu11f}.\textbf{OW}-\textbf{HD}. \ref{phu8f}, \ref{phufff} and \ref{phu9f} are trivial by choices on related maps and semantics of the composition operators for these maps. All compositions shown  let us to derive conclusion for $(\sigma'_1, O'_1, U'_1, T'_1,F'_1) \bullet (\sigma'_2, O'_2, U'_2, T'_2,F'_2) $.
 \end{proof}
 \begin{lemma}[\textsc{ReadStack}]
   \label{lemma:readstack}
\begin{align*}
  \llbracket z:=x \rrbracket (\lfloor \llbracket \Gamma\,, z:\_ \, ,\rcuitrT{x}{G}{k}{k+1}{\_} \rrbracket_{M,tid} * \{m\}\rfloor)  \subseteq \\
                                                              \lfloor \llbracket \Gamma\,, \rcuitrT{x}{G}{k}{k+1}{\_}\, , \rcuitrT{z}{G}{k}{k+1}{\_}  \rrbracket  * \mathcal{R}(\{m\})\rfloor
\end{align*}
 \end{lemma}
 \begin{proof}
We assume
\begin{gather}\label{ahu1sr}
  \begin{aligned}
    (\sigma, O, U, T,F) \, \in &  \llbracket \Gamma\,, z:\_ \, ,\rcuitrT{x}{G}{k}{k+1}{\_} \rrbracket_{M,tid} * \{m\}
    \end{aligned} \\
\textsf{WellFormed}(\sigma,O,U,T,F)
\label{ahu2sr}
\end{gather}
From the assumption in the type rule of \textsc{T-ReadS} we assume that
\begin{gather}
\textsf{FV}(\Gamma) \cap \{z\}  =\emptyset 
  \label{ahu3sr}
\end{gather}
We split the composition in  \ref{ahu1sr} as 
\begin{gather} \label{ahu11sr}
  \begin{aligned}
    (\sigma, O_{1}, U_{1}, T_{1} ,F_1) \in & \llbracket  \Gamma\,, z:\_ \, ,\rcuitrT{x}{G}{k}{k+1}{\_} \rrbracket_{M,tid} \end{aligned}\\
\label{ahu12sr}
(\sigma, O_{2}, U_{2}, T_{2}, F_2) = m
\\
\label{ahusigsr}
\sigma_1 \bullet \sigma_2 = \sigma
\\
\label{ahu13sr}
O_{1} \bullet_{O} O_{2} = O
\\
\label{ahu14sr}
U_{1} \cup U_{2} = U
\\
\label{ahu15sr}
T_{1} \cup T_{2} = T
\\
\label{ahusrf}
F_1 \uplus F_2 = F
\\
\label{ahu16sr}
\textsf{WellFormed}(\sigma_1,O_{1},U_{1},T_{1},F_1)
\\
\label{ahu17sr}
\textsf{WellFormed}(\sigma_2,O_{2},U_{2},T_{2},F_2)
\end{gather}
We must show $\exists_{\sigma'_1, \sigma'_2, O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2}, F'_1 , F'_2}$ such that
\begin{gather}\label{phu5sr}
\begin{aligned}
(\sigma',O'_{1},U'_{1}, T'_{1}, F'_1)  \in \llbracket \Gamma\,, \rcuitrT{x}{G}{k}{k+1}{\_}\, , \rcuitrT{z}{G}{k}{k+1}{\_}  \rrbracket_{M,tid}
\end{aligned}\\
\label{phu6sr}
(\sigma',O'_{2},U'_{2}, T'_{2}, F'_2) \in \mathcal{R}(\{m\})
\\
\label{ahusigsr'}
\sigma'_1 \bullet \sigma'_2 = \sigma'
\\
\label{phu7sr}
O'_{1} \bullet_{O} O'_{2} = O'
\\
\label{phu8sr}
U'_{1} \cup U'_{2} = U'
\\
\label{phu9sr}
T'_{1} \cup T'_{2} = T'
\\
\label{phusrf}
F'_1 \uplus F'_2 = F'
\\
\label{phu10sr}
\textsf{WellFormed}(\sigma_1',O'_{1},U'_{1},T'_{1},F'_1) \\
\label{phu11sr}
\textsf{WellFormed}(\sigma_2',O'_{2},U'_{2},T'_{2}, F'_2)
\end{gather}

Let $s(x,tid)$ be $o_x$. We also know from operational semantics that the machine state has changed as 
\begin{gather}\label{ahussr}
\sigma' =  \sigma[s(z,tid) \mapsto o_x ]
\end{gather}

We know that there exists no change in the observation of heap locations
\begin{gather}\label{ahus1sr}
O'_1 =  O_1
\end{gather}

\ref{ahus2sr} follows from \ref{ahu1sr}
\begin{gather}\label{ahus2sr}
  T_1 = \{tid\} \text{ and } tid = \sigma.l
\end{gather}

$\sigma'_1$ is determined by operational semantics. The undefined map, $T_1$ and free list need not change so we can pick $U'_1$ as $U_1$, $T'_1$  as $T_1$ and $F'_1$ as $F_1$. Assuming \ref{ahu11sr} and choices on maps makes $(\sigma_1',O'_{1},U'_{1}, T'_{1})$ in denotation
\[\llbracket \Gamma\,, \rcuitrT{x}{G}{k}{k+1}{\_}\, , \rcuitrT{z}{G}{k}{k+1}{\_}  \rrbracket_{M,tid}\]

In the rest of the proof, we prove \ref{phu10sr}, \ref{phu11sr} and show the composition of $(\sigma'_1, O'_1, U'_1,T'_1,F'_1)$ and  $(\sigma'_2, O'_2, U'_2,T'_2,F'_2)$. \ref{phu10sr} follows from \ref{ahu16sr} trivially.

To prove \ref{phu6sr}, we need to show interference relation
\[(\sigma, O_2, U_2, T_2,F_2) \mathcal{R} (\sigma', O'_2, U'_2, T'_2,F'_2)  \]
which by definition means that we must show 
\begin{gather}\label{phu17sr}
  \sigma_2.l  \in  T_2 \rightarrow (\sigma_2.h =\sigma'_2.h \land \sigma_2.l=\sigma'_2.l)\\
  \label{phu18sr}
  l\in T_2\rightarrow F_2=F_2'\\
  \label{phu20sr}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma_2.h) \\
  \label{phu21sr}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma'_2.h) \\
  \label{phu22sr}
  O_2 = O_2' \land U_2 = U_2' \land T_2 = T_2'\land \sigma_2.R_2 = \sigma_2'.R_2 \land \sigma_2.rt = \sigma'_2.rt \\
  \label{phu23sr}
  \forall x, t \in T_2 \ldotp \sigma_2.s(x,t) = \sigma'_2.s(x,t)  \\
    \label{phusrrt1}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h) \\
  \label{phusrrt2}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h') 
\end{gather}
To prove all relations (\ref{phu17sr}-\ref{phu23sr}) we assume \ref{ahus2sr} which is to assume $T_2$ as subset of reader threads. Let $\sigma'_2$ be $\sigma_2$. $O_2$ need not change so we pick $O'_2$  as $O_2$. We pick $F'_2$ as $F_2$. Since $T_2$ is subset of reader threads, we pick $T_2$ as  $T'_2$. By assuming \ref{ahu17sr}  we show \ref{phu11sr}. \ref{phu20sr}, \ref{phu21sr}, \ref{phusrrt1} and \ref{phusrrt2} follow trivially. \ref{phu23sr} follows from choice of $\sigma'_2$ and \ref{ahussr}(determined by operational semantics).

 \ref{phu17sr} and \ref{phu18sr} follow from \ref{ahus2sr} and choice of $F_2'$. \ref{phu22sr}, \ref{phusrrt1} and \ref{phusrrt2} are determined by choice of $\sigma'_2$, operational semantics and choices made on maps related to the assertions.

\ref{phu7sr}-\ref{phusrf} are  trivial by choices on related maps and semantics of the composition operators for these maps. \ref{ahusigsr'} follows trivially from \ref{ahusigsr}. All compositions shown  let us to derive conclusion for $(\sigma'_1, O'_1, U'_1, T'_1,F'_1) \bullet (\sigma'_2, O'_2, U'_2, T'_2,F'_2) $ trivial.
 \end{proof}
  \begin{lemma}[\textsc{ReadHeap}]
   \label{lemma:readheap}
\begin{align*}
  \llbracket z:=x.f \rrbracket (\lfloor \llbracket \Gamma\, , z:\_ \, ,  x:\textsf{rcuItr} \, \rho \, \N  \rrbracket_{M,tid} * \{m\}\rfloor)  \subseteq \\
                                                              \lfloor \llbracket \Gamma\,,  x:\textsf{rcuItr} \, \rho \, \N[f\mapsto z]\, ,z:\textsf{rcuItr} \, \rho' \, \N_{\emptyset}  \rrbracket  * \mathcal{R}(\{m\})\rfloor
\end{align*}
 \end{lemma}
 \begin{proof}
We assume
\begin{gather}\label{ahu1hr}
  \begin{aligned}
    (\sigma, O, U, T,F) \, \in &  \llbracket \Gamma\,, z:\textsf{rcuItr}\,\_ \, ,\rcuitrT{x}{G}{k}{k+1}{\_} \rrbracket_{M,tid} * \{m\}
    \end{aligned} \\
\textsf{WellFormed}(\sigma,O,U,T,F)
\label{ahu2hr}
\end{gather}
From the assumption in the type rule of \textsc{T-ReadH} we assume that
\begin{gather}
\textsf{FV}(\Gamma) \cap \{z\}  =\emptyset 
\label{ahu3hr} \\
\rho.f = \rho' 
\label{ahu4hr} \\
\end{gather}
We split the composition in  \ref{ahu1hr} as 
\begin{gather} \label{ahu11hr}
  \begin{aligned}
    (\sigma_1, O_{1}, U_{1}, T_{1} ,F_1) \in & \llbracket  \Gamma\,, z:\textsf{rcuItr}\,\_ \, ,\rcuitrT{x}{G}{k}{k+1}{\_} \rrbracket_{M,tid} \end{aligned}\\
\label{ahu12hr}
(\sigma_2, O_{2}, U_{2}, T_{2},F_2) = m
\\
\label{ahusighr}
\sigma_1 \bullet \sigma_2 = \sigma
\\
\label{ahu13hr}
O_{1} \bullet_{O} O_{2} = O
\\
\label{ahu14hr}
U_{1} \cup U_{2} = U
\\
\label{ahu15hr}
T_{1} \cup T_{2} = T
\\
\label{ahuhrf}
F_1 \uplus F_2 = F
\\
\label{ahu16hr}
\textsf{WellFormed}(\sigma_1,O_{1},U_{1},T_{1})
\\
\label{ahu17hr}
\textsf{WellFormed}(\sigma_2,O_{2},U_{2},T_{2})
\end{gather}
We must show $\exists_{\sigma'_1, \sigma'_2, O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2},F'_1 ,F'_2}$ such that
\begin{gather}\label{phu5hr}
\begin{aligned}
(\sigma',O'_{1},U'_{1}, T'_{1},F_1)  \in \llbracket \Gamma\,,  x:\textsf{rcuItr} \, \rho \, \N[f\mapsto z]\, ,z:\textsf{rcuItr} \, \rho' \, \N_{\emptyset} \rrbracket_{M,tid}
\end{aligned}
\\
\label{phuNhr}
\N(f) = z
\\
\label{phu6hr}
(\sigma',O'_{2},U'_{2}, T'_{2}, F_2) \in \mathcal{R}(\{m\})
\\
\label{ahusighr'}
\sigma'_1 \bullet \sigma'_2 = \sigma'
\\
\label{phu7hr}
O'_{1} \bullet_{O} O'_{2} = O'
\\
\label{phu8hr}
U'_{1} \cup U'_{2} = U'
\\
\label{phu9hr}
T'_{1} \cup T'_{2} = T'
\\
\label{phuhrf}
F'_1 \uplus F'_2 = F'
\\
\label{phu10hr}
\textsf{WellFormed}(\sigma_1',O'_{1},U'_{1},T'_{1}) \\
\label{phu11hr}
\textsf{WellFormed}(\sigma_2',O'_{2},U'_{2},T'_{2})
\end{gather}

Let $h(s(z,tid),f)$ be $o_z$. We also know from operational semantics that the machine state has changed as
\begin{gather}\label{ahushr}
\sigma_1' =  \sigma_1[s(x,tid) \mapsto o_z]
\end{gather}
\ref{phuNhr} is determined directly from operational semantics.

We know that there exists no change in the observation of heap locations
\begin{gather}\label{ahus1hr}
O'_1 =  O_1
\end{gather}

\ref{ahus2hr} follows from \ref{ahu1hr}
\begin{gather}\label{ahus2hr}
  T_1 = \{tid\} \text{ and } tid = \sigma.l
\end{gather}

$\sigma'_1$ is determined by operational semantics. The undefined map, free list and $T_1$ need not change so we can pick $U'_1$ as $U_1$, $F'_1$ as $F_1$ and $T'_1$ and $T_1$. Assuming \ref{ahu11hr} and choices on maps makes $(\sigma_1',O'_{1},U'_{1}, T'_{1})$ in denotation
\[ \llbracket \Gamma\,,  x:\textsf{rcuItr} \, \rho \, \N[f\mapsto z]\, ,z:\textsf{rcuItr} \, \rho' \, \N_{\emptyset} \rrbracket_{M,tid}\]

In the rest of the proof, we prove \ref{phu10hr}, \ref{phu11hr} and show the composition of $(\sigma'_1, O'_1, U'_1,T'_1)$ and  $(\sigma'_2, O'_2, U'_2,T'_2)$. 

To prove \ref{phu6hr}, we need to show that each of the memory axioms in Section \ref{sec:memaxioms} holds for the state $(\sigma',O'_1,U_1',T_1')$.
\begin{case} - \textbf{UNQR} By \ref{ahushr}, \ref{ahu16hr}.\textbf{UNQR} and $\sigma.rt = \sigma.rt'$.
\end{case}
\begin{case} - \textbf{OW} By \ref{ahushr}, \ref{ahus1hr} and \ref{ahu16hr}.\textbf{OW}
\end{case}
\begin{case} - \textbf{RWOW} By \ref{ahushr}, \ref{ahus1hr} and \ref{ahu16hr}.\textbf{RWOW}
\end{case}
\begin{case} - \textbf{AWRT} Trivial. 
\end{case}
\begin{case} - \textbf{IFL}  By \ref{phu5hr}, \ref{ahu16hr}.\textbf{WULK}, \ref{ahus1hr}, choice of $F'_1$ and operational semantics.
\end{case}
\begin{case} - \textbf{FLR}  By operational semantics(\ref{ahushr}), choice for $F'_1$ and \ref{ahu16hr}. 
\end{case}
\begin{case} - \textbf{WULK}  By \ref{ahu16hr}.\textbf{WULK}, \ref{ahus1hr} and operational semantics($\sigma.l = \sigma.l'$).
\end{case}
\begin{case} - \textbf{WF}, \textbf{FNR}, \textbf{FPI} and \textbf{FR} Trivial.
\end{case}
\begin{case} - \textbf{HD} 
\end{case}
\begin{case} - \textbf{WNR} By \ref{ahus2hr} and operational semantics($\sigma.l = \sigma.l'$).
\end{case}
\begin{case} - \textbf{RINFL} By operational semantics(\ref{ahushr}) bounding threads have not changed. We choose $F'_1$ as $F_1$. These two together with \ref{ahu16hr} shows \textbf{RINFL}. 
\end{case}
\begin{case} - \textbf{ULKR} Trivial. 
\end{case}
\begin{case} - \textbf{UNQRT}  By \ref{ahu16hr}.\textbf{UNQRT}, \ref{ahus1hr} and \ref{ahushr}.
\end{case}

To prove \ref{phu6hr}, we need to show interference relation
\[(\sigma, O_2, U_2, T_2,F_2) \mathcal{R} (\sigma', O'_2, U'_2, T'_2,F'_2)  \]
which by definition means that we must show 
\begin{gather}\label{phu17hr}
  \sigma_2.l  \in  T_2 \rightarrow (\sigma_2.h =\sigma'_2.h \land \sigma_2.l=\sigma'_2.l)\\
  \label{phu18hr}
  l\in T_2\rightarrow F_2=F_2'\\
  \label{phu20hr}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma_2.h) \\
  \label{phu21hr}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma'_2.h) \\
  \label{phu22hr}
  O_2 = O_2' \land U_2 = U_2' \land T_2 = T_2'\land \sigma_2.R_2 = \sigma_2'.R_2 \land \sigma_2.rt = \sigma'_2.rt \\
  \label{phu23hr}
  \forall x, t \in T_2 \ldotp \sigma_2.s(x,t) = \sigma'_2.s(x,t) \\
 \label{phuhrrt1}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h) \\
  \label{phuhrrt2}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h') 
\end{gather}
To prove all relations (\ref{phu17hr}-\ref{phu23hr}) we assume \ref{ahus2hr} which is to assume $T_2$ as subset of reader threads.  Let $\sigma'_2$ be $\sigma_2$ and $F'_2$ be $F_2$. $O_2$ need not change so we pick $O'_2$  as $O_2$. Since $T_2$ is subset of reader threads, we pick $T_2$ as  $T'_2$. By assuming \ref{ahu17hr}  we show \ref{phu11hr}. \ref{phu20hr} and \ref{phu21hr} follows trivially. \ref{phu23hr} follows from choice of $\sigma'_2$ and \ref{ahushr}(determined by operational semantics).

\ref{phu17hr} and \ref{phu18hr} follow from \ref{ahus2hr} and choice of $F_2'$.\ref{phu22hr}, \ref{phuhrrt1} and \ref{phuhrrt2} are determined by choice of $\sigma'_2$, operational semantics and choices made on maps related to the assertions. 

\ref{phu7hr}-\ref{phuhrf} are trivial by choices on related maps and semantics of the composition operators for these maps. \ref{ahusighr'} follows trivially from \ref{ahusighr}. All compositions shown let us to derive conclusion for $(\sigma'_1, O'_1, U'_1, T'_1,F'_1) \bullet (\sigma'_2, O'_2, U'_2, T'_2,F'_2) $.
 \end{proof}
 \begin{lemma}[\textsc{WriteFreshField}]
   \label{lemma:writef}
   \begin{align*}
  \llbracket p.f := z \rrbracket (\lfloor \llbracket \Gamma, p:\textsf{rcuFresh}\,\N'_{f,\emptyset},\; x:\textsf{rcuItr}\;\; \rho \;\; \N \rrbracket_{M,tid} * \{m\}\rfloor)  \subseteq \\
  \lfloor \llbracket \Gamma \,, \rcunf{p}{f}{z} \, , x:\textsf{rcuItr}\, \rho \, \N([f\rightharpoonup z]) \rrbracket  * \mathcal{R}(\{m\})\rfloor
\end{align*}
 \end{lemma}
 \begin{proof}
 We assume
\begin{gather}\label{ahu1wf}
  \begin{aligned}
    (\sigma, O, U, T,F) \, \in &  \llbracket \Gamma, p:\textsf{rcuFresh}\,\N'_{f,\emptyset},\; x:\textsf{rcuItr}\;\; \rho \;\; \N \rrbracket_{M,tid} * \{m\}
    \end{aligned} \\
\textsf{WellFormed}(\sigma,O,U,T,F)
\label{ahu2wf}
\end{gather}
From the assumption in the type rule of \textsc{T-WriteFH} we assume that
\begin{gather}
z:\textsf{rcuItr}\,\rho.f\,\_ \text{ and } \N(f) = z \text{ and } f \notin dom(\N')
\label{ahu4wf} 
\end{gather}

We split the composition in  \ref{ahu1wf} as 
\begin{gather} \label{ahu11wf}
  \begin{aligned}
    (\sigma, O_{1}, U_{1}, T_{1},F_1 ) \in & \llbracket  \Gamma, p:\textsf{rcuFresh}\,\N'_{f,\emptyset},\; x:\textsf{rcuItr}\;\; \rho \;\; \N \rrbracket_{M,tid} \end{aligned}\\
\label{ahu12wf}
(\sigma, O_{2}, U_{2}, T_{2}, F_2) = m
\\
\label{ahusigwf}
\sigma_1 \bullet \sigma_2 = \sigma
\\
\label{ahu13wf}
O_{1} \bullet_{O} O_{2} = O
\\
\label{ahu14wf}
U_{1} \cup U_{2} = U
\\
\label{ahu15wf}
T_{1} \cup T_{2} = T
\\
\label{ahuwff}
F_1 \uplus F_2 = F
\\
\label{ahu16wf}
\textsf{WellFormed}(\sigma_1,O_{1},U_{1},T_{1},F_1)
\\
\label{ahu17wf}
\textsf{WellFormed}(\sigma_2,O_{2},U_{2},T_{2}, F_2)
\end{gather}
We must show $\exists_{\sigma'_1, \sigma'_2, O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2},F'_1 , F'_2}$ such that
\begin{gather}\label{phu5wf}
\begin{aligned}
(\sigma',O'_{1},U'_{1}, T'_{1},F'_1)  \in \llbracket \Gamma \,, \rcunf{p}{f}{z} \, , x:\textsf{rcuItr}\, \rho \, \N([f\rightharpoonup z]) \rrbracket_{M,tid}
\end{aligned}
\\
\label{phuNwf}
\N(f) = z \land \N'(f) = z
\\
\label{phu6wf}
(\sigma',O'_{2},U'_{2}, T'_{2},F'_2) \in \mathcal{R}(\{m\})
\\
\label{ahusigwf'}
\sigma'_1 \bullet \sigma'_2 = \sigma'
\\
\label{phu7wf}
O'_{1} \bullet_{O} O'_{2} = O'
\\
\label{phu8wf}
U'_{1} \cup U'_{2} = U'
\\
\label{phu9wf}
T'_{1} \cup T'_{2} = T'
\\
\label{phuwff}
F'_1 \uplus F'_2 = F'
\\
\label{phu10wf}
\textsf{WellFormed}(\sigma_1',O'_{1},U'_{1},T'_{1}, F'_1) \\
\label{phu11wf}
\textsf{WellFormed}(\sigma_2',O'_{2},U'_{2},T'_{2}, F'_2)
\end{gather}

We also know from operational semantics that the machine state has changed as
\begin{gather}\label{ahuswf}
\sigma' =  \sigma[h(s(p,tid),f) \mapsto s(z,tid)]
\end{gather}

There exists no change in the observation of heap locations
\begin{gather}\label{ahus1wf}
O'_1 =  O_1
\end{gather}

\ref{ahus2wf} follows from \ref{ahu1wf}
\begin{gather}\label{ahus2wf}
  T_1 = \{tid\} \text{ and } tid = \sigma.l
\end{gather}

$\sigma'_1$ is determined by operational semantics. The undefined map, free list, $T_1$ need not change so we can pick $U'_1$ as $U_1$, $T'_1$ as $T_1$ and $F'_1$ as $F_1$. Assuming \ref{ahu11wf} and choices on maps makes $(\sigma_1',O'_{1},U'_{1}, T'_{1})$ in denotation
\[\llbracket \Gamma \,, \rcunf{p}{f}{z} \, , x:\textsf{rcuItr}\, \rho \, \N([f\rightharpoonup z]) \rrbracket_{M,tid}\]

In the rest of the proof, we prove \ref{phu10wf} and \ref{phu11wf} and show the composition of $(\sigma'_1, O'_1, U'_1,T'_1,F'_1)$ and  $(\sigma'_2, O'_2, U'_2,T'_2,F'_2)$. To prove \ref{phu10wf}, we need to show that each of the memory axioms in Section \ref{sec:memaxioms} holds for the state $(\sigma',O'_1,U_1',T_1',F'_1)$.
\begin{case} - \textbf{UNQR} By \ref{ahu16wf}.\textbf{UNQR}, \ref{phu10wf}.\textbf{FR}(proved) and $\sigma.rt = \sigma.rt'$.
\end{case}
\begin{case} - \textbf{OW} By \ref{ahuswf},\ref{ahus1wf} and \ref{ahu16wf}.\textbf{OW}
\end{case}
\begin{case} - \textbf{RWOW} By \ref{ahuswf}, \ref{ahus1wf} and \ref{ahu16wf}.\textbf{RWOW}
\end{case}
\begin{case} - \textbf{AWRT} Trivial. 
\end{case}
\begin{case} - \textbf{IFL}  By \ref{ahu16wf}.\textbf{WULK}, \ref{ahus1wf}, choice of $F'_1$ and operational semantics.
\end{case}
\begin{case} - \textbf{FLR}  By operational semantics(\ref{ahuswf}), choice of $F'_1$ and \ref{ahu16wf}. 
\end{case}
\begin{case} - \textbf{WULK}  By \ref{ahu16wf}.\textbf{WULK}, \ref{ahus1wf} and operational semantics($\sigma.l = \sigma.l'$).
\end{case}
\begin{case} - \textbf{WF} By \ref{ahu16wf}.\textbf{WF}, \ref{ahus2wf}, \ref{ahus1wf} and operational semantics(\ref{ahuswf}).
\end{case}
\begin{case} - \textbf{FR} By \ref{ahu16wf}.\textbf{FR}, \ref{ahus2wf}, \ref{ahus1wf} and operational semantics(\ref{ahuswf}).
\end{case}
\begin{case} - \textbf{FNR} By \ref{ahu16wf}.\textbf{FNR}, \ref{ahus2wf}, \ref{ahus1wf} and operational semantics(\ref{ahuswf}).
\end{case}
\begin{case} - \textbf{FPI} By \ref{ahu16wf}.\textbf{FPI}, \ref{ahu11wf} and \ref{ahu4wf}
\end{case} 
\begin{case} - \textbf{HD} 
\end{case}
\begin{case} - \textbf{WNR} By \ref{ahus2wf} and operational semantics($\sigma.l = \sigma.l'$).
\end{case}
\begin{case} - \textbf{RINFL} By operational semantics(\ref{ahuswf} - bounding threads have not changed), choice of $F'_1$ and \ref{ahu16wf}. 
\end{case}
\begin{case} - \textbf{ULKR} Trivial. 
\end{case}
\begin{case} - \textbf{UNQRT} By \ref{ahu16wf}.\textbf{UNQRT}, \ref{ahus1wf} and \ref{ahuswf}.
\end{case}

To prove \ref{phu6wf}, we need to show interference relation
\[(\sigma, O_2, U_2, T_2,F_2) \mathcal{R} (\sigma', O'_2, U'_2, T'_2,F'_2)  \]
which by definition means that we must show 
\begin{gather}\label{phu17wf}
  \sigma_2.l  \in  T_2 \rightarrow (\sigma_2.h =\sigma'_2.h \land \sigma_2.l=\sigma'_2.l)\\
  \label{phu18wf}
  l\in T_2\rightarrow F_2=F_2'\\
  \label{phu20wf}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma_2.h) \\
  \label{phu21wf}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma'_2.h) \\
  \label{phu22wf}
  O_2 = O_2' \land U_2 = U_2' \land T_2 = T_2'\land \sigma_2.R = \sigma'_2.R \land \sigma_2.rt = \sigma'_2.rt \\
  \label{phu23wf}
  \forall x, t \in T_2 \ldotp \sigma_2.s(x,t) = \sigma'_2.s(x,t)\\
  \label{phuwfrt1}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h) \\
  \label{phuwfrt2}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h') 
\end{gather}
To prove all relations (\ref{phu17wf}-\ref{phu23wf}) we assume \ref{ahus2wf} which is to assume $T_2$ as subset of reader threads and \ref{ahu17wf}. Let $\sigma'_2$ be $\sigma_2$ and $F'_2$ be $F_2$. $O_2$ need not change so we pick $O'_2$  as $O_2$. Since $T_2$ is subset of reader threads, we pick $T_2$ as  $T'_2$. By assuming \ref{ahu17wf}  we show \ref{phu11wf}. \ref{phu20wf} and \ref{phu21wf} follows trivially. \ref{phu23wf} follows from choice of $\sigma'_2$ and \ref{ahuswf}(determined by operational semantics).


\ref{phu17wf} and \ref{phu18wf} follow from \ref{ahus2wf} and choice of $F_2'$.  \ref{phu22wf} are determined by operational semantics, choice of $\sigma'_2$ and choices made on maps related to the assertions.

\ref{phu8wf}-\ref{phuwff} are trivial by choices on related maps and semantics of the composition operators for these maps. \ref{phuwfrt1} and \ref{phuwfrt2} follow from choice of $\sigma'_2$.

$O'_1 \bullet O'_2 $ follows from \ref{ahu13wf}, \ref{ahus1wf} and choice of $O_2$. 

We assume $\sigma_1.h \bullet \sigma_2.h$. We know from \ref{ahu4wf} that $f \notin dom(\N')$. From \ref{phu5wf}, \ref{phu10wf}-\ref{phu11wf}.\textbf{FNR}, \ref{phu10wf}-\ref{phu11wf}.\textbf{RITR} and \ref{phu10wf}-\ref{phu11wf}.\textbf{WNR} we show $\sigma'_1.h \bullet \sigma'_2.h$ (with choices for other maps in the machine state we show \ref{ahusighr'}). All compositions shown  let us to derive conclusion for $(\sigma'_1, O'_1, U'_1, T'_1) \bullet (\sigma'_2, O'_2, U'_2, T'_2) $.
 \end{proof}
\begin{lemma}[\textsc{Sycn}]
   \label{lemma:syncstop}
   \begin{align*}
  \llbracket  \textsf{SyncStart};\textsf{SyncStop} \rrbracket (\lfloor \llbracket \Gamma  \rrbracket_{M,tid} * \{m\}\rfloor)  \subseteq \\
                                                              \lfloor \llbracket \Gamma[\overline{x:\textsf{freeable}/x:\textsf{unlinked}}] \rrbracket  * \mathcal{R}(\{m\})\rfloor
\end{align*}
 \end{lemma}
 \begin{proof}
 We assume
\begin{gather}\label{ahu1st}
  \begin{aligned}
    (\sigma, O, U, T,F) \, \in &  \llbracket \Gamma \rrbracket_{M,tid} * \{m\}
    \end{aligned} \\
\textsf{WellFormed}(\sigma,O,U,T,F)
\label{ahu2st}
\end{gather}

We split the composition in  \ref{ahu1st} as 
\begin{gather} \label{ahu11st}
  \begin{aligned}
    (\sigma, O_{1}, U_{1}, T_{1},F_1 ) \in & \llbracket  \Gamma \rrbracket_{M,tid} \end{aligned}\\
  \label{ahu12st}
(\sigma, O_{2}, U_{2}, T_{2},F_2) = m
\\
\label{ahusigst}
\sigma_1 \bullet \sigma_2 = \sigma
\\
\label{ahu13st}
O_{1} \bullet_{O} O_{2} = O
\\
\label{ahu14st}
U_{1} \cup U_{2} = U
\\
\label{ahu15st}
T_{1} \cup T_{2} = T
\\
\label{ahustF}
F_1 \uplus F_2 = F
\\
\label{ahu16st}
\textsf{WellFormed}(\sigma,O_{1},U_{1},T_{1},F_1)
\\
\label{ahu17st}
\textsf{WellFormed}(\sigma,O_{2},U_{2},T_{2},F_2)
\end{gather}
We must show $\exists_{\sigma'_1, \sigma'_2, O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2}},F'_1 ,F'_2$ such that
\begin{gather}\label{phu5st}
\begin{aligned}
(\sigma',O'_{1},U'_{1}, T'_{1},F'_1)  \in \llbracket \Gamma[\overline{x:\textsf{freeable}/x:\textsf{unlinked}}] \rrbracket_{M,tid}
\end{aligned}\\
\label{phu6st}
(\sigma',O'_{2},U'_{2}, T'_{2}, F'_2) \in \mathcal{R}(\{m\})
\\
\label{ahusigst'}
\sigma'_1 \bullet \sigma'_2 = \sigma'
\\
\label{phu7st}
O'_{1} \bullet_{O} O'_{2} = O'
\\
\label{phu8st}
U'_{1} \cup U'_{2} = U'
\\
\label{phu9st}
T'_{1} \cup T'_{2} = T'
\\
\\
\label{phustF}
F'_1 \uplus F'_2 = F'
\\
\label{phu10st}
\textsf{WellFormed}(\sigma',O'_{1},U'_{1},T'_{1},F'_1) \\
\label{phu11st}
\textsf{WellFormed}(\sigma',O'_{2},U'_{2},T'_{2}, F'_2)
\end{gather}
We also know from operational semantics that \lstinline|SyncStart| changes
\begin{gather}\label{ahuB}
  \sigma_1'.B = \sigma_1.B[\emptyset \mapsto R]
\end{gather}
Then \lstinline|SyncStop| changes it to $\emptyset$ so there exists no change in $B$ after \lstinline|SyncStart|;\lstinline|SyncStop|. So there is no change in machine state.
\begin{gather}\label{ahusst}
\sigma_1' =  \sigma_1
\end{gather}

There exists no change in the observation of heap locations
\begin{gather}\label{ahus1st}
  O'_1 =  O_1(\forall_{x \in \Gamma} \ldotp s(x,tid))[\textsf{unlinked} \mapsto \textsf{freeable}]
\end{gather}
and we pick free list to be
\begin{gather}\label{ahusF}
 F'_1 = F_1(\forall_{x:\textsf{unlinked} \in \Gamma, T\subseteq R} \ldotp s(x,tid)[ T \mapsto \{\emptyset\} ])
\end{gather}

\ref{ahus2st} follows from \ref{ahu1st}
\begin{gather}\label{ahus2st}
  T_1 = \{tid\} \text{ and } tid = \sigma.l
\end{gather}

Let $T'_1$ be $T_1$ and $\sigma'_1$(not changed) be determined by operational semantics. The undefined map need not change so we can pick $U'_1$ as $U_1$. Assuming \ref{ahu11st} and choices on maps makes $(\sigma_1',O'_{1},U'_{1}, T'_{1},F'_1)$ in denotation
\[ \llbracket \Gamma[\overline{x:\textsf{freeable}/x:\textsf{unlinked}}] \rrbracket_{M,tid}\]

In the rest of the proof, we prove \ref{phu10st} and \ref{phu11st} and show the composition of $(\sigma'_1, O'_1, U'_1,T'_1,F'_1)$ and $(\sigma'_2, O'_2, U'_2,T'_2,F'_2)$. To prove \ref{phu10st}, we need to show that each of the memory axioms in Section \ref{sec:memaxioms} holds for the state $(\sigma',O'_1,U_1',T_1',F'_1)$ which is trivial by assuming \ref{ahu16st}. We also know \ref{phu5st}(as we showed the support of state to the denotation).

To prove \ref{phu6st}, we need to show interference relation
\[(\sigma, O_2, U_2, T_2,F_2) \mathcal{R} (\sigma', O'_2, U'_2, T'_2,F_2')  \]
which by definition means that we must show 
\begin{gather}\label{phu17st}
  \sigma_2.l  \in  T_2 \rightarrow (\sigma_2.h =\sigma'_2.h \land \sigma_2.l=\sigma'_2.l)\\
  \label{phu18st}
  l\in T_2\rightarrow F_2=F_2'\\
  \label{phu20st}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma_2.h) \\
  \label{phu21st}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma'_2.h) \\
  \label{phu22st}
  O_2 = O_2' \land U_2 = U_2' \land T_2 = T_2'\land \sigma_2.R = \sigma'_2.R \land \sigma_2.rt = \sigma'_2.rt \\
  \label{phu23st}
  \forall x, t \in T_2 \ldotp \sigma_2.s(x,t) = \sigma'_2.s(x,t)\\
    \label{phustrt1}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h) \\
  \label{phustrt2}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h') 
\end{gather}
To prove all relations (\ref{phu17st}-\ref{phu23st}) we assume \ref{ahus2st} which is to assume $T_2$ as subset of reader threads and \ref{ahu17st}. Let $\sigma'_2$ be $\sigma_2$. $O_2$ need not change so we pick $O'_2$  as $O_2$. Since $T_2$ is subset of reader threads, we pick $T_2$ as  $T'_2$. By assuming \ref{ahu17st} we show \ref{phu11st}. \ref{phu20st} and \ref{phu21st} follows trivially. \ref{phu23st} follows from choice of $\sigma'_2$ and \ref{ahusst}(determined by operational semantics). 

\ref{phu17st} and \ref{phu18st} follow from \ref{ahus2st}. \ref{phu22st} are determined by choice of $\sigma'_2$ and operational semantics and choices made on maps related to the assertions.

\ref{phu8st}-\ref{phustF} follow from \ref{ahu13st}-\ref{ahustF} trivially by choices on maps of logical state and semantics of composition operators. \ref{ahusigst'} follow from \ref{ahusigst}, \ref{ahusst}-\ref{ahus2st} and choice of $\sigma'_2$. All compositions shown let us to derive conclusion for $(\sigma'_1, O'_1, U'_1, T'_1,F'_1) \bullet (\sigma'_2, O'_2, U'_2, T'_2,F'_2) $ .
 \end{proof}
 
  \begin{lemma}[\textsc{Alloc}]
   \label{lemma:alloc}
\begin{align*}
  \llbracket x:=new \rrbracket (\lfloor \llbracket \Gamma\, , x:\textsf{undef} \, \rrbracket_{M,tid} * \{m\}\rfloor)  \subseteq \\
                                                              \lfloor \llbracket \Gamma\,,  x:\textsf{rcuFresh} \, \N_{\emptyset}  \rrbracket  * \mathcal{R}(\{m\})\rfloor
\end{align*}
 \end{lemma}
 \begin{proof}
We assume
\begin{gather}\label{ahu1alc}
  \begin{aligned}
    (\sigma, O, U, T,F) \, \in &  \llbracket \Gamma\, , x:\textsf{undef} \, \rrbracket_{M,tid} * \{m\}\rfloor) 
    \end{aligned} \\
\textsf{WellFormed}(\sigma,O,U,T,F)
\label{ahu2alc}
\end{gather}

We split the composition in  \ref{ahu1alc} as 
\begin{gather} \label{ahu11alc}
  \begin{aligned}
    (\sigma, O_{1}, U_{1}, T_{1},F_1 ) \in & \llbracket \Gamma\, , x:\textsf{undef} \, \rrbracket_{M,tid}  \end{aligned}\\
  \label{ahu12alc}
(\sigma, O_{2}, U_{2}, T_{2},F_2) = m
  \\
  \label{ahualcsig}
  \sigma_1 \bullet \sigma_2 = \sigma
  \\
\label{ahu13alc}
O_{1} \bullet_{O} O_{2} = O
\\
\label{ahu14alc}
U_{1} \cup U_{2} = U
\\
\label{ahu15alc}
T_{1} \cup T_{2} = T
\\
\label{ahualcF}
F_1 \uplus F_2 = F
\\
\label{ahu16alc}
\textsf{WellFormed}(\sigma,O_{1},U_{1},T_{1},F_1)
\\
\label{ahu17alc}
\textsf{WellFormed}(\sigma,O_{2},U_{2},T_{2},F_2)
\end{gather}
We must show $\exists_{O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2},F'_1, F'_2}$ such that
\begin{gather}\label{phu5alc}
\begin{aligned}
(\sigma',O'_{1},U'_{1}, T'_{1},F'_1)  \in \llbracket \Gamma\,,  x:\textsf{rcuFresh} \, \N_{\emptyset}  \rrbracket 
\end{aligned}\\
\label{phu6alc}
(\sigma',O'_{2},U'_{2}, T'_{2},F'_2) \in \mathcal{R}(\{m\})
\\
\label{phualcsig}
\sigma'_1 \bullet \sigma'_2 = \sigma'
\\
\label{phu7alc}
O'_{1} \bullet_{O} O'_{2} = O'
\\
\label{phu8alc}
U'_{1} \cup U'_{2} = U'
\\
\label{phu9alc}
T'_{1} \cup T'_{2} = T'
\\
\label{phualcF}
F'_1 \uplus F'_2 = F'
\\
\label{phu10alc}
\textsf{WellFormed}(\sigma',O'_{1},U'_{1},T'_{1}) \\
\label{phu11alc}
\textsf{WellFormed}(\sigma',O'_{2},U'_{2},T'_{2})
\end{gather}

From operational semantics we know that $s(y,tid)$ is $\ell$. We also know from operational semantics that the machine state has changed as
\begin{gather}\label{ahusalc}
\sigma' =  \sigma[h(\ell) \mapsto \textsf{nullmap} ]
\end{gather}

There exists no change in the observation of heap locations
\begin{gather}\label{ahus1alc}
  O'_1 =  O_1(\ell)[\textsf{undef}\mapsto \textsf{fresh}]
\end{gather}

\ref{ahus2alc} follows from \ref{ahu1alc}
\begin{gather}\label{ahus2alc}
  T_1 = \{tid\} \text{ and } tid = \sigma.l
\end{gather}

Let $T'_1$ to be $T_1$. Undefined map and free list need not change so we can pick $U'_1$ as $U_1$ and $F'_1$ as $F_1$ and show(\ref{phu5alc}) that $(\sigma',O'_1,U_1',T_1',F'_1)$ is in denotation of
\[\llbracket \Gamma\,,  x:\textsf{rcuFresh} \, \N_{\emptyset}  \rrbracket \]

In the rest of the proof, we prove \ref{phu10alc}, \ref{phu11alc} and $(\sigma'_1, O'_1, U'_1,T'_1,F'_1)$ and  $(\sigma'_2, O'_2, U'_2,T'_2,F'_2)$. To prove \ref{phu10alc}, we need to show that each of the memory axioms in Section \ref{sec:memaxioms} holds for the state $(\sigma',O'_1,U_1',T_1',F'_1)$.

\begin{case} - \textbf{UNQR} Determined by \ref{phu5alc} and operational semantics($\ell$ is fresh-unique).
\end{case}
\begin{case} - \textbf{RWOW}, \textbf{OW} By \ref{phu5alc}
\end{case}
\begin{case} - \textbf{AWRT} Determined by operational semantics($\ell$ is fresh-unique). 
\end{case}
\begin{case} - \textbf{IFL}, \textbf{ULKR}, \textbf{WULK}, \textbf{RINFL}, \textbf{UNQRT} Trivial.
\end{case}
\begin{case} - \textbf{FLR} determined by operational semantics and \ref{phu5alc}.
\end{case}
\begin{case} - \textbf{WF} By \ref{ahus2alc}, \ref{phu5alc} and \ref{ahus1alc}. 
\end{case}
\begin{case} - \textbf{FR} Determined by operational semantics($\ell$ is fresh-unique).
\end{case}
\begin{case} - \textbf{FNR} By \ref{phu5alc} and operational semantics($\ell$ is fresh-unique).
\end{case}
\begin{case} - \textbf{FPI} By \ref{phu5alc} and $\N_{f,\emptyset}$.
\end{case} 
\begin{case} - \textbf{HD} 
\end{case}
\begin{case} - \textbf{WNR} By \ref{ahus2alc}.
\end{case}

To prove \ref{phu6alc}, we need to show interference relation
\[(\sigma, O_2, U_2, T_2,F_2) \mathcal{R} (\sigma', O'_2, U'_2, T'_2,F'_2)  \]
which by definition means that we must show 
\begin{gather}\label{phu17alc}
  \sigma_2.l  \in  T_2 \rightarrow (\sigma_2.h =\sigma'_2.h \land \sigma_2.l=\sigma'_2.l)\\
  \label{phu18alc}
  l\in T_2\rightarrow F_2=F_2'\\
  \label{phu20alc}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma_2.h) \\
  \label{phu21alc}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma'_2.h) \\
  \label{phu22alc}
  O_2 = O_2' \land U_2 = U_2' \land T_2 = T_2'\land \sigma_2.R = \sigma'_2.R \land \sigma_2.rt = \sigma'_2.rt \\
  \label{phu23alc}
  \forall x, t \in T \ldotp \sigma_2.s(x,t) = \sigma'_2.s(x,t) \\
    \label{phualcrt1}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h) \\
  \label{phualcrt2}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h') 
\end{gather}
To prove all relations (\ref{phu17alc}-\ref{phualcrt2}) we assume \ref{ahus2alc} which is to assume $T_2$ as subset of reader threads and \ref{ahu17alc}. Let $\sigma'_2$ be $\sigma_2$. $F_2$ and $O_2$ need not change so we pick $O'_2$  as $O_2$ and $F'_2$ as $F_2$. Since $T_2$ is subset of reader threads, we pick $T_2$ as  $T'_2$. By assuming \ref{ahu17alc} and choices on maps we show \ref{phu11alc}. \ref{phu20alc} and \ref{phu21alc} follow trivially. \ref{phu23alc} follows from choice of $\sigma'_2$ and \ref{ahusalc}(determined by operational semantics). \ref{phu7alc}-\ref{phualcF} follow from \ref{ahu13alc}-\ref{ahualcF}, semantics of compositions operators and choices made for maps of the logical state.

\ref{phu17alc} and \ref{phu18alc} follow from \ref{ahus2alc} and choice on $F'_2$. \ref{phu22alc} are determined by operational semantics, operational semantics and choices made on maps related to the assertion.

$\sigma'_1.h \cap \sigma'_2.h = \emptyset$ is determined by operational semantics($\ell$ is unique and fresh). So, \ref{phualcsig} follows from \ref{ahualcsig} and choice of $\sigma'_2$. All compositions shown let us to derive conclusion for  $(\sigma'_1, O'_1, U'_1, T'_1,F'_1) \bullet (\sigma'_2, O'_2, U'_2, T'_2,F'_2) $.
 \end{proof}
 \begin{lemma}[\textsc{Free}]
   \label{lemma:free}
\begin{align*}
  \llbracket Free(x) \rrbracket (\lfloor \llbracket x:\textsf{freeable} \rrbracket_{M,tid} * \{m\}\rfloor)  \subseteq \\
                                                              \lfloor \llbracket x:\textsf{undef} \rrbracket  * \mathcal{R}(\{m\})\rfloor
\end{align*}
 \end{lemma}
 \begin{proof}
We assume
\begin{gather}\label{ahu1free}
  \begin{aligned}
    (\sigma, O, U, T,F) \, \in &  \llbracket x:\textsf{freeable} \, \rrbracket_{M,tid} * \{m\}\rfloor) 
    \end{aligned} \\
\textsf{WellFormed}(\sigma,O,U,T,F)
\label{ahu2free}
\end{gather}

We split the composition in  \ref{ahu1free} as 
\begin{gather} \label{ahu11free}
  \begin{aligned}
    (\sigma, O_{1}, U_{1}, T_{1},F_1 ) \in & \llbracket  x:\textsf{freeable}  \rrbracket_{M,tid}  \end{aligned}\\
  \label{ahu12free}
(\sigma, O_{2}, U_{2}, T_{2},F_2) = m
  \\
  \label{ahufreesig}
  \sigma_1 \bullet \sigma_2 = \sigma
  \\
\label{ahu13free}
O_{1} \bullet_{O} O_{2} = O
\\
\label{ahu14free}U
_{1} \cup U_{2} = U
\\
\label{ahu15free}
T_{1} \cup T_{2} = T
\\
\label{ahufreeF}
F_1 \uplus F_2 = F
\\
\label{ahu16free}
\textsf{WellFormed}(\sigma,O_{1},U_{1},T_{1},F_1)
\\
\label{ahu17free}
\textsf{WellFormed}(\sigma,O_{2},U_{2},T_{2},F_2)
\end{gather}
We must show $\exists_{O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2},F'_1, F'_2}$ such that
\begin{gather}\label{phu5free}
\begin{aligned}
(\sigma',O'_{1},U'_{1}, T'_{1},F'_1)  \in \llbracket  x:\textsf{undef}  \rrbracket 
\end{aligned}\\
\label{phu6free}
(\sigma',O'_{2},U'_{2}, T'_{2},F'_2) \in \mathcal{R}(\{m\})
\\
\label{phufreesig}
\sigma'_1 \bullet \sigma'_2 = \sigma'
\\
\label{phu7free}
O'_{1} \bullet_{O} O'_{2} = O'
\\
\label{phu8free}
U'_{1} \cup U'_{2} = U'
\\
\label{phu9free}
T'_{1} \cup T'_{2} = T'
\\
\label{phufreeF}
F'_1 \uplus F'_2 = F'
\\
\label{phu10free}
\textsf{WellFormed}(\sigma',O'_{1},U'_{1},T'_{1}) \\
\label{phu11free}
\textsf{WellFormed}(\sigma',O'_{2},U'_{2},T'_{2})
\end{gather}

From operational semantics we know that
\begin{gather}\label{ahusfree}
\sigma_1' =  \sigma_1
\end{gather}

There exists no change in the observation of heap locations
\begin{gather}\label{ahus1free}
  O'_1 =  O_1(s(x,tid))[\textsf{freeable}\mapsto \textsf{undef}]
\end{gather}

\begin{gather}\label{ahus3free}
  F'_1 = F_1 \setminus \{s(x,tid)\mapsto \{\emptyset\}\}
  \end{gather}

\begin{gather}\label{ahus4free}
  U'_1 = U_1 \cup \{(x,tid)\}
  \end{gather}

\ref{ahus2free} follows from \ref{ahu1free}
\begin{gather}\label{ahus2free}
  T_1 = \{tid\} \text{ and } tid = \sigma.l
\end{gather}

Let $T'_1$ to be $T_1$. All \ref{ahusfree}-\ref{ahus4free} show(\ref{phu5free}) that $(\sigma',O'_1,U_1',T_1',F'_1)$ is in denotation of  
\[\llbracket  x:\textsf{undef}  \rrbracket \]

In the rest of the proof, we prove \ref{phu10free}, \ref{phu11free}\ref{phu10}, \ref{phu11} and show the composition of $(\sigma'_1, O'_1, U'_1,T'_1,F'_1)$ and  $(\sigma'_2, O'_2, U'_2,T'_2,F'_2)$.. To prove \ref{phu10free}, we need to show that each of the memory axioms in Section \ref{sec:memaxioms} holds for the state $(\sigma',O'_1,U_1',T_1',F'_1)$ and it it trivial by \ref{ahusfree}-\ref{ahus4free} and \ref{phu5free}.

To prove \ref{phu6free}, we need to show interference relation
\[(\sigma, O_2, U_2, T_2,F_2) \mathcal{R} (\sigma', O'_2, U'_2, T'_2,F'_2)  \]
which by definition means that we must show 
\begin{gather}\label{phu17free}
  \sigma_2.l  \in  T_2 \rightarrow (\sigma_2.h =\sigma'_2.h \land \sigma_2.l=\sigma'_2.l)\\
  \label{phu18free}
  l\in T_2\rightarrow F_2=F_2'\\
  \label{phu20free}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma_2.h) \\
  \label{phu21free}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma'_2.h) \\
  \label{phu22free}
  O_2 = O_2' \land U_2 = U_2' \land T_2 = T_2'\land \sigma_2.R = \sigma'_2.R \land \sigma_2.rt = \sigma'_2.rt \\
  \label{phu23free}
  \forall x, t \in T \ldotp \sigma_2.s(x,t) = \sigma'_2.s(x,t) \\
    \label{phufreert1}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h) \\
  \label{phufreert2}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h') 
\end{gather}

To prove all relations (\ref{phu17free}-\ref{phufreert2}) we assume \ref{ahus2free} which is to assume $T_2$ as subset of reader threads and \ref{ahu17alc}. Let $\sigma'_2$ be $\sigma_2$. $F_2$ and $O_2$ need not change so we pick $O'_2$  as $O_2$ and $F'_2$ as $F_2$. Since $T_2$ is subset of reader threads, we pick $T_2$ as  $T'_2$. By assuming \ref{ahu17alc} and choices on maps we show \ref{phu11free}. \ref{phu20free} and \ref{phu21free} follow trivially. \ref{phu23free} follows from choice of $\sigma'_2$ and \ref{ahusfree}(determined by operational semantics). \ref{phu7free}-\ref{phufreeF} follow from \ref{ahu14free}-\ref{ahufreeF}, semantics of composition operators and choices on related maps.

\ref{phu17free} and \ref{phu18free} follow from \ref{ahus2free} and choice on $F'_2$. \ref{phu22free} are determined by operational semantics, choice of $\sigma'_2$ and choices made on maps related to the assertion.

Composition for heap for case $\sigma'_1.h \cap \sigma'_2.h = \emptyset$ is trivial. $\sigma'_1.h \cap \sigma'_2.h \neq \emptyset$ is determined by semantics of heap composition operator $\bullet_h$( $v$ has precedence over \textsf{undef}) and this makes showing \ref{phu7free} straightforward. Since other machine components do not change(determined by operational semantics), \ref{phufreesig} follows from \ref{ahufreesig}, \ref{ahusfree} and choice of $\sigma'_2$. All compositions shown let us to derive conclusion for  $(\sigma'_1, O'_1, U'_1, T'_1,F'_1) \bullet (\sigma'_2, O'_2, U'_2, T'_2,F'_2) $.
 \end{proof} 
  \begin{lemma}[\textsc{RReadStack}]
   \label{lemma:rreadstack}
\begin{align*}
  \llbracket z:=x \rrbracket (\lfloor \llbracket \Gamma\,, z:\textsf{rcuItr}\, , x:\textsf{rcuItr} \rrbracket_{R,tid} * \{m\}\rfloor)  \subseteq \\
                                                              \lfloor \llbracket \Gamma\,, x:\textsf{rcuItr} \, , z:\textsf{rcuItr}  \rrbracket  * \mathcal{R}(\{m\})\rfloor
\end{align*}
 \end{lemma}
  \begin{proof}
  We assume
\begin{gather}\label{ahu1srr}
  \begin{aligned}
    (\sigma, O, U, T,F) \, \in & \llbracket \Gamma\,, \Gamma\,, z:\textsf{rcuItr}\, , x:\textsf{rcuItr}   \rrbracket_{R,tid} * \{m\}
    \end{aligned} \\
\textsf{WellFormed}(\sigma,O,U,T,F)
\label{ahu2srr}
\end{gather}

We split the composition in  \ref{ahu1srr} as 
\begin{gather} \label{ahu11srr}
  \begin{aligned}
    (\sigma_1, O_{1}, U_{1}, T_{1},F_1 ) \in & \llbracket \Gamma\,, \Gamma\,, z:\textsf{rcuItr}\, , x:\textsf{rcuItr} \rrbracket_{R,tid} \end{aligned}\\
  \label{ahu12srr}
(\sigma, O_{2}, U_{2}, T_{2},F_2) = m
\\
\label{ahu13srr}
O_{1} \bullet_{O} O_{2} = O
\\
\label{ahusigsrr}
\sigma_1 \bullet \sigma_2 = \sigma
\\
\label{ahu14srr}
U_{1} \cup U_{2} = U
\\
\label{ahu15srr}
T_{1} \cup T_{2} = T
\\
\label{ahusrrf}
F_1 \uplus F_2 = F
\\
\label{ahu16srr}
\textsf{WellFormed}(\sigma,O_{1},U_{1},T_{1},F_1)
\\
\label{ahu17srr}
\textsf{WellFormed}(\sigma,O_{2},U_{2},T_{2},F_2)
\end{gather}
We must show $\exists_{O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2},F'_1,F'_2}$ such that
\begin{gather}\label{phu5srr}
\begin{aligned}
(\sigma',O'_{1},U'_{1}, T'_{1},F'_1)  \in\llbracket \Gamma\,, x:\textsf{rcuItr} \, , z:\textsf{rcuItr}   \rrbracket_{R,tid}
\end{aligned}\\
\label{phu6srr}
(\sigma',O'_{2},U'_{2}, T'_{2},F'_2) \in \mathcal{R}(\{m\})
\\
\label{phu7srr}
O'_{1} \bullet_{O} O'_{2} = O'
\\
\label{ahusigsrr'}
\sigma'_1 \bullet \sigma'_2 = \sigma'
\\
\label{phu8srr}
U'_{1} \cup U'_{2} = U'
\\
\label{phu9srr}
T'_{1} \cup T'_{2} = T'
\\
\label{phusrrf}
F'_1 \uplus F'_2 = F'
\\
\label{phu10srr}
\textsf{WellFormed}(\sigma',O'_{1},U'_{1},T'_{1},F'_1) \\
\label{phu11srr}
\textsf{WellFormed}(\sigma',O'_{2},U'_{2},T'_{2},F'_2)
\end{gather}

We also know from operational semantics that the machine state has changed as
\begin{gather}\label{ahussrr}
\sigma_1' =  \sigma_1
\end{gather}

There exists no change in the observation of heap locations
\begin{gather}\label{ahus1srr}
  O'_1 =  O_1
\end{gather}

\ref{ahus2srr} follows from \ref{ahu1srr}
\begin{gather}\label{ahus2srr}
  T_1 \subseteq R
\end{gather}

Let $T'_1$ be $T_1$ and $\sigma'_1$ be determined by operational semantics as $\sigma_1$. The undefined map and free list need not change so we can pick $U'_1$ as $U_1$ and $F'_1$ as $F_1$. Assuming \ref{ahu11srr} and choices on maps makes $(\sigma_1',O'_{1},U'_{1}, T'_{1},F'_1)$ in denotation
\[ \llbracket \Gamma\,, x:\textsf{rcuItr} \, , z:\textsf{rcuItr}  \rrbracket_{R,tid}\]

In the rest of the proof, we prove \ref{phu10srr}, \ref{phu11srr}\ref{phu10}, \ref{phu11} and show the composition of $(\sigma'_1, O'_1, U'_1,T'_1,F'_1)$ and  $(\sigma'_2, O'_2, U'_2,T'_2,F'_2)$. To prove \ref{phu10srr}, we need to show that each of the memory axioms in Section \ref{sec:memaxioms} holds for the state $(\sigma',O'_1,U_1',T_1',F'_1)$ which is trivial by assuming \ref{ahu16srr} and knowing \ref{ahus2srr}, \ref{ahus1srr} and components of the state determined by operational semantics.

To prove \ref{phu11srr}, we need to show that \textsf{WellFormed}ness is preserved under interference relation
\[(\sigma, O_2, U_2, T_2,F_2) \mathcal{R} (\sigma', O'_2, U'_2, T'_2,F'_2)  \]
which by definition means that we must show 
\begin{gather}\label{phu17srr}
  \sigma_2.l  \in  T_2 \rightarrow (\sigma_2.h =\sigma'_2.h \land \sigma_2.l=\sigma'_2.l)\\
  \label{phu18srr}
  l\in T_2\rightarrow F_2=F_2'\\
  \label{phu20srr}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma_2.h) \\
  \label{phu21srr}
  \forall tid,o\ldotp\textsf{iterator} \, tid \in O_2(o) \rightarrow o \in dom(\sigma'_2.h) \\
  \label{phu22srr}
  O_2 = O_2' \land U_2 = U_2' \land T_2 = T_2'\land \sigma_2.B = \sigma'_2.B \land \sigma_2.rt = \sigma'_2.rt \\
  \label{phu23srr}
  \forall x, t \in T_2 \ldotp \sigma_2.s(x,t) = \sigma'_2.s(x,t) \\
    \label{phusrrrt1}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h) \\
  \label{phusrrrt2}
  \forall tid,o\ldotp\textsf{root} \, tid \in O(o) \rightarrow o \in dom(h') 
\end{gather}
$\sigma_2$, $O_2$, $U_2$ and $T_2$ need not change so that we choose $\sigma'_2$ to be $\sigma'_2$, $O'_2$ to be $O_2$, $U'_2$ to $U_2$ and $T'_2$ to be $T_2$. Let $F'_2$ be $F_2$. These choices make proving \ref{phu17srr}-\ref{phusrrrt2} trivial and  \ref{phu7srr}-\ref{phu9srr} follow from assumptions \ref{ahu13srr}-\ref{ahusrrf}, choices made for related maps and semantics of composition operations. All compositions shown let us derive conclusion for $(\sigma'_1,O'_1,U'_1,T'_1,F'_1) \bullet (\sigma'_2,O'_2,U'_2,T'_2,F'_2)$.
  \end{proof}

    \begin{lemma}[\textsc{RReadHeap}]
   \label{lemma:rreadheap}
\begin{align*}
  \llbracket z:=x.f \rrbracket (\lfloor \llbracket \Gamma\, , z:\textsf{rcuItr}\, ,  x:\textsf{rcuItr} \rrbracket_{R,tid} * \{m\}\rfloor)  \subseteq \\
                                                              \lfloor \llbracket \Gamma\,,  x:\textsf{rcuItr} \, ,z:\textsf{rcuItr}   \rrbracket  * \mathcal{R}(\{m\})\rfloor
\end{align*}
 \end{lemma}
    \begin{proof}
        We assume
\begin{gather}\label{ahu1hrr}
  \begin{aligned}
    (\sigma, O, U, T,F) \, \in &  \llbracket \Gamma\, , z:\textsf{rcuItr}\, ,  x:\textsf{rcuItr} \rrbracket_{R,tid} * \{m\}\rfloor)
    \end{aligned} \\
\textsf{WellFormed}(\sigma,O,U,T,F)
\label{ahu2hrr}
\end{gather}

We split the composition in  \ref{ahu1hrr} as 
\begin{gather} \label{ahu11hrr}
  \begin{aligned}
    (\sigma_1, O_{1}, U_{1}, T_{1},F_1 ) \in &  \llbracket \Gamma\, , z:\textsf{rcuItr}\, ,  x:\textsf{rcuItr}  \rrbracket_{R,tid} \end{aligned}\\
  \label{ahu12hrr}
(\sigma_2, O_{2}, U_{2}, T_{2},F_2) = m
  \\
  \label{ahusighrr}
  \sigma_1 \bullet \sigma_2 = \sigma
  \\
\label{ahu13hrr}
O_{1} \bullet_{O} O_{2} = O
\\
\label{ahu14hrr}
U_{1} \cup U_{2} = U
\\
\label{ahu15hrr}
T_{1} \cup T_{2} = T
\\
\label{ahuhrrf}
F_1 \uplus F_2 = F
\\
\label{ahu16hrr}
\textsf{WellFormed}(\sigma_1,O_{1},U_{1},T_{1},F_1)
\\
\label{ahu17hrr}
\textsf{WellFormed}(\sigma_2,O_{2},U_{2},T_{2},F_2)
\end{gather}
We must show  $\exists_{\sigma'_1,\sigma'_2,O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2},F'_1,F'_2}$ such that
\begin{gather}\label{phu5fhrr}
\begin{aligned}
(\sigma_1',O'_{1},U'_{1}, T'_{1},F'_1)  \in   \lfloor \llbracket \Gamma\,,  x:\textsf{rcuItr} \, ,z:\textsf{rcuItr}  \rrbracket  
\end{aligned}\\
\label{phu6hrr}
(\sigma_2',O'_{2},U'_{2}, T'_{2}, F'_2) \in \mathcal{R}(\{m\})
\\
  \label{ahusighrr'}
  \sigma'_1 \bullet \sigma'_2 = \sigma'
\\
\label{phu7hrr}
O'_{1} \bullet_{O} O'_{2} = O'
\\
\label{phu8hrr}
U'_{1} \cup U'_{2} = U'
\\
\label{phu9hrr}
T'_{1} \cup T'_{2} = T'
\\
\label{phu10hrr}
\textsf{WellFormed}(\sigma_1',O'_{1},U'_{1},T'_{1},F'_1) \\
\label{phu11hrr}
\textsf{WellFormed}(\sigma_2',O'_{2},U'_{2},T'_{2},F'_2)
\end{gather}

Let $h(s(x,tid),f)$ be $o_x$. We also know from operational semantics that the machine state has changed as
\begin{gather}\label{ahushrr}
\sigma_1' =  \sigma_1[s(z,tid)\mapsto o_x]
\end{gather}

There exists no change in the observation of heap locations
\begin{gather}\label{ahus1hrr}
  O'_1 =  O_1
\end{gather}

\ref{ahus2hrr} follows from \ref{ahu1hrr}
\begin{gather}\label{ahus2hrr}
  T_1 \subseteq R
\end{gather}
Proof is similar to Lemma \ref{lemma:rreadstack}.
      \end{proof}
\subsection{Soundness Proof of Structural Program Actions}
\label{lem:lemstructural}
In this section, we introduce soundness Theorem \ref{thm:snd} for structural rules of the type system. We consider the cases of the induction on derivation of  $\Gamma \vdash C \dashv \Gamma$ for all type systems,$R,M$.

Although we have proofs for read-side structural rules, we only present proofs for write-side structural type rules in this section as read-side rules are simple versions of write-side rules and proofs for them are trivial and already captured by proofs for write-side structural rools.
\begin{theorem}[Type System Soundness]
  \label{thm:snd}
\[
\forall_{\Gamma,\Gamma',C}\ldotp \Gamma \vdash C \dashv \Gamma' \implies \llbracket \Gamma \vdash C \dashv \Gamma' \rrbracket 
\]
\end{theorem}

\begin{proof}
  Induction on derivation of $\Gamma \vdash_{M} C \dashv \Gamma$.

  \begin{case}-\textbf{M}: consequence where $C$ has the form $\Gamma \vdash_{M} C \dashv \Gamma'''$.
    We know
    \begin{gather}\label{s'l6a1}
      \Gamma' \vdash_{M}  C \dashv \Gamma'' \\
      \label{s'l6a2}
      \Gamma \subt \Gamma'\\
      \label{s'l6a3}
      \Gamma'' \subt \Gamma''' \\
      \label{s'l6a4}
      \{\llbracket \Gamma' \rrbracket_{M,tid} \}C\{\llbracket \Gamma'' \rrbracket_{M,tid} \}
    \end{gather}

    We need to show
    \begin{gather}\label{s'l6p1}
\{ \llbracket \Gamma \rrbracket_{M,tid} \}C\{\llbracket \Gamma''' \rrbracket_{M,tid}\}
    \end{gather}

    The $\subt$ relation translated to entailment relation in Views Logic. The relation is established over the action judgement for identity label/transition
    
From \ref{s'l6a2} and Lemma \ref{lem:cntxsubt-m} we know 
\begin{gather}\label{s'l6a6}
\llbracket \Gamma \rrbracket_{M,tid} \sqsubseteq \llbracket \Gamma' \rrbracket_{M,tid}
\end{gather}


From \ref{s'l6a3} and \ref{lem:cntxsubt-m} we know 
\begin{gather}\label{s'l6a7}
\llbracket \Gamma'' \rrbracket_{M,tid} \sqsubseteq \llbracket \Gamma''' \rrbracket_{M,tid}
\end{gather}

By using \ref{s'l6a6}, \ref{s'l6a7} and \ref{s'l6a4} as antecedentes of Views Logic's consequence rule, we conclude \ref{s'l6p1}.
  \end{case}
  
%%HERE sequence
  \begin{case}-\textbf{M}: where $C$ is sequence statement. $C$ has the form $C_1;C_2$. Our goal is to prove
  \begin{gather}
    \label{sl1p1}
   \{ \llbracket \Gamma \rrbracket_{M,tid} \} \vdash_{M} C_1;C_2 \dashv \{ \llbracket \Gamma'' \rrbracket_{M,tid} \}
 \end{gather}
We know 
  \begin{gather}\label{sl1a1}
    \Gamma \vdash_{M} C_1 \dashv \Gamma' \\
    \label{sl1a2}
    \Gamma' \vdash_{M} C_2 \dashv \Gamma''\\
    \label{sl1a3}
    \{\llbracket \Gamma \rrbracket_{M,tid}\}   C_1  \{ \llbracket \Gamma' \rrbracket_{M,tid}\} \\
    \label{sl1a4}
    \{ \llbracket \Gamma' \rrbracket_{M,tid} \}  C_2  \{\llbracket \Gamma'' \rrbracket_{M,tid}\} 
  \end{gather} 
  
  By using \ref{sl1a3} and \ref{sl1a4} as the antecedents for the Views sequencing rule, we can derive the conclusion for \ref{sl1p1}.
  \end{case}
  
  \begin{case}-\textbf{M}: where $C$ is loop statement. $C$ has the form $while\left(x\right)\{C\}$.

     \begin{gather}\label{sl2a1}
       \Gamma \vdash_{M} C \dashv \Gamma \\
       \label{sl2a2}
       \Gamma(x) = \textsf{bool} \\ 
       \label{sl2a3}
       \{\llbracket \Gamma \rrbracket_{M,tid} \}  C  \{\llbracket \Gamma \rrbracket_{M,tid}\} 
     \end{gather}
    Our goal is to prove
    \begin{gather}\label{sl2p1}
      \{\llbracket \Gamma \rrbracket_{M,tid} \} \left(assume\left(x\right);C\right)^{*};assume(\lnot x) \{\llbracket \Gamma \rrbracket_{M,tid} \}
    \end{gather}
 We prove \ref{sl2p1} by from the consequence rule, based on the proofs of the following \ref{sl2p2} and \ref{sl2p3}
    \begin{gather}\label{sl2p2}
      \{ \llbracket \Gamma \rrbracket_{M,tid} \}\left(assume\left(x\right);C\right)^{*} \{ \llbracket \Gamma \rrbracket_{M,tid} \}
    \end{gather}
    \begin{gather}\label{sl2p3}
      \{ \llbracket \Gamma \rrbracket_{M,tid} \}assume\left(\lnot x\right)\{ \llbracket \Gamma \rrbracket_{M,tid} \}
    \end{gather}
    
   The poof of \ref{sl2p2} follows from Views Logic's proof rule for assume construct by using
      \[\{\llbracket\Gamma \rrbracket_{M,tid}\} assume\left(x\right) \{\llbracket \Gamma \rrbracket_{M,tid} \}\]
      as antecedant. We can use this antecedant together with the antecedent we know from \ref{sl2a3}
      \[\{\llbracket \Gamma \rrbracket_{M,tid} \}C\{\llbracket \Gamma \rrbracket_{M,tid}\}\]
      as antecedents to the Views Logic's proof rule for sequencing. Then we use the antecedent
      \[ \{\llbracket \Gamma \rrbracket_{M,tid} \}assume\left(x\right);C\{\llbracket \Gamma \rrbracket_{M,tid} \}\] to the proof rule for nondeterministic looping.
  
    The proof of \ref{sl2p3} follows from Views Logic's proof rule for assume construct by using the
    \[ \{ \llbracket \Gamma \rrbracket_{M,tid} \}assume\left(\lnot x\right)\{ \llbracket \Gamma \rrbracket_{M,tid} \}\] as the antecedent.
  \end{case}
  \begin{case}-\textbf{M}: where $C$ is a loop statement. $C$ has the form $while(x.f\neq \texttt{null})\{C\}$
    Proof is similar to the one for \textsc{T-Loop1}. 
  \end{case}
  \begin{case}-\textbf{M}: case where $C$ is branch statement. $C$ has the form $if\left(e\right)then\{C_1\}else\{C_2\}$.
      \begin{gather}\label{sl4a1}
       \Gamma, x:\textsf{rcuItr}\;\rho\;\N([f_1 \rightharpoonup z]) \vdash_{M} C_1 \dashv \Gamma' \\
       \label{sl4a2}
       \Gamma, x:\textsf{rcuItr}\;\rho\;\N([f_2 \rightharpoonup z]) \vdash_{M} C_2 \dashv \Gamma' \\
       \label{sl4a4}
       \{\llbracket \Gamma, \,  x:\textsf{rcuItr}\;\rho\;\N([f_1 \rightharpoonup z]) \rrbracket_{M,tid} \}  C_1  \{\llbracket \Gamma' \rrbracket_{M,tid}\}\\
        \label{sl4a5}
       \{\llbracket \Gamma , \, x:\textsf{rcuItr}\;\rho\;\N([f_2 \rightharpoonup z]) \rrbracket_{M,tid} \}  C_2  \{\llbracket \Gamma' \rrbracket_{M,tid}\}
      \end{gather}
      
    Our goal is to prove
    \begin{gather}\label{sl4p1}
      \begin{array}{l}
      \{\llbracket \Gamma,x:\textsf{rcuItr}\;\rho\;\N([f_1 | f_2 \rightharpoonup z]) \rrbracket_{M,tid} \} \\
      y = x.f_1;\left(assume\left(z = y\right);C_1\right)+\left(assume\left(y \neq z\right);C_2 \right)\\
      \{\llbracket \Gamma' \rrbracket_{M,tid} \}
      \end{array}
    \end{gather}
    where the desugared form includes a fresh variable y. We use fresh variables just for desugaring and they are not included in any type context.
    We prove\ref{sl4p1} from the consequence rule  of Views Logic based on the proofs of the following \ref{sl4p2} and \ref{sl4p3}
    \begin{gather}\label{sl4p2}
      \begin{array}{l}
      \{\llbracket\Gamma,   x:\textsf{rcuItr}\;\rho\;\N([f_1 | f_2 \rightharpoonup z])\rrbracket_{M,tid}\} \\
      \left(assume\left(z = y\right);C_1\right)+\left(assume\left(y \neq z\right);C_2 \right) \\
      \{\llbracket \Gamma' \rrbracket_{M,tid}\}
      \end{array}
    \end{gather}
    and
    \begin{gather}\label{sl4p3}\begin{array}{l}
      \{\llbracket \Gamma,   x:\textsf{rcuItr}\;\rho\;\N[f_1 | f_2 \rightharpoonup z] \rrbracket_{M,tid}\} \\
      y = x.f_1\\
      \{\llbracket \Gamma,   x:\textsf{rcuItr}\;\rho\;\N([f_1 | f_2 \rightharpoonup z]) \llbracket_{M,tid} \cap \llbracket x:\textsf{rcuItr}\;\rho\;\N([f_1 \rightharpoonup y]) \rrbracket_{M,tid} \}
      \end{array}
      \end{gather}

    \ref{sl4p3} is trivial from the fact that y is a fresh variable and it is not included in any type context and just used for desugaring.

    We prove \ref{sl4p2} from the branch rule of Views Logic based on the proofs of the following \ref{sl4p4} and \ref{sl4p5}
    \begin{gather}\label{sl4p4}
      \begin{array}{l}
        \{\llbracket \Gamma, x:\textsf{rcuItr}\;\rho\;\N([f_1 | f_2 \rightharpoonup z]) \rrbracket_{M,tid} \cap \\
        \llbracket x:\textsf{rcuItr}\;\rho\;\N([f_1 \rightharpoonup y]) \rrbracket_{M,tid} \}\\
      \left(assume\left(z = y\right);C_1\right)\\
      \{\llbracket \Gamma' \rrbracket_{M,tid}\}
      \end{array}
    \end{gather}
    and
    \begin{gather}\label{sl4p5}
      \begin{array}{l}
        \{\llbracket \Gamma, x:\textsf{rcuItr}\;\rho\;\N([f_1 | f_2 \rightharpoonup z]) \rrbracket_{M,tid} \cap\\
        \llbracket x:\textsf{rcuItr}\;\rho\;\N([f_1 \rightharpoonup y]) \rrbracket_{M,tid} \}\\
        \left(assume\left(z \neq y\right);C_2\right)\\
      \llbracket \Gamma' \rrbracket_{M,tid}\}
      \end{array}
    \end{gather}
    We show \ref{sl4p4} from Views Logic's proof rule for the assume construct by using 
      \[
      \begin{array}{l}
        \{\llbracket \Gamma, x:\textsf{rcuItr}\;\rho\;\N([f_1 | f_2 \rightharpoonup z]) \rrbracket_{M,tid} \cap \\
        \llbracket x:\textsf{rcuItr}\;\rho\;\N([f_1 \rightharpoonup y]) \rrbracket_{M,tid} \} \\
        assume\left(y=z\right)\\
        \{\llbracket \Gamma, x:\textsf{rcuItr}\;\rho\;\N([f_1 \rightharpoonup z]) \rrbracket_{M,tid} \}
      \end{array}
      \]
      as the antecedent. We can use this antecedent together with 
      \[ \{\llbracket \Gamma, x:\textsf{rcuItr}\rho\N([f_1 \rightharpoonup z]) \rrbracket_{M,tid}\} C_1 \{\llbracket\Gamma' \rrbracket_{M,tid}\} \] as antecedents to the View's Logic's proof rule for sequencing.
    
We show \ref{sl4p5} from Views Logic's proof rule for the assume construct by using 
      \[
      \begin{array}{l}
      \{\llbracket \Gamma, x:\textsf{rcuItr}\;\rho\;\N([f_1 | f_2 \rightharpoonup z]) \cap\\
      x:\textsf{rcuItr}\;\rho\;\N([f_1 \rightharpoonup y]) \rrbracket_{M,tid} \}\\
      assume(x\neq y)\\
      \{\llbracket  \Gamma,x:\textsf{rcuItr}\;\rho\;\N([f_2 \rightharpoonup z]) \rrbracket_{M,tid} \}
      \end{array}
      \]
      as the antecedent. We can use this antecedent together with 
      \[ \{\llbracket\Gamma,   x:\textsf{rcuItr}\rho\N([f_2  \rightharpoonup z])\rrbracket_{M,tid}\} C_2 \{\llbracket\Gamma' \rrbracket_{M,tid}\} \]
      as antecedents to the Views Logic's proof rule for sequencing.
  \end{case}
  
  \begin{case}-\textbf{M}: case where $C$ is branch statement. $C$ has the form $if(x.f == \texttt{null})then\{C_1\}else\{C_2\}$.
    Proof is similar to one for \textsc{T-Branch1}.
   \end{case}

\begin{case}-\textbf{O}: parallel where $C$ has the form $\Gamma_1,\Gamma_2\vdash_{O} C_1 || C_2 \dashv \Gamma'_1,\Gamma'_2$
We know 
\begin{gather} \label{sl7a1}
\Gamma_1 \vdash C_1 \dashv \Gamma'_1\\
\label{sl7a2}
\Gamma_2 \vdash C_2 \dashv \Gamma'_2\\
\label{sl7a3}
\{ \llbracket \Gamma_1 \rrbracket \} C_1 \{ \llbracket \Gamma'_1 \rrbracket\}\\
\label{sl7a4}
\{ \llbracket \Gamma_2 \rrbracket \} C_2  \{ \llbracket \Gamma'_2 \rrbracket \}
\end{gather}

We need to show 
\begin{gather}\label{sl7p1}
\{\llbracket \Gamma_1, \Gamma_2 \rrbracket \} C_1 || C_2 \{\llbracket \Gamma'_1, \Gamma'_2 \rrbracket \}
\end{gather}

By using \ref{sl7a3} and \ref{sl7a4} as antecedents to Views Logic's parallel rule, we can draw conclusion for \ref{sl7p2}
\begin{gather}\label{sl7p2}
\{\llbracket \Gamma_1 \rrbracket * \llbracket \Gamma_2 \rrbracket\} C_1 || C_2\{\llbracket \Gamma'_1 \rrbracket * \llbracket \Gamma'_2 \rrbracket\}
\end{gather}

Showing \ref{sl7p1} requires showing 
\begin{gather}\label{sl7a5}
\llbracket \Gamma_1,\Gamma_2 \rrbracket \sqsubseteq \llbracket \Gamma_1\rrbracket * \llbracket  \Gamma_2 \rrbracket
\end{gather}

\begin{gather}\label{sl7a6}
\llbracket \Gamma'_1 \rrbracket * \llbracket \Gamma'_2 \rrbracket \sqsubseteq \llbracket \Gamma'_1, \Gamma'_2 \rrbracket
\end{gather}

By using \ref{sl7a5} and \ref{sl7a6}(trivial to show as "," and "*" for denotation of type contexts are both semantically equivalent to $\cap$) as antecedents to Views Logic's consequence rule, we can conclude \ref{sl7p1}.
\end{case}
\begin{case}-\textbf{M} where C has form $\textsf{RCUWrite}\, x.f \text{ as } y \text{ in } \bar{s}$
  which desugars into
  \[\textsf{WriteBegin}; x.f:= y ; \bar{s} ;\textsf{WriteEnd}\]

  We assume from the rule \textsc{ToRCUWrite}
 \begin{gather}\label{dsuga1}
       \Gamma, y:\textsf{rcuItr}\;\_ \vdash_{M} \bar{s} \dashv \Gamma' \\
       \label{dsuga2}
       \textsf{FType}(f) = \textsf{RCU} \\
       \label{dsuga3}
       \textsf{NoFresh}(\Gamma') \\
       \label{dsuga4}
       \textsf{NoUnlinked}(\Gamma')\\
        \label{dsuga5}
       \{\llbracket \Gamma\,, y:\textsf{rcuItr}\;\_ \rrbracket_{M,tid} \}  \bar{s}  \{\llbracket \Gamma' \rrbracket_{M,tid}\}
      \end{gather}
      
    Our goal is to prove
    \begin{gather}\label{dsugp1}
      \begin{array}{l}
      \{\llbracket \Gamma \rrbracket_{M,tid} \} 
      \textsf{WriteBegin}; x.f:= y  ;\textsf{WriteEnd}
      \{\llbracket \Gamma' \rrbracket_{M,tid} \}
      \end{array}
    \end{gather}
   Proof starts with application of the sequence rule. Assumptions \ref{dsuga3}-\ref{dsuga4} guarantee that there exists no change in the state(no heap update) due to any action in the body $\bar{s}$ which includes $x.f:=y$. \ref{dsugp1} follows from assumptions \ref{dsuga1}-\ref{dsuga5} trivially.
\end{case}
\end{proof}
%  \end{itemize}
\begin{lemma}[Context-SubTyping-M]\label{lem:cntxsubt-m}
\[ \Gamma \subt \Gamma'  \implies \llbracket \Gamma \rrbracket_{M,tid} \sqsubseteq \llbracket  \Gamma' \rrbracket_{M,tid} \]
\end{lemma}
\begin{proof}
  
Induction on the subtyping derivation. Then inducting on the first entry in the non-empty context(empty case is trivial) which follows from \ref{lem:cntxsubt-m-s}.
\end{proof}
\begin{lemma}[Context-SubTyping-R]\label{lem:cntxsubt-r}
\[ \Gamma \subt \Gamma'  \implies \llbracket \Gamma \rrbracket_{R,tid} \sqsubseteq \llbracket  \Gamma' \rrbracket_{R,tid} \]
\end{lemma}
\begin{proof}
Induction on the subtyping derivation. Then inducting on the first entry in the non-empty context(empty case is trivial) which follows from \ref{lem:cntxsubt-r-s}.
\end{proof}
\begin{lemma}[Singleton-SubTyping-M]\label{lem:cntxsubt-m-s}
  \[ x:T \subt x:T'  \implies \llbracket x:T \rrbracket_{M,tid} \sqsubseteq \llbracket  x:T' \rrbracket_{R,tid} \]
\end{lemma}
\begin{proof}
  Proof by case analysis on structure of $T'$ and $T$. Important case includes the subtyping relation is defined over components of \textsf{rcuItr} type. $T'$ including approximation on the path component
  \[\rho.f_1 \subt \rho.f_1|f_2\]
  together with the approximation on the field map
  \[\N([f_1 \rightharpoonup \_ ]) \subt \N([f_1|f_2 \rightharpoonup \_ ])\]
  lead to subset inclusion in between a set of states defined by denotation of the $x:T'$ the set of states defined by denotation of the $x:T$(which is also obvious for \textsc{T-Sub}). Reflexive relations and relations capturing base cases in subtyping are trivial to show.
  \end{proof}
\begin{lemma}[Singleton-SubTyping-R]\label{lem:cntxsubt-r-s}
  \[ x:T \subt x:T'  \implies \llbracket x:T \rrbracket_{M,tid} \sqsubseteq \llbracket  x:T' \rrbracket_{M,tid} \]
\end{lemma}
\begin{proof}
  Proof is similar to \ref{lem:cntxsubt-m-s} with a single trivial reflexive derivation relation (\textsc{T-TSub2})
\[\textsf{rcuItr} \subt \textsf{rcuItr}\]
  \end{proof}


==> chapters/RCUTypesSoundnessLemmasOld.tex <==
%!TEX root = ./paper.tex
\section{Soundness}
\label{sec:lemmas}

\begin{Lemma}[Safe ReadBlock Traversal]
\begin{gather}
\llbracket x:=x.f \rrbracket \lfloor \llbracket \Gamma,x:\mathsf{rcuIterator} \rrbracket_{\textsf{R},tid} * \{m\}\rfloor  \subseteq \\ 
\lfloor \llbracket \Gamma,x:\mathsf{rcuIterator} \rrbracket_{\textsf{R},tid}  * \mathcal{R}(\{m\})\rfloor 
\end{gather}
\end{Lemma}
\begin{proof}
We assume 
\begin{gather} \label{l1e1}
(\sigma,O,U,T) \, \in \, \llbracket \Gamma,x:\textsf{rcuIterator} \rrbracket_{\textsf{R},tid} * \{m\}
\\
\label{l1ewfa}
\textsf{WellFormed}(\sigma,O,U,T)
\end{gather}
And must show that there exists $O',U',T'$ such that
\begin{gather} \label{l1e3}
%\begin{gather}
(\sigma[ \sigma.s(x,tid) \mapsto \sigma.h(\sigma.s(x,tid),f) ], O',U',T') \in \\
\llbracket \Gamma,x:\textsf{rcuIterator} \rrbracket_{\textsf{R},tid} * \mathcal{R}(\{m\})
%\end{gather}
\\
\label{l1ewfa}
\textsf{WellFormed}(\sigma[ \sigma.s(x,tid) \mapsto \sigma.h(\sigma.s(x,tid),f)  ],O',U',T')
\end{gather}
%
From \ref{l1e1} we can assume
%
%%% gather formats a collection of numbered equations nicely
\begin{gather} \label{l1e4}
(\sigma,O_{1},U_{1},T_{1}) \in \llbracket \Gamma, x:\textsf{rcuIterator} \rrbracket_{\textsf{R},tid}
\\
 \label{l1e5}
(\sigma,O_{2},U_{2},T_{2}) = m 
\\
 \label{l1e6}
O_{1} \bullet O_{2} = O
\\
 \label{l1e7}
U_{1} \cup U_{2} = U 
\\
 \label{l1e8}
T_{1} \uplus T_{2} = T
\\
\label{l1wfa1}
\textsf{WellFormed}(\sigma,O_{1},U_{1},T_{1})
\\
\label{l1wfa2}
\textsf{WellFormed}(\sigma,O_{2},U_{2},T_{2})
\end{gather}
%
To prove \ref{l1e3} choose 
%
\[
\begin{array}{cl}
O' = O[ \sigma.s(x,tid) \mapsto O \setminus \textsf{iterator} \, tid  \cup \textsf{iterator} \, tid ] \\
U' = U \\
T' = T
\end{array}
\]
We must prove there exists $O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2}$ such that
\begin{gather}\label{l1e9}
(\sigma',O'_{1},U'_{1}, T'_{1}) \in \llbracket \Gamma,x:\textsf{rcuIterator} \rrbracket_{R,tid}
\\
\label{l1e10}
(\sigma',O'_{2},U'_{2}, T'_{2}) \in \mathcal{R}(\{m\})
\\
 \label{l1e11}
O'_{1} \bullet O'_{2} = O'
\\
\label{l1e12}
U'_{1} \cup U'_{2} = U' 
\\
\label{l1e13}
T'_{1} \uplus T'_{2} = T
\\
\label{l1wfp1}
\textsf{WellFormed}(\sigma',O_{1}',U_{1}',T_{1}')
\\
\label{l1wfp2}
\textsf{WellFormed}(\sigma',O_{2}',U_{2}',T_{2}')
\end{gather}
%
We choose $O_{2}' = O_{2}$, $U_{1}' = U_{1}$, $U_{2}' = U_{2}$, $T_{1}' = T_{1}$ and $T_{2}' = T_{2}$.
So \ref{l1e12} follows from \ref{l1e7} and \ref{l1e13} follows from \ref{l1e8}.

In the rest of the proof it is useful to know that 
\begin{equation} \label{l1e14}
T_{1} = \{tid\}
\end{equation}
which follows directly from \ref{l1e4}.

To show \ref{l1e11}, pick
\[
O_{1}'  = O_{1}[\sigma.s(x,tid) \mapsto O_{1} \setminus \textsf{iterator} \;  tid \cup \textsf{iterator} \; tid]
\]
$O'_{1} \bullet O'_{2} = O'$, follows, as we know $O'_{2}$ does not include $tid$.

From \ref{l1e4} we can assume 

\begin{gather} \label{l1e18}
(\sigma,\hat{O}'_{1}, U, T) \in \llbracket \Gamma \rrbracket_{R,tid}
\\
 \label{l1e19}
(\sigma,\hat{O}''_{1}, U, T) \in \llbracket x:\textsf{rcuIterator} \rrbracket_{R,tid}
\\
 \label{l1e20}
\hat{O}'_{1} \bullet \hat{O}''_{1} = O_{1}
\end{gather}

To show \ref{l1e9}, we need to show that there exists $O''_{1}$ and $O'''_{1}$ such that
\begin{gather} \label{l1e15}
(\sigma',O''_{1}, U, T) \in \llbracket \Gamma \rrbracket_{R,tid}
\\
 \label{l1e16}
(\sigma',O'''_{1}, U, T) \in \llbracket x:\textsf{rcuIterator} \rrbracket_{R,tid}
\\
 \label{l1e17}
O''_{1} \bullet O'''_{1} = O'_{1}
\end{gather}

Choosing $O''_{1} = \hat{O}'_{1}$, \ref{l1e15} follows  from \ref{l1e18}.

Assume that \[ o = \sigma.s(x,tid)\]

From semantics of \[ \llbracket x:\mathsf{rcuIterator} \rrbracket_{tid} \] we know that \[ \mathsf{iterator} \, tid \in O(o) \land x\notin U \]

By choosing $O'''_{1}$ to contain the new iterator from $O'_{1}$, , we know that

\[ x \notin dom(\Gamma) \]

as \[ \forall y \ldotp \sigma(y) = \sigma'(y) where x \neq y \]

as a result  

\ref{l1e15} implies \ref{l1e9}.

To show \ref{l1e10} we need to show that
\[
(\sigma, O_{2}, U_{2}, T_{2}) \mathcal{R} (\sigma', O_{2}, U_{2}, T_{2})
\]
%$\sigma$ agrees with $\sigma'$ on the heap and the stack for threads other than $tid$. By \ref{l1e8} and \ref{l1e14}, $tid \notin T_{2}$ so this is allowed.
which by definition means we must show
\begin{gather}
\label{l1re1}
\sigma.l \in T_{2} \rightarrow \sigma.h = \sigma'.h
\\
\label{l1re2}
\textsf{iterator} \, tid \in O_{2}(o) \rightarrow  o \in dom(\sigma'.h)
\\
\label{l1re3}
O_{2} = O_{2}
\\
\label{l1re4}
U_{2} = U_{2}
\\
\label{l1re5}
T_{2} = T_{2}
\\
\label{l1re6}
t \in T_{2} \rightarrow \forall x \ldotp \sigma.s(x,t) = \sigma'.s(x,t)
\end{gather}

\ref{l1re3}-\ref{l1re5} hold trivially. To show \ref{l1re1} we know $\sigma' = \sigma [  \sigma.s(x,tid) \mapsto \sigma.h(\sigma.s(x,tid),f)  ]$. So $\sigma'.h = \sigma.h$ as only $\sigma.s$ changes. To show \ref{l1re2} we know by \textsf{\textbf{MustBeAllocated}} that $o \in dom(\sigma.h)$ and thus $o \in dom(\sigma'.h)$. To show \ref{l1re6} we know $T_{1} = \{tid\} \land tid \notin T_{2}$.  We can assume $t \in T_{2} \land t \ne tid$ and must prove that 
\[
\forall x \ldotp \sigma.s(x,t) = \sigma'.s(x,t) 
\]
Which holds by the definition of $\sigma'$ as only $tid$s variables could be updated. 

%%%%%%Equation 21

To show \ref{l1wfp1} we assume \ref{l1wfa1} and pick
\[
O_{1}'  = O_{1}[\sigma.s(x,tid) \mapsto O_{1} \setminus \mathsf{iterator} \,  tid \cup \mathsf{iterator} \, tid]
\]

In addition, we know \ref{l1e14} and $tid  \in R$.

Assume that \[ o = \sigma'.s(x,tid)\]

From semantics of \[ \llbracket x:\mathsf{rcuIterator} \rrbracket_{R,tid} \] we know that \[ \mathsf{iterator} \, tid \in O(o) \land x\notin U \]

(\ref{l1wfp1} $\ldotp$ \textsf{Iterator I}) holds as $\mathsf{iterator} \, tid \in O'_{1}(o)$.

 
\[
O_{1}'  = O_{1}[\sigma.s(x,tid) \mapsto O_{1} \setminus \mathsf{iterator} \,  tid  \cup \mathsf{iterator} \, tid]
\]

\[ o = \sigma.s(x,tid) \in O_{1}\]

\[ o' = \sigma'.s(x,tid) \in O'_{1}\]


 As we know that $o \notin O'_{1}$ but $o' \in O_{1}'$, we can deduce that a thread $tid \in R$ can only have one pointer to a particular memory location.  This implies that (\ref{l1wfp1} $\ldotp$ \textsf{Iterator II}) holds. 

To show (\ref{l1wfp1} $\ldotp$ \textsf{Iterator III}), we know that for some $o$  where $s(x,tid) = o$
\[ \mathsf{iterator} \, tid\, \in O(o) \land  \exists T \ldotp T(T,o) \in F\]
and we need to show that 
\[tid \in T\].

As we know from semantics of 
\[
(\texttt{delayedFree}(x), s,h,l,R,F) 
\;\;\Downarrow_{\mathrm{tid}}\;\;
(s,h,l,R,F \uplus \{ (R,S(x))\} 
\]
that
\[s(x,tid) \in S(x)\]
then we conclude that 
\[tid \in T\]

In addition to (\ref{l1wfp1} $\ldotp$ \textsf{Iterator II}), we know that heap owns all locations that it owns before so  (\ref{l1wfp1} $\ldotp$ \textsf{Ownership}) holds as

\begin{gather*}
 \forall  o'' \, \ldotp \, h(o,f) = v \, \land \, h(o'',f') = v\, \land \, v \in  \mathsf{OID} \, \land \, \mathsf{ftype}(f) = \mathsf{rcu}, \, \implies \\
 o=o'' \land f=f'' \end{gather*}

holds.

(\ref{l1wfp1} $\ldotp$ \textsf{UnlinkedI}), (\ref{l1wfp1}$\ldotp$ \textsf{UnlinkedII}),(\ref{l1wfp1}$\ldotp$ \textsf{UnlinkedIII}), (\ref{l1wfp1}$\ldotp$ \textsf{FreshI}), (\ref{l1wfp1}$\ldotp$ \textsf{Freeing I}),(\ref{l1wfp1}$\ldotp$ \textsf{Freeing II}) and (\ref{l1wfp1}$\ldotp$ \textsf{MustBeAllocated}) are trivial


%%%%%%%%%%%%%Note:Check Equation_21.MustBeAllocated and others. Equation_22 

To show \ref{l1wfp2} we assume \ref{l1wfa2} and we already know that $O_{2}' = O_{2}$,  $U_{2}' = U_{2}$ and $T_{2}' = T_{2}$  .

 We know $tid' \in T_{2}$. (\ref{l1wfp2}$\ldotp$ \textsf{Ownership}), (\ref{l1wfp2}$\ldotp$ \textsf{IteratorI}), (\ref{l1wfp2}$\ldotp$ \textsf{IteratorII}), (\ref{l1wfp2}$\ldotp$ \textsf{UnlinkedI}), (\ref{l1wfp2}$\ldotp$ \textsf{UnlinkedII}),(\ref{l1wfp2}$\ldotp$ \textsf{UnlinkedIII}), (\ref{l1wfp2}$\ldotp$ \textsf{FreshI}), (\ref{l1wfp2}$\ldotp$ \textsf{Freeing I}), (\ref{l1wfp2}$\ldotp$ \textsf{Freeing II}) and (\ref{l1wfp2}$\ldotp$ \textsf{MustBeAllocated}) hold as only $s$ changes and $h$, $F_{2}$, $O_{2}$ do not change. 

\begin{comment}
For proof of  \ref{l1wfp2}$\ldotp$ \textsf{FreshII}, we can assume that 
\[o = O_{2}(x,t) \land o' = O'_{2}(x,t)\]
and we know that 
\[
\sigma' = \sigma [  \sigma.s(x,t) \mapsto \sigma.h(x,f) ]   \land \sigma.h = \sigma.h' 
\]
As heap does not change and assuming that 

\[ \mathsf{fresh} \in O_{2}'(o') \]

there exists only one action that preserves observation of a thread for a node as \textsf{fresh}
\[
\Gamma,\, x:\textsf{fresh } f\,\_ \vdash_{M} x.f := z \dashv x:\textsf{fresh }f\,z \,,\Gamma
\]
 which is a mutator action and this implies that 

\[t = l\]

For another case of \ref{l1wfp2}$\ldotp$ \textsf{FreshII} where 

\[t\in T_{2} \land t \in R\]

proof is trivial.
\end{comment}

%%%%
To show (\ref{l1wfp2}$\ldotp$ \textsf{IteratorIII}) we can assume for all \[x,tid', o\]
we can assume 
\[ \sigma'.s(x,tid') = o \land \mathsf{iterator} \, tid' \in O'_{2}(o) \land \exists T \ldotp (T,o)  \in F' \]
and we must prove 
\[tid' \in T\]
From assumption ( \ref{l1wfa2}$\ldotp$ \textsf{IteratorIII} ) we know for all \[x,tid',o\] 
\[\sigma.s(x,tid') = o \land \mathsf{iterator} \, tid' \, \in O_{2}(o) \land \exists T \ldotp (T,o) \in F \]
As
\[O_{2} = O'_{2} \land T_{2} = T'_{2}\]
and using 
\[\sigma'.s(x,tid') = o \land \mathsf{iterator} \, tid' \, \in O'_{2}(o) \land \exists T \ldotp (T,o) \in F' \]
and 
all updates in $\sigma$ are done to $tid$ associated variables and \[tid \notin T_{2}\]
implies that 
\[tid' \in T_{2} \land tid' \in T\].

%%%%

To prove (\ref{l1wfp2}$\ldotp$ \textsf{FreshII}) we can assume for some \[ x, tid', o \]
we can assume
\[ \sigma'.s(x,tid') = o \land \mathsf{fresh} \in O_{2}(o) \land tid' \in T_{2} \]
and we must prove 
\[tid' = \sigma'.l\]
From assumption ( \ref{l1wfa2}$\ldotp$ \textsf{FreshII} ) we know 
\begin{gather*}
\forall x,tid',o \ldotp \sigma.s(x,tid') = o \land \mathsf{fresh} \in O_{2}(o) \land tid' \in T_{2} \implies \\
tid' = \sigma.l 
\end{gather*}
As
\[O_{2} = O'_{2} \land T_{2} = T'_{2}\]
and using 
\[ \sigma'.s(x,tid') = o \land \mathsf{fresh} \in O_{2}(o) \land tid' \in T_{2} \]
we conclude that 
\[ \forall x,tid',o \ldotp \sigma.s(x,tid') = o \implies tid' = \sigma.l \]

If we knew $\sigma.s(x,tid') = \sigma'.s(x,tid')$ then we would be done. As we know $\sigma$ and $\sigma'$ only differ on variables associated to $tid$, and moreover $tid \notin T_{2}$, then we know that equality, and thus
\[tid' = \sigma.l\]
as required.

\end{proof}

\begin{Lemma}[Safe MutatorBlock Unlink]
\begin{gather}
\llbracket x.f:=z \rrbracket = \lfloor \llbracket \Gamma,x:\mathsf{rcuNext} \, f \, y, y:\mathsf{rcuNext} \, f \, z \rrbracket_{M,tid} * \{m\}\rfloor  \subseteq \\
\lfloor \llbracket \Gamma,x:\mathsf{rcuNext} \, f \, z, y:\mathsf{unlinked} \rrbracket  * \mathcal{R}(\{m\})\rfloor 
\end{gather}

\end{Lemma}

\begin{proof}

We can  assume 

\begin{gather} \label{l2e2}
(\sigma,O,U,T) \, \in \, \llbracket \Gamma,x:\mathsf{rcuNext} \, f \, y, y:\mathsf{rcuNext} \, f \, z \rrbracket_{M,tid} * \{m\}
\\
\label{l2ewfa}
\textsf{WellFormed}(\sigma,O,U,T)
\end{gather}

And must show that there exists $O',U',T'$ such that

\begin{gather} \label{l2e3}
(  \sigma [ \sigma.s(x,tid),f \mapsto \sigma.s(z,tid) ]  , O', U', T') \in \\
 \llbracket \Gamma,x:\mathsf{rcuNext} \, f \,z, y:\mathsf{unlinked} \rrbracket_{M,tid} * \mathcal{R}(\{m\})
\\
\label{l2ewfa}
\textsf{WellFormed}(  \sigma [ (\sigma.s(x,tid),f \mapsto \sigma.s(z,tid) ] , O', U', T')
\end{gather}

From \ref{l2e2} we can assume 


\begin{gather} \label{l2e4}
(\sigma, O_{1}, U_{1}, T_{1}) \in \llbracket \Gamma, x:\mathsf{rcuNext} \, f \, y, y:\mathsf{rcuNext} \, f  \,z\rrbracket_{M,tid}
\\
 \label{l2e5}
(\sigma, O_{2}, U_{2}, T_{2}) = m 
\\
\label{l2e6}
O_{1} \bullet O_{2} = O
\\
 \label{l2e7}
U_{1} \cup U_{2} = U
\\
 \label{l2e8}
T_{1} \uplus T_{2} = T
\\
\label{l2wfa1}
\textsf{WellFormed}(\sigma,O_{1},U_{1},T_{1})
\\
\label{l2wfa2}
\textsf{WellFormed}(\sigma,O_{2},U_{2},T_{2})
\end{gather}

To prove \ref{l2e3} choose

\[
\begin{array}{cl}
&O' = O[\sigma.s(y,tid) \mapsto O \setminus \mathsf{iterator} \, tid  \cup \mathsf{unlinked}]\\
&U' = U\\
&T' = T
\end{array}
\]

We must prove there exists $O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2}$ such that


\begin{gather}\label{l2e9}
(\sigma',O'_{1},U'_{1}, T'_{1}) \in \llbracket \Gamma,x:\mathsf{rcuNext}\,f \, z , \, y :\mathsf{unlinked}  \rrbracket_{M,tid}
\\
\label{l2e10}
(\sigma',O'_{2},U'_{2}, T'_{2}) \in \mathcal{R}(\{m\})
\\
 \label{l2e11}
O'_{1} \bullet O'_{2} = O'
\\
 \label{l2e12}
U'_{1} \cup U'_{2} = U' 
\\
 \label{l2e13}
T'_{1} \uplus T'_{2} = T
\\
\label{l2wfp1}
\textsf{WellFormed}(\sigma',O'_{1},U'_{1},T'_{1})
\\
\label{l2wfp2}
\textsf{WellFormed}(\sigma',O'_{2},U'_{2},T'_{2})
\end{gather}

We choose \[O_{2}' = O_{2}, U_{1}' = U_{1}, U_{2}' = U_{2}, T_{1}' = T_{1}, T_{2}' = T_{2}\]  so \ref{l2e12} follows from \ref{l2e7} and \ref{l2e13} follows from \ref{l2e8}

In the rest of the proof, it is useful to know that 

\begin{equation} \label{l2e14}
T_{1} = \{tid\}
\end{equation}
which follows directly from \ref{l2e4}.


To show \ref{l2e11}, pick

\[O_{1}' = O_{1}[\sigma.s(y,tid) \mapsto O_{1} \setminus \textsf{iterator} \, tid \cup \textsf{unlinked}]\]
$O'_{1} \bullet O'_{2} = O'$, follows, as we know $O'_{2}$ does not include $tid$.


From \ref{l2e4} we can assume


\begin{gather} \label{l2e14}
(\sigma,\hat{O}'_{1},U_{1},T_{1})  \in \llbracket \Gamma \rrbracket_{M,tid}
\\
 \label{l2e15}
(\sigma,\hat{O}''_{1},U_{1},T_{1})  \in \llbracket x:\mathsf{rcuNext} \, f \, y \rrbracket_{M,tid}
\\
\label{l2e16}
(\sigma,\hat{O}'''_{1},U_{1},T_{1}) \in \llbracket y:\mathsf{rcuNext} \, f \, z \rrbracket_{M,tid}
\\
 \label{l2e17}
\hat{O}'_{1} \bullet \hat{O}''_{1} \bullet \hat{O}'''_{1} = O_{1}
\end{gather}


To show \ref{l2e9}, we need to show that there exists  $O''_{1}$, $O'''_{1}$, $O''''_{1}$ such that 

\begin{gather} \label{l2e18}
(\sigma', O''_{1},U ,T) \in \llbracket \Gamma \rrbracket_{M,tid}
\\
 \label{l2e19}
(\sigma', O'''_{1},U ,T) \in \llbracket x:\mathsf{rcuNext} \, f \, z \rrbracket_{M,tid}
\\
 \label{l2e20}
(\sigma', O''''_{1},U ,T) \in \llbracket y:\mathsf{unlinked} \rrbracket_{M,tid}
\\ 
\label{l2e21}
O''_{1} \bullet O'''_{1} \bullet O''''_{1} = O'_{1}
\end{gather}

Choosing $\hat{O}'_{1} = O''_{1}$, \ref{l2e18} follows from \ref{l2e14}.

By choosing $O''''_{1}$ to contain the unlinked node and choosing $O'''_{1}$ to contain the iterator from ${O}'_{1}$, we show \ref{l2e21} where \ref{l2e9} follows from.

To show \ref{l2e10} we need to show that 

\[
(\sigma, O_{2}, U_{2}, T_{2}) \mathcal{R} (\sigma', O_{2}, U_{2}, T_{2})
\]
%$\sigma$ agrees with $\sigma'$ on the heap and the stack for threads other than $tid$. By \ref{l1e8} and \ref{l1e14}, $tid \notin T_{2}$ so this is allowed.
which by definition means we must show
\begin{gather}
\label{l2re1}
\sigma.l \in T_{2} \rightarrow \sigma.h = \sigma'.h
\\
\label{l2re2}
\textsf{iterator} \, tid \in O_{2}(o) \rightarrow  o \in dom(\sigma'.h)
\\
\label{l2re3}
O_{2} = O_{2}
\\
\label{l2re4}
U_{2} = U_{2}
\\
\label{l2re5}
T_{2} = T_{2}
\\
\label{l2re6}
t \in T_{2} \rightarrow \forall x \ldotp \sigma.s(x,t) = \sigma'.s(x,t)
\end{gather}


\ref{l2re3}-\ref{l2re5} holds trivially. We know that 
\[T_{2} \subseteq R\]
so \ref{l2re1} holds trivially.

\ref{l2re2} holds as we know from \textsf{\textbf{MustBeAllocated}} that $o \in dom(\sigma.h)$ and thus $o \in dom(\sigma'.h)$. To show \ref{l2re6} we know $T_{1} = \{tid\} \land tid \notin T_{2}$.  We can assume $t \in T_{2} \land t \ne tid$ and must prove that 
\[
\forall x \ldotp \sigma.s(x,t) = \sigma'.s(x,t) 
\]
which holds by the definition of $\sigma'$ as only $tid$s variables could be updated. 


To show \ref{l2wfp1} we assume \ref{l2wfa1} and pick

\[O_{1}' = O_{1}[\sigma.s(y,tid) \mapsto O_{1} \setminus \mathsf{iterator} \, tid \cup \mathsf{unlinked}] \]

In addition, we know  that 

\[T_{1}=\{tid\} \land tid= l\]
and  assume that 
\[o = \sigma'.s(y,tid)\]

(\ref{l2wfp1}.\textsf{IteratorI}) holds as 

\[ l =  tid \land \textsf{unlinked} \in O'_{1}(o)\]

(\ref{l2wfp1}.\textsf{IteratorII}) is trivial.

 To show (\ref{l2wfp1}.\textsf{IteratorIII}), we know that 

\[F \subseteq R\land tid \notin R\] implies that ( \ref{l2wfp1}.\textsf{IteratorIII}) is trivial.

To show (\ref{l2wfp1}.\textsf{UnlinkedI}), we can assume that 
\[ \sigma'.s(y,tid) = o \land \mathsf{unlinked} \in O'_{1}(o) \]
and we show that 
\[\forall o',f' \ldotp  h(o',f') = o \implies \mathsf{unlinked} \in O'_{1}(o') \lor ( \_ ,o') \in F\]
As 
\[\mathsf{unlinked} \in O'_{1}(\sigma'.s(y,tid)) \]
(\ref{l2wfp1}.\textsf{UnlinkedI}) holds.

(\ref{l2wfp1}.\textsf{UnlinkedII-III}) is trivial.

(\ref{l2wfp1}.\textsf{FreshI-II}), (\ref{l2wfp1}.\textsf{WriterNotReader}), (\ref{l2wfp1}.\textsf{MustBeAllocated}) is trivial.

To show (\ref{l2wfp1}.\textsf{FreeingI}) ...To show (\ref{l2wfp1}.\textsf{FreeingII}) ...
%%%%%%%%%%%%%%%%

To show \ref{l2wfp2} we assume \ref{l2wfa2} and we already know that $O_{2}' = O_{2}$,  $U_{2}' = U_{2}$ and $T_{2}' = T_{2}$  .

To prove (\ref{l2wfp2}.\textsf{IteratorI}), for some 
\[ x, o, tid' \]
we assume
\[
\sigma'.s(x,tid') = o \land (x,tid') \notin U'_{2} \land tid' \in T'_{2}
\]
and it is enough to prove 
\[ \mathsf{iterator} \, tid \in O'_{2} \]
as 
\[tid' \in R\]
From assumption (\ref{l2wfp1}.\textsf{IteratorI}) we know
\[ \sigma.s(x,tid') = o \land (x,tid') \notin U_{2} \land tid' \in T_{2} \implies \mathsf{iterator} \, tid \in O_{2}\]
As
\[  O_{2}' = O_{2}  \land U_{2}' = U_{2} \land T_{2}' = T_{2} \]
and using
\[
\sigma'.s(x,tid') = o \land (x,tid') \notin U'_{2} \land tid' \in T'_{2}
\]
and as heap changes, we can conlclude that 
\[\forall o,x \ldotp \sigma'.s(x,tid') = o \land (x,tid') \notin U'_{2} \land tid' \in T'_{2} \implies \mathsf{iterator} tid' \]

Proving (\ref{l2wfp2}.\textsf{IteratorII}) is trivial.


To prove (\ref{l2wfp2}.\textsf{IteratorIII}),  for some
\[o,tid' \] where 
\[tid' \in R\]
we assume 
\[ \mathsf{iterator} \, tid' \in O'_{2} \land \exists T \ldotp (T,o) \in  F \] to prove
\[tid' \in T\]
From assumption  (\ref{l2wfa2}.\textsf{IteratorIII}), we know that 
\[\mathsf{iterator} \, tid' \in O_{2} \land \exists T \ldotp (T,o) \in  F  \implies tid' \in T \]
and using 
\[O_{2} = O'_{2} \land T_{2} = T'_{2}\] with
\[ \mathsf{iterator} \, tid' \in O'_{2} \land \exists T \ldotp (T,o) \in  F \]
enables us to conclude that 
\[tid' \in T\]

To prove (\ref{l2wfp2}.\textsf{Unlinked I}) for some $o$ we can assume
\[\mathsf{unlinked} \in O'_{2}(o) \] and 
\[\forall o',f' \ldotp \sigma'.h(o',f')= o\] to prove
\[ \mathsf{unlinked} \in O'_{2}(o) \lor (\_,o') \in F\]
From assumption (\ref{l2wfa2}.\textsf{Unlinked I})  we know that 
\begin{gather}\mathsf{unlinked} \in O_{2}(o) \text{then} \forall o',f' \ldotp \sigma.h(o',f') = o \implies \\ 
\mathsf{unlinked} \in O_{2}(o') \lor (\_,o') \in F \end{gather}
Using 
\[O_{2} = O'_{2} \land T_{2} = T'_{2}\] and 
\[\mathsf{unlinked} \in O'_{2}(o) \]
\[\forall o',f' \ldotp \sigma'.h(o',f')= o\] 
we can conclude that 
\[ \mathsf{unlinked} \in O'_{2}(o) \lor (\_,o') \in F\]

Proving (\ref{l2wfp2}.\textsf{UnlinkedII-III}) is trivial.

To prove (\ref{l2wfp2}.\textsf{FreshI}) we assume for some node $o$
\[\mathsf{fresh} \in O'_{2}(o) \]
\[\forall o',f'  \ldotp \sigma'.h(o',f') = o\]
to prove
\[ \mathsf{fresh} \in O'_{2}(o')\]
From assumption (\ref{l2wfa2}.\textsf{FreshI}), we know that 
\[ \forall o \ldotp \mathsf{fresh} \in O_{2}(o) \text{then} \forall o',f' \ldotp \sigma.h(o',f') = o \implies \mathsf{fresh} \in O_{2}(o') \]
and using 
\[ O_{2} = O'_{2} \land T_{2} = T'_{2} \] with 
\[ \mathsf{fresh} \in O'_{2}(o) \]
\[ \forall o',f'  \ldotp \sigma'.h(o',f') = o\]
we conclude that 
\[fresh \in O'_{2}(o')\]

Proving (\ref{l2wfp2}.\textsf{FreshII}), (\ref{l2wfp2}.\textsf{FreeingI-II}) is trivial.

\end{proof}
\newcommand{\newln}{\\&\quad\quad{}} 


\begin{Lemma}[Safe MutatorBlock Link]
\begin{gather}
\llbracket x.f:=z \rrbracket \lfloor \llbracket \Gamma,x:\mathsf{rcuNext} \, f \, y \, , z:\mathsf{fresh} \, f \, y \rrbracket_{\textsf{M},tid} * \{m\}\rfloor  \subseteq \\ 
\lfloor \llbracket \Gamma,x:\mathsf{rcuNext} \, f \, z \, , z:\mathsf{rcuNext} \, f \, y  \rrbracket_{\textsf{M},tid}  * \mathcal{R}(\{m\})\rfloor 
\end{gather}
\end{Lemma}
\begin{proof}
We assume 
\begin{gather} \label{l3e1}
(\sigma,O,U,T) \, \in \, \llbracket \Gamma,x:\mathsf{rcuNext} \, f \, y \, , z:\mathsf{fresh} \, f \, y \rrbracket_{\textsf{M},tid} * \{m\}
\\
\label{l3ewfa}
\textsf{WellFormed}(\sigma,O,U,T)\\
\sigma.h(\sigma.s(x,tid),f) = \sigma.s(y,tid) 
\end{gather}
And must show that there exists $O',U',T'$ such that
\begin{gather} 
\begin{split}
\label{l3e3} 
(\sigma[ \sigma.s(x,tid),f \mapsto\sigma.s(z,tid) ], O',U',T')  \\
\in \llbracket \Gamma,x:\mathsf{rcuNext} \, f \, z \, , z:\mathsf{rcuNext} \, f \, y \rrbracket_{\textsf{M},tid} * \mathcal{R}(\{m\})
\end{split}
\\
\label{l3ewfa}
\textsf{WellFormed}(\sigma[ \sigma.s(x,tid),f \mapsto\sigma.s(z,tid)],O',U',T')
\end{gather}

From \ref{l3e1} we can assume 

\begin{gather} \label{l3e4}
(\sigma, O_{1}, U_{1}, T_{1}) \in \llbracket \Gamma, x:\mathsf{rcuNext} \, f \, y, z:\mathsf{fresh} \, f \, y\rrbracket_{M,tid}
\\
 \label{l3e5}
(\sigma, O_{2}, U_{2}, T_{2}) = m 
\\
\label{l3e6}
O_{1} \bullet O_{2} = O
\\
 \label{l3e7}
U_{1} \cup U_{2} = U
\\
 \label{l3e8}
T_{1} \uplus T_{2} = T
\\
\label{l3wfa1}
\textsf{WellFormed}(\sigma,O_{1},U_{1},T_{1})
\\
\label{l3wfa2}
\textsf{WellFormed}(\sigma,O_{2},U_{2},T_{2})
\end{gather}

To prove \ref{l3e3} choose

\[
\begin{array}{cl}
&O' = O[\sigma.s(z,tid) \mapsto O  \setminus \mathsf{fresh}  \cup \mathsf{iterator} \, tid]\\
&U' = U\\
&T' = T
\end{array}
\]

We must prove there exists $O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2}$ such that


\begin{gather}\label{l3e9}
(\sigma',O'_{1},U'_{1}, T'_{1}) \in \llbracket \Gamma,x:\mathsf{rcuNext}\,f \, z , \, z:\mathsf{rcuNext}\,f \, y  \rrbracket_{M,tid}
\\
\label{l3e10}
(\sigma',O'_{2},U'_{2}, T'_{2}) \in \mathcal{R}(\{m\})
\\
 \label{l3e11}
O'_{1} \bullet O'_{2} = O'
\\
 \label{l3e12}
U'_{1} \cup U'_{2} = U' 
\\
 \label{l3e13}
T'_{1} \uplus T'_{2} = T
\\
\label{l3wfp1}
\textsf{WellFormed}(\sigma',O'_{1},U'_{1},T'_{1})
\\
\label{l3wfp2}
\textsf{WellFormed}(\sigma',O'_{2},U'_{2},T'_{2})
\end{gather}

We choose 

\[O'_{2} = O_{2}, U'_{1} = U_{1}, U'_{2} = U_{2}, T'_{1} = T_{1}, T'_{2} = T_{2}  \] so \ref{l3e12} follows from \ref{l3e7} and \ref{l3e13} follows from \ref{l3e8}.

In the rest of the proof , it is useful to knowthat
\begin{equation} \label{l3e14}
T_{1} = \{tid\}
\end{equation}
which follows directly from \ref{l3e4}.

To show \ref{l3e11}, pick

\[O_{1}' = O_{1}[\sigma.s(z,tid) \mapsto O_{1} \setminus \textsf{fresh}  \cup \textsf{iterator} \, tid]\]
$O'_{1} \bullet O'_{2} = O'$, follows, as we know $O'_{2}$ does not include $tid$.


From \ref{l3e4} we can assume

\begin{gather} \label{l3e14}
(\sigma,\hat{O}'_{1},U_{1},T_{1})  \in \llbracket \Gamma \rrbracket_{M,tid}
\\
 \label{l3e15}
(\sigma,\hat{O}''_{1},U_{1},T_{1})  \in \llbracket x:\mathsf{rcuNext} \, f \, y \rrbracket_{M,tid}
\\
\label{l3e16}
(\sigma,\hat{O}'''_{1},U_{1},T_{1}) \in \llbracket z:\mathsf{fresh} \, f \, y \rrbracket_{M,tid}
\\
 \label{l3e17}
\hat{O}'_{1} \bullet \hat{O}''_{1} \bullet \hat{O}'''_{1} = O_{1}
\end{gather}


To show \ref{l3e9}, we need to show that there exists  $O''_{1}$, $O'''_{1}$, $O''''_{1}$ such that 

\begin{gather} \label{l3e18}
(\sigma', O''_{1},U ,T) \in \llbracket \Gamma \rrbracket_{M,tid}
\\
 \label{l3e19}
(\sigma', O'''_{1},U ,T) \in \llbracket x:\mathsf{rcuNext} \, f \, z \rrbracket_{M,tid}
\\
 \label{l3e20}
(\sigma', O''''_{1},U ,T) \in \llbracket z:\mathsf{rcuNext} \,f \, y \rrbracket_{M,tid}
\\ 
\label{l3e21}
O''_{1} \bullet O'''_{1} \bullet O''''_{1} = O'_{1}
\end{gather}

Choosing $\hat{O}'_{1} = O''_{1}$, \ref{l3e18} follows from \ref{l3e14}.

By choosing $O''''_{1}$ and $O'''_{1}$ to contain the iterators from ${O}'_{1}$, we show \ref{l3e21} where \ref{l3e9} follows from.

To show \ref{l3e10} we need to show that 

\[
(\sigma, O_{2}, U_{2}, T_{2}) \mathcal{R} (\sigma', O_{2}, U_{2}, T_{2})
\]
%$\sigma$ agrees with $\sigma'$ on the heap and the stack for threads other than $tid$. By \ref{l1e8} and \ref{l1e14}, $tid \notin T_{2}$ so this is allowed.
which by definition means we must show
\begin{gather}
\label{l3re1}
\sigma.l \in T_{2} \rightarrow \sigma.h = \sigma'.h
\\
\label{l3re2}
\textsf{iterator} \, tid \in O_{2}(o) \rightarrow  o \in dom(\sigma'.h)
\\
\label{l3re3}
O_{2} = O_{2}
\\
\label{l3re4}
U_{2} = U_{2}
\\
\label{l3re5}
T_{2} = T_{2}
\\
\label{l3re6}
t \in T_{2} \rightarrow \forall x \ldotp \sigma.s(x,t) = \sigma'.s(x,t)
\end{gather}

\ref{l3re3}-\ref{l3re5} holds trivially. We know that 
\[T_{2} \subseteq R\]
so \ref{l3re1} holds trivially.

\ref{l3re2} holds as we know from \textsf{\textbf{MustBeAllocated}} that $o \in dom(\sigma.h)$ and thus $o \in dom(\sigma'.h)$. To show \ref{l3re6} we know $T_{1} = \{tid\} \land tid \notin T_{2}$.  We can assume $t \in T_{2} \land t \ne tid$ and must prove that 
\[
\forall x \ldotp \sigma.s(x,t) = \sigma'.s(x,t) 
\]
which holds by the definition of $\sigma'$ as only $tid$s variables could be updated. 

To prove \ref{l3wfp1} we know 
\[O_{1}' = O_{1}[\sigma.s(z,tid) \mapsto O_{1} \setminus \mathsf{fresh}  \cup \mathsf{iterator} \, tid ] \]
in addition to
\[T_{1}=\{tid\} \land tid= l\]

(\ref{l3wfp1}.\textsf{IteratorI}) holds as 

\[ l =  tid \] for
\[ o' = \sigma'.s(x,tid) \land o'' = \sigma'.s(z,tid) \] with knowing that
\[O'_{1} = O_{1}[\sigma.s(z,tid) \mapsto O_{1}  \setminus \mathsf{fresh}  \cup \mathsf{iterator} \, tid]\]
we can conclude that (\ref{l3wfp1}.\textsf{IteratorI}) holds as  
\[ \textsf{iterator} \, tid \in O'_{1}(o') \land \textsf{iterator} \, tid \in O'_{1}(o'') \]

Proving (\ref{l3wfp1}.\textsf{IteratorII})  is trivial.
 To show (\ref{l3wfp1}.\textsf{IteratorIII}), we know that 

Knowing that \[F \subseteq R\land tid \notin R\] makes ( \ref{l3wfp1}.\textsf{IteratorIII}) is trivial.

Proving (\ref{l3wfp1}.\textsf{Unlinked I}) is trivial.

To prove (\ref{l3wfp1}.\textsf{Unlinked II}) we can assume 
\begin{gather} \forall o \ldotp (T,o) \in F' \implies (\forall o',f' \ldotp h(o',f') = o \implies (T',o') \in F \land T' \subseteq T) \end{gather}

From (\ref{l3wfa1}.\textsf{Unlinked II}), we know that 
\begin{gather} \forall o \ldotp (T,o) \in F \implies (\forall o',f' \ldotp h(o',f') = o \implies (T',o') \in F and T' \subseteq T) \end{gather}
As we know that  $O_{1}$  is updated with a node $o'$ such that 
 \[o=\sigma'.s(y,tid) \land  o' = \sigma'.s(z,tid)   \]
\[z:\mathsf{rcuNext}\,f \, y \land \mathsf{iterator} \, tid \in O'_{1}(o') \land o' \in dom(\sigma'.h) \]
and 
\[tid \notin R \]
we can conclude that 
\[ (\forall o',f' \ldotp \sigma'.h(o',f') = o \implies (T',o') \in F and T' \subseteq T) \]

From assumption of (\ref{l3wfa1}.\textsf{UnlinkedIII}), we know that for some $o$ 
\[ \mathsf{iterator} \; l \in O_{1}(o) \implies \mathsf{unlinked} \notin O_{1}(o)\]
As 
\[ T_{1} = T'_{1} \land tid = l \] and from our assumption from (\ref{l3wfp1}.\textsf{UnlinkedIII})
\[\mathsf{itearator} \; l \in O'_{1}(o) \] and
\[ O_{1}' = O_{1}[\sigma.s(z,tid) \mapsto O_{1} \setminus \mathsf{fresh}  \cup \mathsf{iterator} \, tid ] \] 
we can conclude that 
\[ \mathsf{unlinked} \notin O'_{1} \]  

(\ref{l3wfp1}.\textsf{Fresh I-II}) is trivial.

(\ref{l3wfp1}.\textsf{FreeingI-II, MustbeAllocated, WriterNotReader}) is trivial.
For proof of \ref{l3wfp2}, we know 
\[ tid' \in T_{2} \land T_{2} = T'_{2} \land tid' \subseteq R \land  O_{2} = O'_{2} \land U_{2}  = U'_{2} \]
(\ref{l3wfp2}.\textsf{Ownership}) holds as we know that heap owns all locations that it owns before. 

(\ref{l3wfp2}.\textsf{IteratorI}) holds as from (\ref{l3wfa2}.\textsf{IteratorI}), we assume
\begin{gather*} \forall o \ldotp o \in \mathsf{RCU} \land \sigma.s(x,tid') = o \land (x,tid') \notin U \implies \\
\mathsf{iterator} \, tid' \in O_{2}(o)\end{gather*}From (\ref{l3wfp2}.\textsf{IteratorI}), we can assume that 
\[\forall o \ldotp o \in \mathsf{RCU} \land \sigma'.s(x,tid') = o \land (x,tid') \notin U\] and conclude that 
\[\mathsf{iterator} \, tid' \in O'_{2}(o)\]

(\ref{l3wfp2}.\textsf{IteratorII}) holds as from (\ref{l3wfa2}.\textsf{IteratorII}), we assume
\begin{gather} \forall tid' \in R , o,o' \ldotp \mathsf{iterator} \, tid' \in O_{2}(o) \land \mathsf{iterator} \, tid' \in O_{2}(o') \implies \\
 o=o' \end{gather}
As we know that 
\[O_{2} = O'_{2}\] which makes showing
(\ref{l3wfp2}.\textsf{IteratorII}) trivial.

(\ref{l3wfp2}.\textsf{IteratorIII}) holds as from (\ref{l3wfa2}.\textsf{IteratorIII}), we assume for some $o,tid'$
 \[ \mathsf{iterator} \, tid' \in O_{2}(o) \land \exists T \ldotp (T,o) \in F \implies tid' \in T_{2}\] and we can assume
\[\mathsf{iterator} \, tid' \in O'_{2} \land \exists T \ldotp (T,o) \in F'\] to prove
\[tid' \in T'_{2}\]

As \[ O_{2} = O'_{2} \land T_{2} = T'_{2} \] and using 
\[ \mathsf{iterator} \, tid'  \in O'_{2} \land \exists T \ldotp (T,o) \in F' \] we can conclude that $(T,o)$ stays same because 
\[T \subseteq R\land T \subseteq T'_{2}\] and 
(\ref{l3wfp2}.\textsf{IteratorIII}) holds.

(\ref{l3wfp2}.\textsf{Unlinked I-III-IV}) is trivial.

Proving (\ref{l3wfp2}.\textsf{Unlinked II}) 

Proving (\ref{l3wfp2}.\textsf{Fresh I}) is trivial.

To prove (\ref{l3wfp2}.\textsf{Fresh II})  we can  assume for some $x,tid',o$
\[\sigma'.s(x,tid') = o \land \mathsf{fresh} \in O'_{2}(o) \land tid' \in T'_{2}\]
and must prove 
\[tid' = \sigma'.l\]
From assumption (\ref{l3wfa2}.\textsf{Fresh II}) we know 
\[\forall x,tid',o \ldotp \sigma.s(x,tid') = o \land \mathsf{fresh} \in O_{2}(o) \land tid' \in T_{2} \implies tid' = \sigma.l\]
As we know \[O_{2} = O'_{2} \land T_{2} = T'_{2}\] and \[\sigma'.s(x,tid') = o \land \mathsf{fresh} \in O'_{2}(o) \land tid' \in T'_{2}\] and because $\sigma$ and $\sigma'$ only differ on  variables related to $tid$ and 
\[tid \notin T'_{2}\] (\ref{l3wfa2}.\textsf{Fresh II}) holds.

Proving (\ref{l3wfp2}.\textsf{MustBeAllocated-FreeingI-II}) is  trivial.

\end{proof}

\begin{Lemma}[Safe MutatorBlock Allocate a Node]
\[
\llbracket y := new \rrbracket \lfloor \llbracket \Gamma,y:\_ \rrbracket_{\textsf{M},tid} * \{m\}\rfloor  \subseteq\lfloor \llbracket \Gamma,y:\mathsf{fresh} \rrbracket_{\textsf{M},tid}  * \mathcal{R}(\{m\})\rfloor 
\]
\end{Lemma}
\begin{proof}
We assume 
\begin{gather} \label{l4e1}
(\sigma,O,U,T) \, \in \, \llbracket \Gamma,y:\_ \rrbracket_{\textsf{M},tid} * \{m\}
\\
\label{l4ewfa}
\textsf{WellFormed}(\sigma,O,U,T) 
\end{gather}
And must show that there exists $O',U',T'$ such that
\begin{gather} 
\begin{split}
\label{l4e3} 
(\sigma[ \sigma.s(y,tid) \mapsto \sigma.h(\sigma.s(y,tid),f) ], O',U',T')  \\
\in \llbracket \Gamma, y:\_ \rrbracket_{\textsf{M},tid} * \mathcal{R}(\{m\})
\end{split}
\\
\label{l4ewfa}
\textsf{WellFormed}(\sigma[ \sigma.s(y,tid) \mapsto \sigma.h(\sigma.s(y,tid),f) ],O',U',T')
\end{gather}

From \ref{l4e1} we can assume 

\begin{gather} \label{l4e4}
(\sigma, O_{1}, U_{1}, T_{1}) \in \llbracket \Gamma, y:\_ \rrbracket_{M,tid}
\\
 \label{l4e5}
(\sigma, O_{2}, U_{2}, T_{2}) = m 
\\
\label{l4e6}
O_{1} \bullet O_{2} = O
\\
 \label{l4e7}
U_{1} \cup U_{2} = U
\\
 \label{l4e8}
T_{1} \uplus T_{2} = T
\\
\label{l4wfa1}
\textsf{WellFormed}(\sigma,O_{1},U_{1},T_{1})
\\
\label{l4wfa2}
\textsf{WellFormed}(\sigma,O_{2},U_{2},T_{2})
\end{gather}

To prove \ref{l4e3} choose

\[
\begin{array}{cl}
&O' = O[\sigma.s(y,tid) \mapsto O  \cup \mathsf{fresh}]\\
&U' = U\\
&T' = T
\end{array}
\]

We must prove there exists $O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2}$ such that


\begin{gather}\label{l4e9}
(\sigma',O'_{1},U'_{1}, T'_{1}) \in \llbracket \Gamma,x:\mathsf{fresh}  \rrbracket_{M,tid}
\\
\label{l4e10}
(\sigma',O'_{2},U'_{2}, T'_{2}) \in \mathcal{R}(\{m\})
\\
 \label{l4e11}
O'_{1} \bullet O'_{2} = O'
\\
 \label{l4e12}
U'_{1} \cup U'_{2} = U' 
\\
 \label{l4e13}
T'_{1} \uplus T'_{2} = T
\\
\label{l4wfp1}
\textsf{WellFormed}(\sigma',O'_{1},U'_{1},T'_{1})
\\
\label{l4wfp2}
\textsf{WellFormed}(\sigma',O'_{2},U'_{2},T'_{2})
\end{gather}

We choose 

\[O'_{2} = O_{2}, U'_{1} = U_{1}, U'_{2} = U_{2}, T'_{1} = T_{1}, T'_{2} = T_{2}  \] so \ref{l4e12} follows from \ref{l4e7} and \ref{l4e13} follows from \ref{l4e8}.

In the rest of the proof , it is useful to knowthat
\begin{equation} \label{l4e14}
T_{1} = \{tid\}
\end{equation}
which follows directly from \ref{l4e4}.

To show \ref{l4e11}, pick

\[O_{1}' = O_{1}[\sigma.s(y,tid) \mapsto O_{1} \cup \mathsf{fresh} ]\]
$O'_{1} \bullet O'_{2} = O'$, follows, as we know $O'_{2}$ does not include $tid$.


From \ref{l4e4} we can assume

\begin{gather} \label{l4e14}
(\sigma,\hat{O}'_{1},U_{1},T_{1})  \in \llbracket \Gamma \rrbracket_{M,tid}
\\
 \label{l4e15}
(\sigma,\hat{O}''_{1},U_{1},T_{1})  \in \llbracket y:\_ \rrbracket_{M,tid}
\\
 \label{l4e16}
\hat{O}'_{1} \bullet \hat{O}''_{1} = O_{1}
\end{gather}


To show \ref{l4e9}, we need to show that there exists  $O''_{1}$, $O'''_{1}$ such that 

\begin{gather} 	\label{l4e17}
(\sigma', O''_{1},U ,T) \in \llbracket \Gamma \rrbracket_{M,tid}
\\
 \label{l4e18}
(\sigma', O'''_{1},U ,T) \in \llbracket y:\mathsf{fresh} \rrbracket_{M,tid}
\\
\label{l4e19}
O''_{1} \bullet O'''_{1} = O'_{1}
\end{gather}

Choosing $\hat{O}'_{1} = O''_{1}$, \ref{l4e17} follows from \ref{l4e14}.

By choosing $O'''_{1}$ to contain the fresh node from ${O}'_{1}$, we show \ref{l4e19} where \ref{l4e9} follows from.

To show \ref{l4e10} we need to show that 

\[
(\sigma, O_{2}, U_{2}, T_{2}) \mathcal{R} (\sigma', O_{2}, U_{2}, T_{2})
\]
%$\sigma$ agrees with $\sigma'$ on the heap and the stack for threads other than $tid$. By \ref{l1e8} and \ref{l1e14}, $tid \notin T_{2}$ so this is allowed.
which by definition means we must show
\begin{gather}
\label{l4re1}
\sigma.l \in T_{2} \rightarrow \sigma.h = \sigma'.h
\\
\label{l4re2}
\textsf{iterator} \, tid \in O_{2}(o) \rightarrow  o \in dom(\sigma'.h)
\\
\label{l4re3}
O_{2} = O_{2}
\\
\label{l4re4}
U_{2} = U_{2}
\\
\label{l4re5}
T_{2} = T_{2}
\\
\label{l4re6}
t \in T_{2} \rightarrow \forall x \ldotp \sigma.s(x,t) = \sigma'.s(x,t)
\end{gather}

\ref{l4re3}-\ref{l4re5} holds trivially. We know that 
\[T_{2} \subseteq R\]
so \ref{l4re1} holds trivially. \ref{l4re2} holds trivially.

To show \ref{l4re6} we know $T_{1} = \{tid\} \land tid \notin T_{2}$.  We can assume $t \in T_{2} \land t \ne tid$ and must prove that 
\[
\forall x \ldotp \sigma.s(x,t) = \sigma'.s(x,t) 
\]
which holds by the definition of $\sigma'$ as only $tid$s variables could be updated. 

To prove \ref{l4wfp1} we know 
\[O_{1}' = O_{1}[\sigma.s(y,tid) \mapsto O_{1} \cup \mathsf{fresh} ] \]
in addition to
\[T_{1}=\{tid\} \land tid= l\]

To prove (\ref{l4wfp1}.\textsf{Fresh I}) , we know from \textsf{InDomain} that
 \[\forall o,o',f' \ldotp \sigma.h(o',f') = o \implies o' \in dom(h) \] and
as we know that allocating a new is done from free list or some new heap location which is not in domain of rcu data structure before.  This makes (\ref{l4wfp1}.\textsf{Fresh I}) holds.

To prove (\ref{l4wfp1}.\textsf{Fresh II}) we know from (\ref{l4wfa1}.\textsf{Fresh II}) for some $x,o$ 
\[ \sigma.s(x,tid) = o \land \mathsf{fresh} \in O_{1}(o) \implies tid = l \]
and as we know that 
\[ T_{1} = T'_{1} \land tid = l \]
(\ref{l4wfp1}.\textsf{Fresh II} becomes trivial.

Proving \ref{l4wfp2} is trivial
\end{proof}

\begin{Lemma}[Safe MutatorBlock Free an Unlinked Node]
\begin{gather}
\llbracket  \mathsf{delayedfree}(x) \rrbracket \lfloor \llbracket \Gamma,x:\mathsf{unlinked} \rrbracket_{\textsf{M},tid} * \{m\}\rfloor  \subseteq \\ 
\lfloor \llbracket \Gamma,x:\mathsf{undef} \rrbracket_{\textsf{M},tid}  * \mathcal{R}(\{m\})\rfloor 
\end{gather}
\end{Lemma}
\begin{proof}

We assume 
\begin{gather} \label{l5e1}
(\sigma,O,U,T) \, \in \, \llbracket \Gamma,x:\mathsf{unlinked} \rrbracket_{\textsf{M},tid} * \{m\}
\\
\label{l5ewfa}
\textsf{WellFormed}(\sigma,O,U,T) 
\end{gather}
And must show that there exists $O',U',T'$ such that
\begin{gather} 
\begin{split}
\label{l5e3} 
(\sigma[ \sigma.s(x,tid) \mapsto \_ ], O',U',T')  \\
\in \llbracket \Gamma, x:\mathsf{unlinked} \rrbracket_{\textsf{M},tid} * \mathcal{R}(\{m\})
\end{split}
\\
\label{l5ewfa}
\textsf{WellFormed}(\sigma[ \sigma.s(x,tid) \mapsto \_) ],O',U',T')
\end{gather}

From \ref{l5e1} we can assume 

\begin{gather} \label{l5e4}
(\sigma, O_{1}, U_{1}, T_{1}) \in \llbracket \Gamma, y:\mathsf{unlinked} \rrbracket_{M,tid}
\\
 \label{l5e5}
(\sigma, O_{2}, U_{2}, T_{2}) = m 
\\
\label{l5e6}
O_{1} \bullet O_{2} = O
\\
 \label{l5e7}
U_{1} \cup U_{2} = U
\\
 \label{l5e8}
T_{1} \uplus T_{2} = T
\\
\label{l5wfa1}
\textsf{WellFormed}(\sigma,O_{1},U_{1},T_{1})
\\
\label{l5wfa2}
\textsf{WellFormed}(\sigma,O_{2},U_{2},T_{2})
\end{gather}

To prove \ref{l5e3} choose

\[
\begin{array}{cl}
&O' = O[\sigma.s(x,tid) \mapsto O  \setminus \mathsf{unlinked} \cup \mathsf{undef}]\\
&U' = U[x \mapsto U \cup \mathsf{undef}]\\
&T' = T
\end{array}
\]

We must prove there exists $O'_{1}, O'_{2}, U'_{1}, U'_{2}, T'_{1}, T'_{2}$ such that


\begin{gather}\label{l5e9}
(\sigma',O'_{1},U'_{1}, T'_{1}) \in \llbracket \Gamma,x:\mathsf{undef}  \rrbracket_{M,tid}
\\
\label{l5e10}
(\sigma',O'_{2},U'_{2}, T'_{2}) \in \mathcal{R}(\{m\})
\\
 \label{l5e11}
O'_{1} \bullet O'_{2} = O'
\\
 \label{l5e12}
U'_{1} \cup U'_{2} = U' 
\\
 \label{l5e13}
T'_{1} \uplus T'_{2} = T
\\
\label{l5wfp1}
\textsf{WellFormed}(\sigma',O'_{1},U'_{1},T'_{1})
\\
\label{l5wfp2}
\textsf{WellFormed}(\sigma',O'_{2},U'_{2},T'_{2})
\end{gather}

We choose 

\[O'_{2} = O_{2}, U'_{2} = U_{2}, T'_{1} = T_{1}, T'_{2} = T_{2}  \] so \ref{l5e12} follows from \ref{l5e7} and \ref{l5e13} follows from \ref{l5e8}.

In the rest of the proof , it is useful to knowthat
\begin{equation} \label{l5e14}
T_{1} = \{tid\}
\end{equation}
which follows directly from \ref{l5e4}.

To show \ref{l5e11}, pick

\[O_{1}' = O_{1}[\sigma.s(x,tid) \mapsto O_{1} \setminus \mathsf{unlinked} \cup \mathsf{undef} ]\]
$O'_{1} \bullet O'_{2} = O'$, follows, as we know $O'_{2}$ does not include $tid$.

And pick

\[U_{1}' = U_{1}[x \mapsto U \cup \mathsf{undef}]\]
$U'_{1} \cup U'_{2} = U'$, follows, as we know $U'_{2}$ does not include $tid$.

From \ref{l5e4} we can assume

\begin{gather} \label{l5e14}
(\sigma,\hat{O}'_{1},U_{1},T_{1})  \in \llbracket \Gamma \rrbracket_{M,tid}
\\
 \label{l5e15}
(\sigma,\hat{O}''_{1},U_{1},T_{1})  \in \llbracket x:\mathsf{unlinked} \rrbracket_{M,tid}
\\
 \label{l5e16}
\hat{O}'_{1} \bullet \hat{O}''_{1} = O_{1}
\end{gather}


To show \ref{l5e9}, we need to show that there exists  $O''_{1}$, $O'''_{1}$ such that 

\begin{gather} 	\label{l5e17}
(\sigma', O''_{1},U ,T) \in \llbracket \Gamma \rrbracket_{M,tid}
\\
 \label{l5e18}
(\sigma', O'''_{1},U ,T) \in \llbracket y:\mathsf{undef} \rrbracket_{M,tid}
\\
\label{l5e19}
O''_{1} \bullet O'''_{1} = O'_{1}
\end{gather}

Choosing $\hat{O}'_{1} = O''_{1}$, \ref{l5e17} follows from \ref{l5e14}.

By choosing $O'''_{1}$ to contain the undefined node from ${O}'_{1}$, we show \ref{l5e19} where \ref{l5e9} follows from.

To show \ref{l5e10} we need to show that 

\[
(\sigma, O_{2}, U_{2}, T_{2}) \mathcal{R} (\sigma', O_{2}, U_{2}, T_{2})
\]
%$\sigma$ agrees with $\sigma'$ on the heap and the stack for threads other than $tid$. By \ref{l1e8} and \ref{l1e14}, $tid \notin T_{2}$ so this is allowed.
which by definition means that we must show
\begin{gather}
\label{l5re1}
\sigma.l \in T_{2} \rightarrow \sigma.h = \sigma'.h
\\
\label{l5re2}
\textsf{iterator} \, tid \in O_{2}(o) \rightarrow  o \in dom(\sigma'.h)
\\
\label{l5re3}
O_{2} = O_{2}
\\
\label{l5re4}
U_{2} = U_{2}
\\
\label{l5re5}
T_{2} = T_{2}
\\
\label{l5re6}
t \in T_{2} \rightarrow \forall x \ldotp \sigma.s(x,t) = \sigma'.s(x,t)
\end{gather}

\ref{l5re3}-\ref{l5re5} holds trivially. We know that 
\[T_{2} \subseteq R\]
so \ref{l5re1} holds trivially. \ref{l5re2} holds trivially.

To show \ref{l5re6} we know $T_{1} = \{tid\} \land tid \notin T_{2}$.  We can assume $t \in T_{2} \land t \ne tid$ and must prove that 
\[
\forall x \ldotp \sigma.s(x,t) = \sigma'.s(x,t) 
\]
which holds by the definition of $\sigma'$ as only $tid$s variables could be updated. 

To prove \ref{l5wfp1} and we know \ref{l5wfp2}
\[O_{1}' = O_{1}[\sigma.s(x,tid) \mapsto O_{1} \setminus \mathsf{unlinked} \cup \mathsf{undef} ] \]
\[T_{1}=\{tid\} \land tid= l\]
\[O_{2} = O'_{2}\]
Proving \ref{l5wfp1} and \ref{l5wfp2} is trivial.
\end{proof}



==> chapters/RCUTypesSoundnessOld.tex <==
%!TEX root = ./paper.tex
\section{Soundness}
\label{sec:meminv}
To prove soundness, we define dynamic language semantics and relate with typing rules. We relate the type rules to the semantics by defining a denotation of type environments in terms of an extended machine state.

We define logic states, $\textsf{LState}$, ranged over by $\Sigma$ to be 
\begin{itemize}
\item A machine state, $\sigma$; 
\item An observation map, O, of type $ \textsf{Loc} \to \mathcal{P}(\textsf{obs})$
\item Undefined variable map, $U$, of type $\mathcal{P}(\textsf{Var})$
\item Set of threads, $T$, of type $\mathcal{P}(\textsf{TIDS})$
\end{itemize}
Reification is then trivially given by the first component.

Each memory region can be observed in the following types in a snapshot taken at any time.
\[
\textsf{obs} := \texttt{iterator} \; \mathrm{tid} \mid
			    \texttt{unlinked} \mid
			    \texttt{fresh}
\]

[Perhaps add a toBeFreed observation, that accounts for the time after the deferred free call, before it is actually freed.]

\[
\begin{array}{cl}
\mathcal{M}_{RCU} \stackrel{def}{=} &\{ m \in \textsf{MState} \times O \times U \times T \mid  \textsf{WellFormed}( m) \}
\end{array}
\]
and we define the set of objects that are involved in an RCU datastructure as:
\[
\textsf{RCU} =  
\{ o \mid \textsf{ftype}(f) = \textsf{rcu} \land \exists o' \ldotp h(o',f) = o \}
\]
where
\[
\begin{array}{cl}
\textsf{WellFormed}(\sigma,O,U,T) \stackrel{def}{=} 		&\textbf{\textsf{Ownership}}(\sigma,O,U,T)\\
								&\land$ $\textbf{\textsf{Iterator I}}(\sigma,O,U,T)\\
								&\land$ $\textbf{\textsf{Iterator II}}(\sigma,O,U,T)\\
								&\land$ $\textbf{\textsf{Iterator III}}(\sigma,O,U,T)\\
								&\land$ $\textbf{\textsf{Unlinked I}}(\sigma,O,U,T)\\
								&\land$ $\textbf{\textsf{Unlinked II}}(\sigma,O,U,T)\\	
								&\land$ $\textbf{\textsf{Unlinked III}}(\sigma,O,U,T)\\					
								&\land$ $\textbf{\textsf{Fresh I}}(\sigma,O,U,T)\\
								&\land$ $\textbf{\textsf{Fresh II}}(\sigma,O,U,T)\\
								&\land$ $\textbf{\textsf{Writer Not Reader}}(\sigma,O,U,T)\\
								&\land$ $\textbf{\textsf{Freeing I}}(\sigma,O,U,T)\\
								&\land$ $\textbf{\textsf{Freeing II}}(\sigma,O,U,T)\\
								&\land$ $\textbf{\textsf{MustBeAllocated}}(\sigma,O,U,T)\\
								&\land$ $\textbf{\textsf{InDomain}}(\sigma,O,U,T)\\
\end{array}
\]

\begin{figure*}[!htbp]
\footnotesize

\[
\textbf{IdenticalSequences}((f_1 \ldots f_n), (f'_1 \ldots f'_m) ) =
\left\{
\begin{array}{cl}
	& n = m \\
	& \land \forall_{1 \leq i \leq n} \ldotp \textsf{ftype}(f_i) = \textsf{ftype}(f'_i) = \textsf{rcu} \\
	& \land  f_i = f'_i 
\end{array}
\right\}
\]

\[
\textbf{h$^{*}$}(o = \textsf{UniqueRoot}, (f_1 \ldots f_n)) = 
\left\{
\begin{array}{cl}
	&\textbf{h$^{*}$}_{0}(o,(f_1 \ldots f_n)) \\
	&\textbf{h$^{*}$}_{1}( h(o,f_1), (f_2 \ldots f_n))   \\ 
	&\textbf{h$^{*}$}_{2}(h( h(o,f_1), f_2), (f_3 \ldots f_n))  \\
	&\ldotp \\ 
	&\ldotp \\
	&\textbf{h$^{*}$}_{n-1}(h(\ldots(h(o,f_1),\ldots, f_{n-1}),f_n)\\
	&\textbf{h$^{*}$}_{n}(h(\ldots(h(o,f_1),\ldots, f_{n}), \_)
\end{array}
\right\}
\]
\[
\textbf{PathsToNode}(o = \textsf{UniqueRoot} , o') = 
\left\{ (f_1 \ldots f_n) | \textbf{h$^{*}$}(o,f_1 \ldots f_n ) = o' \right\}
\]
\[
\textbf{IsSingleton}(S = \{\ldots\} ) = \mid S \mid = 1
\]

\caption{Utility Definitions for Memory Invariants}
\label{fig:definitionWellFormed-Utility}
\end{figure*}

\begin{figure*}[!htbp]
\footnotesize
\[
\textbf{Ownership}(\sigma,O,U,T) =
\left\{
\begin{array}{cl}
 	 & \forall f,o,o',f' \ldotp \\
	& \sigma.h(o,f) = v \land \sigma.h(o',f') = v \\
	& \land v \in \textsf{OID} \\
	& \land  \textsf{ftype}(f) = \textsf{rcu} \\
 	&\implies\left\{ 
		\begin{array}{cl} 
			&  o=o' \land f=f' \\
			& \lor\textsf{unlinked} \in O(o) \\ 
			& \lor \textsf{unlinked} \in O(o') \\
			& \lor  (\_, o) \in \sigma.F \\ 
			& \lor  (\_, o') \in \sigma.F 
		\end{array}
		\right\}
\end{array}
\right\}
\]
\[
\textbf{A Reference Cross Read/Write Blocks-Iterator I}(\sigma,O,U,T)=
\left\{
\begin{array}{cl}
	& \forall tid,o \in \textsf{RCU} \ldotp \\ 
	& \sigma.s(x,tid) = o  \\
	& \land (x,tid) \notin U \\
&\implies \left\{
		\begin{array}{cl}
 			& \textsf{iterator } \, tid \in O(o) \\
 			& \lor \sigma.l=tid \land (\textsf{unlinked} \in O(o) \\
			& \lor (\_,o) \in \sigma.F) 
		\end{array}
	\right\}
\end{array}
\right\}
\]
\[
\textbf{Single Reader Reference-Iterator II}(\sigma,O,U,T) =
\left\{
\begin{array}{cl}
 & \forall tid \in \sigma.R, o,o' \ldotp \\
&\textsf{iterator } \, tid \in O(o)  \\
&\land \textsf{iterator} \, tid \in O(o') \\
&\implies \left\{ 
		\begin{array}{cl}
			o=o'
		\end{array}
	\right\}
\end{array}
\right\}
\]
\[
\textbf{References In Free List-Iterator III}(\sigma,O,U,T)=
\left\{
\begin{array}{cl}
	&\forall tid, o \ldotp \\ 
	& \textsf{iterator} \, tid \in O(o) \\
	& \land \exists T \ldotp (T,o) \in \sigma.F \\
& \implies \left\{ 
		\begin{array}{cl}
  			tid \in T
		\end{array}
	\right\}
\end{array}
\right\}
\]
%%%
\[
\textbf{Aliasing Path-Iterator IV} = 
\left\{
\begin{array}{cl}
\left\{
\begin{array}{cl}
& \forall x,y \ldotp \sigma.s(x,tid) = o' \land \sigma.s(y,tid) = o'' \\
&\land \textsf{iterator} \, tid \in O(o') \land \textsf{iterator} \, tid \in O(o'') \\
& \land P_1 = \textsf{PathToNode}(o = \textsf{UniqueRoot}, o') \\
&\land P_2 = \textsf{PathToNode}(o = \textsf{UniqueRoot}, o'') \\
& \land \textsf{IsSingleton}(P_1) \land \textsf{IsSingleton}(P_2) \\
&\textsf{IdenticalSequences}( P_1, P_2) \\
\end{array}
\right\}
& \implies \left\{
		\begin{array}{cl}
		 \sigma.h^{*}(o,P_1) = \sigma.h^{*}(o,P_2) 
		\end{array}
	\right\}
\end{array}
\right\}
\]
\[
\textbf{Disjoint Path-Iterator V} =
\left\{
\begin{array}{cl}
\left\{
\begin{array}{cl}
& \forall_{x,y \in VA} \ldotp \sigma.s(x,tid) = o' \land \sigma.s(y,tid) = o'' \\
&\land \textsf{iterator} \, tid \in O(o') \land \textsf{iterator} \, tid \in O(o'') \\
& \land P_1 = \textsf{PathToNode}(o = \textsf{UniqueRoot}, o') \\ 
&\land P_2 = \textsf{PathToNode}(o = \textsf{UniqueRoot}, o'') \\
& \land \textsf{IsSingleton}(P_1) \land \textsf{IsSingleton}(P_2) \\
&\lnot \textsf{IdenticalSequences}( P_1, P_2) \\
\end{array}
\right\}
& \implies \left\{
		\begin{array}{cl}
	             \sigma.h^{*}(o,P_1) \neq \sigma.h^{*}(o,P_2) 
		\end{array}
	\right\}
\end{array}
\right\}
\]
%%%
\[
\textbf{Unlinked Points To Unlinked-Unlinked I}(\sigma,O,U,T) =
\left\{
\begin{array}{cl}
&\forall o \ldotp \textsf{unlinked} \in O(o) \\
&\implies\left\{ 
	\begin{array}{cl}
		&\forall o',f '\ldotp \\ 
 		&\sigma.h(o',f') = o \\
		&\implies \left\{
			\begin{array}{cl} 
				&\textsf{unlinked} \in O(o') \\
				&\lor (\_,o') \in \sigma.F
			\end{array}
		\right\}
	\end{array}
	\right\}
\end{array}
\right\}
\]
\[
\textbf{Free List Inclusion-Unlinked II}(\sigma,O,U,T) =
\left\{
\begin{array}{cl}
	&\forall o \ldotp (T, o) \in \sigma.F \\
	&\implies \left\{
 	\begin{array}{cl}
		&\forall o',f' \ldotp \sigma.h(o',f') = o \\
		&\implies \left\{
   		\begin{array}{cl}
   	 		&(T',o') \in \sigma.F \\
    			&\land T' \subseteq T
    		\end{array}
 		\right\}
 	\end{array}
 	\right\}
\end{array}
\right\}
\]
\[
\textbf{Unlinked Not Iterator-Unlinked III}(\sigma,O,U,T) =
\left\{
\begin{array}{cl}
	&\forall o \ldotp \textsf{iterator} \, \sigma.l \in O(o) \\
	& \implies \left\{ 
	\begin{array}{cl}
		&\textsf{unlinked} \notin O(o)	
	\end{array}
	\right\}
\end{array}
\right\}
\]
\[
\textbf{Unlinked Refences In Free List-Unlinked IV}(\sigma,O,U,T) =
\left\{
\begin{array}{cl}
 \lnot (\forall o \ldotp \textsf{unlinked} \in O(o) \land (\_,o) \notin \sigma.F)
\end{array}
\right\}
\]
\[
\textbf{Fresh Points To Fresh-Fresh I}(\sigma,O,U,T) =
\left\{
\begin{array}{cl}
&\forall o \ldotp \textsf{fresh} \in O(o) \\
&\implies \left\{ 
          \begin{array}{cl}
	&\forall o',f' \ldotp  \sigma.h(o',f') = o \\
&\implies \left\{ 
	\begin{array}{cl}
	&\textsf{fresh} \in O(o')
	\end{array}
\right\}
\end{array}
\right \}
\end{array}
\right\}
\]
\[
\textbf{Fresh Reference In Write Block-Fresh II}(\sigma,O,U,T) =
\left\{
\begin{array}{cl}
& \forall tid,x,o \ldotp \sigma.s(x,tid) = o \\
&\land \textsf{fresh} \in O(o)\\
&\implies \left \{
	tid = \sigma.l
\right\}
\end{array}
\right\}
\]
\[
\textbf{Writer Not Reader}(\sigma,O,U,T) =
\left\{
\begin{array}{cl}
 \sigma.l \notin \sigma.R
\end{array}
\right\}
\]
\[
\textbf{Free List Threads Subset Of Readers-Freeing I}(\sigma,O,U,T) =
\left\{
\begin{array}{cl}
\forall o \ldotp (T,o) \in \sigma.F \implies T \subseteq \sigma.R
\end{array}
\right\}
\]
\[
\textbf{Type of Reference in Free List-Freeing II}(\sigma,O,U,T) =
\left\{
\begin{array}{cl}
&\forall tid,o \ldotp (T,o) \in \sigma.F \\ 
&\land \textsf{iterator} \, tid \in O(o)\\ 
&\implies \left\{ 
	tid \in T
\right\}
\end{array}
\right\}
\]
\[
\textbf{MustBeAllocated}(\sigma,O,U,T) =
\left\{
\begin{array}{cl}
 &\textbf{\textsf{MustBeAllocated}}_{0}(\sigma,O,U,T) = \{o | \mathsf{iterator} \, tid \in O(o)\} \\
 &\textbf{\textsf{MustBeAllocated}}_{n+1} (\sigma,O,U,T)= \{ o' | o \in \textbf{\textsf{MustBeAllocated}}_{n}(\sigma,O,U,T) \lor \sigma.h(o,f) =o'\}
\end{array}
\right\}
\]
\[
\textbf{InDomain}(\sigma,O,U,T) =
\left\{
\begin{array}{cl}
&\forall o,f',o' \ldotp  \sigma.h(o,f) = o' \\
&\implies \left\{ o' \in dom(\sigma.h) \right\}
	\end{array}
\right\}
\]

\caption{Definition of WellFormedness: Memory Invariants}
\label{fig:definitionWellFormed}
\end{figure*}

We view type environments denotationally, in terms of the set of instrumented states permitted by a given environment. Figure \ref{fig:denotingtypeenviroment} defines the type environment denotation :
\[ \llbracket \Gamma  \rrbracket_{tid} \] 
Type denotations are mostly straightforward, though they rely on a notion of partial separating conjunction ∗ of instrumented states. To define this separation, we must first define composition of instrumented states which is an operation $\bullet$ : $\mathcal{M} \longrightarrow \mathcal{M} \longrightarrow \mathcal{M}$ that is commutative and associative. It is defined over observation map as exclusive union of observed type states:

\[O_{1} \bullet O_{2}(loc) =  O_{1}(loc) \uplus O_{2}(loc)\]

Separation algebra is define as :

\begin{gather}
 * = ( \land,\bullet,\uplus,\uplus) 
\\
\textsf{iterator} \, tid \in O \rightarrow tid \in T
\\
\textsf{unlinked} \in O \rightarrow \sigma.l \in T
\\
\textsf{fresh} \in O \rightarrow \sigma.l \in T
\end{gather}

Partial separating conjunction then simply requires the existence of two states that compose:
\[ m \in P \ast Q   \stackrel{def}{=} \exists m' \ldotp \exists m'' \ldotp m' \in P \land m'' \in Q \land m \in m' \bullet m''  \]

[TODO : Explain previous separating conjuction clearly]

\subsection{Views Framework}
Our soundness proof builds upon a version of the Views Framework [15], which is in some sense a generalization of the ideas behind separation logic and rely-guarantee reasoning. We gave the definitions required by Views Framework, $\mathcal{M}_{RCU}$, $*$ and $\bullet$. We define some relations over $\mathcal{M}$ to enable Views Framework give us structure to the soundness proof as an embedding of the type derivations into the view's program logic.

Thread interference relation $\mathcal{R} \subseteq \mathcal{M} \times \mathcal{M}$  defines permissible interference on an instrumented state. The relation must distribute over composition:
\[
   \forall m_{1}, m_{2}, m\ldotp (m_{1} \bullet  m_{2}) \Longrightarrow \exists  m'_{1} m'_{2} \ldotp m_{1} \mathcal{R} m'_{1} \land m_{2} \mathcal{R} m'_{2} \land m \in m'_{1} \bullet m'_{2}
\]

where $\mathcal{R}$ is transitive-reflexive closure of $\mathcal{R}_{0}$ shown at Figure \ref{fig:threadInterferenceRel}. A unit $\in \mathcal{M}$, a state with all maps are empty, to $\bullet$ is closed with respect to $\mathcal{R}$.
\begin{figure*}[!htbp]
\[
(\sigma, O, U, T) \, \mathcal{R}_{0} \, (\sigma', O', U', T') = \left\{
 \begin{array}{ll}
  \sigma.l  \in  T \rightarrow \sigma.h = \sigma'.h \land\\
  \textsf{iterator} \, tid \in O(o) \rightarrow o \in dom(\sigma'.h) \land \\
  O = O' \land U = U' \land T = T' \land\\
 t \in T \rightarrow \forall x \ldotp \sigma.s(x,t) = \sigma'(x,t)
 \end{array}
 \right.
\]
\caption{Thread Interference Relation}
\label{fig:threadInterferenceRel}
\end{figure*}

In the Views Framework, program logic itself contains judgements of the form $\{ p \} C \{ q \}$ for views p and q and commands $C$. A denotation of static assertions are in terms of instrumented states : $\llbracket \Gamma \rrbracket_{tid}$. Proving derivation of typing, ($\llbracket  \Gamma \vdash C \dashv \Gamma \rrbracket$ ) forms the basis of soundness.

This rule shows how types changed soundly in a concurrent setting. Denotation of a typing context:
\[
 \llbracket \Gamma \rrbracket : \mathcal{P}(\textsf{LState})
\]

\begin{figure*}[!htbp]
\centering
\[
\begin{array}{l@{\;\;=\;\;}l}
\llbracket \, x : \textsf{rcuIterator}\,  \rrbracket_{tid}
&
\{ (s,h,l,R,F), O,U \mid \textsf{iterator } \, tid\in  O(s(x)) 
\land x \notin U
\}
\\

\llbracket \, x : \textsf{unlinked} \, \rrbracket_{tid}
&
\{ (s,h,l,R,F), O,U \mid \textsf{unlinked}\in  O(s(x)) 
\land l = tid 
\land x \notin U
\}

\\

\llbracket \, x : \textsf{rcuNext } f_1\,x_1, \ldots f_n\,x_n  \, \rrbracket_{tid}
&
\left
\{ 
\begin{array}{l|l}
(s,h,l,R,F), O,U 
&
\textsf{iterator } \, tid\in  O(s(x)) 
\land x \notin U\\
&{}\land  s(x_1) = h(s(x), f_1) \\
&{}\ldots \\
&{}\land s(x_n) = h(s(x), f_n)
\end{array}
\right\}
\\
%x : rcuNext ft : y
\llbracket \, x : \textsf{rcuNext} f_1 \ldots f_n \, | \, y  \, \rrbracket_{tid}
&
\left
\{
\begin{array}{l|l}
(s,h,l,R,F),O,U
&
  \textsf{iterator } \, tid \in  O(s(x)) \\
&{}\textsf{iterator } \, tid \in O(s(y)) \\
&{}\land x \notin U \land y \notin U \,  \\
&{}\land  s(x_1) = h(s(x), f_1)  \\ &{}\ldots  \\ &{}\land s(y) = h(s(x), f_n)
\end{array}
\right\}
\\
%x:rcuIterator | y
\llbracket \, x : \textsf{rcuIterator} \, | \text{Bounding Set} = \mathcal{P}(\textsf{VAR})  \, \rrbracket_{tid}
&
\left
\{
\begin{array}{l|l}
(s,h,l,R,F),O,U
&
  \forall y \in \text{Bounding Set} \ldotp \\
&{}\textsf{iterator } \, tid\in  O(s(y)) \\
&{}\textsf{iterator }\, tid \in O(s(x)) \\
&{}\land y \notin U \land x \notin U\\
&{}\land  s(y_1) = h(s(y), f_1) \\ &{} \ldots \\ &{}\land s(x) = h(s(y), f_n)
\end{array}
\right\}
\\
\llbracket \, x : \textsf{fresh } f_1\,x_1, \ldots f_n\,x_n \,  \rrbracket_{tid}
&
\left
\{ 
\begin{array}{l|l}
(s,h,l,R,F), O,U 
&
\textsf{fresh}\in  O(s(x)) 
\land x \notin U\\
&{}\land  s(x_1) = h(s(x), f_1) \\
&{}\ldots \\
&{}\land s(x_n) = h(s(x), f_n)
\end{array}
\right\}
\\


\llbracket \, x : \textsf{undef }\rrbracket_{tid}
&

\{ 
(s,h,l,R,F), O,U 
\mid
x \in U\}
\\

\llbracket \, x : \textsf{normal }\rrbracket_{tid}
&

\{ 
(s,h,l,R,F), O,U 
\mid
x \notin U\}
\\
\end{array}
\]
\caption{Denoting Types and Type Environments}
\label{fig:denotingtypeenviroment}
\end{figure*}

We then define this on typing contexts as 
\begin{gather*}
\llbracket x_1 : T_1, \ldots x_n : T_n \rrbracket_{tid,\textsf{RMO}} = \\
\llbracket x_1 : T_1 \rrbracket_{tid}*_{local} \ldots *_{local} \llbracket x_n : T_n \rrbracket_{tid} *_{local} \llbracket \textsf{RMO} \rrbracket_{tid}
\end{gather*}
where
$\llbracket \textsf{R} \rrbracket_{tid} = \{ (s,h,l,R,F), O,U  \mid tid \in R \}$, 
$\llbracket \textsf{M} \rrbracket_{tid} = \{ (s,h,l,R,F), O,U  \mid tid = l \}$, and
$\llbracket \textsf{O} \rrbracket_{tid} = \{ (s,h,l,R,F), O,U  \mid tid \neq l \land tid \notin R \}$, and


Given the specific definitions of composition and interference, the Views Framework defines a number of useful concepts to help structure and simplify the soundness proof. First, it defines a view as the subset of instrumented states that are stable under interference:
\[ \textsf{View} \stackrel{def}{=} \{ M \in \mathcal{M} | \mathcal{R}(M) \subseteq M\} \] such that: 
The program logic is proven sound with respect to views, and our denotation of type environments is a valid view (stable with respect to R). The framework also describes a useful concept called the view shift operator $\subseteq$, that describes a way to reinterpret a set of instrumented states as a new set of instrumented states. It requires that :
\[p \sqsubseteq q \stackrel{def}{\Leftrightarrow} \forall m\in\mathcal{M} \ldotp \lfloor p * \{ m \} \rfloor \subseteq \lfloor q* \mathcal{R}(\{m\})\rfloor\]
This specifies how the region information can be changed soundly. That is, we can only change the region information such that all other possible threads can maintain compatible views.

To use the Views Framework soundness result we need to show for each axiom, $\Gamma_{1} \vdash_{\textsf{RMO}} \alpha \dashv \Gamma_{2}$, that
\[
\forall r\ldotp   \llbracket \alpha \rrbracket  \lfloor \llbracket \Gamma_{1} \rrbracket_{\textsf{RMO},tid}  * \{m\} \rfloor \subseteq \\
  \lfloor \llbracket \Gamma_{2} \rrbracket_{\textsf{RMO},tid} * \mathcal{R}(\{m\}) \rfloor
\]
\begin{theorem}[Axiom Soundness]
For each axiom, $\Gamma_{1} \vdash_{\textsf{RMO}} \alpha \dashv \Gamma_{2}$, we must show
\[
\forall r\ldotp   \llbracket \alpha \rrbracket  \lfloor \llbracket \Gamma_{1} \rrbracket_{\textsf{RMO},tid}  * \{m\} \rfloor \subseteq  \lfloor \llbracket \Gamma_{2} \rrbracket_{\textsf{RMO},tid} * \mathcal{R}(\{m\}) \rfloor
\]
\end{theorem}

We can define the denotation typing judgement as: 

\[ \llbracket \Gamma_{1} \vdash C \dashv \Gamma_{2} \rrbracket \stackrel{def}{=} \{ \llbracket \Gamma_{1} \rrbracket_{tid}\} C \{ \llbracket \Gamma_{2} \rrbracket_{tid}\} \]

%%%
For soundness proof, we describe the important lemmas supporting soundness proof, and omit natural uninteresting lemmas. Lemmas of the proof are described in detail in Appendix \ref{sec:lemmas}.
%%%
[TODO: Matthew, Is it ok or enough to give pointer to the real proofs of these lemmas at appendix in here ?]
\begin{Lemma}[Safe ReadBlock Traversal]
\begin{gather*}
\llbracket x:=x.f \rrbracket \lfloor \llbracket \Gamma,x:\mathsf{rcuIterator} \rrbracket_{\textsf{R},tid} * \{m\}\rfloor\subseteq \\
\lfloor \llbracket \Gamma,x:\mathsf{rcuIterator} \rrbracket_{\textsf{R},tid}  * \mathcal{R}(\{m\})\rfloor 
\end{gather*}
\end{Lemma}
\begin{proof}
\end{proof}

[TODO: Explain what we prove and tell detailed is in Appendix]

\begin{Lemma}[Safe MutatorBlock Unlink]
\begin{gather*}
\llbracket x.f:=z \rrbracket = \lfloor \llbracket \Gamma,x:\mathsf{rcuNext} \, f \, y, y:\mathsf{rcuNext} \, f \, z \rrbracket_{M,tid} * \{m\}\rfloor  \subseteq 
\\ \lfloor \llbracket \Gamma,x:\mathsf{rcuNext} \, f \, z, y:\mathsf{unlinked} \rrbracket  * \mathcal{R}(\{m\})\rfloor 
\end{gather*}
\end{Lemma}
\begin{proof}
\end{proof}

[TODO: Explain what we prove and tell detailed is in Appendix]

\begin{Lemma}[Safe MutatorBlock Link]
\begin{gather*}
\llbracket x.f:=z \rrbracket \lfloor \llbracket \Gamma,x:\mathsf{rcuNext} \, f \, y \, , z:\mathsf{fresh} \, f \, y \rrbracket_{\textsf{M},tid} * \{m\}\rfloor \subseteq \\ \lfloor \llbracket \Gamma,x:\mathsf{rcuNext} \, f \, z \, , z:\mathsf{rcuNext} \, f \, y  \rrbracket_{\textsf{M},tid}  * \mathcal{R}(\{m\})\rfloor 
\end{gather*}
\end{Lemma}
\begin{proof}
\end{proof}

[TODO: Explain what we prove and tell detailed is in Appendix]

\begin{Lemma}[Safe MutatorBlock Allocate a Node]
\[
\llbracket y := new \rrbracket \lfloor \llbracket \Gamma,y:\_ \rrbracket_{\textsf{M},tid} * \{m\}\rfloor  \subseteq \lfloor \llbracket \Gamma,y:\mathsf{fresh} \rrbracket_{\textsf{M},tid}  * \mathcal{R}(\{m\})\rfloor 
\]
\end{Lemma}
\begin{proof}
\end{proof}

[TODO: Explain what we prove and tell detailed is in Appendix]

\begin{Lemma}[Safe MutatorBlock Free an Unlinked Node]
\begin{gather*}
\llbracket  \mathsf{delayedfree}(x) \rrbracket \lfloor \llbracket \Gamma,x:\mathsf{unlinked} \rrbracket_{\textsf{M},tid} * \{m\}\rfloor  \subseteq \\ 
\lfloor \llbracket \Gamma,x:\mathsf{undef} \rrbracket_{\textsf{M},tid} * \mathcal{R}(\{m\})\rfloor 
\end{gather*}
\end{Lemma}
\begin{proof}
\end{proof}

[TODO: Explain what we prove and tell detailed is in Appendix]
%%%

Using the soundness theorem from the Views framework ~\cite{views} with the previous theorem we can show our type system is sound.

\begin{theorem}[Type Soundness]
\[ \Gamma_{1} \vdash C \dashv \Gamma_{2} \Longrightarrow \llbracket \Gamma_{1} \vdash C \dashv \Gamma_{2} \rrbracket \]
\end{theorem}
\begin{proof}
By induction on the derivation $ \Gamma_{1} \vdash C \dashv \Gamma_{2}$. 
\end{proof}

